Learning in repeated auctions

Online auctions are one of the most fundamental facets of the modern economy and power an industry generating hundreds of billions of dollars a year in revenue. Auction theory has historically focused on the question of designing the best way to sell a single item to potential buyers, with the concurrent objectives of maximizing revenue generated or welfare created. Theoretical results in this area have typically relied on some prior Bayesian knowledge agents were assumed to have on each-other. This assumption is no longer satisfied in new markets such as online advertising: similar items are sold repeatedly, and agents are unaware of each other or might try to manipulate each-other. On the other hand, statistical learning theory now provides tools to supplement those missing pieces of information given enough data, as agents can learn from their environment to improve their strategies. This survey covers recent advances in learning in repeated auctions, starting from the traditional economic study of optimal one-shot auctions with a Bayesian prior. We then focus on the question of learning optimal mechanisms from a dataset of bidders' past values. The sample complexity as well as the computational efficiency of different methods will be studied. We will also investigate online variants where gathering data has a cost to be accounted for, either by seller or buyers ("earning while learning"). Later in the survey, we will further assume that bidders are also adaptive to the mechanism as they interact repeatedly with the same seller. We will show how strategic agents can actually manipulate repeated auctions, to their own advantage. All the questions discussed in this survey are grounded in real-world applications and many of the ideas and algorithms we describe are used every day to power the Internet economy.

==> NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> chapters/SafetyCopy09031638/chapter2_some_classical_results.tex <==
%!TEX root = ../main.tex
\chapter{Bayesian mechanism design}
\label{Chapter:Bayes}

Auctions mechanisms involve many different agents, sellers and/or buyers, with possibly different and conflicting objectives as they all seek to optimize of their own utility functions. These interactions can be modeled using game-theoretic concepts. More specifically, we are going to focus on a specific types of games with \emph{incomplete information} that are called \textit{mechanisms}. In those games, each player has some private information (i.e. unknown from everyone else), and send a \emph{message} to a central authority.  Based on those gathered messages, the latter decides on the final outcome.  The utility of each player then solely depends on this outcome. 

Mechanisms model appropriately  many practical situations such as the celebrated  problems of assigning students to schools, or matchings in organ-transplant applications.  In these problems, a central authority forms pairs between school and students or donors and recipients. In selling mechanisms, the central authority is the seller of a specific item and the players are the buyers.  \emph{Auctions} are mechanisms used to sell a particular item. In the case of a sale of a single non-divisible item, they have the following specific features. 


%\clem{The notation defined here is not used later on and even conflicts with later notation.}{\color{red}VP : agreed !}
%A \textit{normal-form game} is defined by a set of of players $\mathcal{N}$ of cardinality $N$, the set of actions  $\mathcal{A}_i$ and the payoff function  of player $i \in \mathcal{N}$
%$u_i:\mathcal{A}_1 \times \dots \times \mathcal{A}_N \rightarrow \mathds{R}.$ 
%
%In such a game, each player chooses independently an action $a_i \in \mathcal{A}_i$ and gets a utility of $u_i(a_1,\ldots,a_N)=u_i(a_i,a_{-i})$
%that depends on both the action $a_i \in   \mathcal{A}_i$ of the player and the profile of actions of other players, denoted by $a_{-i} := (a_1,\ldots, a_{i-1}, a_{i+1},a_N) \in \prod_{j \neq i} \mathcal{A}_j$.
%
% 
%\begin{definition2}[Normal-form game]
%A normal-form game is:
%\begin{itemize}
%\item a set of players $\mathcal{N}$ of cardinality $N$.
%\item for each player $i \in [1,N]$, a set of possible actions $\mathcal{A}_i$.
%\item a set of payoff functions which gives for each player her payoff corresponding to her action and actions of other players
%$$u_i:\mathcal{A}_1 \times \dots \times \mathcal{A}_N \rightarrow \mathds{R}\;.$$
%\end{itemize}
%In a normal-form game of complete information, actions, outcomes and payoff functions are common knowledge to all players. In a game of incomplete information, every player's payoff function depends on a variable $X$ called private information and which is only known to each specific player. If we denote by $\mathcal{X}$ the set of private information, the payoff function of player $i$ is defined as $u_i:\mathcal{A}^{N} \times \mathcal{X} \rightarrow \mathds{R}$.
%\end{definition2}


%In the different settings we are going to consider,  players have some private information that actually impacts their payoff functions. Formally, let us denote by  $\mathcal{X}$ the set of private information, so that the payoff function of player $i$ rewrites as  $u_i:\prod_{j \in \mathcal{N}} \mathcal{A}_j \times \mathcal{X} \rightarrow \mathds{R}$. Those games are called with \textit{incomplete information}.


\medskip


%and decides each player's outcome according to these messages. In these games, players' actions correspond to the message they send to the central authority. 

%In a game of incomplete information, every player's payoff function depends on a variable $X$ called private information and which is only known to each specific player. If we denote by, the payoff function of player $i$ is defined as 

%In this survey, we are focusing on a certain type of games with incomplete information where there exists a central authority which gathers messages from the different players and decides each player's outcome according to these messages. In these games, players' actions correspond to the message they send to the central authority. This type of centralized gamed is called mechanism. 
%\begin{definition2}[Mechanism]
%A mechanism is a game of incomplete information where players send a message to a central authority who does not know the private information of each player. The central authority decides based on messages it receives and some predefined rules every player's outcome.  
%\end{definition2}

Auctions are games of incomplete information as each buyer has some private valuation for the item to be sold, i.e. the highest price they are willing to  pay to acquire  this item. This valuation might be different from one buyer to another. We denote by $\mathcal{N}$ the set of buyers, of cardinality $n \in \mathbb{N}$, by  $x_i \in \mathcal{X}_i$ the  private value of bidder $i \in \mathcal{N}$, $\mathcal{X}_i $ the set of private values of bidder $i$, and by  $x = (x_1,\dots,x_n)\in \mathbb{R}^n$, the so-called profile of private values. 
The possible messages (or actions) of buyer $i\in \mathcal{N}$ are called ``bids'' and the set of bids of buyer $i$ is denoted by $\mathcal{B}_i$. The outcome of an auction mechanism is defined by two different rules~:
\begin{enumerate}
\item an \textit{allocation rule} $q:\mathcal{B}_1 \times \dots \times  \mathcal{B}_n \rightarrow \Delta_n$ where $\Delta_n$ is the set of probability distributions over the set of $n$ buyers. It specifies the probability that each player gets the item.
\item a \textit{payment rule} $p: \mathcal{B}_1 \times \dots \times  \mathcal{B}_n \rightarrow \mathds{R}^{n}$. It specifies the expected payment of each player, whether or not they get the item.
\end{enumerate}

We also denote by $b = (b_1,\dots,b_n)$ the vector of bids of the bidders.  With these notations, the expected utility of bidder $i \in \mathcal{N}$ is then defined as
%$$u_i(b,x_i) = q_i(b)\big(x_i -p_i(b)\nig)\;;$$
$$u_i(b,x_i) = q_i(b)x_i -p_i(b)\;;$$
on the other hand, the seller aims at maximizing her expected revenue
%$$\sum_{i=1}^n q_i(b)p_i(b)\;.$$
$$\sum_{i=1}^n p_i(b)\;.$$

%\begin{definition2}[Auction mechanism]
%An auction mechanism is a mechanism defined by three features: 
%\begin{itemize}
%\item a set of possible messages $\mathcal{B}_i$ for each buyer (bids in most cases). 
%\item an allocation rule $q:\mathcal{B}_1 \times \dots \times  \mathcal{B}_N \rightarrow \Delta_N$ where $\Delta_N$ is the set of probability distributions over the set of $N$ buyers. It gives the probability that each player gets the object.
%\item a payment rule $p: \mathcal{B}_1 \times \dots \times  \mathcal{B}_N \rightarrow \mathds{R}^{N}$. It defines the expected payment of each player whether he got or not the object.
%\end{itemize}
%A selling mechanism is nothing more than a set of rules explaining how a group of buyers and a seller interact. 
%
%The private information owned by each buyer which conditions their payoff function is their own value for the item, i.e., the highest price they are ready to pay to own the item. We denote by $\mathcal{X}_i$ the set of all possible values for one item for bidder $i$.  The value vector which contains the values of all the different players is denoted by $x = (x_1,\dots,x_N)$. The \textit{messages} sent to the seller are called \textit{bids}.  We denote by $b = (b_1,\dots,b_N)$ the corresponding bid vector. 
%
%Depending on the information they have on the mechanism and the other bidders, the ultimate goal of the bidders is to maximize their utility 
%$$u_i(x_i, (b_1,...,b_N)) = q_i(b_1,...,b_N)(x_i -p_i(b_1,...,b_N))\;,$$
%and the objective of the seller is to maximize her revenue
%$$\sum_{i=1}^N q_i(b_1,...,b_N)p_i(b_1,...,b_N))\;.$$
%\end{definition2}
\section{The Bayesian setting}
The auction literature has often considered  a Bayesian setting where the value $x_i$ of bidder $i \in \mathcal{N}$ is random, drawn according to his \emph{value distribution} that ``represents the seller assessment of the probability of bidder $i$ having a value estimate of $x_i$ or less''  \citep{Myerson81}. The value distribution quantifies the uncertainty of the seller on the maximum price that one buyer is willing to pay for the item and is represented as a Bayesian prior on the private information of each buyer. 


A widely made assumption is that value distributions are common knowledge among bidders and seller.  As a consequence, we denote by $F_i$ the value distribution - i.e. the cumulative distribution function of the value -  of buyer $i \in \mathcal{N}$ and by $f_i$ its corresponding density function, assuming it exists, an assumption we are going to make repeatedly (removing this assumption is almost always a matter of technicalities and has little to no impact on conceptual questions). We implicitly identify the distribution $F_i$ with its cumulative distribution function (cdf) and use both terms exchangeably. We are also going to assume that values $x_i \in {\mathcal X}_i$ are non-negative, i.e. the support of $F_i$ is included in (but not necessarily equal to)  $\mathds{R}_+ = [0,\infty)$. Unless otherwise noted, we assume that $\mathds{E}_{x_i \sim F_i} [x_i] < +\infty$ to get optimality results (and not just $\varepsilon$-optimality). A crucial assumption throughout this survey is that, unless otherwise noted, the values $x_i$ are drawn independently for different $i$'s and hence they are statistically independent as random variables. We shall  denote by $\mathcal{F} = \mathcal{F}^{(n)} =  F_1\otimes \ldots\otimes F_n$ the joint - and hence - product distribution of $x=(x_1,\ldots,x_n)$, the vector of values. 


\medskip

\paragraph{Examples} Typical examples of value distributions are the \emph{uniform} distribution, which is widely used in textbook examples due to its simplicity,  the \emph{exponential} and the \emph{log-normal} distributions as they are similar to some empirical distributions encountered on modern internet platforms. Power law distributions (also known as \emph{Pareto} distributions) are also widely used, as they capture the idea that the value in real time bidding and online advertising comes from few matches of very high quality, such as consumers who recently viewed a product \citep{arnosti2016adverse} (this situation where 20\% of individuals own/generate 80\% of wealth is also referred as the Pareto principle in economics). \emph{Generalized Pareto} distributions are also often used as examples because their virtual value - an important concept we will define later - is linear. 
\begin{definition}[Symmetric setting]
The auction setting is  called \textit{symmetric} if all bidders have the same value distribution.
\end{definition} 

For the sake of clarity, we use pronouns her/she for the seller and he/his for one specific bidder.

\subsubsection*{Assumptions on Value Distributions and Notations}
If $v$ is a vector (of scalars or functions) in $\mathbb{R}^n$, we call $v_{-i}$ the vector in $\mathbb{R}^{n-1}$ that contains all entries of $v$ except the $i$-th one, $v_i$. 
In other words, $v_{-i}=(v_1,\ldots,v_{i-1},v_{i+1},\ldots,v_n)$.  We also use the notation $v_{-i}(j)$ to denote the $j$-th entry of $v_{-i}$. Similarly, the notation  $F_{-i}$ will denote the product distribution of values of all bidders except $i$ and $b_{-i}$ is the vector of all bids except bidder's $i$. 

Finally, we are always going to make the following key default assumption on distributions, unless explicitly noted. Each value distribution $F_{i}$ is assumed to be continuous, supported on some interval $[0,b]$, with $b$ being possibly infinite. Moreover, we assume that $f_i>0$ on $(0,b)$, except possibly on a set of Lebesgue measure 0. 

\medskip

Note that if ${\cal G}_i$ is the cdf of the largest value of a vector $x_{-i}$ drawn according to $F_{-i}$, ${\cal G}_i(t)=\prod_{j\neq i}F_j(t)$. In particular, with our key default assumption on distributions, ${\cal G}_i$ is differentiable and its density is strictly positive except possibly on a set of measure zero. 

When we say that a function $\beta$ is increasing, we use the standard convention that it means that if $l>u$, $\beta(l)>\beta(u)$. A non-decreasing function is such that if $l>u$, $\beta(l)\geq \beta(u)$.

We use $\partial f$ to denote the subdifferential of a convex function $f$ (see \cite{HULLbook01}, Chapter D). 

\nek{this is ongoing and needs to be completed}

{\color{red} Faudrait finir cette section}


%{\color{red} VP: Je pense qu'il faut elaborer un peu sur le "typical". Ca veut dire quoi exactement ? Soit on met des refs, soit on vire}

%The notion of information owned by the seller and value distribution have progressively changed with several new applications of auction systems. One of the goal of this thesis is to clarify this change and show how sellers and bidders can adapt to this new information structure of the game. For instance, in a repeated setting, where multiple different items are sold successively, the value distribution could also represent the variety of values that a specific buyer can give to one item. 

\subsection{Properties of auction systems}
\label{subsec_prop_auction}
A bidder's \textit{strategy} is the mapping indicating which bids he sends to the seller to buy one specific item, conditional on his private information, a.k.a his value. Stated otherwise, a strategy is a mapping $\beta: \mathcal{X} \rightarrow \mathcal{B}$ that maps private values to bids. %\nek{technical detail: is this mapping possibly random? or is it a function?}
%Bidders have the choice on the bids they send to the seller to get one specific item. A strategy defines how these bids depend on buyer's original private value.
%\begin{definition2}[Strategy]
%A strategy is a function $\beta: \mathcal{X} \rightarrow \mathcal{B}$ that maps private values to bids.
%\end{definition2}
We will denote by $\mathds{B}_i$ the set of all strategies of player $i$, $\beta_i$ the strategy chosen by $i$ and $\beta_{-i}$ the profile of strategies corresponding to all bidders except bidder $i$. %COMMENTED (deja introduit plus haut) Similarly, the notation  $F_{-i}$ will denote the product distribution of values of all bidders except $i$ and $b_{-i}$ is the vector of all bids except bidder's $i$. 

In Bayesian games, it is important to differentiate between \textit{ex ante}, \textit{interim} and \textit{ex post} properties \citep{hartline2013bayesian}. These notions depend on the information available to buyers when they decide to participate in the game and choose their strategy.  
\begin{itemize}
\item For  \emph{ex-ante} properties, bidders do not know yet their own value for the item; i.e. they only know $F_i$ and $F_{-i}$.
\item For \emph{interim} properties, bidders know their valuation but do not know the values of other players, i.e. they know $x_i$ and $F_{-i}$.
\item For \emph{ex-post} properties, bidders know both their and the other players' valuations, i.e. they know  $x_i$ and $x_{-i}$.
\end{itemize}
In the next sections, we will mostly focus on  interim properties. It is the starting point of most of the auction literature: we assume that value distributions are common knowledge and that exact valuations are private information to each bidder.  We will mention  explicitly when  we refer to ex-ante or ex-post properties.

We are also assuming that bidders are risk-neutral. In other words, they seek to maximize their expected utility and use utility-maximizing strategies: %over all other bidders' possible valuations and with respect to their strategies\nek{awkward; need to rephrase; need to def for interim and ex-ante. review that.}.  
Given the strategy $\beta_{-i}$ of other players, the  expected utility  of the strategy $\beta_i$  given bidder $i$'s value $x_i$ is denoted by
$$
U_{i}(\beta_i,\beta_{-i},x_i) = \mathds{E}_{x_{-i} \sim F_{-i}}\Big[u_{i}\big((\beta_1(x_1), \dots,\beta_{i-1}(x_{i-1}),\beta_i(x_i),\beta_{i+1}(x_{i+1}),\beta_n(x_n)), x_i\big)\Big]\;.
$$
%\nek{this is awkward as interim doesn't mean we know other people's strategies... and a strategy is a mapping but technically here we just need to know $\beta_i(x_i)$; also if $\beta_i(x_i)$ included in the stuff?}


\paragraph{Optimality and characterization of strategies} Maybe one of the most central concept in game theory is \emph{(Bayesian) Nash equilibrium}. %It is a characteristic of the vector of strategies $(\beta_1,\ldots,\beta_n)$ and the valuation distributions $F_1,\ldots,F_n$.
 At a Bayesian Nash Equilibrium, for any bidder $i$, his strategy $\beta_i$ maximizes his expected utility, given his valuation distribution $F_i$, and given the strategies of his opponents and their valuation distributions, i.e. $\beta_{-i}$ and $F_{-i}$. A stronger concept is that of \emph{weak dominance}: a strategy  $\beta_i$ is weakly dominant when it is optimal in terms of expected utility of bidder $i$ against any strategies used in $\beta_{-i}$ and not only those at a Bayesian Nash Equilibrium. The strongest concept is ex-post dominance, where optimality is achieved at any possible profile of valuations.
\begin{definition2}
\begin{itemize}
\item \emph{Nash equilibrium:} 
A profile of strategies $(\beta_{1},\dots,\beta_{n})$ is \textit{a Bayesian Nash equilibrium} if for all players $i \in \mathcal{N}$, 
\begin{equation*}
\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \quad U_{i}(\beta_i,\beta_{-i},x_i)  \geq U_{i}(\beta,\beta_{-i},x_i) \;.
\end{equation*} 
\item \emph{Weak dominance:} A strategy $\beta_i$ is  weakly dominant for player $i \in \mathcal{N}$ if
\begin{equation*}
\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \forall \beta_{-i} \in  \mathds{B}_{-i}, \quad U_{i}(\beta_i,\beta_{-i},x_i)  \geq U_{i}(\beta,\beta_{-i},x_i) \;.
\end{equation*}
\item \emph{Ex-Post Weak dominance:} A strategy $\beta_i$ is  ex-post weakly dominant for player $i \in \mathcal{N}$ if
\begin{equation*}
%\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \forall \beta_{-i} \in  \mathds{B}_{-i}, \forall x_{-i} \in \mathcal{X}^{N-1},\quad u_{i}((\beta_1(x_1),\dots,\beta_i(x_i),\dots,\beta_N(x_N)),x_i)  \geq u_{i}((\beta_1(x_1),\dots,\beta(x_i),\dots,\beta_N(x_N)),x_i) \;.
\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \forall \beta_{-i} \in  \mathds{B}_{-i}, \forall x_{-i} \in \mathcal{X}^{N-1},\quad u_{i}((\beta_i(x_i),\beta_{-i}(x_{-i})),x_i)  \geq u_{i}((\beta(x_i),\beta_{-i}(x_{-i})),x_i) \;.
\end{equation*}
\end{itemize}
\end{definition2}

%
%
%A strategy which is optimising the expected utility of one bidder for any valuation and for any strategies of the other bidders is said dominant. 
%\begin{definition2}[(Weakly) dominant strategy]
%A strategy $\beta^{*}$ is  ex-post weakly dominant for player $i$ if for all $\beta_{-i} \in  \mathds{B}^{N-1}$, for all $\beta \in \mathds{B}$ and for all $x \in X^{N}$:
%
%\end{definition2}

Those properties of strategies are classical concepts in game theory. On the other hand, it is also possible to introduce and study different properties of mechanisms. Some of them require the concept of \emph{``truthful bidding''} which correspond to the specific strategy $\beta_i(x)= x$. We will denote by $\beta_{i,\text{tr}}$ this truthful strategy.


\paragraph{Characterization of mechanisms}
\begin{definition2} A mechanism is
\begin{description}
\item[(BIC)] Bayesian Incentive-Compatible:  if bidding truthfully for all bidders is a Bayesian Nash equilibrium.
\item[(DSIC)] Dominant Strategy Incentive-Compatible:  if bidding truthfully is a weakly dominant strategy for all bidders.
\item[(Standard)] if it allocates the item to the buyer with the highest bid.
\item[(Efficient)] if it allocates the item to the buyer with the highest valuation (at least at some equilibrium).
\item[(IR)]  interim Individually-Rational: if 
\begin{equation*}
\forall \, i \in \mathcal{N}, \; \forall x_i \in \mathcal{X}_i, \quad U_{i}((\beta_{i,\text{tr}}, \beta_{-i,\text{tr}}),x_i) \geq 0\;.
 \end{equation*}
 and ex-post Individually-Rational: if 
 \begin{equation*}
\forall \, i \in \mathcal{N},\; \forall x_i \in \mathcal{X}_i,  \forall x_{-i} \in \mathcal{X}_{-i}, \quad u_{i}\big((x_i, x_{-i}), x_i\big) \geq 0\;.
\end{equation*}
\end{description}
\end{definition2}

A DSIC mechanism is obviously a BIC mechanism. More generally,  Incentive Compatible (IC) auctions have the nice property of being ``simple'' for the buyers from a strategic standpoint:  bidding their (known in the interim setting) valuation is optimal for them. Notice  that this unfortunately does not ensure the uniqueness of the equilibrium where each bidder bids truthfully (we will call this equilibrium the  \textsl{truthful equilibrium}). See Section \ref{sec:NashIsDifficult} for more details. \nek{move that to section \ref{sec:NashIsDifficult}} Indeed, there exist many other equilibria such as the following one: every bidder always bids 0 except one of them bidding arbitrarily high\nek{this is unclear; this is really an example with unif[0,1], one bids zero one bids one. given the strategy of the other, second price is dsic. but obviously non-uniqueness of equilibrium.Probably give this example later after intro 2nd price; and point to it now}. Those are pathological equilibria and will be discarded in the following. As we will see later on, being DSIC is one of the main reasons explaining the tremendous success of second-price auctions in practice. Another reason is that if bidders are bidding truthfully, then the seller can, in a first step, elicit their value distributions through a DSIC mechanism and then  move to another  mechanism that maximizes her revenue (this is detailed in Section \ref{Section:RevenueMax}).

% - even if it is at the cost of efficiency\nek{efficiency as in what?}.


 
\medskip
Finally, before presenting and analyzing two classical types of auction, we indicate that individual rationality simply ensures that bidders have an interest in taking part in these auctions.

\section{Sealed-bid auctions}
In a sealed-bid auction bidders privately send their bid to the seller. We present below two of the most well-known sealed-bid auctions, the \emph{second-price} and the \emph{first-price} auctions. This class of auctions does not include the well-known - in popular culture -  ascending auction, a.k.a English auction, where bidders can observe bids from other bidders and progressively choose to increase their bids until only one bidder remains. On the other hand,  if bidders' valuations are independent, there exists a strategic-equivalence between the ascending and the second-price auction. 
\subsection{The sealed-bid second-price auction}
The second-price auction allocates the item to the highest bidder who pays the highest bid among other bidders, i.e., the second highest bid. A key property of this auction is the following result \citep{vickrey1961counterspeculation}, which does not require any assumption on bidders' value distributions. 

\begin{theorem2}
The second-price auction is DSIC. In other words, bidding truthfully is weakly dominant. 
\end{theorem2}
\begin{proof}
Let us denote by $x_i$ the private value of bidder $i$ and by $b^*_{-i}$ the highest bid of the competition. We are going to compare the utility of bidding  $b$ instead of $x_i$.
\begin{itemize}
\item Case $b > x_i$. The only case where his (ex-post) utility is changed is when $x_i < b^*_{-i} < b$. With a bid $b$, he now wins the auction but his utility is negative since $x_i - b^*_{-i} < 0 $.
\item  Case $b < x_i$. The only case where his (ex-post) utility is changed is when $x_i > b^*_{-i} > b$. With a bid $b$, he now loses a profitable  (i.e. with a positive utility) auction.
\end{itemize}
Hence, bidder $i$ has no incentive to deviate  from truthful bidding. 
\end{proof}
The classical second-price auction was used until recently \citep{feng2020reserve} by most of the biggest online platforms to sell ad placements on publishers' websites. Another widely used and studied sealed-bid auction is the first-price auction.
\subsection{The sealed-bid first-price auction} 
\label{first-price-auction}
The first-price auction allocates the item to the highest bidder who pays his own bid.

\medskip

Before studying Nash equilibria of symmetric first-price auction, we derive the general best reply of player $i$ to the bid distribution of the competition, specifically the distribution of the maximum bid of the competition. This result is of increasing interest to practitioners as many online auctions are now first price auctions.

\begin{proposition2}\label{Prop:BestReply1st}
	Let $G_i$ be the cdf of the highest bid of the competition of bidder $i$, i.e. $\max_{j\neq i} b_j$. 
In a sealed-bid first price auction, a best response of bidder $i$  to $G_i$ is the function $\beta_i$ defined by
\begin{equation*}\label{eq:bestresponsefirstpriceSemiAbstract}
%\beta(x_i):  \beta(x_i)=b(x_i) \text{ where } b(x_i)\in \argmax_{b \in \mathbb{R}} G_i(b)(x_i-b)\;.    COMMENT: trop complique
\beta_i(x_i) \in \argmax_{b \in \mathbb{R}} G_i(b)(x_i-b)\;.   
\end{equation*}
When $G_i$ is log-concave and $G_i(x_i)>0$, the best response is unique.  If we further assume that $G_i$ has a pdf $g_i$, first order conditions also give, if $G_i(x_i)>0$, 
\begin{equation*} \label{eq:bestresponsefirstprice}
\beta_i(x_i)  \text{ is a solution (in }b \text{) of } b + \frac{G_{i}(b)}{g_{i}(b)}= x_i\,.
\end{equation*}
If $G_i(x_i)=0$ a best response is $\beta_i(x_i)=x_i$.

 \end{proposition2}
Calling $Y_{-i}$ a random variable with cdf $G_i$, it can also be shown that under mild technical conditions that $\beta_i$ is increasing and satisfies the equation $\beta_i(x)=\Exp{\beta_i^{-1}(Y_{-i})|Y_{-i}\leq \beta_i(x)}$. We also have the following interesting corollary.

\begin{corollary2}\label{coro:1stPriceNotBIC}
Proposition \ref{Prop:BestReply1st} implies that the first price auction is in general not BIC.	
\end{corollary2}
The corollary simply follows by  showing that the best response of bidder $i$ when all other bidders bid truthfully (and hence the top bid of the competition is the largest value of the other bidders) consists in bidding something else than $x_i$. If $G_i(x_i)>0$ it follows immediately than they are better strategies than bidding $b_i=x_i$~: for instance, take any $\tilde{b}_i$ such that $G_i(\tilde{b}_i)=G_i(x_i)/2$ ($\tilde{b}_i$ exists by continuity of $G_i$ and $G_i(a_i)=0$). The utility of bidder $i$ is strictly positive at $\tilde{b}_i$ and is 0 at $x_i$. 
\begin{proof}
Let us denote by $B_{-i}$ the random variable corresponding to the maximum bid of the competition of bidder $i$, so that its cdf and pdf are $G_i$ and $g_i$.

When bidder $i$ has private value is $x_i$ and bids $b_i$, the utility he derives from the auction is $u_i(b_i,x_i)=(x_i-b_i)\mathds{1}\{b_i>B_{-i}\}$; in other words, it is his value minus his cost when he wins the auction and zero otherwise. 

We denote by $\mathcal{U}_i(b_i,x_{i}):\mathds{R}^{+}\times\mathds{R}^{+}\rightarrow \mathds{R}$ the associated expected utility of bidder $i$ when his private value is $x_i$ and he bids $b_i$. We have 
$$
\mathcal{U}_i(b_i,x_i) = \mathds{E}_{B_{-i}}\Big[(x_i-b_i)\mathds{1}\{b_i>B_{-i}\}\Big] = G_i(b_i)(x_i-b_i)\;.
$$
A best response is therefore any $b(x_i)\in \argmax_{b\in \mathds{R}^+}G_i(b)(x_i-b)$. Note that when $G_i$ is log-concave and $G_i(x_i)>0$, we can verify by inspection that $\mathcal{U}_i(b_i,x_i)$ is strictly log-concave in $b_i$ on the support of $F_i$  and therefore it has a unique maximum smaller than $x_i$ \citep{boydvandenberghe04}. This property follows also immediately from the definition of a strictly concave function.

Note that since $G_i$ has a pdf, it is continuous and differentiable and therefore so is $\mathcal{U}_i(b_i,x_i)$ as a function of $b_i$. 
The derivative with respect to $b_i$ is then equal to 
$$
\frac{\partial \mathcal{U}_i}{\partial b_i}(b_i,x_i) = g_i(b_i)(x_i-b_i) - G_i(b_i).
$$
Let us assume that $G_i(x_i) >0$, then $\mathcal{U}_i(x_i,x_i)=0$ but $\left.\frac{\partial \mathcal{U}_i(b_i,x_i)}{\partial b_i}\right|_{b=x_i} <0$. This first implies by continuity that there exists  bids where the utility is positive. Rolle's theorem applied to $t\mapsto G_i(t)(x_i-t)$ also gives the existence of a stationary point $b_i^* \leq x_i$ where  $\frac{\partial \mathcal{U}_i}{\partial b_i}(b^*_i,x_i) =0$, as $\mathcal{U}_i(0,x_i)=0$, too (since we assumed non-negative bids). 
Since we showed above that $\mathcal{U}_i(b_i,x_i)$ is  positive somewhere in a neighborhood of $x_i$, then necessarily  $\mathcal{U}_i(b_i^*,x_i)>0$. Finally, if $g_i(b^*_i)=0$ then this  would imply that  $G_i(b^*_i)=0$ to satisfy the first order condition and therefore $\mathcal{U}_i(b_i^*,x_i)$ would be equal to 0 which is impossible.

The case where $G_i(x_i)=0$ is trivial as bidder $i$ cannot have a positive utility (recall that $G_i$ is a non-decreasing and non-negative function, so $0\leq G_i(b_i)\leq G_i(x_i)$ if $b_i\leq x_i$). Bidding $x_i$ is then optimal.
\end{proof}


There is a very rich line of work focusing on deriving Nash equilibria in first-price auctions when bidders have different value distributions. This involves solving complex systems of coupled first-order differential equations (at least with continuous value distributions, see \cite{krishna2009auction}, Section 4.3; see also p. \pageref{thm:SystemEquiAsymetricFirstPrice}). On the other hand, with symmetric bidders, i.e. with identical value distributions, it is possible to solve explicitly this system of equations and to derive the unique symmetric  Nash equilibrium with increasing strategy. From now on, we will call an Nash equilibrium  \emph{increasing} if the  strategies  are all increasing mappings. 
\begin{theorem2}%[Nash equilibrium in a first-price auction]
In the symmetric case, where all bidders  have the same cdf $F$, if the pdf $f$ is such that $f(x)>0$ (except  on a set of Lebesgue measure 0 within the support of $F$), there exists a symmetric increasing Nash-equilibrium whose strategy is described by:  
\begin{equation*}
\beta(x) = \mathds{E}[X^{(1)}_{-i} | X^{(1)}_{-i} < x]\;.
\end{equation*}
where $X^{(1)}_{-i}$ is the highest value among bidders except bidder $i$.
\end{theorem2}
% \nek{tech question: if we assume $f>0$ then $\beta$ is increasing and we have zero problems below. If $f\geq 0$, $\beta$ is only non-decreasing; then we have to deal with possible ties, how to break them and make sure that the PWin is $G_i(x)$. when they all bid $\beta(x_j)$ I haven't done this. this minor tech stuff would preferably done in an appendix; probably need to replace $x_j$ by $x_j^-$, i.e. the $inf_x F(x)=t$. I leave the proof with non-decreasing but worth a check}.
This bidding strategy can be interpreted as bidding the expectation of the largest value of the competition, conditionally on the fact that this value is smaller than bidder $i$'s value. We note that this bidding strategy can be derived from the proof of the revenue-equivalence Theorem \ref{Th:RevEquivalence}, and specifically the expected payment formula. This is another common method for finding equilibrium bidding strategies. The proof presented below might lead more directly to the solution.  
\begin{proof}
We assume that $n\geq 2$ and that all bidders are using the function $\beta$ described above. As we will show below, this function is increasing on the support of $F$ under our assumptions. Furthermore  when all bidders are using the same \emph{increasing} strategy on the union of the support of their value distributions, the probability that bidder $i$ wins the auction is the same as the probability that he has the highest value; this would not always be true if the strategy were only non-decreasing. 

Furthermore, elementary properties of conditional expectations give, if $G_i$ and $g_i$ are the cdf and pdf of $X_{-i}^{(1)}$,
$$
\beta(x)=\beta_i(x)=\frac{\int_{0}^{x} y g_i(y) dy}{G_i(x)}=x-\frac{\int_0^x G_i(u)du}{G_i(x)}\;, \text{ whenever } G_i(x)>0\;.
$$
Under our assumptions, $G_i=F^{n-1}$ and hence $g_i(x)=(n-1)f(x)F^{n-2}(x)$. Note that under our assumptions $g_i(x)>0$ on the support of $F$, except possibly on a set of Lebesgue measure 0, and thus  $\beta'(x)=\frac{g_i(x)\int_0^x G_i(u)du}{[G_i(x)]^2}$. Hence, restricted to the support of $F$, $\beta$ is a non-decreasing function whose derivative is 0 on a set of Lebesgue measure 0 . We conclude that $\beta$ is actually increasing on the support of $F$ under our assumptions. 

We denote by $x_i$ the private value of bidder $i$, by $b_i$ his bid and by $H$ the supremum of the support of $F$. Bidder $i$ has no incentive to bid higher than $\beta(H)$~: suppose he did bid $b>\beta(H)$. Clearly since the other bidders bid according to $\beta$, their maximum bid is lower than $\beta(H)$. Then, bidding $b$, bidder $i$'s probability of winning the auction would be 1 and his cost $x-b$. He could achieve the same probability of winning by bidding $\beta(H)$ but his cost would be lower~: $x-\beta(H)$. Then, any other bid $b$ will satisfy $b \in [0,\beta(H)]$ and since $\beta(0) =0$ and $\beta$ continuous (because $F$ is continuous and by construction of $\beta$), there exists $z \in [0,H]$ such that $b = \beta(z)$. Finally, note that the probability that bidder $i$ wins the auction when bidding $\beta(z)$ is just $G_i(z)$, since $\beta$ is increasing on the support of $F$. Therefore,
\begin{align*}
\mathcal{U}_i(\beta(x),x) - \mathcal{U}_i(b,x) &= \mathcal{U}_i(\beta(x),x) - \mathcal{U}_i(\beta(z),x)
\\&= G_i(x)\left(x - \frac{\int_{0}^{x} y g_i(y) dy}{G_i(x)}\right) - G_i(z)\left(x - \frac{\int_{0}^{z} y g_i(y) dy}{G_i(z)}\right)
\\&= x(G_i(x) - G_i(z)) + \int_{x}^{z} y g_i(y) dy = 
\int_x^z(y-x)g_i(y)dy 
\geq 0\;.
\end{align*}
This shows that the best response  is $\beta$, therefore, $(\beta,\dots,\beta)$ is a symmetric (increasing) Nash equilibrium.   We will prove unicity of this increasing differentiable symmetric Nash equilibrium in symmetric first-price auctions in Section \ref{sec_rev_equi}. 
\end{proof}

Unlike second-price auctions, first price auctions are not incentive compatible (see e.g. Corollary \ref{coro:1stPriceNotBIC}). As a consequence, the strategy of a bidder at an equilibrium  depends on the bidding strategy of the other bidders, and ultimately on other bidders' valuation distributions (see Proposition \ref{Prop:BestReply1st}). So in practice, computing a good or optimal bidding strategy would require estimating the distribution of the highest bid of the competition, which can be very challenging. Nevertheless, because of their relative transparency for bidders (who know ahead of time what they might pay if they win), first-price auctions are increasingly used in online advertising auctions \citep{feng2020reserve}. However, optimal bidding becomes much more complex for bidders than it is in second price or other BIC/DSIC/``truthful'' auctions.
\paragraph{Nash equilibrium in the asymmetric case}

Asymmetric first price auctions are much more intricate than symmetric ones as  the equilibrium strategy of each  bidder depends in a very subtle manner of the other bidders' strategies  \citep{LebrunFirstPriceAsymmetric1999}. Indeed, let us assume that the distributions $F_1,\ldots,F_n$ are supported on $[h,H]$, have a density  bounded away from 0 on $(h,H)$ and possibly have a point mass  at $h$. 
%This assumption comes from practical  -- as many auctions have 0 value to online advertisers -- and technical -- if a common reserve price is set at $r>h$, then distributions can be assumed to be  supported on $[r,H]$ with a point mass at $r$  \citep{LebrunFirstPriceAsymmetric1999}. 
\begin{theorem2}[\cite{LebrunFirstPriceAsymmetric1999}]\label{thm:SystemEquiAsymetricFirstPrice}
Under these  assumptions, there exist deterministic Nash equilibrium strategies that are increasing. Let us denote them by $\beta_i$ and by $x_i(b)=\beta_i^{-1}(b)\geq b$ their inverse, i.e. the value inducing the bid $b$. Then the increasing functions $b\rightarrow x_i(b)$ solve  the system of differential equations : 
\begin{equation}\label{eq:equilibrium1stPriceAsymmetric}
\forall \, i \;, 1\leq i \leq n\;, \frac{\partial}{\partial b}\log(F_i(x_i(b)))=\frac{-1}{x_i(b)-b}+\frac{1}{n-1}\sum_{j=1}^n \frac{1}{x_j(b)-b}\;. 
\end{equation}	
When the distributions are without atoms, the boundary conditions are 
$x_i(h)=h$ for all $i \in \mathcal{N}$, and there exists $\eta>0$ such that for all $i$, $\beta_i(H)=\eta$. 
\end{theorem2}
The boundary conditions mean that bidders bid their value at $h$ and have a common maximal bid \citep{FibichGaviousAsymmetricFirstPricePerturbApproach2003}.
\paragraph{Numerical issues in computing Nash equilibrium}
Finding the solution to the differential system \eqref{eq:equilibrium1stPriceAsymmetric} is considered hard essentially because the solutions are unstable near the boundary \citep{MarshallNumericalAnalysis1stPrice94}. The case of $n=2$ bidders has received a fair amount of attention both from both theoretical and numerical perspectives \citep{FibichGaviousDynamicalSystem2012}. Another approach finds yet another form of the differential system of equations and expands the functions appearing in it in a fixed polynomial basis.  \citep{NumericalSolutionsFirstPriceGayle2008}. 
\section{A revenue equivalence theorem}
\label{sec_rev_equi}
Revenue equivalence theorems are general results showing that different auction systems  -- sharing nonetheless some properties -- are equivalent in terms of expected revenue \emph{at a specific equilibrium}.  The first revenue equivalence theorem showed that the sealed-bid second-price auction and the ascending/English auction lead to the same revenue for the seller \citep{vickrey1961counterspeculation}. This result was later extended to all standard auctions - under rather minimal assumptions. 



\begin{theorem2}%[Revenue equivalence]
\label{Th:RevEquivalence}
Consider the family of auctions that are both

 i) \textsl{standard} (i.e. the winner is the bidder with the highest bid)

 ii) \textsl{0-rational} (i.e. winning the auction with a bid of 0 induces a payment of 0).

\noindent When all bidders have the same value distribution, %and their bids are statistically independent,
 i.e. in the symmetric case, the seller's expected revenue and bidders' expected utilities at a symmetric increasing Nash equilibrium are independent of the  specific payment rule. 
\end{theorem2}
\begin{remark2} The revenue equivalence Theorem \ref{Th:RevEquivalence} applies in particular to first and second price auctions, in the symmetric case where all bidders have the same value distribution \citep{Myerson81} and use an increasing strategy at equilibrium. The revenue equivalence theorem assumes that bidders have all the same value distributions. There exists asymmetric cases where the first-price auction brings more revenue than the second-price auction and vice-versa (\cite{krishna2009auction}, Section 4.3.2). 
\end{remark2}
\begin{proof} 
Given a specific standard auction, let $\beta$  be a  strategy at an increasing symmetric Nash equilibrium. Let us denote by $P(t)$ the corresponding expected payment of bidder~$i$ when he bids $\beta(t)$ and the other bidders are using the same strategy $\beta$. As before, we  denote by $G_i$ the distribution of $X^{(1)}_{-i}$, the highest value among all the bidders except bidder $i$. Using the fact that $\beta$ is increasing, that all players use this strategy - at the Nash equilibrium -  and the fact that the auction is standard, the probability that bidder $i$ wins when he bids $\beta(t)$ is $G_i(t)$.

We can still assume that a deviation of bidder $i$ consists in  bidding $\beta(z)$ instead of $\beta(x_i)$ because the auction is standard and $\beta$ is increasing.  In particular, the expected utility for bidder $i$ of this deviation can be written as
\begin{align*}
\mathcal{U}_i(z,x_i) = x_iG_{i}(z) - P_i(z)\;.
\end{align*}
% If $p_i(t,x_{-i})$ is the payment of bidder $i$ when bidding $\beta(t)$ and the other players have value $x_{-i}$,
% $$P_{i}(t) =  \mathds{E}_{F_{-i}}\Big[p_i(t_i,x_{-i})\Big] = \int_{\mathcal{X}_{-i}} p_i(t,x_{-i})f_{-i}(x_{-i})dx_{-i} \;.$$

Since $\beta$ is a strategy corresponding to a Nash equilibrium, bidder $i$'s expected utility is maximized when he bids $\beta(x_i)$ and hence 
$$
\mathcal{U}_i(x_i,x_i) =\max_{z} \mathcal{U}_i(z,x_i) =\max_{z}  \, x_iG_i(z) - P_i(z)  \;.
$$
We denote ${\mathcal V}(x_i)=\mathcal{U}_i(x_i,x_i)$. 
Clearly $x_i \mapsto \mathcal{V}_i(x_i)$ is convex - as a max of linear and hence convex functions - and hence almost everywhere differentiable \citep{HULLbook01}, p. 115). Recall also that (Lemma 4.4.1 in \citep{HULLbook01}, p. 188) the subdifferential at a point $x$ of a supremum of convex functions contains the convex hull of the subdifferentials of the functions achieving this supremum (and is empty if the supremum is not achieved). Here the functions we consider have a very simple differential in $x$: it is simply $G_i(z)$. This suggests informally that when $\mathcal{V}$ is differentiable, ``${\mathcal V}'(x)=G_i(z^*(x))$", where $z^*(x)=\argmax_z \mathcal{U}_i(z,x)$. In particular in our case it suggests that ``${\mathcal V}'(x)=G_i(x)$". The envelope theorem allows us to make this intuition formal. 

The envelope Theorem in its Theorem 2 form in \citep{MilgromSegal2002} applies because $\mathcal{U}_i(z,\cdot)$ is linear for all $z$ and hence differentiable and therefore absolutely continuous. Furthermore $\frac{\partial \mathcal{U}_i(z,x)}{\partial x} =G_i(z)\in[0,1]$ for all $z$. Since the max of $z\mapsto \mathcal{U}_i(z,x_i)$ is attained for $z=x_i$ at the Nash equilibrium, the envelope theorem then gives 
$$
{\mathcal V}(x)-{\mathcal V}(0)=\int_0^{x}G_i(u)du\;.
$$
However, almost by definition, ${\mathcal V}(x)-{\mathcal V}(0)=xG_i(x)-P_i(x)+P_i(0)$. 
Thus, since $P_i(0)=0$ because of 0-rationality, we finally get that, by integration by parts,
$$
P_i(x)=P_i(0)+xG_i(x)-\int_0^x G_i(u)du = \int_0^x tdG_i(t) dt=G_i(x)\mathds{E}[X^{(1)}_{-i}|X^{(1)}_{-i} < x]\;.
$$
%\iffalse
%\nek{I changed the argument to above}
%Assuming differentiability, it  holds that, since $\mathcal{U}_i(z,x_i)$ attains its maximum at $x_i$, 
%\begin{equation*}
%\left.\frac{\partial \mathcal{U}_i}{\partial z} (\cdot,x_i)\right|_{z=x_i} = x_ig_i(x_i) - P_i'(x_i) = 0\;.  
%\end{equation*}
%Thus, since $P_i(0)=0$ because of 0-rationality, we finally get that
%\begin{equation*}
%P_i(x) = P_i(0) + \int_{0}^{x} sg_i(s)ds = G_i(x)\mathds{E}[X^{(1)}_{-i}|X^{(1)}_{-i} < x]\;.
%\end{equation*}
%In the case where $\mathcal{U}_i$ is not everywhere differentiable, the same argument holds using standard mean-value theorems for the subdifferential \citep{HULLbook01}, pp.178-180. \nek{check with Thomas, Vianney, Clem} \nek{note to thomas: there's a slight confusion around the function of the first variable and the function $\gamma(x_i)=\mathcal{U}_i(x_i,x_i)$}
%\nek{keep below}
%\fi
Hence the expected payment of bidder $i$ is independent of the specific auction format. As a consequence, so are  the expected seller's revenue and the expected utility of bidder $i$, because the auction is standard.
%\iffalse
%Finally, we assumed in the proof that $P$ is  differentiable (for the sake of simplifying the exposition). This assumption is not necessary and can be removed using the convexity of $x_i \mapsto \mathcal{U}_i(x_i,x_i)$ in a way that is similar to the proof of the more general Theorem \ref{Th:MyersonLemma}. \nek{je pense qu'il faut faire très gaffe; l'exemple d'Hartline a un payoff discontinu (a l'equilibre je sais pas parce que son contre example est faux)}
%\fi

\end{proof}




\begin{remark2} 
This proof shows a principled way to get necessary conditions on bidding strategies forming an increasing Nash equilibrium, through the payment formula derived above.
% COMMENT : c'est fait juste apres
%Finally, a maybe more informal but perhaps more intuitive derivation of this result is the following. Assuming differentiability of $P_i(z)$ and $G_i(z)$, it holds that, since $\mathcal{U}_i(z,x_i)$ attains its maximum at $x_i$, 
%\begin{equation*}
%\left.\frac{\partial \mathcal{U}_i}{\partial z} (\cdot,x_i)\right|_{z=x_i} = x_ig_i(x_i) - P_i'(x_i) = 0\;.  
%\end{equation*}
%Thus, since $P_i(0)=0$ because of 0-rationality, we get 
%\begin{equation*}
%P_i(x) = P_i(0) + \int_{0}^{x} sg_i(s)ds = G_i(x)\mathds{E}[X^{(1)}_{-i}|X^{(1)}_{-i} < x]\;.
%\end{equation*}
\end{remark2}



\subsubsection{Informal derivation of symmetric first-price auction equilibrium strategy} The proof of Theorem \ref{Th:RevEquivalence} is a bit formal and technical as it relies on convex analysis arguments; however, it provides insight on how to easily and informally derive symmetric equilibrium. Denote by $\beta$ the common strategy of an increasing Nash equilibrium of the first-price auction, postulated at this point for this informal derivation to exist. Note that by symmetry, $G_j=G_i=G$ for all $i,j$ and similarly for the pdfs. So we use the notations $G$ and $g$ for cdf and pdf below. Conducting the same computations as in the proof of Theorem \ref{Th:RevEquivalence}, assume that all bidders  but $i$  follow $\beta$ and that bidder $i$ is bidding $\beta(z)$ instead of $\beta(x_i)$  rewrites his utility in the specific case of first price auction as 
\begin{equation*}
\mathcal{U}_i(\beta(z),x_i) = (x_i - \beta(z))G(z)\;. 
\end{equation*}
Since $\beta$  is a  symmetric increasing Nash equilibrium,  the maximum utility is attained by bidding $b=\beta(x_i)$. Differentiating with respect to $z$, temporarily assuming that $\beta$ is differentiable, then yields 
\begin{equation*}
0=\left.\frac{\partial \mathcal{U}_i}{\partial z} (\beta(z),x_i)\right|_{z=x_i} = (x_i-\beta(x_i))g(x_i) - \beta'(x_i)G(x_i)\;.
\end{equation*}
Notice that the above equation can be rewritten in the more compact form
\begin{equation*}
(\beta(x)G(x))' = xg(x)\;.
\end{equation*}
Integrating the above equation and using the fact that $G(0)=0$, we can compute explicitly the symmetric equilibrium strategy
\begin{equation*}
\beta(x) = \frac{\int_{s=0}^{x}sg(s)ds}{G(x)}= \mathds{E}[X^{(1)}_{-1}|X^{(1)}_{-1}<x]\;.
\end{equation*}
We can verify as posteriori that $\beta$ is differentiable and increasing when $g>0$. 

This also proves the uniqueness of  increasing differentiable Nash equilibria  in a symmetric first-price auction. 



% \begin{remark2} The system of equations corresponding to the Nash Equilibrium in the asymmetric setting presented in Theorem \ref{thm:SystemEquiAsymetricFirstPrice} can actually be easily deduced by applying the same perturbative approach.\nek{this is very unclear; we should drop it I think or do it} \end{remark2}

\section{Deriving revenue-maximizing auctions}
\label{Section:RevenueMax}
We now focus on how the seller can design her auction system to maximize her revenue. A large part of the recent literature on auctions have focused on this objective since most of the auctioneers have a choice in designing the rules of their respective auction platforms.

To compute the optimal revenue-maximizing auction, we assume that the seller has prior knowledge on the distribution $F_i$ on each bidders' valuations.  These value distributions quantify the information that the seller has on each bidder. 

\subsection{The role of reserve prices}
Setting reserve prices is a crucial tool used to improve or maximize seller's revenue in classical auctions. To illustrate its role, we focus on  second-price auctions. 
\begin{definition2}
The reserve price is the minimum price a bidder must pay to acquire an  item. The reserve price is  \textit{anonymous} (respectively, \emph{personalized}) if it is the same for all bidders (resp., if it is different from one bidder to the other).
\end{definition2}
In a second-price auction with reserve prices the buyer that wins the auction must have bid above his reserve price. He then pays the maximum between his reserve price and the second highest bid. A crucial and perhaps surprising point  is that, in expectation,  it can be beneficial for the seller to sometimes not allocate the item. However, whenever the item is sold, the payment is higher with this reserve price than without. 

To illustrate this point, we quickly recall a historical example, the New-Zealand radio spectrum rights auction \citep{milgrom2004putting}. In 1990, the NZ government decided to sell some radio spectrum rights through multiple simultaneous sealed-bid second-price auctions without reserve prices for the corresponding licenses. These auctions were expected to raise around NZ\$250 million. Instead, the government revenue was around NZ\$36 million. On many licenses, there was a huge discrepancy between the first and the second bid. For instance, a firm bid NZ\$100 000 and the second price was only NZ\$36\dots If reserve prices had been set beforehand, it would have ensured to the government that the firm who made a bid of NZ\$100 000 would have paid a price sufficiently high. This example illustrates the importance of setting reserve prices. A first way to do it would be to assume that the seller can compute an intrinsic value for keeping the item. This could be a reasonable assumption for housing or wine auctions. However, in many other situations (TV rights, radio spectrum rights auctions..), the seller does not have any intrinsic value for the item. 

For illustration purpose,  we will compute in the following the optimal reserve price in the simple case of a single buyer. As before, we denote by $F$ the cdf of the buyer valuation, and for the sake of simplicity, we assume it has a density $f$ (again, all the following results generalize to arbitrary distributions, but at the cost of technicalities) and has finite expectation.


%\iffalse and the need for a careful modelisation of the different incentives of the system. {\color{red}VP: la phrase suivante est moche, et il faut une reference et/ou plus d'explications} For instance, in the recent sell of French football TV rights, in 2017, the auctioneer was very careful on its definition of the reserve prices by setting very specific reserve prices for every TV rights packages. 
%\fi
\subsection{The posted price setting: monopoly pricing}
\label{monopoly-pricing}
In this  particularly simple through practically very common setting, designing an auction simply reduces to  a \textit{take-it-or-leave-it} offer, also called \emph{posted price}. In other words, a fixed selling price is offered and a rational bidder will accept to pay it to acquire the item if and only if the price is smaller than his valuation. 
\begin{lemma2}\label{TH:Monopoly}
In a posted price setting, the seller's expected revenue is 
\begin{equation} \label{eq:defPiOfr}
\Pi(r) = r(1-F(r))\;.
\end{equation}
In the same setting, when $F$ is differentiable and has finite expectation, the optimal reserve price, called \emph{the monopoly price}, is a solution of :
\begin{equation*}
0=-[r(1-F(r))]'=rf(r) - (1-F(r)) = f(r)\Big(r- \frac{1-F(r)}{f(r)}\Big)\;. 
\end{equation*}
\end{lemma2}
\begin{proof}
The seller's revenue can be written as a function of $r$ as: in expectation, the seller's revenue is just the fixed price $r$ multiplied by the probability that the buyer buys the item. This latter probability is just the probability that the value of the buyer is above $r$. Formally, if $x$ is the value of the item for the buyer, the revenue of the seller $\Pi(r)$ when selling at the fixed price $r$ is 
\begin{equation*} 
\Pi(r) = r P(x\geq r)=r \int_{r}^{+\infty} f(x)dx = r(1-F(r))\;.
\end{equation*}
The result on the monopoly price follows from differentiating the previous relation, since
\begin{equation*} 
\frac{d\Pi(r)}{dr} = (1-F(r)) - rf(r) \;.
\end{equation*}
Furthermore choosing $r=0$ or $r$ arbitrarily high gives 0 revenue, the latter because $F$ is assumed to have finite expectation, which then implies that $\lim_{t\tendsto \infty} t(1-F(t))=0$ by the dominated convergence theorem. Indeed, if $x$ has distribution $F$, $t(1-F(t))\leq \mathds{E}_{x\sim F}[x\indicator{x\geq t}]\leq \mathds{E}_{x\sim F}[x]<\infty$.  Hence a maximum of the function $\Pi$ exists among its stationary points, finishing the proof. 
\end{proof}
%\iffalse
%\begin{figure}[H]
%\includegraphics[width=.5\linewidth]{images/monopolistic_revenue}
%\caption{Seller's revenue as a function of the reserve price. The revenue is computed based on $r(1-F(r))$ with $F = \mathcal{U}([0,1])$.}
%\end{figure}
%{\color{red} VP: Quel est l'interet du paragraphe suivant ?} 
%The setting of posted price is very related to the setting where a monopolistic firm sells a service to different customers. She must define a single price for all her clients. She will choose the monopoly price corresponding to the distribution of values representing her customers. Sometimes, the firm prefers not to sell the item and sacrifies a bit of short-term revenue to insure that in most other cases, buyers will pay a price sufficiently high.  
%\fi
\bigskip
Notice that without the assumption that $F$ has a finite expectation, the optimal reserve price could be arbitrarily high: take for instance $F(r)=1-r^{-\alpha}$ with $0<\alpha<1$.
Such an example might actually be relevant in luxury items markets.
 
One of the purpose of discussing the single bidder case was to introduce organically the crucial concept of \textit{virtual value} \citep{Myerson81}. 
\begin{definition2}%[Virtual value]
The virtual value function $\psi : \mathcal{X} \to \mathds{R}$ of a distribution $F$ (with pdf $f$) is: 
\begin{equation} \label{eq:defVirtualValue}
%\boxed.  VP: Pourquoi une box ?
{
\psi(x) = x - \frac{1-F(x)}{f(x)}\;.
}
\end{equation}
\end{definition2}
The virtual value function can be either positive or negative, irrespective of the support of the value distribution. The expectation  under $F$ of the virtual value,  i.e. $\mathds{E}_{X \sim F} [ \psi(X)]$, is actually equal to the infimum of the support of $F$, when $F$ has finite expectation. In particular, it is equal to 0 if the support of $F$ ``starts" at 0. 
%\nek{maybe stop here; afterwards it kind of implies that $\psi_F$ is increasing...} and in that case, the virtual value is necessarily sometimes negative (at least around $x=0$) and sometimes positive (at least around the supremum of the support of $F$) \nek{latter is false unless virtual value is assumed to be increasing}.

The virtual value $\psi(x)$ is a crucial concept that can be interpreted as  \emph{virtual payment}, as we explain now. If the bidder has value $x$ and decides to buy the item, so $x\geq r$, his (virtual) payment can be thought of as $\psi(x)$,  \textsl{independently} of the price $r$ set by the seller. Indeed, the revenue generated by such a price $r$ is
\begin{gather*}
\mathds{E}_{X \sim F} [ \psi(X) \mathds{1}\{X \geq r\}]=
\int_r^\infty \psi(x) f(x)dx= \int_r^\infty xf(x) - (1-F(x)) dx \\
= -\int_r^\infty (x(1-F(x)))' dx=
r(1-F(r))=\Pi(r)\;.
\end{gather*}
The last equality comes from the definition of $\Pi(r)$, see Equation \eqref{eq:defPiOfr}. As a consequence, even though it is traditionally called virtual value, $\psi(x)$ could rather be understood as a virtual \textsl{payment}~: the buyer pays on average $\psi(x)$ when his value is $x$ and he buys/wins the item, i.e. $x\geq r$. See also Proposition \ref{prop:virtualValueIsVirtualPaymentGeneralCase} for an explanation of why this interpretation holds for general auction systems and buyers optimizing their expected utility.

\subsubsection{Examples of virtual value functions:} 
\begin{itemize}
\item if $x\sim\mathfrak{U}([0,1])$, the uniform distribution over $[0,1]$, then $\psi(x)=2x-1$ for $x \in [0,1]$.
\item if $x\sim \mathfrak{E}\mathrm{xp}(\lambda)$, the exponential distribution, then  $\psi(x)=x-\lambda$ for $x \in \mathds{R}_+$ ($F(x)=1-\exp(-x/\lambda)$).
\item Generalized Pareto (GP) distributions, parametrized by $(\mu,\sigma,\xi)$ where $\sigma >0$ and $\xi\leq 0$, have cdf 
\begin{equation*}
F_{\mu,\xi,\sigma}(x)   = \begin{cases} 1-(1 +\frac{\xi (x-\mu)}{\sigma})^{-1/\xi} & \text{for } \xi < 0 \\
1-e^{-(x-\mu)/\sigma} & \text{for } \xi= 0\end{cases}\;.
\end{equation*} 
Their virtual value is affine \citep{balseiro2020multistage}
$$\psi_{\mu,\xi,\sigma}(x) = (1-\xi)x+\xi\mu-\sigma$$
\end{itemize}
%\begin{remark2}
%With $\xi = -1 , \mu = 0, \sigma = 1 $, we recover the uniform distribution. With $\xi = 0 , \mu = 0 , \sigma = 1$, we recover the exponential distribution. With  $ \mu = 1, \sigma = \xi$ , this corresponds the power law (a.k.a the Pareto distribution) with parameter $\alpha = 1/\xi$. Hence, the generalized Pareto distribution are widely used in auction theory due to their flexibility (they model a large spectrum of distributions) and the fact that their virtual value is easy to compute (the virtual value is affine).
%\end{remark2}
\subsubsection{Relationship between  monopoly price and virtual value/payment}
Lemma \ref{TH:Monopoly} states that the optimal reserve price against  a single bidder (which was called the monopoly price)  is, in the case where the virtual value/payment function  $\psi$ is increasing and changes sign, necessarily the root of $\psi$ (or the point where the sign changes if $\psi$ is not continuous). If $\psi$ is strictly positive everywhere, which can happen if the  infimum of the support of $F_i$ is positive, then the optimal reserve price is that specific point (or equivalently 0). Note that if $\Pi(t)$ is the expected revenue of the seller at reserve price $t$ (see Equation \eqref{eq:defPiOfr}), $\Pi'(t)=-f(t)\psi(t)$.  Quite interestingly, even with multiple other bidders, the optimal reserve price for bidder $i$ is still $i$'s monopoly price, i.e. the same as if he were the only bidder. This is illustrated in the following Section \ref{optimal_reserve_for_lazy} under the same assumptions of $\psi$ being increasing and/or changing sign once. 

As a consequence, in the following,  our main focus will be on these distributions which are called \textsl{regular}. The results we will prove can be generalized to non-regular distribution with a technique called \textsl{ironing}, see Section \ref{Se:Ironing}.  
 \begin{definition2} 
The distribution $F$ is  regular if the corresponding virtual value $\psi$ is increasing.
\end{definition2}

The uniform, exponential and generalized Pareto distributions with $\xi <1$, are all regular distributions. % 
%\begin{proposition2}
%If $\psi$ increasing and crossing zero exactly once and F is defined over its full support, then r is the monopoly price if and only if
%$$\psi(r) = 0$$ 
%\end{proposition2}
%\begin{proof}
%The monopoly price r is defined as $$\argmax_r R(r) = r(1-F(r)).$$
%Then, 
%$$
%\frac{dR(r)}{dr} = -f(r)\psi(r)\;.
%$$
%Since $\psi$ increasing, R is concave and $\psi(r)=0$.
%\end{proof}
%If $\psi$ is crossing zero multiple times, the monopoly price also verifies $\psi(r)=0$. 
%One of the beauty of auction theory is that this notion of monopoly price can be extended to auctions with multiple buyers.
\subsection{Optimal reserve prices in a second-price auction}
\label{optimal_reserve_for_lazy}
We  focus in this section on second-price auctions with reserve prices \citep{riley1981optimal} where  $n$ buyers are asymmetric, i.e. their value distribution can be different. As a consequence, the seller might also set different, personalized, reserve prices so as to increase her revenue. When introducing the concept of reserve price, we mentioned that a bidder can only win the auction if his bid was higher than his reserve price and that the latter is the minimal payment that bidder might pay. There however remains some ambiguity on how the auction unfolds (depending on which condition ``highest bidders" or ``bid above reserve price" is checked first). As a consequence, there exist at least two different types of second-price auction with reserve prices.

\begin{description}
\item[``Lazy" 2nd-price auction:] The winner can only be the highest bidder. He gets the item only if he  clears his reserve price (i.e. he bids above it), and pays the maximum between his reserve price and the second highest bid overall (regardless of whether the second highest bid cleared its reserve).
\item[``Eager" 2nd-price auction:] Bidders that have not cleared their respective reserve price are  disregarded. Thus the winner is the highest bidder amongst those that have cleared their reserve price and he pays the maximum between his reserve price and the second highest cleared bid.
\end{description}


First of all, notice that if the reserve prices are anonymous, i.e. the same for all bidders, as they should be in the symmetric case for instance, both types of auctions coincide.  Optimal reserve prices are easy to compute in lazy auctions, as they have an explicit form. They are on the other hand hard to compute for eager auctions. Moreover, the eager 2nd-price auction is also not the revenue-maximizing auction for the seller. So this concept is neither simple (as is the lazy auction) nor optimal (as is the Myerson auction, see Section \ref{emp_Myerson}). As a consequence, we will not put too much emphasis on eager auctions. In practice, if one wishes to implement eager 2nd-price auctions, a good idea would be to use the reserve prices of the corresponding lazy 2nd-price auction.



\medskip

It is quite immediate to see that lazy and eager second price auctions are still DSIC mechanism (the proof follows the exact same lines as that without reserve prices), hence we shall again only consider the truthful equilibrium. We now derive the expected payment of a bidder at this equilibrium.
%\begin{theorem2}[Expected payment in a lazy second-price auction]\label{myerson_for_second_price}
%Consider bidder $i$ with virtual value $\psi_i$ and reserve price $r_i$. We denote by $G_i$ the cdf of $Y_{-i} = max_{j\neq i} X_j$. The expected payment $P_i(\beta_{tr})$ of bidder $i$ in a lazy second-price auction when all bidders are bidding truthfully is equal to:
%\begin{equation*}
%P_i(\beta_{tr}) = \mathds{E}_{x_i\sim F_{i}}\bigg(\psi_i(x_i)G_i(x_i)\textbf{1}_{x_i\geq r_i}\bigg)\;.
%\end{equation*}
%\end{theorem2}
\begin{theorem2}\label{myerson_for_second_price}
Let   $P_i$ be the expected payment of bidder $i$ facing reserve price $r_i$ at the truthful equilibrium of a lazy second-price auction. %Assume the bidders are statistically independent. 
Then 
\begin{equation*}
P_i = \mathds{E}_{x_i\sim F_{i}}\Big[\psi_i(x_i)G_i(x_i)\mathds{1}\{x_i\geq r_i\|\Big]\;,
\end{equation*} 
where $G_i$ the cdf of $\max_{j\neq i} X_j$ and $r_i$ is the personalized reserve price of bidder $i$.

\end{theorem2}
\begin{proof} 
Let us introduce the notation $y_{-i}= \max_{j\neq i} x_j$ so that the pointwise payment of bidder $i$, when he has value $x_i$, given all the values $x_j$ is equal to: 
\begin{equation*}
\max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x_i\geq r_i\}\;,
\end{equation*}
We note that 
$$
\max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x_i\geq r_i\}=
\mathds{1}\{x_i\geq r_i\}(r_i\mathds{1}\{y_{-i}\leq r_i\}+\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{ y_{-i}\geq r_i\}y_{-i})\;.
$$
As a consequence,
\allowdisplaybreaks
\begin{align*}
P_i&= \mathds{E}_{F_1,\dots,F_n}\Big[\max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x\geq r_i\}\Big]
\\& = \int_{x_i} \int_{y_{-i}} \max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x_i\geq r_i\}f_i(x_i)g_i(y_{-i})dy_{-i}dx_i
\\& =\Big(1-F_i(r_i)\Big)G_i(r_i)r_i + \int_{x_i=r_i}^{+\infty}\int_{y_{-i}=r_i}^{+\infty}y_{-i}g_i(y_{-i})f_i(x_i)\textbf{1}(x_i \geq y_{-i})dy_{-i}dx_i
\\& = \Big(1-F_i(r_i)\Big)G_i(r_i)r_i + \int_{y_{-i} = r_i}^{+\infty}y_{-i}g_i(y_{-i})\int_{x_i=y_{-i}}^{+\infty}f_i(x_i)dy_{-i}dx_i \hspace{2cm} \text{ (by Fubini)}
\\& = \Big(1-F_i(r_i)\Big)G_i(r_i)r_i + \int_{y_{-i} = r_i}^{+\infty}y_{-i}g_i(y_{-i})(1-F_i(y_{-i}))dy_{-i} 
\\& = \int_{y_{-i} = r_i}^{+\infty} \Big(f(y_{-i})y_{-i} - (1-F_i(y_{-i}))\Big)G_i(y_{-i})dy_{-i} \hspace{2.5cm} \text{(by integration by parts)}
\\& = \mathds{E}_{F_i}\Big[\psi_i(x)G_i(x)\mathds{1}\{x\geq r_i\}\Big]\;.
\end{align*}
\end{proof}
We can therefore easily derive the optimal reserve prices, as a function of $\psi_i$ at least for regular distributions.%\begin{definition2} 
%The distribution F  is said regular if its corresponding virtual value $\psi$ is increasing.
%\end{definition2}
%\redtext{changement}
%{\color{red} VP: est-ce qu'on a besoin de ce graphique ? En plus celui en haut a droite deconne, le vert n'est pas aligne avec le trait pointille rouge}
%\begin{figure}[h!]
%\begin{tabular}{cc}
%\includegraphics[width=.50\linewidth]{images/r025}&
%\includegraphics[width=.50\linewidth]{images/r075}\\
%\multicolumn{2}{c}{\includegraphics[width=.50\linewidth]{images/r05}}
%\end{tabular}
%\caption{\textbf{Change in bidder payment as a function of the reserve price.} The value distribution of the bidder is uniform [0,1] with $\psi(x) = 2x -1$, and is represented by the blue line. The dashed red vertical line corresponds to the current reserve price. We picked $G=1$, i.e. no competition. The bidder payment is equal to the area under the curve. The seller has no incentive to set the reserve price lower than $\psi_i^{-1}(0)$ since it decreases her total expected payment (because of the negative contribution of the red area). It is also clear that $r \ge \psi_i^{-1}(0)$ is suboptimal since it results in lost revenue for the seller.}
%\label{fig:visualOptimalR} % I can do without the label too
%\end{figure}
\begin{theorem2}%[Optimal reserve price in lazy second-price auction]
If  $F_i$ are regular, the optimal reserve prices in a lazy second-price auction are:
\begin{equation*}
\bigg(r_1,\dots,r_n\bigg) = \bigg(\psi_1^{-1}(0),\dots,\psi_n^{-1}(0)\bigg)\;,
\end{equation*}
with the convention that $\psi_1^{-1}(0)$ is the minimum of the support of $F_i$ is $\psi_i$ is  positive everywhere and the point where $\psi_i$ changes its sign if it is discontinuous.
\end{theorem2}
\begin{proof} 
The seller maximizes the sum of expected payment: 
\begin{align*}
\mathds{E}_{F_1,\dots,F_N}\Big[\sum_{i=1}^{n} P_i\Big] &= \sum_{i=1}^{n}  \mathds{E}_{F_i}\Big[\psi_i(x_i)G_i(x_i)\mathds{1}\{x_i\geq r_i\}\Big]\;.
\end{align*}
Since $F_i$ is regular, $\psi_i$ has one zero and is negative before the zero and positive after. Thus, the optimal choice for $r_i$ is clearly $\psi_i^{-1}(0)$. Indeed, the function $t\rightarrow \mathds{E}_{F_i}\Big[\psi_i(x_i)G_i(x_i)\mathds{1}\{x_i\geq t\}\Big]$ is increasing before $\psi_i^{-1}(0)$ and decreasing afterwards, owing to the sign of the integrand on both sides of $\psi_i^{-1}(0)$.
\end{proof}
We see in the proof that in a lazy second-price auction, the seller can safely maximize the payment of each bidder one by one independently. Indeed, in a lazy second price auction, changing the reserve price of one specific bidder does not change the probability of winning and the payment of the other bidders. This is not the case for eager second-price auctions on the other hand, which explains the complexity of computing the optimal reserve prices in them. Finally, the optimal reserve prices in a lazy second-price auction correspond to the monopoly prices of each bidder.



\begin{corollary2}The optimal reserve price for a bidder in a lazy second-price auction is independent of the presence, or not, of other bidders. In particular, it is the same as in the situation where he is the only bidder.
\end{corollary2}

\begin{figure}[H]
\includegraphics[width=.6\linewidth]{images/optimalmonopolyprice.pdf}
\caption{Bidder's payment as a function of the reserve price depending on the number of players in second-price auction with bidders all having a uniform value distribution $\mathfrak{U}([0,1])$.}
\end{figure}
%The proof also shows that when the distribution is not regular, the optimal reserve prices for each bidder verifies: $r_i \in \argmax(\mathds{E}_{F_i}(\psi_i(x)G(x)\textbf{1}_{x\geq r_i}))$.

The seller's revenue increases through the use of personalized reserve prices when bidders have very different value distributions. Intuitively, it is in the her best interest to set a high reserve price to bidders with high values most of the time  (or very high values sometimes) and low reserve prices to bidders with  low values most the time.

\bigskip
So far, we have only focused on the seller's revenue when designing auctions. An alternative objective can be the maximization of the  \textsl{global welfare} of the system, which is the sum of the seller's revenue and all bidders' utility. 




Even though reserve prices largely increase the seller's revenue, they actually significantly decrease the expected total welfare, as the item will sometimes not be allocated. This happens when all bidders (or at least the highest one in lazy auctions) have values below their reserve prices.

\begin{example2}
To illustrate this decrease in welfare, we are going to consider a simple example.  There are $n=2$ symmetric bidders with a value drawn uniformly over $[0,1]$. Because of the  symmetry, the optimal reserve price is the same for both bidders hence lazy and eager auctions coincide (and we do not need to specify the rule).  In this simple case, $r^* = \psi^{-1}(0) = 1/2$. As a consequence, the item is allocated as soon as one  bidder bids above 1/2, which happens with probability $3/4$. Otherwise, the item is not sold (which obviously happens with probability $1/4$). Simple computations show that changing the design from a second-price auction without reserve price to a second-price auction with optimal reserve price yields 
\begin{itemize}
\item a \textbf{12,5 \% decrease} of the global welfare (from $2/3$ to $7/12$).
\item a \textbf{50 \% decrease} of every single  bidder's utility  (from $1/6$ to $1/12$).
\item a \textbf{25 \%  increase} of the seller's revenue (from $1/3$ to $5/12$).
\end{itemize}
\end{example2}
\subsection{Myerson's lemma and characterization of BIC and DSIC auctions}
We mentioned before that the virtual value could (and maybe should) be understood as a virtual payment in a single bidder auction and/or in lazy second price auctions. The following lemma (that will be referred to as the ``Myerson Lemma'') is a crucial result \citep{Myerson81}. It states that the virtual payment of a bidder is the correct quantity to study in any  incentive-compatible auctions, and not just lazy second-price ones. The proof, while conceptually profound, is not very hard technically and requires integration by part and Fubini's theorem as we used in the case of the lazy second-price auction. This result holds for any Bayesian Incentive Compatible auction (if bidding truthfully is weakly dominant) that is 0-rational (if bidding 0 ensures a payment of 0). The latter assumption can be weakened, at the cost of an additive constant in the payment formula. 
\begin{theorem2}%[Myerson lemma]
\label{Th:MyersonLemma}
For any BIC and 0-rational auction, the expected payment of bidder $i$ at the truthful equilibrium is 
\begin{equation*} 
\mathds{E}_{x_i\sim F_i}[P_i(x_i)] = \mathds{E}_{x_i \sim F_{i}}[\psi_i(x_i)Q_i(x_i)] = \mathds{E}_{x \sim \mathcal{F}^{(n)}}[\psi_i(x_i)q_i(x)]\;.
\end{equation*}
Here $Q_i(x_i)$ is the winning probability  of bidder $i$  at the truthful equilibrium given his value  $x_i$ and $q_i(x)$ is the probability that the item is attributed to bidder $i$ when the values are $x=(x_1,\ldots,x_n)$. 
\label{myerson_lemma}
\end{theorem2}
\begin{proof}
Let us consider only  the truthful equilibrium of the BIC auction. In particular, we assume that all bidders except possibly $i$ bid their values, i.e. they bid truthful. Let us call $Q_i(z)$ the probability that bidder $i$ bidding $z$ wins the auction (when all other bidders bid truthful) and $P_i(z)$ his expected payment (when all other bidders bid truthful). The expected utility of bidder $i$ when he has value $x_i$ and bids $z$ is simply $Q_i(z)x_i - P_i(z)$. 
By definition of Bayesian incentive-compatibility, at the truthful equilibrium the auction must verify: 
\begin{equation*}
\forall z \in \mathds{R}^{+}, \forall x_i \in \mathds{R}^{+}, Q_i(x_i)x_i - P_i(x_i) \geq Q_i(z)x_i - P_i(z)\;,
\end{equation*}
since at the truthful equilibrium bidder $i$ gets maximum utility by bidding his value. 
Thus, if we denote by $\mathcal{U}_i(x_i)$ the expected utility of bidder $i$ when he has value $x_i$, 
\begin{equation*}
\mathcal{U}_i(x_i) = \max_{z} Q_i(z)x_i - P_i(z) = x_i Q_i(x_i)-P_i(x_i)\;.
\end{equation*}
As a consequence, $\mathcal{U}_i$ is a  convex mapping (the maximum of affine mappings) and therefore is differentiable almost everywhere and absolutely continuous (i.e. it is equal to the integral of its derivative).

Bayesian-incentive compatibility also implies that
\begin{equation*}
\forall z \in \mathds{R}^{+}, \mathcal{U}_i(z) =\max_t zQ_i(t)-P_i(t)\geq z Q_i(x_i)-P_i(x_i)= \mathcal{U}_i(x_i) + Q_i(x_i)(z-x_i)\;.
\end{equation*}
Since $\mathcal{U}_i$ is convex, this means that $Q_i(x_i)$ belongs to the subdifferential of $\mathcal{U}_i$ at $x_i$, i.e.
\begin{equation*}
Q_i(x_i) \in \partial \mathcal{U}_i(x_i)\;,
\end{equation*}
and  $\nabla \mathcal{U}_{i}(x_i) = Q_i(x_i)$  if  $\mathcal{U}_i$ differentiable at  $x_i$. Therefore, using Theorem  D.2.3.4 in \citep{HULLbook01}, 
$$
\mathcal{U}_i(x_i)-\mathcal{U}_i(0)=\int_0^{x_i}Q_i(z)dz\;,
$$
and since $\mathcal{U}_i(x_i)=x_i Q_i(x_i)-P_i(x_i)$, 
\begin{equation*}
P_i(x_i) = P_i(0) + Q_i(x_i)x_i - \int_{0}^{x_i}Q_i(z)dz\;.
\end{equation*}
Taking expectation over $x_i$ now gives~: 
\begin{align*}
 \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] &= \int_{x_i}P_i(x_i)f_i(x_i)dx_i 
\\&=  P_i(0) + \int_{x_i} \Big(Q_i(x_i)x_i - \int_{0}^{x_i}Q_i(z)dz\Big)f_i(x_i)dx_i
\\& = P_i(0) + \int_{x_i} Q_i(x_i)x_if_i(x_i)dx_i - \int_{z}Q_i(z)\Big(\int_{z}^\infty f_i(x_i)dx_i\Big)dz \qquad \text{ (Fubini) }
\\& = P_i(0) + \int_{x_i} \Big(x_i - \frac{1-F_i(x_i)}{f_i(x_i)}\Big)Q_i(x_i)f_i(x_i)dx_i 
%\\&= P_i(0) + \int_{x} \Big(x_i - \frac{1-F_i(x_i)}{f_i(x_i)}\Big)q_i(x)f(x)dx
\\& =  
 P_i(0) + \mathds{E}_{x_i \sim F_i}[\psi_i(x_i)Q_i(x_i)]\;.
% P_i(0) + \mathds{E}_{x \sim \mathcal{F}}[\psi_i(x_i)q_i(x)] =
\end{align*}
The result follows from the fact that $P_i(0) =0$ since the auction is 0-rational.

The last equality comes from the fact that $Q_i(x_i)= \mathds{E}_{x \sim \mathcal{F}^{(n)}}[q_i(x)|x_i]$ and the tower property of conditional expectations.
\end{proof}
\begin{remark2}
Theorem \ref{myerson_for_second_price} is a direct consequence  of this result with the specific choice of $Q_i(x_i) = G_i(x_i)\mathds{1}\{x_i\geq r_i\}$.
\end{remark2}
Myerson's lemma indicates that the expected payment of a 0-rational BIC auction only depends on the allocation rule and the virtual value; the proof actually gives a characterization of any incentive-compatible auction.  However, this characterization is slightly different for  BIC and DSIC auctions. 
\nek{Thomas: in coro below, do we need the auction to be 0-rational? }
\begin{corollary2}%[characterization of BIC auctions]
[\cite{Myerson81}]
\label{characterization_inc_comp}
Using the notations of Theorem \ref{Th:MyersonLemma}, an auction is BIC if and only if
\begin{itemize}
\item[i)] the allocation rule is monotone, i.e.  the probability of winning, as a function of the bid, is non-decreasing (for any fixed bids of others bidders)  and
\item[ii)] the expected payment verifies 
$$P_i(x_i) = Q_{i}(x_i)x_i - \int_{0}^{x_i} Q_{i}(z)dz.$$
\end{itemize}
\end{corollary2}
\begin{proof} 
The proof of Theorem \ref{myerson_lemma} gives the first implication. For the reverse, 
let us assume that all bidders except $i$ bid truthfully; and let us show that $i$ has an incentive to also bid truthfully. This will show that truthful bidding constitutes a Nash equilibrium and hence the auction is BIC. 

Note that because we have assumed that all other bidders bid truthfully, if bidder $i$ bids $z$, the probability that he wins is $Q_i(z)$. Hence, the expected utility derived by bidder $i$ when bidding $z$ and his value is $x_i$ is 
$$
\mathcal{U}_i(z,x_i)=x_i Q_i(z)-P_i(z)=(x_i-z)Q_i(z)+\int_0^z Q_i(t) dt\;.
$$
The second equality comes from assumption ii). 
Let us call $b_i^*$, the optimal bid of bidder $i$. 
% \nek{version 1}
% $b_i^*$ satisfies
% $$
% b_i^*=\argmax_z (x_i-z)Q_i(z)+\int_0^z Q_i(t) dt\;.
% $$
% Let us now show that $b_i^*=x_i$, which would conclude the proof.
% Consider the function $H: y\mapsto \int_0^y Q_i(t) dt$\;. This function is differentiable, with derivative $H'(y)=Q_i(y)$; as a consequence of assumption i) it is convex, since $Q_i(y)$ is non-decreasing in $y$. Therefore it is above all of its tangents, i.e~:
% $$
% \forall z\;, H(x_i)\geq H(z)+(x_i-z)H'(z)=H(z)+(x_i-z)Q_i(z)\;.
% $$
% In other words,
% $$
% \forall z\;, \mathcal{U}_i(x_i,x_i)=\int_0^{x_i}Q_i(t)dt\geq (x_i-z)Q_i(z)+\int_0^z Q_i(t) dt=\mathcal{U}_i(z,x_i)\;.
% $$
% This shows that $b_i^*=x_i$ and the auction is BIC.
%
% \nek{alternative}
Let us now show that $b_i^*=x_i$. To do so, we simply need to establish that 
$$
\forall z\in \mathds{R}_+,\; \mathcal{U}_i(x_i,x_i)=\int_0^{x_i} Q_i(t) dt \geq (x_i-z)Q_i(z)+\int_0^z Q_i(t) dt\;.
$$
This is equivalent to showing that 
$$
\forall z \in \mathds{R}_+\;, \int_z^{x_i} Q_i(t) dt \geq (x_i-z)Q_i(z)\;.
$$
If $z\leq x_i$, since $Q_i$ is non-decreasing, $Q_i(t)\geq Q_i(z)$ on $[z,x_i]$ and hence 
$$
\int_z^{x_i} Q_i(t) dt \geq (x_i-z)Q_i(z)\;.
$$
If $z\geq x_i$, since $Q_i$ is non-decreasing, $Q_i(t)\leq Q_i(z)$ on $[z,x_i]$ and hence
$$
\int_{x_i}^z Q_i(t) dt \leq (z-x_i) Q_i(z)\;.
$$
Multiplying the previous inequality by $(-1)$ on both sides shows that if $z\leq x_i$, we also have 
$$
\int_z^{x_i} Q_i(t) dt \geq (x_i-z)Q_i(z)\;.
$$
So we have shown that 
$$
\forall z\in \mathds{R}_+\;, \mathcal{U}_i(x_i,x_i)\geq \mathcal{U}_i(z,x_i)\;.
$$
Therefore, bidding truthfully is an optimal strategy for bidder $i$ and the auction is BIC. %(Note that the inequalities needed also follow from realizing that the function $H: y\mapsto \int_0^y Q_i(t) dt$ is convex.) COMMENT: I think adding alternative arguments just complicate things and scramble the message

% if the auction verifies
% $$P_i(x_i) = Q_{i}(x_i)x_i - \int_{0}^{x_i} Q_{i}(z)dz\;,$$
% then it implies that the auction verifies  $\nabla \mathcal{U}_i(x_i) = Q_{i}(x_i)$.\nek{do you mean this with subdifferentials?}
% \nek{I don't understand below}
% Since the probability of winning is increasing as a function of the bid, $$\mathcal{U}_i(x_i) - \mathcal{U}_i(z) = \int_{x_i}^{z}Q_{i}(s)ds \geq Q_i(x_i)(z - x_i)$$ which entails that $$\mathcal{U}_{i}(x)\geq Q_i(z)x - P(z).$$ This is the definition of bayesian incentive-compatibility (BIC).
%
%
% \nek{alternative}
% not clear yet that we know the gradient of $U_i$.
%
% Increasing allocation+others are truthful means $PWin(z)=Q_i(z)$ if we use $z$ instead of $x_i$ in $\beta(z)$.
%
% Now optimal strategy means $U_i(x_i)=\max_z x_iQ_i(z)-P(z)$. use convexity.
%
% see krishna pp.64-65 and possibly 69.
%
% Since the probability of winning is increasing as a function of the bid, the function
% $\mathcal{U}_i(x_i)$ is convex since its derivative is increasing. It is in particular above all of its tangents, hence
% $$
% \forall z\;,\mathcal{U}_i(x_i)\geq \mathcal{U}_i(z)+\mathcal{Q}_i(z)(x_i-z)\;.
% $$
% Since $\mathcal{U}_i(z)=z\mathcal{Q}_i(z)-P(z)$, we have
% $$
% \forall z\;,\mathcal{U}_i(x_i)\geq x_i \mathcal{Q}_i(z)-P(z)\;.
% $$
% This is the definition of bayesian incentive-compatibility (BIC).


\end{proof}
\begin{corollary2}%[characterization of DSIC auctions]
[\cite{Myerson81}]
\label{corollary_charect_DSIC}
An auction is DSIC if and only if
\begin{itemize}
\item[i)] the allocation rule is monotone and
\item[ii)]  the payment  of the winning bidder is the minimum bid guaranteeing that he would still have won the auction.\end{itemize}
 Given a monotone allocation rule and assuming 0-rationality, the payment rule is unique. 
\end{corollary2}
\begin{proof} 
The proof is almost identical, one just needs to make the various computations pointwise (for any vector $x_{-i}$) instead of in expectation.
\end{proof}
This characterization can be extended to very general mechanisms \citep{archer2001truthful}.
\subsection{The Myerson auction : revenue maximization for BIC auctions}
After having established the Myerson lemma, it is now possible to derive the  revenue-maximizing auction among all BIC auctions. 
\begin{definition2}%[Myerson auction]
The Myerson auction, for regular value distribution $F_i$ with associated virtual value $\psi_i$,  is defined by the two following rules: 
\begin{description}
\item[Allocation rule:] Given the bids $b=(b_1,\ldots,b_n)$, the winner is the bidder with the highest non-negative virtual value $\psi_i(b_i)$, i.e.
$$
q_i(b) = \mathds{1}\Big\{ i = \arg\max \big\{ \psi_j(b_j) \, ; \, j \text{ s.t. } \psi_j(b_j) \geq 0 \big\} \Big\}
$$
with the convention that if  all virtual values are negative, then the item is not allocated and $q_i(b) = 0$. Ties are broken arbitrarily.
\item[Payment rule:] If bidder $i$ wins the auction, he pays
$$p_i(b)=\max \Big\{ \psi_i^{-1}(0), \psi_i^{-1}\Big(\max_{j\neq i} \big\{\psi_j(b_j)\big\}\Big) \Big\}$$
\end{description}
\end{definition2}
This auction amounts to running a second price auction with reserve prices 0 among the \emph{virtualized bids} $\psi_k(b_k)$ and converting back this ``virtual cost" in the original bid space of the winner $i$ through the function $\psi_{i}^{-1}$\;.
\begin{theorem2} \label{theorem_regular_distributions}
If $F_1,\dots,F_n$ are regular, the Myerson auction maximizes seller's revenue among all BIC and  interim-IR  auctions.
\end{theorem2}
\begin{proof}
The Myerson auction is BIC as it verifies the condition of Corollary \ref{characterization_inc_comp}. Since $\psi_i$ are non-decreasing (as $F_i$ are regular), the probability of winning is non-decreasing. %\nek{do we need to explain how to check the payment condition?}

To show individual-rationality, we remark that since the auction is BIC, $$\mathcal{U}_{i}(x_i) = \mathcal{U}_{i}(0) + \int_{0}^{x_i}Q_i(s_i)ds_i = -P_{i}(0) + \int_{0}^{x_i}Q_i(s_i)ds_i \geq 0,$$ because $P_i(0) = 0$.  Thanks to  Myerson's lemma, Theorem \ref{Th:MyersonLemma}, the payment of each BIC auction is equal to 
$$
 P_i(0) + \mathds{E}_{x_i \sim F_{i}}(\psi_i(x_i)Q_i(x_i))\;. 
$$
The Myerson auction maximizes the two terms of this expression since for any rational auction, $P_i(0)\leq0$.  Since the winner in the Myerson auction is the bidder who verifies
\begin{equation*} 
\psi_i(x_i) = \max_{j \in S}\psi_j(x_j)\;,
\end{equation*}
and the item is not allocated when all $\psi_i$ are negative, the second term, is also maximized pointwise. 
Indeed, note that we can rewrite this second term
$$
\mathds{E}_{x_i \sim F_{i}}(\psi_i(x_i)Q_i(x_i))=\mathds{E}_{x \sim \mathcal{F}^{(n)}}[\langle\psi(x),q(x)\rangle]\;,
$$
where $\langle \cdot,\cdot\rangle $ is the standard inner product. 
\end{proof}
\begin{corollary2} In the symmetric case, the second-price auction with reserve prices set to  monopoly prices is the revenue-maximizing auction.
\end{corollary2}
\begin{remark2} 
The seller can increase her revenue if the mechanism is  only required to satisfy ex-ante rationality instead of interim rationality, as shown in 	
\citep{cremer1988full}. Indeed, there exists a BIC auction that is ex ante individually rational that accomplishes full-surplus extraction for the seller. In other words, the utility of bidders in this auction is equal to zero. This auction is not interim individually-rational since the expected utility when the bidder's value is zero is strictly negative. This setting of ex-ante individual rationality only makes sense when bidders have to decide to take part in the auction before understanding their value for the item. We shall come back in more details to this setting in Section \ref{sub_full_surplus_extraction}.
\end{remark2}
\subsection{Generalization of optimality result}
\label{SE:General_OptimalityResults}
\subsubsection{Non Incentive-Compatible mechanism: the revelation principle}
Myerson's optimality result can be extended to any incentive-compatible auctions, as long as there is a Nash equilibrium between bidders.
\begin{theorem2}%[Revelation principle]
Given a mechanism and a specific Nash equilibrium for this mechanism, there exists another BIC mechanism where the bidders' expected utility and seller's revenue at the truthful equilibrium are equal to the ones at the original Nash equilibrium. 
\end{theorem2}
\begin{proof}
Consider a mechanism and  $\beta = (\beta_1,\dots,\beta_n)$ a profile of strategies that is a Nash equilibrium. This mechanism is defined by an allocation rule $q:\mathcal{B}^{n}\rightarrow \mathds{R}^{n}$ and a payment rule  $p:\mathcal{B}^n\rightarrow \mathds{R}^{n}$. The mechanism $(q \circ \beta, p \circ \beta)$ is then clearly BIC and bidding truthful generate the same bids distributions, allocation and paiement as in the original mechanism; hence utilities and revenue are unchanged.
\end{proof}
\begin{corollary2} 
If value distributions are regular, the Myerson auction is the revenue-maximizing mechanism among all individually-rational mechanisms which have a Nash equilibrium.
\end{corollary2} 
\begin{proof}
This is a direct application of the revelation principle.
\end{proof}
We now extend the Myerson auction to cases where value distributions are not regular. 
\subsubsection{Non-regular distribution: the ironing technique}\label{Se:Ironing}

If $F_i$'s are not regular, the Myerson auction is not always defined as $\psi_i$'s may not be invertible. From an allocation standpoint, since $\psi_i$ is not necessarily increasing,  the allocation rule may not be monotone. Hence a bidder might have incentive to ``shade" (or lower) his bid to increase his virtual bid and his probability of winning. Non-regular distributions are not uncommon, as a mixture of two distributions typically is not regular (for instance the mixture of two uniforms, Gaussians, etc...). It is therefore crucial to adapt the Myerson mechanism to non-regular distributions. The canonical way is to define a slightly different allocation rule based on a modified virtual value \citep{Myerson81} called the \textit{ironed virtual value}. 

Recall that one key consequence of having a non-decreasing virtual value is that the monopoly revenue $\Pi(r) = r(1-F(r)) = \int_r^\infty \psi(v)f(v)dv$ is ``almost''  concave, in the sense that $\Pi\circ F^{-1}$ is concave with derivative  $-\psi\circ F^{-1}(\cdot)$. As a consequence, optimizing the monopoly revenue boils down to finding the root of $\psi$.  The ironing technique consists in replacing $\Pi\circ F^{-1}$, which is not necessarily concave, by its concavification. 

\begin{definition2}\label{def:Concavification}
For a function $h$, we call  $\mathrm{cav}(h)$ is the concavification of the  function $h$, which is its smallest concave majorant of $h$, i.e. the smallest concave function above it: its hypograph is the convex hull of the hypograph of $h$.
\end{definition2}
We can now define the ironed virtual value. 
\begin{definition2} \label{def:IronedVirtualValue}
For any non-regular distribution $F$, the \emph{ironed virtual value} of $\psi$, denoted by $\tilde{\psi}$ is defined by
$$
 \tilde{\psi}(x)= \partial \Big(-\mathrm{cav}(\Pi\circ F^{-1})\Big)(F(x))\;, \text{ where } \partial \text{ denotes the subdifferential}. 
$$
\end{definition2}

In general, the concavification of a function $g$ is either equal to $g$ at some point or linear on some interval otherwise. Luckily enough, the ironed virtual value has a closed form on intervals where it is not equal to the virtual value.


\begin{lemma2}%[Expression of ironed virtual value on [a,b]] 
Assume that for some $a<b$, it holds that \begin{itemize}
\item[--] $\mathrm{cav}(\Pi\circ F^{-1})(F(a))=\Pi (a)$,  
\item[--]$\mathrm{cav}({\Pi}\circ F^{-1})(F(b))=\Pi(b)$
\item[--] $\mathrm{cav}({\Pi}\circ F^{-1})(F(x)) > \Pi (x)$ for $x \in(a,b)$ 
\end{itemize}then
the ironed virtual value  of $\psi$ on $(a,b)$ is constant and equal to
$$
\tilde{\psi}(x)= \frac{\int_{a}^b \psi(t) f(t) \mathrm{d} t}{F(b)-F(a)}$$
\end{lemma2}
\begin{proof}
By definition of the concavification, $\mathrm{cav}(\Pi\circ F^{-1})$ is linear on $[F(a),F(b)]$ and the results comes from linear interpolation.
\end{proof}
%Typically, non-increasing virtual value function are ironed on an interval where it is non-increasing. On the other hand, if the ironing is limited to the smallest interval  where the virtual value is non-increasing, this might not guarantee that the ironed virtual value is increasing. To insure that the ironed virtual value is non-decreasing, the ironing should be extended a larger interval. The final minimal interval $[a_{opt},b_{opt}]$ where the virtual value is ironed should verify the following conditions:
%$$\psi(a_{opt}) \leq \psi([a_{opt},b_{opt}]) \leq \psi(b) \text{ and } \forall c,d \in [a_{opt},b_{opt}], \psi(c) \geq \psi([c,d]) \geq \psi(d)$$
%A good way to visualize how to set $a_{opt}$ and $b_{opt}$ is to plot $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$ as a function of $F(t)$.  We recall that $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t = -b(1-F(b))$, the opposite of the monopoly revenue. The intervals where the virtual value should be ironed are the ones where the convex envelop of $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$ is different from $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$.
%
%\begin{definition2}[Ironed virtual value] Consider a value distribuion F with corresponding virtual value $\phi$. Let $[a_1,b_1],...,[a_k,b_k]$ be the intervals that are straightened out when one takes the convex hull for the plot of the cumulative virtual value $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$ against F(b). The ironed virtual value  of $\psi_i$ denoted by $\tilde{\psi}_i$ is defined as 
%$$
%\tilde{\psi}_i(x)=\left\{\begin{array}{ll}{\psi([a,b]) = \frac{\int_{a}^{b} \psi(t) f(t) \mathrm{d} t}{F\left(b\right)-F\left(a\right)},} & {x \in\left[a_i, b_i\right]} \\ {\psi(x),} & {\text { otherwise }}\end{array}\right.
%$$
%\end{definition2}
We refer to \citep{note_ironings} for more technical details. In particular, the ironed virtual value, since  it is defined as a sub-differential, is not a function but a multi-valued mapping. On the other hand, selecting the aforementioned $\tilde{\psi}(x)$ as $\psi(x)$ when the sub-differential is not reduced to a singleton is also perfectly valid and implicitly used as convention from now on.  With this latter expression, either $\tilde{\psi}$ is equal to $\psi$ or it is constant on some interval around $x$. It is  non-decreasing everywhere and intervals where $\psi$ is  decreasing are ``flattened'', as illustrated in Figure \ref{Ironed}.



Recall that the purpose of ironing is to replace the - possibly somewhere decreasing - virtual value function $\psi$ in the Myerson auction (that might then not be BIC) by $\tilde{\psi}$. We now show that ironing the virtual value does not decrease the revenue of the Myerson auction.

\begin{figure}[h!]
\centering
œ\begin{tabular}{cc}
\includegraphics[width=.5\linewidth]{images/convex_hull.pdf}&
\includegraphics[width=.5\linewidth]{images/virtual_value_ironing.pdf}
\end{tabular}
\includegraphics[width=.55\linewidth]{images/ironed_revenue_curve.pdf}

\caption{\textbf{Left:} Concavification of $\Pi\circ F^{-1}$ for a  mixture of $\mathfrak{U}(0,0.5)$ and $\mathfrak{U}(0,1)$. \textbf{Right:} Associated virtual value (plain black) and ironed one (dashed orange).
\textbf{Center:} Original (plain black) and ironed (dashed orange) monopoly revenue.}
\label{Ironed}
\end{figure}
\begin{lemma2} 
The payment of bidder $i$ at the truthful equilibrium of any BIC auction satisfies 
$$ \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] \leq P_i(0) + \mathbf{E}_{x_{i} \sim F_{i}}\left[Q_{i}\left(x_{i}\right) \tilde{\psi}_{i}\left(x_{i}\right)\right]\;,$$
where $\tilde{\psi}_i$ is his ironed virtual value.\end{lemma2} 
\begin{proof} 
The proof is based on  the Harris inequality \citep{harris1960lower}, a direct application of Chebyschev' sum inequality. 
\begin{lemma2}[Harris inequality]
For any  non-decreasing mapping $\rho$ and  non-increasing mapping $\gamma$, the following holds for any random variable $X$, 
$$\mathds{E}[\rho(X)\gamma(X)] \leq \mathds{E}[\rho(X)]\mathds{E}[\gamma(X)]\;.$$
\end{lemma2}
Consider a BIC auction. According to Theorem \ref{Th:MyersonLemma}, 
$$
\mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] = P_i(0) + \mathbf{E}_{x_{i} \sim F_{i}}\left[Q_{i}\left(x_{i}\right) \psi_{i}\left(x_{i}\right)\right]\;.
$$
Furthemore, since the auction is BIC, Corollary \ref{characterization_inc_comp} implies that $Q_i$ must be non-decreasing. 

Let  $[c,d]$ be an interval where $\psi$ requires ironing and let $[a,b]$ be the largest interval that contains $[c,d]$ over which $\psi(x)\neq \tilde{\psi}(x)$. In other words, $[a,b]$ is the whole interval over which  $\psi$ has been ironed. We consider the function $\tilde{\psi}$ defined above on the corresponding $[a,b]$ interval. Furthermore, note that $f_i(x)/(F_i(b)-F_i(a))$ is a valid probability density on $[a,b]$. We then have
\begin{align*}
&\int_{a}^{b}Q_i(x)\psi_{i}(x)f_i(x)dx =(F_i(b) - F_i(a)) \int_{a}^{b}Q_i(x)\psi_{i}(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx
\\&\leq (F_i(b) - F_i(a)) \int_{a}^{b}Q_i(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx\int_{a}^{b}\psi_i(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx
\\&=\int_{a}^{b}Q_i(x)\tilde{\psi}_{i}(x)f_i(x)dx\;.
\end{align*}
from where the result follows. The first inequality comes from applying Harris' inequality. \nek{c'est faux non? $\psi$ est justement pas monotone sur l'interval, donc pourquoi appliquer Harris?} The last equality comes from the definition of $\tilde{\psi}$ which is a constant and equal to $\int_{a}^{b}\psi_i(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx$ on the interval $[a,b]$ by definition. Here it is important that we use the whole ironing interval for $[a,b]$. The same argument applies on all intervals where $\psi$ requires ironing.  
The statement of the Lemma is shown by applying Theorem \ref{Th:MyersonLemma} to compute expected revenue. 
\end{proof}
We now generalize Theorem \ref{theorem_regular_distributions} to the case of non-regular value distributions.
 \begin{theorem2}[\cite{Myerson81}]%[Optimal auctions for general value distribution]
  In a single item auction, with general value distribution, a revenue-maximing auction is an auction where the seller allocates the item to the bidder with the highest non-negative ironed virtual value. The payment rule is defined such that the auction is incentive compatible - see Corollary \ref{characterization_inc_comp}.
 \end{theorem2}
 
 \subsection{Reserve prices in first price auctions}
%\nek{need to read his assumptions carefully and state them} 
We start with an abstract result that we then apply to first price auctions. 

\begin{proposition2}\label{prop:virtualValueIsVirtualPaymentGeneralCase}
Suppose bidder $i$ participates in an auction such that the probability of winning the auction when bidding $b$ is $G_i(b)$ and the corresponding expected payment is $P_i(b)$. Call $\beta_i$ an optimal strategy for bidder $i$ in this setup, i.e. one that maximizes their utility. 	
Then the seller revenue coming from bidder $i$ is 
\begin{equation}\label{eq:RevSellerGeneralPriceWithVValue}
 \mathds{E}_{x_i\sim F_{i}}[P_i(\beta_i(x_i))]-P_i(\beta_i(0)) =\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;,
\end{equation}
where $\psi_i$ is the virtual value (see Equation \eqref{eq:defVirtualValue}) associated with the value distribution of $x_i$. 
\end{proposition2}
\begin{remark2}
This proposition helps explain how our interpretation of the $\psi_i(x_i)$ as a virtual payment makes sense for utility-maximizing bidders in general and not only in the case of BIC or DSIC auctions we encountered previously. It can also be seen as a more quantitative version of the revelation principle. 
\end{remark2}
\begin{proof}
Note that since bidder $i$ tries to maximize his utility, 
$$
\beta_i(x_i)=\argmax_b x_iG_i(b)-P_i(b)\;. 
$$
Let us call 
$$
W(x)=x G_i(\beta_i(x))-P_i(\beta_i(x))
$$
The envelope theorem in the form of Theorem 2 of \cite{MilgromSegal2002} applies since $0\leq G_i(t)\leq 1$ for all $t$ and hence 
$$
W(x)-W(0)=\int_0^x G_i(\beta_i(t)) dt\;.
$$
Therefore, the expected payment satisfies
$$
P_i(\beta_i(x))-P_i(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(t)) dt\;.
$$
Taking expectation with respect to $x_i$ with cdf $F_i$ in the previous equation gives
\begin{align*}
\mathds{E}_{x_i\sim F_{i}}[P_i(\beta_i(x_i))]-P_i(\beta_i(0))&=\int_0^{\infty} xG_i(\beta_i(x)) f_i(x)dx-\int_0^{\infty}\int_0^{\infty} f_i(x)\indicator{t\leq x}G_i(\beta_i(t))dt\, dx\;,\\
&=\int_0^{\infty} xG_i(\beta_i(x)) f_i(x)dx-\int_0^{\infty} (1-F_i(t))G_i(\beta_i(t))dt\;,\\
&=\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
\end{align*}
% $$
% \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
% $$

% This is not limited to first price... as long as $P(\beta_i(0))=0$\\
% En gros,  1st order conditions give $xG_i'(\beta_i(x))=P'(\beta_i(x))$. Multiply both sides by $\beta'_i(x)$ and integrate to get $P(\beta_i(x))-P(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(u))du\;.$ Then doing the same as below, we get that
% $$
% \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)]-P(\beta_i(0))=\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
% $$
% Ou: envelope theorem says that if $W_i(x)=\max_b xG_i(b)-P(b)$, and $\beta_i$ is an optimal strategy, $W_i'(x)=G(\beta_i(x))$. Hence, $W_i(x)-W_i(0)=\int_0^x G_i(\beta_i(u))du=xG_i(\beta_i(x))-P(\beta_i(x))+P(\beta_i(0))$. We conclude that
% $P(\beta_i(x))-P(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(u))du\;.$ And the result follows as above.

	
	
\end{proof}




In the case of first price auctions, we have $P_i(\beta_i(x_i))=\beta_i(x_i)G_i(\beta_i(x_i))$, since the probability of winning is $G_i(\beta_i(x_i))$. 
So the arguments given in the proof above allow us to recover a result from \citep{KirkegaardAsymmetricFirstPrice2009}~: the optimal strategy for bidder $i$ when the top bid of the competition has cdf $G_i$ and $P_i(\beta_i(0))=0$ satisfies 
\begin{equation}\label{eq:OptStrat1stPriceEnvelope}
\beta_{i}(x)=x-\frac{\int_0^x G_i(\beta_i(t))dt}{G_i(\beta_i(x))}\;.
\end{equation}

%Because of the the envelope theorem and arguments similar to those used to derived the revenue maximizing auctions, the equilibrium strategy must satisfy 
\iffalse
Using the envelope theorem, one can show \citep{KirkegaardAsymmetricFirstPrice2009} that the optimal strategy for bidder $i$ when the top bid of the competition has cdf $G_i$ satisfies 
\begin{equation}\label{eq:OptStrat1stPriceEnvelope}
\beta_{i}(x)=x-\frac{\int_0^x G_i(\beta_i(t))dt}{G_i(\beta_i(x))}\;.
\end{equation}
\fi
The expected payoff of player $i$ at $x$ is then equal to $u_i(x,\beta_{i}(x))=\int_0^x G_i(\beta_i(t))dt$ and in particular it holds  that $\mathds{E} U_i (\beta,x_i)=\ \mathds{E}_{x_i\sim F_{i}}\big[G_i(\beta_i(x_i))(x_i-\psi(x_i))\big]$. 
\iffalse
\nek{I think with the envelope theorem we can show that if I'm a utility maximizer, i.e. I pick 
$$
\beta(x)=\argmax_b xG(b)-P(b)\;,
$$
regardless of the payment rule, then 
$$
\mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
$$
This is not limited to first price... as long as $P(\beta_i(0))=0$\\
En gros,  1st order conditions give $xG_i'(\beta_i(x))=P'(\beta_i(x))$. Multiply both sides by $\beta'_i(x)$ and integrate to get $P(\beta_i(x))-P(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(u))du\;.$ Then doing the same as below, we get that 
$$ 
\mathds{E}_{x_i\sim F_{i}}[P_i(x_i)]-P(\beta_i(0))=\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
$$
Ou: envelope theorem says that if $W_i(x)=\max_b xG_i(b)-P(b)$, and $\beta_i$ is an optimal strategy, $W_i'(x)=G(\beta_i(x))$. Hence, $W_i(x)-W_i(0)=\int_0^x G_i(\beta_i(u))du=xG_i(\beta_i(x))-P(\beta_i(x))+P(\beta_i(0))$. We conclude that 
$P(\beta_i(x))-P(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(u))du\;.$ And the result follows as above. 
}
\fi
\begin{corollary2}\label{coro:RevSeller1stPriceWithVValue}
In a first price auction, when bidder $i$ uses the strategy implicitly defined in Equation \eqref{eq:OptStrat1stPriceEnvelope}, the seller revenue coming from bidder $i$ is 
\begin{equation}\label{eq:RevSeller1stPriceWithVValue}
 \mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;,
\end{equation}
where $\psi_i$ is the virtual value associated with the value distribution of $x_i$. 
\end{corollary2}
The corollary follows from Proposition \ref{prop:virtualValueIsVirtualPaymentGeneralCase} after noticing that $P_i(\beta_i(0))=\beta_i(0)G_i(\beta_i(0))=0$ when bidder $i$ uses $\beta_i$ defined in Equation \eqref{eq:OptStrat1stPriceEnvelope}.

\iffalse
\begin{proof}
We note that 
$$
 \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\int_0^{\infty}\beta_{i}(x) G_i(\beta_i(x)) f_i(x) dx =\int_0^{\infty} xG_i(\beta_i(x))f_i(x)dx - \int_0^{\infty}f_i(x)\int_0^x G_i(\beta_i(t))dt dx\;.
$$	
Using Fubini's theorem, we have 
$$
\int_0^{\infty}f_i(x)\int_0^x G_i(\beta_i(t)))dt dx=\int_0^{\infty}f_i(x)G_i(\beta_i(t))dt \indicator{t\leq x} dx dt=\int_0^{\infty}(1-F_i(t))G_i(\beta_i(t))) dt\;.
$$
We conclude that 
$$
 \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\int_0^\infty G_i(\beta_i(x))\left[x-\frac{1-F_i(x)}{f_i(x)}\right]f_i(x) dx = \mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi(x_i)\big]\;.
$$
\end{proof}
\fi

\paragraph{Good or optimal reserve prices} Proposition \ref{prop:virtualValueIsVirtualPaymentGeneralCase} and Corollary \ref{coro:RevSeller1stPriceWithVValue} suggest that from a seller revenue standpoint it would be good to avoid bids corresponding to values that have negative virtual values. In other words, setting individual reserve values at $\psi_i^{-1}(0)$ for bidders may have positive impact for seller revenue. However, this interpretation ignores the impact of setting such reserve values on the strategic response of the bidder that is optimizing his utility. 


Finding optimal reserve prices for first price auctions is much more complicated than finding them for the second price auctions, even with $n=2$ symmetric bidders \citep{KotowskiAsymmetricReserves2018} for the following two reasons. First, if the distribution $F$ is not regular and its density is discontinuous at the monopoly price, giving two different reserve prices to the two symmetric buyers actually increases the seller revenue at equilibrium, at least when $r_1$ and $r_2$ are close.
Second, in the specific case where those two reserve prices $r_1$ and $r_2$ are sufficiently close,  the equilibrium bid distribution of the player with the lower reserve price becomes discontinuous.


Many further difficulties arise when the seller tries to learn good reserve prices for first price auctions from data and does not have access to the bidders' value distributions. We further detail them in Section \ref{learning_reserve_prices_first_price}.

\section{Prior-independent optimal auctions} 
\label{sec-Bulow}
In the previous section, we  derived the revenue-maximizing auction given the prior of the seller on the possible valuations of the different bidders. In some cases, the seller does not have access to a reliable prior and she has to choose an auction without this information. An associated challenge is to understand what auctions are robust to a lack of knowledge about (or some mis-specification in) the bidders' value distributions.

The following theorem shows that a basic second-price auction without reserve price -  referred to henceforth as the Vickrey auction - with just one extra bidder, leads to a higher revenue than the optimal Myerson auction \citep{bulow1996auction}. Only the symmetric case is considered, so that the comparison of two auctions with different set of bidders is possible.
\begin{theorem2}[\cite{bulow1996auction}]%[Bulow-Klemperer Theorem]
In the symmetric setting and with regular distributions, the revenue of the Myerson auction with $n$ bidders is lower than the revenue of the Vickrey auction with $n+1$ bidders. 
\end{theorem2}
\begin{figure}[H]
\includegraphics[width=.5\linewidth]{images/BulowKlemperer.pdf}
\caption{Illustration of the Bulow-Klemperer theorem for the case with value distributions  $\mathfrak{U}([0,1])$.}
%{\color{red} Ca ne devrait pas etre $K$ bidders mais $n$ bidders ; choix des couleurs discutables ; on ne dit pas Nb bidders en Anglais }}
\label{fig:BK}
\end{figure}
Before proving the Bulow-Klemperer theorem, we introduce a useful lemma.
\begin{lemma2}\label{second_price_without_reserve}
In the symmetric case and with regular distributions, the Vickrey auction is revenue-maximizing in the class of individually-rational auctions where the item is always attributed. 
\end{lemma2}
\begin{proof}
Based on the revelation principle, we shall only consider incentive-compatible auctions. Theorem \ref{Th:MyersonLemma} then applies. Since the item must always be attributed, in order to maximize the seller's revenue it should be allocated to the bidder with the highest virtual value, regardless of whether the highest virtual value is non-negative or not. This is a consequence of the proof of Theorem \ref{Th:MyersonLemma}. Since the distributions are regular and identical, the bidder with the highest virtual value is also the bidder with the highest value. As a consequence, the mechanism we just described is exactly the Vickrey auction.
\end{proof}
The proof of the Bulow-Klemperer theorem can now be derived from the previous lemma.
\begin{proof} 
Let us assume that there are $n+1$ bidders, and consider the following mechanism. First, the seller runs a Myerson auction on  $n$ bidders (chosen arbitrarily). If the item is not allocated by the Myerson auction, it is allocated for free (i.e. without any payment) the $(n+1)$-th bidder. The revenue of this auction is equal to the revenue of the Myerson auction with $n$ bidder, yet it is  an auction that always allocate an item amongst $n+1$ bidders. Lemma \ref{second_price_without_reserve} implies that the revenue of this auction is smaller than the one of the Vickrey auction. 
This gives the result.
\end{proof}

As a consequence, it is more interesting,  from a seller revenue maximization standpoint to have one more bidder in the auction than to implement a complex mechanism. This is the reason why one of the first recommendations of most economists dealing with institutions organizing auctions is to maximize the competition  before implementing complex mechanisms \citep{bulow1996auction,milgrom2004putting}. This is sometimes referred to as the Wilson doctrine.

\bigskip

Nonetheless, let us assume that a specific mechanism has been chosen, independently of the value distributions (which are unknown in this setup). A crucial  question that remains is the evaluation of this specific choice of mechanism in the worst-case analysis. We will restrict ourselves to DSIC auctions. We will use the notion of \textsl{competitive ratio} defined as the infimum, over all possible value distributions, of the revenue of this auction divided by the optimal revenue of the Myerson auction for these distributions. 

The competitive ratio is obviously smaller than 1, and the bigger the better. Unfortunately, if the class of value distributions is not restricted when computing this infimum, there does not exist any auction with a positive competitive ratio \citep{allouah2018prior}. As a consequence, we will use different types of restrictions to achieve non-trivial approximation results. Based on the Bulow-Klemperer theorem, we can derive some revenue guarantees on the second price auction without reserve price. 
\begin{corollary2} \label{compet-ratio}
The Vickrey auction  with $n$ symmetric bidders and regular value distributions is at least a $\left(\frac{n-1}{n}\right)$-approximation of the Myerson auction. 
\end{corollary2}
\begin{proof}
We denote  respectively by $R(\mathrm{Vickrey}_n)$ and $R(\mathrm{Myerson}_n)$ the expected revenue of the seller  in the Vickrey or  Myerson auction with $n$ bidders and by $P_i(\mathrm{Vickrey}_n)$ and $P_i(\mathrm{Myerson}_n)$ the expected payment of the bidder $i$ in those auctions (so that $R(\cdot) = \sum_{i=1}^n P_i(\cdot)$).


Let us first prove that $P_i(\mathrm{Myerson}_n)\geq P_i(\mathrm{Myerson}_{n+1})$.

By symmetry and with regular distributions, their exists a unique monopoly price $r^*$ which is independent of the number of players. Note that $\psi(x)\geq 0$ when $x\geq r^*$. Furthermore, in the symmetric case, the probability that bidder $i$ wins the auction when facing $k$ competitors is just $F^k(x)$. Hence, 
\begin{align*}
	P_i(\mathrm{Myerson}_{n})&= \int  \psi(x) F^{n-1}(x)f(x)\mathds{1}\{x\geq r^*\} dx\\&\geq \int \psi(x) F^{n}(x)f(x)\mathds{1}\{x\geq r^*\}dx\\&=P_i(\mathrm{Myerson}_{n+1}),\end{align*}
which proves the inequality.



Then, based on the Bulow-Klemperer theorem, 
$$R(\mathrm{Vickrey}_n)\geq R(\mathrm{Myerson}_{n-1}) = (n-1)  P_i(\mathrm{Myerson}_{n-1}) \geq (1-\frac{1}{n})  R(\mathrm{Myerson}_{n})$$
which gives the result. \end{proof}
We proved in Corollary \ref{compet-ratio}, through the Bulow-Klemperer theorem that the competitive ratio of the Vickrey auction is at least 0.5, when the distributions are restricted to regular ones. Interestingly, it is possible to do better with a slightly different auction. 
\begin{theorem2}[\cite{fu2015randomization}]
There exists an incentive-compatible auction with a competitive ratio of 0.512 against regular value distributions. 
\end{theorem2}
The mechanism considered was the first  with a higher competitive ratio than 0.5  against regular distributions. It is a slight modification  of the Vickrey auction where the seller inflates the second highest bid. Formally, the mechanism is the following: with probability $1-\varepsilon$,  a second price auction without reserve price is run. With the  probability $\varepsilon$, the mechanism allocates the object to the bidder with the highest valuation, but only if his valuation is greater than $1+\delta$  times the valuation of the second highest bidder and pays  $(1+\delta)$ the second highest bid. Otherwise, the mechanism does not allocate the item. 

The idea behind this theorem is the following. The Bulow-Klemperer bound of $0.5$ on the competitive ratio is rather tight for regular distributions that would induce a high optimal reserve price. On the other hand, it is rather loose for regular distribution with a low associated reserve price. Inflating the second highest bid has a positive effect for the former type of distribution (as it somehow emulates a high reserve price) and a negative effect for the later type (because it induces some reserve price, bigger than what it should be). As a consequence, the ratio of revenues increase in the first case, and decreases in the second one; but thanks to the looseness in the Bulow-Klemperer bound of $0.5$, the infimum globally increases. 

On the other hand, when restricted to MHR distributions, the ratio is equal to 0.7153 and this result is tight. 

For regular distribution, this result was then improved up to 0.519 \citep{allouah2018prior}  and further improved in \citep{hartline2020benchmark} which identified the optimal prior-independent mechanism. The optimal mechanism is a mixture between a second price auction and the same auction where the prices are scaled up by a factor of about 2.5. The authors find the worst-case family of distributions and use these distributions to derive the optimal mechanism and solve the problem. 

\section{Further reading: non-unicity of Nash equilibria and related complications}
\label{sec:NashIsDifficult}
\nek{Add the two counter examples here...}


==> chapters/chapter2_some_classical_results_discarded.tex <==
%!TEX root = ../main.tex
\chapter{Bayesian mechanism design}
\label{Chapter:Bayes}

Auctions mechanisms involve many different agents, sellers and/or buyers, with possibly different and conflicting objectives, the optimization of their own utility functions. These interactions can be modelled using game-theoretic concepts. More specifically, we are going to focus on a specific types of games with \emph{incomplete information}, that are called \textit{mechanisms}. In those games, each player has some private information (i.e., unknown from everyone else), and send some \emph{message} to a central authority.  Base on those messages  gathered, the latter  decides on the final outcome:  the utility of a player then solely depends on it. 

Mechanisms model appropriately  many practical situations such as the celebrated  problems of affecting student to schools, or organs transplantation matchings. In these problems, a central authority forms pairs between school and students or donors and recipients. In selling mechanisms, the central authority is the seller of a specific item and the players are the buyers.  \emph{Auctions} are mechanisms used to sell a particular item. In the case of a sale of a single non-divisible item, they have the following particular features. 


%\clem{The notation defined here is not used later on and even conflicts with later notation.}{\color{red}VP : agreed !}
%A \textit{normal-form game} is defined by a set of of players $\mathcal{N}$ of cardinality $N$, the set of actions  $\mathcal{A}_i$ and the payoff function  of player $i \in \mathcal{N}$
%$u_i:\mathcal{A}_1 \times \dots \times \mathcal{A}_N \rightarrow \mathds{R}.$ 
%
%In such a game, each player chooses independently an action $a_i \in \mathcal{A}_i$ and gets a utility of $u_i(a_1,\ldots,a_N)=u_i(a_i,a_{-i})$
%that depends on both the action $a_i \in   \mathcal{A}_i$ of the player and the profile of actions of other players, denoted by $a_{-i} := (a_1,\ldots, a_{i-1}, a_{i+1},a_N) \in \prod_{j \neq i} \mathcal{A}_j$.
%
% 
%\begin{definition2}[Normal-form game]
%A normal-form game is:
%\begin{itemize}
%\item a set of players $\mathcal{N}$ of cardinality $N$.
%\item for each player $i \in [1,N]$, a set of possible actions $\mathcal{A}_i$.
%\item a set of payoff functions which gives for each player her payoff corresponding to her action and actions of other players
%$$u_i:\mathcal{A}_1 \times \dots \times \mathcal{A}_N \rightarrow \mathds{R}\;.$$
%\end{itemize}
%In a normal-form game of complete information, actions, outcomes and payoff functions are common knowledge to all players. In a game of incomplete information, every player's payoff function depends on a variable $X$ called private information and which is only known to each specific player. If we denote by $\mathcal{X}$ the set of private information, the payoff function of player $i$ is defined as $u_i:\mathcal{A}^{N} \times \mathcal{X} \rightarrow \mathds{R}$.
%\end{definition2}


%In the different settings we are going to consider,  players have some private information that actually impacts their payoff functions. Formally, let us denote by  $\mathcal{X}$ the set of private information, so that the payoff function of player $i$ rewrites as  $u_i:\prod_{j \in \mathcal{N}} \mathcal{A}_j \times \mathcal{X} \rightarrow \mathds{R}$. Those games are called with \textit{incomplete information}.


\medskip


%and decides each player's outcome according to these messages. In these games, players' actions correspond to the message they send to the central authority. 

%In a game of incomplete information, every player's payoff function depends on a variable $X$ called private information and which is only known to each specific player. If we denote by, the payoff function of player $i$ is defined as 

%In this survey, we are focusing on a certain type of games with incomplete information where there exists a central authority which gathers messages from the different players and decides each player's outcome according to these messages. In these games, players' actions correspond to the message they send to the central authority. This type of centralized gamed is called mechanism. 
%\begin{definition2}[Mechanism]
%A mechanism is a game of incomplete information where players send a message to a central authority who does not know the private information of each player. The central authority decides based on messages it receives and some predefined rules every player's outcome.  
%\end{definition2}

Auctions are games with incomplete information as each buyer has some private valuation for the item,  the highest price they are willing to  pay to acquire  the item (which might be different from one buyer to another). We denote by $\mathcal{N}$ the set of buyers, of cardinality $n \in \mathbb{N}$, by  $x_i \in \mathcal{X}$ the  private value or bidder $i \in \mathcal{N}$ and by  $x = (x_1,\dots,x_n)$ the profile of private values. 
The possible messages (or actions) of buyer $i\in \mathcal{N}$ are called ``bids'' and their set is denoted by $\mathcal{B}_i$. The outcome of an auction mechanism is defined by two different rules
\begin{enumerate}
\item an \textit{allocation rule} $q:\mathcal{B}_1 \times \dots \times  \mathcal{B}_n \rightarrow \Delta_n$ where $\Delta_n$ is the set of probability distributions over the set of $n$ buyers. It gives the probability that each player gets the object.
\item a \textit{payment rule} $p: \mathcal{B}_1 \times \dots \times  \mathcal{B}_n \rightarrow \mathds{R}^{n}$. It defines the expected payment of each player whether he got or not the object.
\end{enumerate}

 We also denote by $b = (b_1,\dots,b_n)$ the vector of bids sent by the buyers.  With these notations, the utility of bidder $i \in \mathcal{N}$ is then defined as
$$u_i(b,x_i) = q_i(b)\big(x_i -p_i(b)\big)\;;$$
on the other hand, the seller aims at maximizing her revenue
$$\sum_{i=1}^n q_i(b)p_i(b)\;.$$

%\begin{definition2}[Auction mechanism]
%An auction mechanism is a mechanism defined by three features: 
%\begin{itemize}
%\item a set of possible messages $\mathcal{B}_i$ for each buyer (bids in most cases). 
%\item an allocation rule $q:\mathcal{B}_1 \times \dots \times  \mathcal{B}_N \rightarrow \Delta_N$ where $\Delta_N$ is the set of probability distributions over the set of $N$ buyers. It gives the probability that each player gets the object.
%\item a payment rule $p: \mathcal{B}_1 \times \dots \times  \mathcal{B}_N \rightarrow \mathds{R}^{N}$. It defines the expected payment of each player whether he got or not the object.
%\end{itemize}
%A selling mechanism is nothing more than a set of rules explaining how a group of buyers and a seller interact. 
%
%The private information owned by each buyer which conditions their payoff function is their own value for the item, i.e., the highest price they are ready to pay to own the item. We denote by $\mathcal{X}_i$ the set of all possible values for one item for bidder $i$.  The value vector which contains the values of all the different players is denoted by $x = (x_1,\dots,x_N)$. The \textit{messages} sent to the seller are called \textit{bids}.  We denote by $b = (b_1,\dots,b_N)$ the corresponding bid vector. 
%
%Depending on the information they have on the mechanism and the other bidders, the ultimate goal of the bidders is to maximize their utility 
%$$u_i(x_i, (b_1,...,b_N)) = q_i(b_1,...,b_N)(x_i -p_i(b_1,...,b_N))\;,$$
%and the objective of the seller is to maximize her revenue
%$$\sum_{i=1}^N q_i(b_1,...,b_N)p_i(b_1,...,b_N))\;.$$
%\end{definition2}
\section{The Bayesian setting}
The auction literature historically considered  a Bayesian setting where the value $x_i$ of bidder $i \in \mathcal{N}$ is random, and drawn accordingly to the \emph{value distribution} that ``represents the seller assessment of the probability of bidder $i$ has a value estimate of $x_i$ or less''  \citep{Myerson81}. It quantifies the uncertainty of the seller on the maximum price that  one buyer is willing to pay for  the item and is represented as a Bayesian prior on the private information of each buyer. 

The traditional assumption is that  value distributions are common knowledge to bidders and seller.  As a consequence, we denote by $F_i$ the cumulative distribution function of the value of buyer $i \in \mathcal{N}$ and by $f_i$ its corresponding density function, assuming it exists, an assumption we are going to make repeatedly (removing it is quite always a matter of technicalities). We implicitly identify the distribution $F_i$ with its cumulative distribution function (cdf) and use both terms exchangeably. We are also going to assume that values are non-negative, i.e., the support of $F_i$ is included (but not necessarily equal to) in $\mathds{R}_+$ and also that $\mathds{E}_{x_i \sim F_i} [x_i] < +\infty$ to get optimality results (and not just $\varepsilon$-optimality). A crucial assumption throughout this survey is that the values $x_i$ are independent; we shall  denote by $\mathcal{F} = F_1\otimes \ldots\otimes F_n$ the joint product distribution of $x=(x_1,\ldots,x_n)$ the vector of values.

\medskip

Typical value distributions are the uniform distribution for its simplicity in textbook examples,  the exponential and the log-normal distribution as they are similar to some empirical distributions encountered on modern internet platforms or any power law distribution (also known as Pareto distributions) capturing the idea that the value in real time bidding and online advertising comes from few matches of very high quality, such as consumers who recently viewed a product \citep{arnosti2016adverse} (this situation where 20\% of individuals own/generate 80\% of wealth is also refered as the Pareto principle in economics).

The auction setting will be called \textit{symmetric} if all bidders have the same value distribution. For the sake of clarity, we use pronouns her/she for the seller and he/his for one specific bidder


%{\color{red} VP: Je pense qu'il faut elaborer un peu sur le "typical". Ca veut dire quoi exactement ? Soit on met des refs, soit on vire}

%The notion of information owned by the seller and value distribution have progressively changed with several new applications of auction systems. One of the goal of this thesis is to clarify this change and show how sellers and bidders can adapt to this new information structure of the game. For instance, in a repeated setting, where multiple different items are sold successively, the value distribution could also represent the variety of values that a specific buyer can give to one item. 

\subsection{Properties of auction systems}
\label{subsec_prop_auction}
A bidder \textit{strategy} is the mapping indicating which bids he sends to the seller to buy one specific item, conditionally to his private information, his value. Stated otherwise, a strategy is a mapping $\beta: \mathcal{X} \rightarrow \mathcal{B}$ that maps private values to bids.

%Bidders have the choice on the bids they send to the seller to get one specific item. A strategy defines how these bids depend on buyer's original private value.
%\begin{definition2}[Strategy]
%A strategy is a function $\beta: \mathcal{X} \rightarrow \mathcal{B}$ that maps private values to bids.
%\end{definition2}

We will denote by $\mathds{B}_i$ the set of all strategies of player $i$, $\beta_i$ the chosen strategy and $\beta_{-i}$ the profile of strategies corresponding to all bidders except bidder $i$ (similarly, the notation  $F_{-i}$ will denotes the product distribution of values of all bidders except  $i$).

We emphasize here that in Bayesian games, it is important to differentiate between \textit{ex ante}, \textit{interim} and \textit{ex post} properties \citep{hartline2013bayesian}. They depend on the information available to buyers when they decide to participate in the game and choose their strategy.  
\begin{itemize}
\item For  \emph{ex-ante} properties, bidders do not know yet their own value for the item; i.e., they only know $F_i$ and $F_{-i}$.
\item For \emph{interim} properties, bidders know their valuation but do not know the values of other players, i.e., $x_i$ and $F_{-i}$
\item For \emph{ex-post} properties, bidders know their valuations and the ones from the other players, i.e., both $x_i$ and $x_{-i}$.
\end{itemize}
In the next sections, we will mostly focus on  interim properties. It is the starting point of the auction literature assuming the value distributions are common knowledge and the exact valuation are private information to each bidder.  

We are also assuming that bidders are risk-neutral, i.e., maximizing their expected utility over all other bidders' possible valuations and with respect to their strategies.  Stated otherwise, assuming the other bidders are using the strategy $\beta_{-i}$, the  expected utility  of the strategy $\beta_i$  given his value $x_i$ is then denoted by
$$
U_{i}(\beta_i,\beta_{-i},x_i) = \mathds{E}_{x_{-i} \sim F_{-i}}\Big[u_{i}\big((\beta_1(x_1), \dots\beta_n(x_n)), x_i\big)\Big]\;.
$$
Maybe one of the most central concept in game theory is (Bayesian) Nash equilibrium, a situation where the strategy of a bidder maximize his utility, given his valuation, the strategies of his opponents and their valuation distributions. A stronger concept is weakly dominance (where optimality is against any strategies) and the strongest is  ex-post dominance, where optimality is achieved at any possible profile of valuations.
\begin{definition2}

\textbf{Nash equilibrium} 
A profile of strategies $(\beta_{1},\dots,\beta_{n})$ is \textit{a Bayesian Nash equilibrium} if for all player $i \in \mathcal{N}$, 
\begin{equation*}
\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \quad U_{i}(\beta_i,\beta_{-i},x_i)  \geq U_{i}(\beta,\beta_{-i},x_i) \;.
\end{equation*} 

\noindent \textbf{Weak dominance} A strategy $\beta_i$ is  weakly dominant for player $i \in \mathcal{N}$, 
\begin{equation*}
\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \forall \beta_{-i} \in  \mathds{B}_{-i}, \quad U_{i}(\beta_i,\beta_{-i},x_i)  \geq U_{i}(\beta,\beta_{-i},x_i) \;.
\end{equation*}

\noindent \textbf{Ex-Post Weak dominance} A strategy $\beta_i$ is  ex-post weakly dominant for player $i \in \mathcal{N}$ if
\begin{equation*}
%\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \forall \beta_{-i} \in  \mathds{B}_{-i}, \forall x_{-i} \in \mathcal{X}^{N-1},\quad u_{i}((\beta_1(x_1),\dots,\beta_i(x_i),\dots,\beta_N(x_N)),x_i)  \geq u_{i}((\beta_1(x_1),\dots,\beta(x_i),\dots,\beta_N(x_N)),x_i) \;.
\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \forall \beta_{-i} \in  \mathds{B}_{-i}, \forall x_{-i} \in \mathcal{X}^{N-1},\quad u_{i}((\beta_i(x_i),\beta_{-i}(x_{-i})),x_i)  \geq u_{i}((\beta(x_i),\beta_{-i}(x_{-i})),x_i) \;.
\end{equation*}
\end{definition2}

%
%
%A strategy which is optimising the expected utility of one bidder for any valuation and for any strategies of the other bidders is said dominant. 
%\begin{definition2}[(Weakly) dominant strategy]
%A strategy $\beta^{*}$ is  ex-post weakly dominant for player $i$ if for all $\beta_{-i} \in  \mathds{B}^{N-1}$, for all $\beta \in \mathds{B}$ and for all $x \in X^{N}$:
%
%\end{definition2}

As mentioned before, those properties of strategies are classical in game theory. On the other hand, it is also possible to introduce and study different properties of mechanisms. Some of them require the concept of ``truthful bidding'' which correspond to the specific strategy $\beta_i(x)= x$. We will denote by $\beta_{tr}$ this truthful strategy.

\begin{definition2} A mechanism is
\begin{description}
\item[(BIC)] Bayesian Incentive-Compatible:  if all bidders bidding truthfully is a Bayesian Nash equilibrium.
\item[(DSIC)] Dominant Strategic Incentive-Compatible:  if bidding truthfully is a weakly dominant strategy for all bidder.
\item[(Standard)] if it allocates the item to the buyer with the highest bid.
\item[(Efficient)] if it allocates the item to the buyer with the highest valuation (at least for some equilibrium).
\item[(IR)]  interim Individually-Rational: if 
\begin{equation*}
 \forall x_i \in \mathcal{X}_i, \quad U_{i}((\beta_{tr}, \beta_{tr}),x_i) \geq 0\;.
 \end{equation*}
 and ex-post Individually-Rational: if 
 \begin{equation*}
 \forall x_i \in \mathcal{X}_i,  \forall x_{-i} \in \mathcal{X}_{-i}, \quad u_{i}\big((x_i, x_{-i}), x_i\big) \geq 0\;.
\end{equation*}
\end{description}
\end{definition2}

A DSIC mechanism is obviously a BIC mechanism. More generally,  Incentive Compatible (IC) auctions have the nice property of being ``simple'' for the buyers:  bidding the true valuation is optimal. Notice  that this unfortunately does not ensure the uniqueness of equilibrium where each bidder bids truthfully (we will call this equilibrium the  \textsl{truthful equilibrium}). Indeed, there exist many other equilibria such as the following one: every bidder always bids 0 except one of them bidding arbitrarily high. Those are pathological equilibria and will be discarded in the following. As we will see later on, being DSIC is one of the main reasons explaining the tremendous success of second-price auctions. Another reason is that if bidders are bidding truthfully, then the  the seller can elicit their value distribution to deviate to another  mechanism that maximizes her revenue (this is detailed in Section \ref{Section:RevenueMax}) - even if it is at the cost of efficiency.


 
\medskip
Finally, before presenting and analyzing two classical types of auction, we indicate that individual rationality simply ensures that bidders have interest to take part in these auctions.

\section{Sealed-bid auctions}
In a sealed-bid auction bidders privately send their bid to the seller. This class of auctions excludes the well-known ascending auction where bidders can observe bids from other bidders and progressively accept to increase their bid until only one bidder remains. On the other hand,  if bidders' valuations are independent, there exists a strategic-equivalence between the ascending auction and a classical sealed-bid auction which is called the \emph{second-price auction}, introduced below along with another classical sealed bid auction, the \emph{first-price auction}.
\subsection{The sealed-bid second-price auction}
The second-price auction allocates the item to the highest bidder who pays the highest bid among other bidders, i.e., the second highest bid. A key property of this auction is the following result, that does not require any assumption on bidders' value distributions. 

\begin{theorem2}
The second-price auction is DSIC (bidding truthfully is weakly dominant). 
\end{theorem2}
\begin{proof}
Let us denote by $x_i$ the private value of bidder $i$ and by $b^*_{-i}$ the highest bid of the competition. We are going to compare the utility of bidding  $b$ instead of $x_i$.
\begin{itemize}
\item If $b > x_i$. The only case where his (ex-post) utility is changed is when $x_i < b^*_{-i} < b$. With a bid $b$, he now wins the auction but his utility is negative since $x_i - b^*_{-i} < 0 $.
\item  if $b < x_i$. The only case where his (ex-post) utility is changed is when $x_i > b^*_{-i} > b$. With a bid $b$, he now loses a profitable  (i.e., with a positive utility) auction.
\end{itemize}
Hence, bidder $i$ has not interest to deviate  from truthful bidding. 
\end{proof}
The classical second-price auction was used until recently by most of the biggest online platforms to sell ad placements on publishers' websites. Another widely used and studied sealed-bid auction is the first-price auction.
\subsection{The sealed-bid first-price auction} 
\label{first-price-auction}
The first-price auction allocates the item to the highest bidder who pays his own bid.

\medskip

Before studying Nash equilibria of symmetric first-price auction, we derive the general best reply of player $i$ to the bid distribution of the competition, and in particular the distribution of the maximum bid of the competition.

\begin{proposition2}\label{Prop:BestReply1st}
The best reply of bidder $i$ to the distribution of the highest bid of the competition with a cdf denoted by $G_i$ and a pdf denoted by $g_i$ is 
\begin{equation*} \label{eq:bestresponsefirstprice}
\beta_i(x_i), \text{ a solution of } b = x_i - \frac{G_{i}(b)}{g_{i}(b)}\,,
\end{equation*}
which as a meaning  as soon as $G_i(x_i)>0$. In the other case, if $G(x_i)=0$ the best response is $\beta_i(x_i)=x_i$.
 \end{proposition2}
\begin{proof}
Let us denote by $B_{-i}$ the random variable corresponding to the maximum bid of the competition of bidder $i$, so that its cdf and pdf are $G_i$ and $g_i$. We denote by $\mathcal{U}_i(b_i,x_{i}):\mathds{R}^{+}\times\mathds{R}^{+}\rightarrow \mathds{R}$ the associated expected utility of bidder $i$ when his private value is $x_i$ and he bids $b_i$. 
$$
\mathcal{U}_i(b_i,x_i) = \mathds{E}_{B_{-i}}\Big[(x_i-b_i)\mathds{1}\{b_i>B_{-i}\}\Big] = G_i(b_i)(x_i-b_i)\;.
$$
The derivative with respect to $b_i$ is then equal to 
$$
\frac{\partial \mathcal{U}_i(b_i,x_i)}{\partial b_i} = g(b_i)(x_i-b_i) - G(b_i).
$$
Let us assume that $G(x_i) >0$, then $\mathcal{U}_i(x_i,x_i)=0$ but $\frac{\partial \mathcal{U}_i}{\partial b_i}(b_i,x_i) <0$. This first implies that there exists  bids where the utility is positive; moreover,   Rolle theorem also gives the existence of a point $b_i^*$ where  $
\frac{\partial \mathcal{U}_i}{\partial b_i}(b^*_i,x_i) =0$. If $g(b^*_i)=0$ then necessarily $G(b^*_i)$ is also equal to 0 and $\mathcal{U}_i(b_i^*,x_i)$ would be equal to 0 which contradict the fact that $b^*_i$ maximizes the utility.

The case where $G(x_i)=0$ is trivial as bidder $i$ cannot have a positive utility. Bidding $x_i$ is then optimal.
\end{proof}


With symmetric bidders (i.e., with identical value distributions), it is possible to solve explicitly this system of equations and to derive the unique symmetric  Nash equilibrium with increasing strategy. From now on, we will call an Nash equilibrium  \emph{increasing} if the  strategies  are all increasing mappings. 
\begin{theorem2}%[Nash equilibrium in a first-price auction]
If bidders are symmetric, there exists a symmetric Nash-equilibrium whose strategy is described by:  
\begin{equation*}
\beta(x) = \mathds{E}[X^{(1)}_{-i} | X^{(1)}_{-i} < x]\;.
\end{equation*}
where $X^{(1)}_{-i}$ the highest value among bidders except bidder $i$. As a consequence, the first-price auction is not BIC.
\end{theorem2}
\begin{proof}
Let us assume that all bidders are using the function $\beta$ described above. We denote by $x_i$ the private value of bidder $i$, by $b_i$ his bid and by $H$ the maximum of the support of $F$. Bidder $i$ has no interest to bid higher than $\beta(H)$. Then,  $b \in [0,\beta(H)]$ and since $\beta(0) =0$ and $\beta$ continuous, there exists $z \in [0,H]$ such that $b = \beta(z)$:
\begin{align*}
\mathcal{U}_i(\beta(x),x) - \mathcal{U}_i(b,x) &= \mathcal{U}_i(\beta(x),x) - \mathcal{U}_i(\beta(z),x)
\\&= G_i(x)\left(x - \frac{\int_{0}^{x} y g(y) dx}{G_i(x)}\right) - G_i(z)\left(x - \frac{\int_{0}^{z} y g_i(y) dx}{G_i(z)}\right)
\\& = x(G_i(x) - G_i(z)) - \int_{x}^{z} y g_i(y) dx 
\\&\leq 0\;.
\end{align*}
Thus, bidder $i$ has no interest to deviate from $\beta$ and   $(\beta,\dots,\beta)$ is a symmetric Nash equilibrium.   We will prove the unicity of this increasing symmetric Nash equilibrium  in symmetric first-price auctions later on,  in Section \ref{sec_rev_equi}. 
\end{proof}

There exists a very rich line of work focusing on deriving Nash equilibria in first-price auctions when bidders have different value distributions. This involves solving complex systems of coupled first-order differential equations (at least with continuous value distributions). The equilibrium strategy of each  bidder depends in a very subtle manner of the other bidders strategies  \citep{LebrunFirstPriceAsymmetric1999}. Indeed, let us assume that the distributions $F_1,\ldots,F_n$ are supported on $[h,H]$ with a density  bounded away from 0 on this interval and, possibly, a point mass  at $h$. This assumption comes from practical  -- as many auctions have 0 value to online advertisers -- and technical -- if a common reserve price is set at $r>h$, then distributions can be assumed to be  supported on $[r,H]$ with a point mass at $r$  \citep{LebrunFirstPriceAsymmetric1999}. 
\begin{theorem2}\label{thm:SystemEquiAsymetricFirstPrice}
Under these  assumptions, there exist deterministic Nash equilibrium strategies that are increasing that satisfy the following equation. Let us denote them by $\beta_i$ and by $x_i(b)=\beta_i^{-1}(b)\geq b$ their inverse, i.e., the value inducing the bid $b$. Then the increasing functions $x_i$ are solution of the system of differential equations for $1\leq i \leq n$: 
\begin{equation}\label{eq:equilibrium1stPriceAsymmetric}
\frac{\partial}{\partial b}\log(F_i(x_i(b)))=\frac{-1}{x_i(b)-b}+\frac{1}{n-1}\sum_{j=1}^n \frac{1}{x_j(b)-b}\;. 
\end{equation}	
When the distributions are without atoms, the boundary conditions are that 
$x_i(h)=h$ for all $i \in \mathcal{N}$, and there must exists $\eta>0$ such that $\beta_i(H)=\eta$. 
\end{theorem2}
The boundary conditions mean that the bidders bid their value at $h$ and have a common maximal bid \citep{FibichGaviousAsymmetricFirstPricePerturbApproach2003}. The system of equations can actually be easily deduced by applying a perturbative approach similar to that demonstrated earlier. 

Because of the the envelope theorem and arguments similar to those used to derived the revenue maximizing auctions, the equilibrium strategy must satisfy 
$$
\beta_{i}(x)=x-\frac{\int_0^x G_i(\beta_i(t))dt}{G_i(\beta_i(x))}\;,
$$ with $G_i$ the distribution of the highest bid of the competition \citep{KirkegaardAsymmetricFirstPrice2009}.
The expected payoff of player $i$ at $x$ is then equal to $u_i(x,\beta_{i}(x))=\int_0^x G_i(\beta_i(t))dt$ and in particular it holds  that $\mathds{E} U_i (\beta,x_i)=\ \mathds{E}_{x_i\sim F_{i}}\big[G_i(\beta_i(x_i))(x_i-\psi(x_i))\big]$. 

\begin{proposition2}
At equilibrium, the seller revenue coming from bidder $i$ is 
\begin{equation}\label{eq:RevSeller1stPriceWithVValue}
 \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;,
\end{equation}
where $\psi_i$ is the virtual value associated with the value distribution of $X_i$. 
\end{proposition2}
\begin{proof}
We note that 
$$
 \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\int_0^{\infty}\beta_{i,\text{eq}}(x) G_i(\beta_i(x)) f_i(x) dx =\int_0^{\infty} xG_i(\beta_i(x))f_i(x)dx - \int_0^{\infty}f_i(x)\int_0^x G_i(\beta_i(t))dt dx\;.
$$	
Using Fubini's theorem, we have 
$$
\int_0^{\infty}f_i(x)\int_0^x G_i(\beta_i(t)))dt dx=\int_0^{\infty}f_i(x)G_i(\beta_i(t))dt \indicator{t\leq x} dx dt=\int_0^{\infty}(1-F_i(t))G_i(\beta_i(t))) dt\;.
$$
We conclude that 
$$
 \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\int_0^\infty G_i(\beta_i(x))\left[x-\frac{1-F_i(x)}{f_i(x)}\right]f_i(x) dx = \mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi(x_i)\big]\;.
$$
\end{proof}
Finding the solution to the differential system \eqref{eq:equilibrium1stPriceAsymmetric} is considered hard essentially because the solutions are instable near the boundary \citep{MarshallNumericalAnalysis1stPrice94}. The case of $n=2$ bidders has received a fair amount of attention both from a theoretical and numerical perspectives \citep{FibichGaviousDynamicalSystem2012}. A concurrent approach  expands the functions appearing in yet another form of the differential system of equations in a fixed polynomial basis \citep{NumericalSolutionsFirstPriceGayle2008}. 

Hence, unlike second-price auctions, first price auctions are not incentive compatible. As a consequence, the strategy of a bidder at an equilibrium  depends on the bidding strategy of the other bidders, and ultimately on their valuations distribution, see Proposition \ref{Prop:BestReply1st}. So in practice, computing the ``appropriate'' bidding strategy would require estimating the distribution of the highest bid of the competition, which is quite challenging. Nevertheless, first-price auctions are more and more used in online advertising auctions which results in more complexity for bidders.

\section{A revenue equivalence theorem}
\label{sec_rev_equi}
Revenue equivalence theorems are general results claiming that different auction systems  -- sharing similar properties -- are equivalent in terms of expected revenue \emph{at a specific equilibrium}.  The first revenue equivalence theorem showed that the sealed-bid second-price auction and the ascending auction lead to the same revenue for the seller \citep{vickrey1961counterspeculation}. This result has later on be extended to all standard auctions showing the equivalence, for instance, between a first-price and a second-price auction in the case where all bidders have the same value distribution \citep{Myerson81}. 

\begin{theorem2}%[Revenue equivalence]
\label{Th:RevEquivalence}
Consider the family of auctions that are both

 i) \textsl{standard} (i.e., the winner is the bidder with the highest bid)

 ii) \textsl{0-rational} (i.e., winning the auction with a bid of 0 induces a payment of 0).

\noindent Then in the symmetric case, the seller's revenue and bidders' utilities at a symmetric increasing Nash equilibrium are independent of the  specific payment and allocation rules.
\end{theorem2}
\begin{proof} 
Given a specific standard auction, let $\beta$  be an  strategy at an increasing symmetric Nash equilibrium. Let us denote by $P(x_i)$ the corresponding expected payment of player $i$ when his value is $x_i$ and the other bidders are using $\beta$. As before, we  denote by $G_i$ the distribution of $X^{(1)}_{-i}$, the highest value among all the bidders except bidder $i$. We can still assume that a deviation of bidder $i$ consists in  bidding $\beta(z)$ instead of $\beta(x_i)$ (because the auction is standard and $\beta$ is increasing). In particular, the expected utility for bidder $i$ of this deviation writes as
\begin{align*}
\mathcal{U}_i(z,x_i) = x_iG_{i}(z) - P_i(z)\;.
\end{align*}
where  $$P_{i}(x_i) =  \mathds{E}_{F_{-i}}\Big[p(x_i,x_{-i})\Big] = \int_{\mathcal{X}_{-i}} p(x_i,x_{-i})f_{-i}(x_{-i})dx_{-i} \;.$$

Since $\beta$ is a strategy corresponding to a Nash equilibrium, then necessarily 
$$
\mathcal{U}_i(x_i,x_i) = \max_{z}  \, x_iG_i(z) - P_i(z)  \quad 
$$
(which implies that $x_i \mapsto \mathcal{U}_i(x_i,x_i)$ is convex) and, assuming differentiability, it  holds that
\begin{equation*}
\frac{\partial \mathcal{U}_i}{\partial z} (x,x) = xg_i(x) - P_i'(x) = 0\;.  
\end{equation*}
Thus, since $P_i(0)=0$ because of 0-rationality, we finally get that
\begin{equation*}
P_i(x) = P_i(0) + \int_{0}^{x} sg_i(s)ds = G_i(x)\mathds{E}[X^{(1)}_{-i}|X^{(1)}_{-i} < x]\;.
\end{equation*}
In particular.  the expected payment of bidder $i$ is independent of the specific auction. As a consequence, so are  the expected seller's revenue and the utility of bidder $i$, because  the auction is standard.

Finally, we assumed in the proof that $P$ is  differentiable (for the sake of exposition). This assumption is not necessary and can be handled using the convexity of $x_i \mapsto \mathcal{U}_i(x_i,x_i)$ similarly to the proof of the more general Theorem \ref{Th:MyersonLemma}.
\end{proof}
\begin{remark2} This proof exhibits a principled way to get necessary conditions on bidding strategies satisfying a Nash equilibrium, as illustrated below. \end{remark2}

\subsubsection{Informal derivation of first-price auction equilibrium} Denote by $\beta$ the common strategy of an increasing Nash equilibrium of the first-price auction. Conducting the same computations than in the proof of Theorem \ref{Th:RevEquivalence}, assume that all bidders  but $i$  follow $\beta$ and that bidder $i$ is bidding $\beta(z)$ instead of $\beta(x)$ -- we remove the index $i$ by symmetry here to lighten notations. Then his utility rewrites in the specific case of first price auction into 
\begin{equation*}
\mathcal{U}(\beta(z),x) = (x - \beta(z))G(z)\;. 
\end{equation*}
Differentiating with respect to $z$, since $\beta$  is a  symmetric increasing Nash equilibrium, yields 
\begin{equation*}
0=\frac{\partial \mathcal{U}}{\partial z} (x,x) = (x-\beta(x))g(x) - \beta'(x)G(x)\;.
\end{equation*}
Notice that the above equation can be rewritten in the following more compact form, 
\begin{equation*}
(\beta(x)G(x))' = xg(x)\;.
\end{equation*}
so that we can finally compute explicitly the symmetric equilibrium strategy
\begin{equation*}
\beta(x) = \frac{\int_{s=0}^{x}sg(s)ds}{G(x)}= \mathds{E}[X^{(1)}_{-1}|X^{(1)}_{-1}<x]\;.
\end{equation*}
This proves the uniqueness of  increasing Nash equilibria  in a symmetric first-price auction. 

\begin{remark2} Importantly, the revenue equivalence theorem assumes that bidders have all the same value distributions. There exists asymmetric cases where the first-price auction brings more revenue than the second-price auction and conversely \citep{krishna2009auction}. \end{remark2}
\section{Deriving revenue-maximizing auctions}
\label{Section:RevenueMax}
We now focus on how the seller can design her auction system to maximize her revenue. A large part of the recent literature on auctions have focused on this objective since most of the auctioneers have the choice to design the rules of their respective auction platform.

To compute the optimal revenue-maximizing auction, we assume that the seller has a prior distribution $F_i$ on each bidders' valuations.  By design, these value distributions quantify the information that the seller owns on each specific bidder. 

\subsection{The role of reserve prices}
Setting reserve prices is a crucial tool to maximize seller's revenue in classical auctions. To illustrate its role, we focus on the second-price auction. 
\begin{definition2}
The reserve price is the minimum price a bidder must pay to acquire an  item. The reserve price is  \textit{anonymous} (respectively \emph{personalized}) if it is the same for all bidders (if it is different from one bidder to the other).
\end{definition2}
In a second-price auction with reserve prices, the buyer that wins the auction, must have bid above his reserve price and is paying the maximum between the latter and the second highest bid. A crucial point  is that, in expectation,  it can be beneficial for the seller to sometimes not allocate the item, so that when it is sold, the payment is higher because of the reserve price. 

To illustrate this point, we quickly recall a historical example, the New-Zealand radio spectrum rights auction \citep{milgrom2004putting}. In 1990, the NZ government decided to sell some radio spectrum rights through multiple simultaneous sealed-bid second-price auctions without reserve prices. These auctions were expected to raise around NZ\$250 millions. Instead, the government revenue was around NZ\$36 millions. On many licenses, there was a huge discrepancy between the first and the second bid. For instance, a firm bid NZ\$100 000 and the second price was only NZ\$36\dots If some reserve price were imposed beforehand, it would have insured to the government that the firm who made a bid of NZ\$100 000 would have paid a price sufficiently high. 

This example illustrates the importance of reserve prices. A first way to set a reserve price would be to assume that the seller can give an intrinsic value for keeping the item. This could be a valid assumption for the housing or wine auctions. However, in many other situations (TV rights, radio spectrum rights auctions..), the seller does not have any intrinsic value for the item. For illustrating purpose, we compute in the simple case of a single buyer the optimal reserve price. As before, we denote by $F$ the cdf of the buyer valuation, and for the sake of simplicity, we assume it has a density $f$ (again, all the following results generalize to arbitrary distributions, but at the cost of technicalities) and has finite expectation.


%\iffalse and the need for a careful modelisation of the different incentives of the system. {\color{red}VP: la phrase suivante est moche, et il faut une reference et/ou plus d'explications} For instance, in the recent sell of French football TV rights, in 2017, the auctioneer was very careful on its definition of the reserve prices by setting very specific reserve prices for every TV rights packages. 
%\fi
\subsection{The posted price setting: monopoly pricing}
\label{monopoly-pricing}
In this  warming-up, simple  setting, designing an auction simply reduces to  a \textit{take-it-or-leave-it} offer, i.e.,  a fixed selling price. A rational bidder will accept to pay it to acquire the item if, and only if, it is smaller than his valuation. 
\begin{lemma2}\label{TH:Monopoly}
The optimal reserve price, called \emph{the monopoly price}, is a solution of :
\begin{equation*}
0=rf(r) - (1-F(r)) = f(r)\Big(r- \frac{1-F(r)}{f(r)}\Big)\;. 
\end{equation*}
\end{lemma2}
\begin{proof}
The seller's revenue can be written as a function of $r$ as:
\begin{equation*} 
\Pi(r) = \int_{r}^{+\infty} rf(x)dx = r(1-F(r))\;.
\end{equation*}
The result follows from differentiating, since
\begin{equation*} 
\frac{d\Pi(r)}{dr} = (1-F(r)) - rf(r) \;,
\end{equation*}
and choosing $r=0$ or $r$ arbitrarily high gives a 0 revenue (because of the mild assumption on $F$).
\end{proof}
%\iffalse
%\begin{figure}[H]
%\includegraphics[width=.5\linewidth]{images/monopolistic_revenue}
%\caption{Seller's revenue as a function of the reserve price. The revenue is computed based on $r(1-F(r))$ with $F = \mathcal{U}([0,1])$.}
%\end{figure}
%{\color{red} VP: Quel est l'interet du paragraphe suivant ?} 
%The setting of posted price is very related to the setting where a monopolistic firm sells a service to different customers. She must define a single price for all her clients. She will choose the monopoly price corresponding to the distribution of values representing her customers. Sometimes, the firm prefers not to sell the item and sacrifies a bit of short-term revenue to insure that in most other cases, buyers will pay a price sufficiently high.  
%\fi
\bigskip
Notice that without the assumption that $F$ has a finite expectation, the optimal reserve price could be arbitrarily high. 
Actually,  the main purpose of the single bidder case is  to introduce the crucial concept of \textit{virtual value}. 
\begin{definition2}%[Virtual value]
The virtual value function $\psi : \mathcal{X} \to \mathds{R}$ of a distribution $F$ (with pdf $f$) is: 
\begin{equation*} 
\psi(x) = x - \frac{1-F(x)}{f(x)}\;.
\end{equation*}
\end{definition2}
We emphasize here that the virtual value function can be either positive or negative, irrespectively of the support of the (true) value distribution. The expected virtual value is actually equal to the minimum of the support of $F$. In particular, it is equal to 0 if the support of $F$ starts at 0 and in that case, the virtual value is necessarily sometimes negative (at least around $x=0$) and sometimes positive (at least around the supremum of the support of $F$).

The virtual value $\psi(x)$ is a crucial concept that can be interpreted as follows. If the bidder has a value $x$ and decides to buy the item, his (virtual) payment can be set as $\psi(x)$,  \textsl{independently} of the price $r$ fixed by the seller. Indeed, the revenue generated by such a price $r$ is
$$
r(1-F(r) ) = \int_r^\infty xf(x) - (1-F(x)) dx = \int_r^\infty \psi(x) f(x)dx = \mathds{E}_{X \sim F} [ \psi(X) \mathds{1}\{X \geq r\}]\,.
$$
As a consequence, even though it is traditionally called virtual value, $\psi(x)$ should rather be understood as a virtual \textsl{payment}.

\subsubsection{Examples of virtual value/payment functions:} 
\begin{itemize}
\item if $x\sim\mathfrak{U}([0,1))$, the uniform distribution over $[0,1]$, then $\psi(x)=2x-1$ for $x \in [0,1]$
\item if $x\sim \mathfrak{E}\mathrm{xp}(\lambda)$, the exponential distribution, then  $\psi(x)=x-\lambda$ for $x \in \mathds{R}_+$
\item The family of Generalized Pareto distributions, parametrized by $(\mu,\sigma,\xi)$ where $\sigma >0$ and $\xi\leq 0$, has distribution 
\begin{equation*}
F_{\mu,\xi,\sigma}(x)   = \begin{cases} 1-(1 +\frac{\xi (x-\mu)}{\sigma})^{-1/\xi} & \text{for } \xi < 0 \\
1-e^{-(x-\mu)/\sigma} & \text{for } \xi= 0\end{cases}
\end{equation*} and its virtual value is affine \citep{balseiro2020multistage}
$$\psi_{\mu,\xi,\sigma}(x) = (1-\xi)x+\xi\mu-\sigma$$
\end{itemize}
%\begin{remark2}
%With $\xi = -1 , \mu = 0, \sigma = 1 $, we recover the uniform distribution. With $\xi = 0 , \mu = 0 , \sigma = 1$, we recover the exponential distribution. With  $ \mu = 1, \sigma = \xi$ , this corresponds the power law (a.k.a the Pareto distribution) with parameter $\alpha = 1/\xi$. Hence, the generalized Pareto distribution are widely used in auction theory due to their flexibility (they model a large spectrum of distributions) and the fact that their virtual value is easy to compute (the virtual value is affine).
%\end{remark2}
\subsubsection{Relationship between  monopoly price and virtual value/payment}
Lemma \ref{TH:Monopoly} states that the optimal reserve price against  a single bidder (which was called the monopoly price)  is, in the case where the virtual value/payment function  $\psi$ is increasing and changes sign, necessarily the root of $\psi$ (or the point where the sign changes if it is not continuous). If $\psi$ is strictly positive everywhere, which can happen if the  the minimum of the support of $F_i$ is positive, then the optimal reserve price is that specific point (or equivalently 0). Quite interestingly, the optimal reserve price of bidder $i$ is still the monopoly price (when facing solely that bidder), even with several other bidders, as illustrated in the following Section \ref{optimal_reserve_for_lazy} under the same assumption on $\psi$. 

 As a consequence, in the following,  we will focus more intensively on these distributions that are called \textsl{regular}. The results we will prove can be generalized to non-regular distribution can be  with a technique called \textsl{ironing}, see Section \ref{Se:Ironing}.  
 \begin{definition2} 
The distribution $F$ is  regular if its corresponding virtual value $\psi$ is increasing.
\end{definition2}

This condition is verified among others by the uniform, the exponential and generalized Pareto distributions with $\xi <1$. % 
%\begin{proposition2}
%If $\psi$ increasing and crossing zero exactly once and F is defined over its full support, then r is the monopoly price if and only if
%$$\psi(r) = 0$$ 
%\end{proposition2}
%\begin{proof}
%The monopoly price r is defined as $$\argmax_r R(r) = r(1-F(r)).$$
%Then, 
%$$
%\frac{dR(r)}{dr} = -f(r)\psi(r)\;.
%$$
%Since $\psi$ increasing, R is concave and $\psi(r)=0$.
%\end{proof}
%If $\psi$ is crossing zero multiple times, the monopoly price also verifies $\psi(r)=0$. 
%One of the beauty of auction theory is that this notion of monopoly price can be extended to auctions with multiple buyers.
\subsection{Optimal reserve prices in a second-price auction}
\label{optimal_reserve_for_lazy}
We  focus in this section on second-price auctions with reserve prices \citep{riley1981optimal} where  $n$ buyers are asymmetric, i.e., their value distribution can be different. As a consequence, the seller might also set different, personalized reserve prices. When introducing the concept of reserve price, we mentioned that a bidder can only win the auction if his bid was bigger than his reserve price and that the latter is the minimal payment he might pay.  This said, there still are some ambiguities on how the auction unfolds (depending on which condition "highest bidders" or "bid above reserve price" is checked first). As a consequence, there exist at least two different types of second-price auction with reserve prices.

\begin{description}
\item[Lazy 2nd-price auction:] The winner can only be the highest bidder. He gets the item only if he  clears his reserve price (i.e., his bid is above it),  and he pays the maximum between his reserve price and the second bid. 
\item[Eager 2nd-price auction:] Bidders that have not cleared their respective reserve price are  disregarded. Thus the winner is the highest bidder amongst those that have cleared their reserve price and he pays the maximum between his reserve price and the second highest cleared bid.
\end{description}


First of all, notice that if the reserve prices are anonymous, as they should be in the symmetric case for instance, both concepts of auctions coincide.  Optimal reserve prices are easy to compute in the lazy auctions, with an explicit form (which is not the case for the eager ones). Moreover, the eager 2nd-price auction is also not the revenue-maximizing auction for the seller, so this concept is neither simple (as the lazy auction) nor optimal (as the Myerson auction, see Section \ref{emp_Myerson}). As a consequence, we will not put too much focus on it. In practice, if one desires to implement eager 2nd-price auction, a good idea would be to use the reserve prices of the lazy one.



\medskip

It is quite immediate to see that lazy and eager second price auctions are still DSIC mechanism (the proof follows the exact same lines that without reserve prices), hence we shall again only consider the truthful equilibrium. We now derive the expected payment of a bidder at this equilibrium.
%\begin{theorem2}[Expected payment in a lazy second-price auction]\label{myerson_for_second_price}
%Consider bidder $i$ with virtual value $\psi_i$ and reserve price $r_i$. We denote by $G_i$ the cdf of $Y_{-i} = max_{j\neq i} X_j$. The expected payment $P_i(\beta_{tr})$ of bidder $i$ in a lazy second-price auction when all bidders are bidding truthfully is equal to:
%\begin{equation*}
%P_i(\beta_{tr}) = \mathds{E}_{x_i\sim F_{i}}\bigg(\psi_i(x_i)G_i(x_i)\textbf{1}_{x_i\geq r_i}\bigg)\;.
%\end{equation*}
%\end{theorem2}
\begin{theorem2}\label{myerson_for_second_price}
Let   $P_i$ be the expected payment of bidder $i$ at the truthful equilibrium of a lazy second-price auction, then \begin{equation*}
P_i = \mathds{E}_{x_i\sim F_{i}}\Big[\psi_i(x_i)G_i(x_i)\mathds{1}\{x_i\geq r_i\|\Big]\;,
\end{equation*} where $G_i$ the cdf of $\max_{j\neq i} X_j$ and $r_i$ is the personalized reserve price of bidder $i$.

\end{theorem2}
\begin{proof} 
Let us introduce the notation $y_{-i}= \max_{j\neq i} x_j$ so that the pointwise payment of bidder $i$ given all the values $x_j$ is equal to: 
\begin{equation*}
\max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x\geq r_i\}\;,
\end{equation*}
As a consequence,
\allowdisplaybreaks
\begin{align*}
P_i&= \mathds{E}_{F_1,\dots,F_n}\Big[\max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x\geq r_i\}\Big]
\\& = \int_{x_i} \int_{y_{-i}} \max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x\geq r_i\}f_i(x_i)g(y_{-i})dy_{-i}dx_i
\\& =\Big(1-F_i(r_i)\Big)G(r_i)r_i + \int_{x_i=r_i}^{+\infty}\int_{y_{-i}=r_i}^{+\infty}y_{-i}g(y_{-i})f_i(x_i)\textbf{1}(x_i \geq y_{-i})dy_{-i}dx_i
\\& = \Big(1-F_i(r_i)\Big)G(r_i)r_i + \int_{y_{-i} = r_i}^{+\infty}y_{-i}g(y_{-i})\int_{x_i=y_{-i}}^{+\infty}f_i(x_i)dy_{-i}dx_i \hspace{2cm} \text{ (by Fubini)}
\\& = \Big(1-F_i(r_i)\Big)G(r_i)r_i + \int_{y_{-i} = r_i}^{+\infty}y_{-i}g(y_{-i})(1-F_i(y_{-i}))dy_{-i} 
\\& = \int_{y_{-i} = r_i}^{+\infty} \Big(f(y_{-i})y_{-i} - (1-F_i(y_{-i}))\Big)G(y_{-i})dy_{-i} \hspace{2.5cm} \text{(by integration by part)}
\\& = \mathds{E}_{F_i}\Big[\psi_i(x)G(x)\mathds{1}\{x\geq r_i\}\Big]\;.
\end{align*}
\end{proof}
We can therefore easily derive the optimal reserve prices, as a function of $\psi_i$ at least for regular distribution.%\begin{definition2} 
%The distribution F  is said regular if its corresponding virtual value $\psi$ is increasing.
%\end{definition2}
%\redtext{changement}
%{\color{red} VP: est-ce qu'on a besoin de ce graphique ? En plus celui en haut a droite deconne, le vert n'est pas aligne avec le trait pointille rouge}
%\begin{figure}[h!]
%\begin{tabular}{cc}
%\includegraphics[width=.50\linewidth]{images/r025}&
%\includegraphics[width=.50\linewidth]{images/r075}\\
%\multicolumn{2}{c}{\includegraphics[width=.50\linewidth]{images/r05}}
%\end{tabular}
%\caption{\textbf{Change in bidder payment as a function of the reserve price.} The value distribution of the bidder is uniform [0,1] with $\psi(x) = 2x -1$, and is represented by the blue line. The dashed red vertical line corresponds to the current reserve price. We picked $G=1$, i.e. no competition. The bidder payment is equal to the area under the curve. The seller has no incentive to set the reserve price lower than $\psi_i^{-1}(0)$ since it decreases her total expected payment (because of the negative contribution of the red area). It is also clear that $r \ge \psi_i^{-1}(0)$ is suboptimal since it results in lost revenue for the seller.}
%\label{fig:visualOptimalR} % I can do without the label too
%\end{figure}
\begin{theorem2}%[Optimal reserve price in lazy second-price auction]
If  $F_i$ are regular, the optimal reserve prices in a lazy second-price auction are:
\begin{equation*}
\bigg(r_1,\dots,r_n\bigg) = \bigg(\psi_1^{-1}(0),\dots,\psi_n^{-1}(0)\bigg)\;,
\end{equation*}
with the convention that $\psi_1^{-1}(0)$ is the minimum of the support of $F_i$ is $\psi_i$ is  positive everywhere and the point where $\psi_i$ changes its sign if it is discontinuous.
\end{theorem2}
\begin{proof} 
The seller maximizes the sum of expected payment: 
\begin{align*}
\mathds{E}_{F_1,\dots,F_N}\Big[\sum_{i=1}^{n} P_i\Big] &= \sum_{i=1}^{n}  \mathds{E}_{F_i}\Big[\psi_i(x_i)G_i(x_i)\mathds{1}\{x_i\geq r_i\}\Big]\;.
\end{align*}
Since $F_i$ is regular, $\psi_i$ has one zero and is negative before the zero and positive after. Thus, the optimal choice for $r_i$ is clearly $\psi_i^{-1}(0)$.
\end{proof}
We see in the proof that in a lazy second-price auction, the seller can safely maximize the payment of each bidder one by one independently. Indeed, in a lazy second price auction, changing the reserve price of one specific bidder does not change the probability of winning and the payment of the other bidders. This is not the case for greedy second-price auction on the other hand, which explains the complexity of computing the optimal reserve prices in them. Finally, the optimal reserve prices in a lazy second-price auction correspond to the monopoly prices of each bidder.



\begin{corollary2}The optimal reserve price for a bidder in a lazy second-price auction is independent of the presence, or not, of other bidders. In particular, it is the same as in the situation where he is the only and single bidder.
\end{corollary2}

\begin{figure}[H]
\includegraphics[width=.6\linewidth]{images/optimalmonopolyprice.pdf}
\caption{Bidder's payment as a function of the reserve price depending on the number of players in second-price auction with bidders all having a uniform value distribution $\mathfrak{U}([0,1])$.}
\end{figure}
%The proof also shows that when the distribution is not regular, the optimal reserve prices for each bidder verifies: $r_i \in \argmax(\mathds{E}_{F_i}(\psi_i(x)G(x)\textbf{1}_{x\geq r_i}))$.

The seller's revenue increases through the use of personalized reserve prices when bidders have very different value distributions. Intuitively, it is in the seller's best interest to set a high reserve price to bidders who have most of the time high values and low reserve prices to bidders who have most the time low values.

So far, we have only focused on the seller's revenue when designing auctions. An alternative objective can be the maximization of the  \textsl{global welfare} of the system, which is the sum of the seller's revenue and all bidders' utility. 

\bigskip


Even though reserve prices largely increase the seller's revenue, they actually significantly decrease of the expected total welfare, as the item will sometimes not be allocated, as soon as  all (or at least the highest in lazy auction) bidders have values below their reserve prices.

\begin{example2}
To illustrate this decrease in welfare, we are going to consider a simple toy example.  There are $n=2$ symmetric bidders with a value drawn uniformly over $[0,1]$. Because of the  symmetry, the optimal reserve price is the same for both bidders hence lazy and eager auctions coincide (and we do not need to specify the rule).  In this simple case, $r^* = \psi^{-1}(0) = 1/2$. As a consequence, the item is allocated as soon as one  bidder bids above 1/2, which happens with probability $3/4$. Otherwise, the item is not sold (which obviously happens with probability $1/4$). Simple computations shows that changing the design from a second-price auction without reserve price to a second-price auction with optimal reserve price yields 
\begin{itemize}
\item a \textbf{12,5 \% decrease} of the global welfare (from $2/3$ to $7/12$).
\item a \textbf{50 \% decrease} of a bidder's utility  (from $1/6$ to $1/12$).
\item a \textbf{25 \%  increase} of the seller's revenue (from $1/3$ to $5/12$).
\end{itemize}
\end{example2}



\subsection{Myerson's lemma}
We mentioned before that the virtual value could (and probably should) be understood rather as a virtual payment in a single bidder auction and/or in lazy second price auctions. The following lemma (that will be referred to as the ``Myerson Lemma'') is a crucial result \citep{Myerson81}. It states that virtual payment of a bidder is the correct quantity to study in any  incentive-compatible auctions, and not just lazy second-price. The proof, while conceptually profound, is not very hard technically and requires integration by part and Fubini's theorem as we used in the case of the lazy second-price auction. This result holds for any Bayesian Incentive Compatible auction (if bidding truthfully is weakly dominant) that is 0-rational (if bidding 0 ensures a payment of 0). The latter assumption can be weakened, at the cost of an additive constant in the payment formula. 
\begin{theorem2}%[Myerson lemma]
\label{Th:MyersonLemma}
For any BIC and 0-rational auction, the expected payment of bidder $i$ at the truthful equilibrium is 
\begin{equation*} 
\mathds{E}_{x_i\sim F_i}[P_i(x_i)] = \mathds{E}_{x_i \sim F_{i}}[\psi_i(x_i)Q_i(x_i)] = \mathds{E}_{x \sim \mathcal{F}}[\psi_i(x_i)q_i(x)]
\end{equation*}
where $Q_i(x_i)$ is the winning probability  of bidder $i$  at the truthful equilibrium given his value  $x_i$.
\label{myerson_lemma}
\end{theorem2}
\begin{proof}
By definition of Bayesian incentive-compatibility, the auction must verify: 
\begin{equation*}
\forall z \in \mathds{R}^{+}, \forall x_i \in \mathds{R}^{+}, Q_i(x_i)x_i - P_i(x_i) \geq Q_i(z)x_i - P_i(z)
\end{equation*}
Thus, if we denote by $\mathcal{U}_i(x_i)$ the expected utility of bidder $i$ when he has value $x_i$, 
\begin{equation*}
\mathcal{U}_i(x_i) = \max_{z} Q_i(z)x_i - P_i(z)
\end{equation*}
As a consequence, $\mathcal{U}_i$ is a  convex mapping (the maximum of affine mappings) and therefore is differentiable almost everywhere and absolutely continuous (i.e., it is equal to the integral of its derivative).

Bayesian-incentive compatibility also implies that
\begin{equation*}
\forall z \in \mathds{R}^{+}, \mathcal{U}_i(z) \geq \mathcal{U}_i(x_i) + Q_i(x_i)(z-x_i) \;,
\end{equation*}
and since $\mathcal{U}$ is convex, this yields
\begin{equation*}
Q_i(x_i) \in \partial \mathcal{U}_i(x_i)\;,
\end{equation*}
and  $\nabla \mathcal{U}_{i}(x_i) = Q_i(x_i)$  if  $\mathcal{U}_i$ differentiable at  $x_i$. Therefore,
\begin{equation*}
P_i(x_i) = P_i(0) + Q_i(x_i)x_i - \int_{0}^{x_i}Q_i(z)dz
\end{equation*}
and taking the expectation over $x_i$ gives: 
\begin{align*}
 \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] &= \int_{x_i}P_i(x_i)f_i(x_i)dx_i 
\\&=  P_i(0) + \int_{x_i} \Big(Q_i(x_i)x_i - \int_{0}^{x_i}Q_i(z)dz\Big)f_i(x_i)dx_i
\\& = P_i(0) + \int_{x_i} Q_i(x_i)x_if_i(x_i)dx_i - \int_{z}Q_i(z)\Big(\int_{z}^\infty f_i(x_i)dx_i\Big)dz \qquad \text{ (Fubini) }
\\& = P_i(0) + \int_{x_i} \Big(x_i - \frac{1-F_i(x_i)}{f_i(x_i)}\Big)Q_i(x_i)f_i(x_i)dx_i 
\\&= P_i(0) + \int_{x} \Big(x_i - \frac{1-F_i(x_i)}{f_i(x_i)}\Big)q_i(x)f(x)dx
\\& =  P_i(0) + \mathds{E}_{x \sim \mathcal{F}}[\psi_i(x_i)q_i(x)] = P_i(0) + \mathds{E}_{x_i \sim F_i}[\psi_i(x_i)Q_i(x_i)]\;.
\end{align*}
The result follows from the fact that $P_i(0) =0$ since the auction is 0-rational.
\end{proof}
\begin{remark2}
Notice that Theorem \ref{myerson_for_second_price} is a direct consequence  of this result with the specific choice of $Q_i(x_i) = G_i(x_i)\mathds{1}\{x_i\geq r_i\}$
\end{remark2}
Myerson lemma indicates that the expected payment of a BIC auction only depends on the allocation rule and the virtual value; the proof actually gives a characterization of any incentive-compatible auction.  However, this characterization is slightly different for  BIC and DSIC auctions. 
\begin{corollary2}%[characterization of BIC auctions]
[\cite{Myerson81}]
\label{characterization_inc_comp}
An auction is BIC if and only if
\begin{itemize}
\item[i)] the allocation rule is monotone, i.e.,  the probability of winning, as a function of the bid, is non-decreasing (for any fixed bids of others bidders)  and
\item[ii)] the expected payment verifies 
$$P_i(x_i) = Q_{i}(x_i)x_i - \int_{0}^{x_i} Q_{i}(z)dz.$$
\end{itemize}
\end{corollary2}
\begin{proof} 
The proof of Theorem \ref{myerson_lemma} gives the first implication. For the reverse, if the auction verifies 
$$P_i(x_i) = Q_{i}(x_i)x_i - \int_{0}^{x_i} Q_{i}(z)dz\;,$$
then it implies that the auction verifies  $\nabla \mathcal{U}_i(x_i) = Q_{i}(x_i)$.

Since the probability of winning is increasing as a function of the bid, $$\mathcal{U}_i(x) - \mathcal{U}_i(z) = \int_{x_i}^{z}Q_{i}(s)ds \geq Q_i(x_i)(z - x_i)$$ which entails that $$\mathcal{U}_{i}(x)\geq Q_i(z)x - P(z).$$ This is the definition of bayesian incentive-compatibility (BIC).
\end{proof}
\begin{corollary2}%[characterization of DSIC auctions]
[\cite{Myerson81}]
\label{corollary_charect_DSIC}
An auction is DSIC if and only if

\begin{itemize}
\item[i)] the allocation rule is monotone and
\item[ii)]  the payment  of the winning bidder is the minimum bid guaranteeing that he would still have won the auction.\end{itemize}
 Given a monotone allocation rule and assuming 0-rationality, the payment rule is unique. 
\end{corollary2}
\begin{proof} 
The proof is almost identical, one just need to make the various computations pointwise (for any vector $x_{-i}$) instead than in expectation.
\end{proof}
This characterization can be extended to very general mechanisms in \citep{archer2001truthful}.
\subsection{The Myerson auction}
Equiped with the Myerson lemma, it is now possible to derive the  revenue-maximizing auction among all BIC auctions. 
\begin{definition2}%[Myerson auction]
The Myerson auction is defined by the two following rules
\begin{description}
\item[Allocation rule:] Given the bids $b=(b_1,\ldots,b_n)$, the winner is the bidder with the highest non-negative virtual value $\psi_i(b_i)$, i.e.,
$$
q(b) = \arg\max \big\{ \psi_i(b_i) \, ; \, i \text{ s.t. } \psi_i(b_i) \geq 0 \big\} 
$$
with the convention that if the set is empty (when all virtual values are negative), then the item is not allocated and $q(b) = 0$. Ties are broken arbitrarily.
\item[Payment rule:] The winner pays the smallest winning bid, i.e., if bidder $i$ won the auction, he pays
$$p_i(b)=\max \Big\{ \psi_i^{-1}(0), \psi_i^{-1}\Big(\max_{j\neq i} \big\{\psi_j(b_j)\big\}\Big) \Big\}$$
\end{description}
\end{definition2}
\begin{theorem2} \label{theorem_regular_distributions}
If $F_1,\dots,F_n$ are regular, the Myerson auction maximizes seller's revenue among all BIC and  interim-IR  auctions.
\end{theorem2}
\begin{proof}
The Myerson auction is BIC as it verifies the condition of Corollary \ref{characterization_inc_comp}. Since $\psi_i$ are non-decreasing (as $F_i$ are regular), the probability of winning is non-decreasing.

To show individual-rationality, we remark that since the auction is BIC, $$\mathcal{U}_{i}(x_i) = \mathcal{U}_{i}(0) + \int_{0}^{x_i}Q_i(s_i)ds_i = -P_{i}(0) + \int_{0}^{x_i}Q_i(s_i)ds_i \geq 0,$$ because $P_i(0) = 0$.  Thanks to  Myerson lemma, the payment of each BIC auction is equal to 
$$
 P_i(0) + \mathds{E}_{x_i \sim F_{i}}(\psi_i(x_i)Q_i(x_i))\;. 
$$
The Myerson auction maximizes the two terms of this expression since for any rational auction, $P_i(0)\leq0$.  Since the winner in the Myerson auction is the bidder who verifies
\begin{equation*} 
\psi_i(x_i) = \arg\max_{j \in S}(\psi_j(x_j))\;,
\end{equation*}
and the item is not allocated when all $\psi_i$ are negative, the second term is also maximized pointwise in the Myerson auction.
\end{proof}
\begin{corollary2} In the symmetric case, the second-price auction with reserve prices set to  monopoly prices is the revenue-maximizing auction.
\end{corollary2}
\begin{remark2} The interim individual rationality assumption can be relaxed \citep{cremer1988full}. Indeed, there exists a BIC auction that accomplishes full-surplus extraction for the seller, i.e., the utility of bidders in this auction is equal to zero and which is ex ante individual rational. This auction is not interim individually-rational since the expected utility when value is zero is strictly negative. It only makes sense when bidders should decide to take part in the auction before understanding their value for the item. We come back in more details on this setting in Section \ref{sub_full_surplus_extraction}.
\end{remark2}
\subsection{Generalization of optimality result}
\label{SE:General_OptimalityResults}
\subsubsection{Non Incentive-Compatible mechanism: the revelation principle}
Myerson's optimality result can be extended to any incentive-compatible auctions, as long as there is a Nash equilibrium between bidders.
\begin{theorem2}%[Revelation principle]
Given a mechanism and a specific Nash equilibrium for this mechanism, there exists another BIC mechanism where the bidders' expected utility and seller's revenue at the truthful equilibrium are equal to the ones at the original Nash equilibrium. 
\end{theorem2}
\begin{proof}
Consider a mechanism and  $\beta = (\beta_1,\dots,\beta_n)$ a profile of strategies that is a Nash equilibrium. This mechanism is defined by an allocation rule $q:\mathcal{B}^{n}\rightarrow \mathds{R}^{n}$ and a payment rule  $p:\mathcal{B}^n\rightarrow \mathds{R}^{n}$. The mechanism $(q \circ \beta, p \circ \beta)$ is then clearly BIC and bidding truthful generate the same bids distributions, allocation and paiement; hence utilities and revenue are unchanged.
\end{proof}
\begin{corollary2} 
The Myerson auction is the revenue-maximizing mechanism among all individually-rational mechanisms which have a Nash equilibrium.
\end{corollary2} 
\begin{proof}
This is a direct application of the revelation principle.
\end{proof}
We now extend the Myerson auction to cases where value distributions are not regular. 
\subsubsection{Non-regular distribution: the ironing technique}\label{Se:Ironing}

If $F_i$ are not regular, the Myerson auction might not be incentive-compatible. Indeed, since $\psi_i$ is non-increasing,  the allocation is not monotone:  a bidder might have incentive to shade (or lower) his bid to increase his virtual bid and his probability of winning. Non-regular distributions are not that uncommon either, as a mixture of two distributions typically is (for instance the mixture of two uniform, Gaussian, etc.). It is therefore crucial to adapt the Myerson mechanism to non-regular distributions. The canonical way is to define a slightly different allocation rule based on a modified virtual value \citep{Myerson81} called the \textit{ironed virtual value}. 

Recall that the principal and most convenient consequence of non-decreasing virtual value is that the monopoly revenue $\Pi(r) = r(1-F(r)) = \int_r^\infty \psi(v)f(v)dv$ is ``almost''  concave, in the sense that $\Pi(F^{-1})(\cdot)$ is concave with derivative  $-\psi\circ F^{-1}(\cdot)$. As a consequence, optimizing the revenue boils down to finding the root of $\psi$.  The ironing technique consists in replacing $\Pi\circ F^{-1}$, which is not necessarily concave, by its concavification. We recall that $\mathrm{cav}(f)$, the concavification of a function $f$, is the the smallest concave function above it; its hypograph is the convex hull of the hypograph of $f$.


\begin{definition2}%[Ironed virtual value] 
For any non-regular distribution $F$, the ironed virtual value of $\psi$, denoted by $\tilde{\psi}$ is defined by
$$
 \tilde{\psi}(x)= - \partial \Big(\mathrm{cav}(\Pi\circ F^{-1})\Big)(F(x))
$$
\end{definition2}

In general, the concavification of a function $g$ is either equal to $g$ at some point or linear on some interval otherwise. Luckily enough, the ironed virtual value as a closed form on intervals where it is not equal to the virtual value.


\begin{lemma2}%[Expression of ironed virtual value on [a,b]] 
Assume that for some $a<b$, it holds that \begin{itemize}
\item[--] $\mathrm{cav}(\Pi\circ F^{-1})(F(a))=\Pi (a)$,  
\item[--]$\mathrm{cav}({\Pi}\circ F^{-1})(F(b))=\Pi(b)$
\item[--] $\mathrm{cav}({\Pi}\circ F^{-1})(F(x)) > \Pi (x)$ for $x \in(a,b)$ 
\end{itemize}then
the ironed virtual value  of $\psi$ on $(a,b)$ is constant and equal to
$$
\tilde{\psi}(x)= \frac{\int_{a}^b \psi(t) f(t) \mathrm{d} t}{F(b)-F(a)}$$
\end{lemma2}
\begin{proof}
By definition of the concavification, $\tilde{\Pi}\circ F^{-1}$ is linear on $[F(a),F(b)]$ and the results comes from linear interpolation.
\end{proof}
%Typically, non-increasing virtual value function are ironed on an interval where it is non-increasing. On the other hand, if the ironing is limited to the smallest interval  where the virtual value is non-increasing, this might not guarantee that the ironed virtual value is increasing. To insure that the ironed virtual value is non-decreasing, the ironing should be extended a larger interval. The final minimal interval $[a_{opt},b_{opt}]$ where the virtual value is ironed should verify the following conditions:
%$$\psi(a_{opt}) \leq \psi([a_{opt},b_{opt}]) \leq \psi(b) \text{ and } \forall c,d \in [a_{opt},b_{opt}], \psi(c) \geq \psi([c,d]) \geq \psi(d)$$
%A good way to visualize how to set $a_{opt}$ and $b_{opt}$ is to plot $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$ as a function of $F(t)$.  We recall that $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t = -b(1-F(b))$, the opposite of the monopoly revenue. The intervals where the virtual value should be ironed are the ones where the convex envelop of $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$ is different from $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$.
%
%\begin{definition2}[Ironed virtual value] Consider a value distribuion F with corresponding virtual value $\phi$. Let $[a_1,b_1],...,[a_k,b_k]$ be the intervals that are straightened out when one takes the convex hull for the plot of the cumulative virtual value $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$ against F(b). The ironed virtual value  of $\psi_i$ denoted by $\tilde{\psi}_i$ is defined as 
%$$
%\tilde{\psi}_i(x)=\left\{\begin{array}{ll}{\psi([a,b]) = \frac{\int_{a}^{b} \psi(t) f(t) \mathrm{d} t}{F\left(b\right)-F\left(a\right)},} & {x \in\left[a_i, b_i\right]} \\ {\psi(x),} & {\text { otherwise }}\end{array}\right.
%$$
%\end{definition2}
We refer to \citep{note_ironings} for more technical details. In particular, the ironed virtual value, since  defined as a sub-differential, is not a function but a multi-valued mapping. On the other hand, selecting $\tilde{\psi}(x) = \psi(x)$ when the sub-differential is not reduced to a singleton is also perfectly valid and implicitly stated from now on.  With this later expression, either $\tilde{\psi}$ is equal to $\psi$ or it is constant on some interval around $x$. It is  non-decreasing everywhere and intervals where $\psi$ is  decreasing are ``flattened'', as illustrated on Figure \ref{Ironed}.



Recall that the purpose of ironing is to replace the non-increasing value function $\psi$ in the Myerson auction (that might not be BIC) by $\tilde{\psi}$. We now show that ironing the virtual value does not decrease the revenue of the Myerson auction.

\begin{figure}[h!]
\centering
\begin{tabular}{cc}
\includegraphics[width=.5\linewidth]{images/convex_hull.pdf}&
\includegraphics[width=.5\linewidth]{images/virtual_value_ironing.pdf}
\end{tabular}
\includegraphics[width=.55\linewidth]{images/ironed_revenue_curve.pdf}

\caption{\textbf{Left:} Concavification of $\Pi\circ F^{-1}$ for a  mixture of $\mathfrak{U}(0,0.5)$ and $\mathfrak{U}(0,1)$. \textbf{Right:} Associated virtual value (plain black) and ironed one (dashed orange). \textbf{Center:} Associated monopoly revenue curve (plain black) and ironed one (dashed orange).}
\label{Ironed}
\end{figure}
\begin{lemma2} 
The payment of bidder $i$ at the truthful equilibrium of any BIC auction satisfies 
$$ \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] \leq P_i(0) + \mathbf{E}_{x_{i} \sim F_{i}}\left[Q_{i}\left(x_{i}\right) \tilde{\psi}_{i}\left(x_{i}\right)\right]\;,$$
where $\tilde{\psi}_i$ is his ironed virtual value.\end{lemma2} 
\begin{proof} 
The proof is based on  the Harris inequality \citep{harris1960lower}, a direct application of Chebyschev' sum inequality. 
\begin{lemma2}%[Harris inequality]
For any  non-decreasing mapping $f$ and  non-increasing mapping $g$, the following holds for any random variable $X$, 
$$\mathds{E}[f(X)g(X)] \leq \mathds{E}[f(X)]\mathds{E}[g(X)]$$
\end{lemma2}
Consider an incentive-compatible auction; by monotonicity,  $Q_i$ must be non-decreasing. Let assume there exists $[a,b]$ where $\psi_i$ is non increasing:
\begin{align*}
&\int_{a}^{b}Q_i(x)\psi_{i}(x)f_i(x)dx =(F_i(b) - F_i(a)) \int_{a}^{b}Q_i(x)\psi_{i}(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx
\\&\leq (F_i(b) - F_i(a)) \int_{a}^{b}Q_i(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx\int_{a}^{b}\psi_i(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx
\\&=\int_{a}^{b}Q_i(x)\tilde{\psi}_{i}(x)f_i(x)dx\;.
\end{align*}
from where the result follows.
\end{proof}
We now generalize Theorem \ref{theorem_regular_distributions} to the case of non-regular value distributions.
 \begin{theorem2}[\cite{Myerson81}]%[Optimal auctions for general value distribution]
  In a single item auction, with general value distribution, a revenue-maximing auction is an auction where the seller allocates the item to the bidder with the highest non-negative ironed virtual value. The payment rule is defined such that the auction is incentive compatible.
 \end{theorem2}
 
\section{Prior-free optimal auctions} 
\label{sec-Bulow}
In the previous section, we  derived the revenue-maximizing auction given the prior of the seller on the possible valuations of the different bidders. In some cases, the seller do not have access to a reliable prior and he has to choose an auction without it. The associated challenge is to understand what are  the auctions robust to a lack of knowledge (or some mis-specification) on the bidders' value distributions.

The following theorem claims that a basic second-price auction without reserve price (that will be refereed to as the Vickrey auction from now on), yet with just one additional more bidder, leads to a higher revenue than the optimal Myerson auction \citep{bulow1996auction} . Only the symmetric case is concerned, so that the comparison of two auctions with different set of bidders is possible.
\begin{theorem2}[\cite{bulow1996auction}]%[Bulow-Klemperer Theorem]
In the symmetric setting and with regular distributions, the revenue of the Myerson auction with $n$ bidders is lower than the revenue of the Vicrey auction with $n+1$ bidders. 
\end{theorem2}
\begin{figure}[H]
\includegraphics[width=.5\linewidth]{images/BulowKlemperer.pdf}
\caption{Illustration of the Bulow-Klemperer theorem for the case with value distributions  $\mathfrak{U}([0,1])$.}
%{\color{red} Ca ne devrait pas etre $K$ bidders mais $n$ bidders ; choix des couleurs discutables ; on ne dit pas Nb bidders en Anglais }}
\label{fig:BK}
\end{figure}
Before proving the Bulow-Klemperer theorem, we introduce a helpful Lemma.
\begin{lemma2}\label{second_price_without_reserve}
In the symmetric case and with regular distributions, the Vickrey auction is revenue-maximizing in the class of individually-rational auctions where the item is always attributed. 
\end{lemma2}
\begin{proof}
Based on the revelation principle, we shall only consider incentive-compatible auctions. Since the item must always be attributed, in order to maximize the seller's revenue, see Theorem \ref{Th:MyersonLemma},  it should be allocated to the bidder with the highest virtual value, irrespectively if its non-negative or not. Since the distributions are regular and identical, the bidder with the highest virtual value is also the bidder with the highest value. As a consequence, the mechanism we just described is exactly the Vickrey auction.
\end{proof}
The proof of the Bulow-Klemperer theorem can now be derived from the previous lemma.
\begin{proof} 
Let us assume that there are $n+1$ bidders, and consider the following mechanism. First, the seller runs a Myerson auction on  $n$ bidders (chosen arbitrarily). If the item is not allocated by the Myerson auction, it is allocated for free (i.e., without any payment) the $(n+1)$-th bidder. The revenue of this auction is equal to the revenue of the Myerson auction with $n$ bidders, yet it is  an auction that always allocate an item amongst $n+1$ bidders. Lemma \ref{second_price_without_reserve} implies that the revenue of this auction is smaller than the one of the Vickrey auction. 
This gives the result.
\end{proof}

As a consequence, it would be more interesting,  revenue speaking for  the seller, to have one more bidder than implementing a complex mechanism. This is the reason why one of the first recommendation of most economists dealing with institutions organizing auctions is to maximize the competition on the platform before implementing complex mechanisms \citep{bulow1996auction,milgrom2004putting}.

\bigskip

Nonetheless, let us assume that a specific mechanism has been chosen, independently of the value distributions (that are unknown). The crucial remaining question is the evaluation of this specific choice of an auction (we will restrict ourselves to DSIC auctions) in the worst-case analysis. We will use the notion of \textsl{competitive ratio} defined as the infimum, over all possible value distributions, of the revenue of this auction divided by the optimal revenue of the Myerson auction for these distributions. 

The competitive ratio is obviously smaller than 1, and the bigger the better. Unfortunately, if the class of value distributions is not restricted when computing this infimum, there does not exist any auction with a positive competitive ratio \citep{allouah2018prior}. As a consequence, we will use different types of restrictions to achieve non-trivial approximation results. Based on the Bulow-Klemperer theorem, we can derive some revenue guarantees on the second price auction without reserve price. 
\begin{corollary2} \label{compet-ratio}
The Vickrey symmetric auction  with $n$ bidders and regular value distributions is a $\left(\frac{n-1}{n}\right)$-approximation of the Myerson auction.
\end{corollary2}
\begin{proof}
We denote  respectively by $R(\mathrm{Vickrey}_n)$ and $R(\mathrm{Myerson}_n)$ the revenue of the seller  in the Vickrey or  Myerson auction with $n$ bidders and by $P_i(\mathrm{Vickrey}_n)$ and $P_i(\mathrm{Myerson}_n)$ the payment of the bidder $i$ in those auctions (so that $R(\cdot) = \sum_{i=1}^n P_i(\cdot)$).


Let us first prove that $P_i(\mathrm{Myerson}_n)\geq P_i(\mathrm{Myerson}_{n+1})$.

By symmetry and with regular distributions, their exists a unique monopoly price $r^*$ which is independent of the number of players. Hence, 
\begin{align*}P_i(\mathrm{Myerson}_{n})&= \int  (x - F(x))F^{n-1}(x)\mathds{1}\{x\geq r^*\} dx\\&\geq \int (x - F(x))F^{n}(x)\mathds{1}\{x\geq r^*\}dx\\&=P_i(\mathrm{Myerson}_{n+1}),\end{align*}
which proves the inequality.

Then, based on the Bulow-Klemperer theorem, 
$$R(\mathrm{Vickrey}_n)\geq R(\mathrm{Myerson}_{n-1}) = (n-1)  P_i(\mathrm{Myerson}_{n-1}) \geq (1-\frac{1}{n})  R(\mathrm{Myerson}_{n})$$
which gives the result. \end{proof}
We proved in Corollary \ref{compet-ratio}, through the Bulow-Klemperer theorem that the competitive ratio of the Vickrey auction is at least 0.5, when the distributions are restricted to regular ones. Interestingly, it is possible to do better with a slightly different auction. 
\begin{theorem2}[\cite{fu2015randomization}]
There exists an incentive-compatible auction with a competitive ratio of 0.512 against regular value distributions. 
\end{theorem2}
The mechanism considered was the first  with a higher competitive ratio than 0.5  against regular distributions. It is a slight modification  of the Vickrey where the seller inflates the second highest bid. Formally, the mechanism is the following: with probability $1-\varepsilon$,  a second price auction without reserve price is run. With the  probability $\varepsilon$, the mechanism allocates the object to the bidder with the highest valuation, but only if his valuation is greater than $1+\delta$  times the valuation of the second highest bidder and pays  $(1+\delta)$ the second highest bid. Otherwise, the mechanism does not allocate the item. 

The idea behind this theorem is the following. The Bulow-Klemperer bound of $0.5$ on the competitive ratio is rather tight for regular distributions that would induce a high optimal reserve price. On the other hand, it is rather loose for regular distribution with a low associated reserve price. Inflating the second highest bid has a positive effect for the former type of distribution (as it somehow emulates a high reserve price) and a negative effect for the later type (because it induces some reserve price, bigger than what it should be). As a consequence, the ratio of revenues increase in the first case, and decreases in the second one; but thanks to the looseness in the Bulow-Klemperer bound of $0.5$, the infimum globally increases. 

This result was further improved up to 0.519 \citep{allouah2018prior} for regular distributions, yet the tightness of this bound is still open. On the other hand, when restricted to MHR distributions, the ratio is equal to 0.7153 and this result is tight. 

\iffalse
\section{New applications of auctions}
We now briefly overview some of the main applications of auctions in modern economy.
\paragraph{Online advertising}
Billions of auctions are run worldwide everyday. One of the main supplier of such auctions is the online advertising market \citep{AllouahBesbes2017,Balseiro2015MultiStage,AmiKeaKey12}. Most of the ad slots are sold to advertisers by a publisher, typically a website, following  more or less explicit mechanisms, i.e., a type of auctions with specific rules. Those auctions take place on platforms known as ``ad exchanges'' \citep{Mut09}, such as AppNexus or AdEx (Google). Each time a person is browsing a publisher website (the New York Times, the Washington Post, le Monde\dots), an auction is run to decide which advertiser (Macys, Walmart, Nike, CDiscount) will have the opportunity to display an ad on the website. In this framework, the value distribution makes perfectly sense. It represents the distributions of values that a specific advertiser gives to all the users arriving on publishers' websites represented by the ``ad exchanges'' in a specific day for instance. These differences in value between users or accross time for a specific user can come from different reasons: the amount of data gathered to estimate precisely the value of displaying an ad, the intent to buy at a specific point in time, the budget that a specific advertiser is likely to spend to attract new customers\dots 
%
%\iffalse
%In practice, there exists intermediaries in the chain between the ad exchanger and the advertisers. They are callled a Demand Side Platform (DSP). A DSP (e.g. Criteo) represents many advertisers and compute the optimal bid to place on the ad exchanger and the optimal ad to display if the advertiser wins the auction. 
%
%The two-stage game presented in the previous sections is a reasonable model for relationships between buyers and sellers on online ad platforms. No clear contracts exhibit the exact rules implemented by the seller to define the allocation and the payment rule. Initially, big ad networks advertized that they are implementing a second-price auction which is incentive-compatible for the bidders. If advertisers or DSPs are bidding truthfully, ad exchanges could have interest to learn the value distributions of the various advertisers on their platform and deviate to a revenue-maximizing auction. In plot \ref{monopoly_reserve_ads}, we show how the monopoly price is a good predictor of the reserve price sent by a big online advertising platform to one of the biggest DSPs on its platform.
%\begin{figure}[H]
%\includegraphics[width=.5\linewidth]{images/reserve_price2}
%\caption{Reserve price sent by one of the biggest ad platform function of the monopoly price of Criteo.}
%\label{monopoly_reserve_ads}
%\end{figure}
%\fi
The importance of reserve prices in these specific auctions is explained by the low number of participants per auction (the median number of bidders is equal to 6 \citep{celis2014buy}) and the strong asymmetries between bidders. For a long time and until recently, the typical auction used in ad exchanger was an eager second-price auction with monopoly prices. Very recently, most of the biggest platforms switched to a first-price auction forcing bidders to develop complex bidding strategies to bid optimally in a first-price auction. The problem of reserve price remains very important since it still impacts very strongly seller's revenue in first-price auctions. 

\paragraph{Modern Internet marketplaces:} In one Ebay auction, the seller can define an anonymous reserve price. Then, most of the time, Ebay runs an ascending auction which is equivalent to a sealed bid second-price auction. At the end of a certain period of time, the winner of the item is the one with the highest bid. There exists some bots that can be used by bidders to automatically raise their bid once another bidder is ready to pay a higher price. Most of the pricing problems also faced by big online platforms such as Uber, Airbnb or Amazon can be seen as a posted price setting as described in Section \ref{monopoly-pricing}.

\paragraph{Electricity market.} With the development of renewable energies which are by definition intermittent, the offer of electricity can have very high variations. The United Sates and European states are more and more implementing and designing complex auction systems to be able to compute a fair price between suppliers and consumers. They want to insure the efficiency of the system to make sure that the producers have the right incentives to invest and develop the right infrastructures. 

\paragraph{European pollution permits.} Since 2013, the European Union have implemented an auction system to sell pollution permits every year. The European commission sees auction as \textit{an open, transparent, harmonised and non-discriminatory process}. To be able to pollute, most of the European firms need to match the number of permits they own at the end of the year with their corresponding CO2 emissions. If a company does not manage to provide enough permits corresponding to its CO2 impact, heavy fines apply. Some of the permits are given freely by the different European governments but more and more are sold through an auction platform. Auctioning share is supposed to increase each year over 2013 to 2020 to reach 75\% of the permits.  The revenue that the European union gets through these auctions is then reinvested in some environmental projects \citep{dietz2018climate}.

The auction system that is used to sell these permits is the following. A certain number of permits are sold every week. A bid is made of a price and a given number of permits. The auction is a sealed-bid auction. Bids are ordered by price and the number of permits is added until reach the limit given for this run of the auction. The clearing price is the price where the demand matches or exceed this limit. All the winning bidders who provided a bid higher than the clearing price pay the clearing price times the number of permit they bid for. 

The European union generated around 16 billion euros from the auctioning of permits over the period 2013-2016. Around 57\% of the total amount of allowances are auctioned, while the remaining ones are available for free allocation to maintain international competitiveness of some of the main European industries. 
\paragraph{Other applications.}
Recently, the French football TV rights were sold through a sealed-bid  first-price auction with carefully tuned reserve prices. In the US, the government sold for 14 billion dollars spectrum licenses to big telecommunication companies. Some other applications are detailed in \citep{klemperer2000every}.y results on the ironing in the next chapters, so we skip the technical details explaining how to precisely define the intervals where the virtual value is ironed \citep{Myerson81,note_ironings,hartline2013mechanism}.
\fi



==> chapters/chapter4_repeated_learning_online_ad_old.tex <==
 %!TEX root = ../main.tex
\chapter{Adaptive and strategic learning agents}
\label{Chapter:Learning}

A crucial assumption behind the results of Chapter 3 is that the seller has access to some large sample batch  of bidders' valuations. The objectives were to learn the optimal (or at least the best possible in some class) mechanism based on this dataset. This model particularly fits problems where the bidders are different from one auction to the other (typically such as on Ebay) so that it is legitimate to assume that they bid their values (as long as they were facing an incentive compatible auction) myopically, i.e., non strategically. Unfortunately, this assumption  of facing new bidders for each different item  no longer holds in many important economical situations, such as online advertising. Indeed, in that market the so-called \emph{demand-side platforms} (DSP), that are aggregate of bidders, repeatedly interact with a single seller (called \emph{Supply-side platforms (SSP)}), billions of times a day \citep{choi2019online}. 

The global objective of the seller remains identical: maximize the total revenue, certainly by learning (or trying to) the value distributions of the bidders. Indeed, it is still interesting for SSP   to optimize the reserve prices (personalized per DSP) since the number of participants per auction is relatively low (the median number of bidders is equal to 6 \citep{celis2014buy}). The difficulty is now that bidders are also present in the game for a long period optimize their cumulative  utility, instead of best-replying myopically to the seller design of mechanism. Thanks to this long-term optimization, it is possible for a bidder to sequentially learn his ``optimal'' bidding strategy, if the mechanism or his opponent's strategy or even his own distribution of valuations are unknown at first. Such a bidder is \emph{adaptive} to his environment, but he could even be \emph{strategic}.
Intuitively, and this will be detailed later on, a strategic buyer might be tempted to modify his bids if he knows that the seller is using them to set reserve prices. It can be much more profitable to face a low reserve price by bidding non-truthfully than facing a high reserve price with truthful bids.



\medskip

It might be worth mentioning here that the DSP might have different values for different auctions because the intrinsic value of an ad is strongly related to the probability that the user seeing it clicks on it. As a consequence, the value distribution of bidders in this chapter represents the time-variability of valuations for one specific bidder for the different items that are sold successively. Notice, on the contrary, that in the precedent chapter, the value of a buyer was fixed, but unknown to the seller that only had some prior (the distribution) on its realization.

\medskip

For simplicity, we shall assume in this section that values always belong to $[0,1]$; this assumption can be weakened, but at the cost of technicalities.
\section{Adaptive bidders - Online learning to bid}

As mentioned above, the buyers were assumed to be myopic in the previous chapters (or equivalently, only present for one single auctions), a crucial hypothesis that should be removed, at least in online ads markets. We will on the contrary assume that a single buyer bids at each auction and that he can use these repetitions to \textsl{improve} his bidding strategy by adapting to his unknown environment; there are at least two different aspects that can be learned sequentially, depending on where the lack of information lies.

\begin{enumerate}
\item \textit{Bidding without knowing its own value:}  the bidder does not know the expected value it gives to the item but could learn his own value distribution, by gathering a new value sample each time he wins an auction. This is particularly relevant in online advertising where advertisers has to show ads to potential buyers to understand their propensity to buy a certain product (or at least, the propensity to click on an ad). 
\item \textit{Bidding without knowing the mechanism:} a strategic bidder does not know precisely the mechanism used by the seller (or alternatively, has few or no information on the other bidders valuation distributions). The bidder can sequentially and incrementally adapt his bidding strategy during  the $T$ successive auctions to maximise his expected  cumulative utility, hopefully achieving (almost) the same performances as if he knew the whole mechanism in advance.
\item \textit{Bidding with budget constraints:} a strategic bidder could have a pre-specified constraint that on the budget he can spend during the $T$ successive auctions. In this setting, at each round, he should bid (and spend some of his budget if he wins the auction) without knowing the exact valuation he will get for the future rounds. The bidder can sequentially and incrementally adapt his bidding strategy during  the $T$ successive auctions to maximise his expected  cumulative utility, without respecting the constraint on his budget.
\end{enumerate}

\subsection{Online learning the value distribution to bid}
In some oversimplified online ad example, a publisher (the website where an ad is displayed) gets paid by the advertiser each time a user clicks on that ad because this is that random event that is relevant (as it might generate a sale afterwards), and not simply the fact that the ad is displayed (as the user might not see it). As a consequence, the actual value of an ad is random -- either 0 or 1 to simplify things again, i.e., whether the user actually clicks or not -- of  expectation $x$, i.e., the probability of click. If $x$ is known before participating in a DSIC auction, then due to the linearity of expectation, the optimal strategy remains to bid truthfully $x$.

Unfortunately for the seller, there are manny examples where the probability of click is unknown to the advertiser before starting a new campaign; he would be willing to bid truthfully this probability repeatedly, but it is unknown. This is an example where multi-armed bandit techniques can be used to learn on the fly the probability of clicks based on the feedback received. Notice that an ad that is not displayed will never be clicked, hence the advertiser must acquire some data to estimate this probability.

\medskip

The simplest model to study this sequential learning problem is the following \citep{Weed16}. Bidder $i$ participates in a sequence $t=1,\ldots,T$ of second price auctions (without reserve prices) where the realized values $v_t \in \{0,1\}$ are i.i.d.\ of unknown expectation $x$. Of course, $v_t$ is not observed before participating to the auction $t$, and only if that auction is won. Let us denote by $b^{(1)}_{-i,t}$ the maximal bids of the opponents (that could actually include a reserve price) and by $b_{i,t}$ the bid of bidder $i$ at that stage then the performance of the optimal truthful strategy is 
$
\sum_{t=1}^T \mathds{E} \big[ x \mathds{1}\{x \geq b^{(1)}_{-i,t}\} \big]
$
while  the learning to bid policy has gathered $
\sum_{t=1}^T \mathds{E} \big[ x \mathds{1}\{b_t \geq b^{(1)}_{-i,t}\} \big]
$. As a consequence, the cost of learning to bid is measured in terms of regret 
$$
R(T) = \sum_{t=1}^T \mathds{E} \big[ x \mathds{1}\{x \geq b^{(1)}_{-i,t}\} \big] -  \mathds{E} \big[ x \mathds{1}\{b_{i,t} \geq b^{(1)}_{-i,t}\} \big]\, .
$$
As in multi-armed bandit, the empirical average $\overline{x}_t = \frac{\sum_{s \leq t} v_x \mathds{1}\{b_{i,s} \geq b^{(1)}_{-i,s} \} }{ \sharp \{s \leq t\, ;\,  b_{i,s} \geq b^{(1)}_{-i,s} \} }$ is negatively biased. As a consequence, the algorithm $\text{UCB}_\text{id}$ slightly biased it positively by adding a small error term in its bid
$$
b_{i,t+1} = \overline{x}_t + 2\sqrt{\frac{\log(T)}{\omega_{i,t}}} \quad \text{ where } \omega_{i,t}=\sharp \{s \leq t\, ;\,  b_{i,s} \geq b^{(1)}_{-i,s} \},
$$
is the number of auctions won until stage $t$.
\begin{proposition2}The $\text{UCB}_\text{id}$ algorithm has a sublinear regret against any sequence of opponent bids $b^{(1)}_{-i,t}$, as long as they are independent of $v_t$, as 
$$
R(T) \leq \mathcal{O}\big(\sqrt{T\log(T)}\big).
$$
Moreover, if the sequence $b^{(1)}_{-i,t}$ is also i.i.d.\ (of unknown law to bidder $i$), then the regret grows is even much slower as 
$$
R(T) \leq \left\{ \begin{array}{ll} c_1 T^{\frac{1-\alpha}{2}}\log^{\frac{1+\alpha}{2}}(T) & \text{if}\ \alpha <1\\
c_2\log^2(T) & \text{if}\ \alpha =1\\
c_3\log(T) & \text{if}\ \alpha >1\end{array}\right.
$$
for some constants $c_i$ independent of $T$ and where $\alpha$ is some regularity parameter called margin and such that, for some $C>0$ and for any $\varepsilon >0$,  
$$\mathds{P}\big\{b^{(1)}_{-i,t} \in (x,x+\varepsilon)\big\} \leq C \varepsilon^\alpha.$$
\end{proposition2}
\begin{proof}
The proof is a bit technical and only sketched; the main ingredients are more or less classical multi-armed bandit techniques. First of all, noticed that, as a direct consequence of Hoeffding inequality, with  probability  of the order of $1/T$, all bids are bigger than $x$. As a consequence, we shall  only focus on this event where  regret is only incurred on  auctions such that 
$$
x < b^{(1)}_{-i,t} <  \overline{x}_t + 2\sqrt{\frac{\log(T)}{\omega_{i,t}}}.
$$ 
Indeed, the optimal bid  $b_{i,t}=x$ loses this auction while $\text{UCB}_\text{id}$ overbids and wins it. It unfortunately pays more than its expected value. The net cost  of this specific auction is
$$
b^{(1)}_{-i,t} -v \leq \overline{x}_t + 2\sqrt{\frac{\log(T)}{\omega_{i,t}}} -x \leq 4\sqrt{\frac{\log(T)}{\omega_{i,t}}}, 
$$
where the last inequality holds for all auction on the event considered (that holds with probability at least $1/T$). Summing over all the auctions $t=1,\ldots,T$  gives the first bound.

The other bounds are derived from careful computations of 
\begin{align*}
&\ \mathds{E} \Big[ (b^{(1)}_{-i,t} -x)  \mathds{1} \big\{ x \leq b^{(1)}_{-i,t} \leq \overline{x}_t  + 2\sqrt{\frac{\log(T)}{\omega_{i,t}}}\big\}\Big]\\
=\ &\  \mathds{E} \Big[ (b^{(1)}_{-i,t} -x)  \mathds{1} \big\{ 0 \leq b^{(1)}_{-i,t}-x \leq \overline{x}_t -x + 2\sqrt{\frac{\log(T)}{\omega_{i,t}}}\big\}\Big]\\
\leq\  &\ C\mathds{E} \Big[ \big( \overline{x}_t -x + 2\sqrt{\frac{\log(T)}{\omega_{i,t}}}\big)_+^{1+\alpha}\Big]\, ,
\end{align*}
where the last inequality is a consequence of the margin definition (and $x_+=\max\{x.0\}$). An important fact is that, if some regret is incurred at auction $t \in \mathds{N}$, then this auction is necessarily won hence the counter $\omega_{i,t}$ increases by one. As a consequence, the overall regret can be controlled by 
$$
C\mathds{E} \Big[ \sum_{s=1}^T\big( \overline{X}_s -x + 2\sqrt{\frac{\log(T)}{s}}\big)_+^{1+\alpha}\Big]\, 
$$
where $\overline{X}_s$ is the average value of the first $s$ auctions won.  Hoeffding inequality implies that $\mathds{P}\{\overline{X}_s -x \geq \varepsilon\} \leq e^{-2s\varepsilon^2}$, hence we get that the total regret is smaller than
\begin{align*}
&\ C\mathds{E} \Big[ \sum_{s=1}^T\big( \overline{X}_s -x + 2\sqrt{\frac{\log(T)}{s}}\big)_+^{1+\alpha}\Big]\\
\ \leq &\ C(1+\alpha)\sum_{s=1}^T\int_{- 2\sqrt{\frac{\log(T)}{s}}}^\infty \Big(\varepsilon + 2\sqrt{\frac{\log(T)}{s}}\Big)^\alpha e^{-2s\varepsilon^2}d\varepsilon\\
\ = \ & \ C(1+\alpha)\sum_{s=1}^T \frac{1}{(2s)^{\frac{1+\alpha}{2}}} \int_{- 4\sqrt{\log(T)}}^\infty \Big(u + 4\sqrt{\log(T)}\Big)^\alpha e^{-\frac{u^2}{2}}du\\
\ \leq \ &C(1+\alpha)\sum_{s=1}^T \Big(\frac{16\log(T)}{t}\Big)^{\frac{1+\alpha}{2}}+ C\frac{(1+\alpha)}{2}\sum_{s=1}^T \frac{1}{s^{\frac{1+\alpha}{2}}}\int_{4\sqrt{\log(T)}}^\infty u^\alpha e^{-\frac{u^2}{2}}du\, .
\end{align*}
The result follows from instantiating the above sum over different values of $\alpha$. For $\alpha >1$, the first sum is controlled  using the fact that all terms are necessarily smaller than 1.
\end{proof}
These results only hold if the value $v_t$ are i.i.d.\ of unknown expectation $x$, using the basic ideas of stochastic multi-armed bandits and devising a new bidding algorithm based on UCB.  If values $v_t$ can be any sequence, then it is also possible to achieve non-trivial regret bounds by using as a building block EXP.3 algorithm instead of UCB \citep{Weed16}. 

Those results and techniques can also be exported to other auctions settings than Vickrey \citep{feng2018learning}.

\subsection{Adaptivity to the mechanism and other bidders}
If a bidder has, at first, not enough information on the auction mechanism and/or the distributions of values of his competitors, he can not compute an appropriate bidding strategy even if he knows perfectly the values he gives to item. The repeated auction setting can then be helpful for him to learn, on the fly, a strategy. A possible approach is again to use ides from multi-armed bandits, but more precisely on contextual bandits. 

For simplicity, assume that the value distribution of the bidder has a finite support included in $[0,1]$, denoted by $\{x^*_1,\ldots, x^*_L\}$. Then a bidding strategy consists in finding, for each possible values $x^*_\ell$ a corresponding bid. A classical contextual bandits technique consists in discretizing the set of bids $[0,1]$ in $\{b^*_1,\ldots,B^*_K\}$ and  in running independent versions of a base bandit algorithm (such as EXP.3 for instance), one for each possible values, where the set of arms is the discrete set of bids.    Such regret minimizing algorithms have indeed been reported in the online advertising industry \citep{nekipelov2015econometrics}.  

\medskip

In this setting, we can even assume that the opponents change through time, so that their sequence of bids  might be arbitrary (but, conditionally to the past and to the actual value $x_\ell$,  their bids at some given auction $t \in \mathds{N}$ are independent from the bid of player $i$). Then the optimal (stationary) strategy of bidder would get an expected cumulative utility of 
$$
\max_{\beta_i \in \mathds{B}_i} \sum_{t=1}^T \mathds{E}\big[ U_i((\beta_i(x_t),b_{-i,t}),x_t)\big]\,,
$$
where $x_t$ is the value for the item $t$ of bidder $i$, $b_{-i,t}$ is the vector of bid of his opponent and $\beta_i$ is a possible strategy. This quantity will serve as a benchmark for a learning to bid policy; for instance, if the mechanism is DSIC, then the optimal mapping in the above equation is $\beta(x)= x$, i.e., bidding truthfully.  On the other hand, the realized cumulative utility of Bidder $i$ is equal to 
$$
\sum_{t=1}^T \mathds{E} [ U_i(b_{i,t},b_{-i,t}),x_t) ]\,,
$$
where $b_{i,t}$ is his bid at stage $t$, after observing the value $x_t$. As a consequence, we can consider the overall regret of bidder $i$ as the difference between those two terms, the benchmark, and the cumulative utility
$$
R(T) = \max_{\beta_i \in \mathds{B}_i} \sum_{t=1}^T \mathds{E} [ U_i((\beta_i(x_t),b_{-i,t}),x_t) ]  - \sum_{t=1}^T \mathds{E} [ U_i(b_{i,t},b_{-i,t}),x_t) ]\, .
$$
As mentioned above, let us assume that bidder $i$ is running independent versions of EXP.3 (one per possible value) then using the standard results of multi-armed bandits recalled in Section \ref{Section:Bandits}, we get that 
\begin{equation}\label{EQ:Reg_Contextual}
R(T) \leq 2\sum_{\ell=1}^L \sqrt{K\log(K)T_\ell} + \max_{b_\ell \in [0,1]} \sum_{t: x_t=x^*_\ell} \mathds{E} [ U_i((b_\ell,b_{-i,t}),x^*_\ell)  ] -   \max_{b^*_\ell \in [0,1]} \sum_{t: x_t=x^*_\ell}^T \mathds{E} [ U_i((b^*_\ell,b_{-i,t}),x^*_\ell)  ] 
\end{equation}
where $T_\ell = \sharp \{t\leq T: x_t=x^*_\ell\}$ is the number of times the values was equal to $x^*_\ell$. The first term of Equation \ref{EQ:Reg_Contextual} corresponds to the estimation error, and the second term to the approximation error, because EXP.3 are restricted to bid in the discretization of $[0,1]$ while the optimal bidding strategy does not have this restriction.

We will need some regularity assumption on the mechanism used by the seller; we will assume that it is ``$C$-almost Lipchitz'', for some constant $C>0$, in the following sense. For any value $x_i \in [0,1]$, for any bids $b_{-i}$ of the opponents and any bids $b_i$ of bidder $i$, there exists a point $b^\varepsilon_k$ in the $\varepsilon$-regular grid of $[0,1]$ (i.e., $b^\varepsilon_k = k\varepsilon$ for some integer $k$) such that $U_i((b_i,b_{-i}),x_i) \leq U_i((b_k^\varepsilon,b_{-i}),x_i)+C\varepsilon$. Classical auction mechanisms  (first and second price auctions, with or without reserve prices, Myerson auction...) all satisfy this assumption that ensures the approximation error is of order $T\varepsilon$ if $\{b^*_1,\ldots,b^*_K\}$ is the $\varepsilon$-regular grid (in particular, this implies that $K=1/\varepsilon$). We emphasize here that auction mechanism are usually not Lipschitz (as there are discontinuities around the smallest winning bid).

\begin{proposition2}
If the mechanism is $C$-almost Lipchitz (with $C$ unknown)  and the value distribution has a finite support $L$, then there exists a learning to bid policy whose regret, with respect to the optimal in hindsight bidding strategy smaller than 
$$
R(T) \leq(2+C) (LT^2\log(T))^{\frac{1}{3}}
$$
\end{proposition2}
\begin{proof}
One just need to put the definition of $C$-almost Lipschitzness  in Equation \ref{EQ:Reg_Contextual}, as this  gives that regret scales as 
$$
R(T) \leq 2\sqrt{\frac{1}{\varepsilon}\log(\frac{1}{\varepsilon})LT} + C T \varepsilon \leq (2+C) (LT^2\log(T))^{\frac{1}{3}}
$$
with the specific choice of $\varepsilon = (L\log(T)/T)^{1/3}$.
\end{proof}

This result only holds for distribution with finite support; for continuous distribution, the trick consists in bucketing the support of value distribution into small bins of size $\varepsilon$ and using, as before, an independent version of EXP.3 per bin. This only works with some regularity assumption on a bin. Specifically, given a small bin $\mathcal{I}$, we shall assume that there exist a constant bid $b$ that is $\varepsilon$-optimal on the set of stages where the values $x_s$ belongs to $\mathcal{I}$, i.e.,
$$
\max_{\beta: \mathcal{I} \to [0,1]} \frac{\sum_{s \leq T: x_s \in \mathcal{I}} U_i((\beta(x_s),b_{-i,s}),x_s)}{\sharp \{s \leq T: x_s \in \mathcal{I}\}} \leq \max_{b \in [0,1]} \frac{\sum_{s \leq T: x_s \in \mathcal{I}} U_i((b,b_{-i,s}),x_s)}{\sharp \{s \leq T: x_s \in \mathcal{I}\}} +C'\varepsilon.
$$
In particular, this assumption is satisfied if $U_i$ is $C'$-Lipschitz and the bids $b_{-i,t}$ does not depend (too much, at most in a Lipschitz fashion) on $x_t$. Once again, balancing the approximation (both in the bid  and the value spaces) and estimations errors gives the optimal choice of $\varepsilon = (\log(T)/T)^{1/4}$ for a regret scalling as 
$$
R(T) \leq (2+C+C') (T^3 \log(T))^{\frac{1}{4}}.
$$
If the utility function $U_i$ (and/or the opponents bid $b_{-i,t}$) is not Lipschitz but less regular (such as $\beta$-H\"older), then the rate of regret growth would be impacted as one should find better tradeoffs in approximation vs estimation errors. This would typically lead to a regret scaling as $(T\log(T))^\alpha$ where $\alpha \in [\frac{1}{2},1)$ is some parameter depending on the different regularities of the mappings at hand.

\subsection{Adaptivity to budget constraints and pacing options}
In practice, a common problem for the bidder is to find strategies  maximizing the number of some actions (e.g. clicks, views) or a buyer's utility subject to some budget constraint \citep{BalBesWei15,gummadi2012optimal,FernandezTapiaAnalyticalSolution2015,FernandezTapiaGueantLasryOptimalRealTimeBidding2017}. 

As an example, in the case of utility maximization, a bidder can be facing the following problem in second price auctions. Given his budget $\mathbf{B}$, $g_t$ the maximum bid of the competition at time $t$ (possibly including reserve prices), $x_t$ the value of the item at time $t$ for the bidder, and $b_t$ the bid of the bidder at time $t$. The bidder's problem in second price auction is~:
\begin{gather*}
\max_{\{b_t\}_{t=1}^T} \sum_{t=1}^T \indicator{b_t>g_t} (x_t-g_t)\;,\\
\text{subject to } 	\sum_{t=1}^T g_t \indicator{b_t>g_t}  \leq \mathbf{B}\;.
\end{gather*}
Under the assumption that bids are much smaller than total budget, the problem loses much of its stochastic component and is often approximated by its so-called fluid approximation (which replaces both objective and constraint by their expectations, effectively appealing to uniform laws of large numbers \citep{dudley_2014}), turning the problem to 
\begin{gather*}
\max_{\{b_t\}_{t=1}^T} \sum_{t=1}^T  \mathds{E}[\indicator{b_t>g_t} (v_t-g_t)]\;,\\
\text{subject to } 	\sum_{t=1}^T \mathds{E}[\indicator{b_t>g_t} g_t] \leq \mathbf{B}\;.
\end{gather*}
Under mild assumptions, and this is a consequence of some strong duality properties,  an optimal bidding strategy is  
$$
b_t=\frac{x_t}{1+\mu^*}\;,
$$
where $\mu^*$ is the optimal solution of the dual problem associated with the constrained optimization mentioned above (Proposition 3.1, \citep{BalBesWei15}). The bidding strategy is similar to the optimal bidding strategy in a second price auction, however the value of each item is discounted by a factor accounting for the constraint. 

This result can be extended to a much broader set of auctions, such as  first price, generalized second price etc... where optimal bidding turns out to be of a similar form to optimal bidding without constraint, the value of each item being linearly discounted by a constant accounting for the budget constraint \citep{gummadi2012optimal}.

\medskip

Three important conceptual ideas emerge from this type of problems. The first one concerns the question of pacing.  For a wide variety of auctions (and payment rules), the optimal strategy to maximize the purchased inventory amounts to spending one's budget smoothly, i.e. at the rate of arrival of auction requests \citep{FernandezTapiaAnalyticalSolution2015,FeedbackSystemsBook}. However, a crucial assumption for this result to hold is that the price paid as a function of win rate does not depend on time and hence the environment is stationary. Not surprisingly, when this assumption does not hold, ``smooth-spending'' at the rate of arrival of auction requests is no longer optimal. These general techniques  can however be used in that more general case to understand the optimal rate of winning auctions and of spending in these more general cases. 

To be implemented in practice, these ideas require of course a forecast for both the arrival rate of auction requests and the price paid at a certain win rate. When the bidder has access to such information, ideas of model-predictive control and re-optimization can be used  \citep{CiocanFariasMPC2012}. 

A third important line of work concerns online estimation of the parameter $\mu$ mentioned above, possibly without forecast \citep{BalseiroGur2019}. The essential idea is to use the fact that $\mu^*$ mentioned above in the solution of an optimization problem and to solve this optimization problem online, using online gradient descent \citep{shalev-shwartz_ben-david_2014}. To be slightly more specific, in the problem mentioned above, the optimal solution for $\mu$ in hindsight is determined through 
$$
\inf_{\mu\geq 0} \sum_{t=1}^T (x_t-(1+\mu)g_t)_+ + \mu \mathbf{B}\; \triangleq: \inf_{\mu \geq 0} \sum_{t=1}^T \ell_t(\mu).
$$
The functions $\ell_t$ are observable at time $t$ and  are a sequence of functions arriving in a streaming fashion. As a consequence, the estimate of the parameter $\mu^*$ can be updated in an online fashion, without a forecast, by using for instance the online (sub)-gradient descent rule
$$
\mu_{t+1}=\mu_t - \gamma \partial_\mu \ell_t(\mu_t)\;,
$$
where $\partial$ is the  (sub)gradient operator and $\gamma$ is the stepsize in the online gradient descent algorithm. Various theoretical guarantees about this scheme, under a variety of optimistic and pessimistic assumptions about the amount of information that is known about the environment in which the bidder evolves, can be proved \citep{BalseiroGur2019}. 

The literature on this topic is very large, with many different variations \citep{GhoshEtal20009,ChoiMela2018,LeeAli2013,YuanWang2013,XuKuang2015}. The question of handling the situation where the bid to budget ratio is not close to 0, and hence the fluid approximation is not well justified, is quite open and  appears to be more of a genuine stochastic control type. An interesting approach seems to use ideas coming out of the analysis of the online knapsack and related problems \citep{Arlotto_2019}. 
\section{Exploitation of adaptive bidders \& Full surplus extraction}

\subsection{Learning against bidders using zero-regret algorithms}
As illustrated in the previous section, the standard techniques of bandits and online learning can be used by bidders to choose their bidding strategy... assuming that the seller let them do it. Indeed, it was more or less implicitly assume that the mechanism was fixed during the whole interaction, an other assumption that is way too restrictive and should be taken care of, as the seller could actually largely leverage this almost predictive behavior for her own interest. 

Let us consider the simple case where all  bidders are independently running regret minimizing algorithms  \citep{braverman2018selling,deng2019prior}, and more precisely where they are using algorithms such as EXP.3, that base their decisions on the mean reward observed. Their particularity is that they rarely pick an arm whose current mean is significantly worse than the current highest mean; for instance if during the first $t$ stages an arm $k$ has generated an average reward (denoted by  $\overline{X}_{k,t}$) that is smaller than the one of arm $\ell$, then the probability of choosing $k$ over $j$ is exponentially small.

\begin{definition2}%[Mean-based algorithm] 
In the standard multi-armed problem, an algorithm is $\eta$-mean-based, for some $\eta \in (0,1)$, if at any stage $t \in \mathds{N}$ and for any pair of arms $(k,\ell)$, if $\overline{X}_{k,t} < \overline{X}_{\ell,t}- \eta$ then  the probability $p_{k,t+1}$ that the algorithm pulls arm $k$ at time $t+1$ is smaller than $\eta$. 
An algorithm is (asymptotically) mean-based if $\eta = o_{T\rightarrow\infty}(1)$.
\end{definition2}

For simplicity, we are even going to assume that there is only one bidder, whose  value distribution $F$ is known beforehand (an assumption that can be fairly weakened \citep{deng2019prior}). If the seller was using the same mechanisms at each auction $t \in \{1,\ldots,T\}$, then the optimal one would obviously to post the monopoly price. This generates a total revenue of $T$ times the monopoly revenue (because the bidder will quickly learn the optimal strategy). On the other hand, if the seller knows that the bidder is using a mean-based algorithm, she can generate a much higher revenue \citep{braverman2018selling}, almost as high as the total welfare denoted by $\mathfrak{W}(F) = \mathds{E}_{x\sim F}[x]$; with $n$ bidders, the total welfare would be $\mathfrak{W}(\mathcal{F}) = \mathds{E}_{x\sim \mathcal{F}}[\max_i x_i]$

To achieve this, the mechanism must change through time and possibly be itself adaptive to the sequence of bids of the buyer. We therefore introduce the concept of dynamic mechanism, so that the actual auction rules might change from stage to stage.

Recall that at each stage $t \in\{1,\ldots,T\}$, bidders valuations for the item are sampled through  distributions $F_i$. These distributions are fixed from one auction to the other. We denote by $a_t \in \mathcal{A}$ the auction mechanism chosen at time $t$ by the seller and by $b_{i,t}$ the bid of buyer $i$. We also denote by $\mathcal{H}_t = \{a_1,b_{1,1},b_{1,N}\dots,a_{t-1},b_{1,t-1},b_{N,t-1}\}$ the finite history at time stage $t$, that consists of past auctions and past buyer's bids. 
\begin{definition2}
A dynamic mechanism $\mathcal{D}\mathcal{M}: \bigcup_t \mathcal{H}_t \rightarrow  \mathcal{A}$ is a mapping that associates to any finite history  $\mathcal{H}_t$ an auction $a_t=: \mathcal{D}\mathcal{M}(\mathcal{H}_t)$. A bidder's dynamic strategy, $\mathcal{S}$, is a mapping from $\mathcal{H}_t$ to the set $\mathds{B}$  of strategies (i.e., functions from values to bids). 
\end{definition2}

The following theorem states that a seller can \emph{extract the full surplus} of the system, if the bidder is using na\"ive learning algorithms.


\begin{theorem2}
If the bidder is running a mean-based algorithm, for any $\varepsilon > 0$, there exists a dynamic selling mechanism such that the seller can get $(1-\varepsilon)\mathfrak{W}(F)T - o(T)$.
\end{theorem2}

The intuition behind this result is that  the seller can lure the na\"ive algorithms such as EXP.3 by setting low prices during a first (large) period of time and then by increasing drastically the reserve price during a second stage. This is illustrated in the following example \citep{braverman2018selling}. 

Assume the bidder value $x_t$ has the following distribution 
$$
x_t = \left\{ \begin{array}{cl} \frac{1}{4} & \text{with probability }\ \frac{1}{2}\\
\frac{1}{2} & \text{with probability }\ \frac{1}{4}\\
1& \text{with probability }\ \frac{1}{4}
\end{array}\right.
$$ Simple computations shows that corresponding monopoly price is $1/4$ and setting it at each time generate a revenue of $T/4$ after $T$ auctions.

 To fool a mean-based algorithm, the seller can use the following scheme. At any stage, it will only allocate the item if the bid is exactly $1$ (any other bid gives a utility of 0). It remains to define the payment associated to a winning bid of 1. During the first $T/2$ stages, it is equal to 0, while it will be equal to 1 during the last $T/2$ stages.
 
Recall that the bidder runs multiple  independent instances of EXP.3, one for each possible values ($1/4$, $1/2$ and $1$), so we can focus independently on the set of stages where the value is constant, and for the sake of simplicity we are going to assume that this value equals $1/2$ (resp.\ 1) exactly $T/8$ times during the first and second half of the game.
\begin{itemize}
\item On the set of stages where the value is 1, EXP.3 quickly learns that bidding 1 is optimal during the first half of the game. This generates a cumulative utility of $T / 8$ to the buyer. As a consequence, EXP.3 will keep bidding 1 when the value
is 1 at each stage of the second half with exponentially high probability. The revenue generated on those stages by the seller is then  approximatively $T / 8$.
\item When the value is $1/2$, bidding 1 during the first half generates a revenue of $T/16$ to the buyer. During the second half, bidding 1 generates a negative utility of $-1/2$ per stage, so that the cumulative utility of bidding 1 decreases, but remains positive during the whole process (and EXP.3 will keep bidding 1 with arbitrarily high probability for almost all stages).  The revenue generated on those stages by the seller is then also  approximatively $T / 8$.
\item When the value is $1/4$, bidding 1 during the first half generates a revenue of $T/16$ to the buyer.    During the second half, bidding 1 generates a negative utility of $3/4$ per stage, so that the cumulative utility of bidding 1 decreases, but remains positive during $T/12$ additional stages where EXP.3 will bid 1 with high probability (and afterwards stop bidding 1 as the cumulative utility of this bid is negative). The revenue generated on those stages by the seller is then also  approximatively $T / 12$.
\end{itemize}
At the end, the total revenue of the seller is therefore of the order of $T/8+T/8+T/12= T/3$ which is much bigger than $T/4$. The trick for the seller was to make the bidder overpay on many  auctions by exploiting the behavior of mean-based algorithms that keep bidding~1 even when instantaneous negative utilities occur. Unfortunately for the seller, this theorem only holds for mean-based buying algorithms.  Even worse, for any dynamic selling mechanism, there exists a buyer's strategy such that he does not pay more than $T$ times the monopoly price  \citep{braverman2018selling}.


\subsection{Trading off ex-post individual rationality for full surplus extraction}
\label{sub_full_surplus_extraction}
If the buyers are using na\"ive algorithms, and the seller knows this, then we proved that she can extract (almost) the full surplus from the system. This was possible because of the asymmetry of information between agents. There are other settings where this full surplus extraction by the seller is possible. The first example we consider is the case where the individual-rationality assumption of the mechanism is removed. This will induce another strong asymmetry between agents, as bidders are somehow ``forced'' to participate in auctions. The idea is to consider the weaker concept of ex-ante, instead of interim, individual-rationality (see Section  \ref{subsec_prop_auction} for more details on the differences).  In the \textit{ex-ante} setting, the bidder does not know the value he will give to the item before he agrees to take part in the auction - he therefore has the same information as the seller on his private valuation.  An ex-ante individually rational mechanism must give a non-negative expected  utility to the bidder.

\begin{theorem2}%[full surplus extraction]
[\cite{cremer1988full}]
There exists an ex-ante individually rational and incentive-compatible auction where the bidders' utilities are all equal to zero and the seller extracts the full surplus.
\end{theorem2}
\begin{proof}Since the seller knows the bidders' value distributions, she  can compute their expected utilities in a second price auction. 

The mechanism constructed is simple. It consists of an entry fee that must be paid before participating to the auction (stated otherwise, the bidder has to pay this amount no matter the outcome of the auction); afterwards, a standard second price auction without reserve price is run. Choosing for the entry fee the expected utility in the second price auction gives an expected  utility of zero to each buyer and the seller extracts the full surplus of the game. This mechanism is of course ex-ante-incentive-compatible. 
\end{proof}
This mechanism is not interim nor ex-post individually rational since for all valuation vectors, the utility of all losing bidders is negative. In order to slightly overcome  this issue, \citep{balseiro2017dynamic} and \citep{mirrokni2016dynamic} refined  this mechanism to ensure that bidders' utilities are not too negative at some point in the game; the trick is to  dispatch the fee on the different time steps instead of being paid at the beginning of the game. They also generalize the original setting to more complex dynamic auctions.

Considering the ex-ante setting makes sense only in auctions where the buyers do not know before participating their own valuation (but only the distribution). It is quite unrealistic in many single item auction, but it could make some sense 
when  $T$ successive auctions are run as in online ad market: indeed, the fee must be paid  before taking part in any of the $T$ auctions. While bidder can compute their distribution of values in the future, they do not know in advance what will be the exact future realizations. This unfortunately requires the bidders to also know perfectly the number $T$ of future auctions. This assumption has been weakened by \citep{agrawal2018robust} that adapted the above mechanisms to bidders that do not believe that there will be $T$ auctions. In this case, they are quite likely to refuse to pay a fee computed on $T$ auctions early in the game. %{\color{red} Ideas of techniques and proof?}

A crucial assumption of this line of work is to assume that bidder's value distributions are known to the seller beforehand; this enables her to compute precisely the extra-fees that can be charged to the bidders without breaking the ex-ante individually rational assumption. Similarly, it implicitly assumes that bidders are able to compute best response to dynamic mechanism (and that they implement them); this assumption is weakened in the following section.

\subsection{Learning against (almost) myopic buyers}

A first attempt to remove the prior knowledge of  bidder's value distributions, and instead to learn them \citep{amin2014repeated,mohri2015revenue,golrezaei2018dynamic}, is to consider mechanisms that are incentive compatible (up to a small number of bids) under the assumption that bidders are \emph{almost} myopic or impatient -- i.e. they have a fixed discount on future utilities. This agains introduces  an asymmetry between the bidders with a discounted long-term utility, and the seller with an undiscounted long-term revenue (infinitely patient). 

To simplify the exposure, we will focus on the posted price case. Formally, let us denote by  $p_t$ the price of the item at time $t$ chosen by the mechanism  and by  $d_t$ the decision of the buyer to buy ($d_t=1$) or to refuse the item ($d_t=0$). Since the distribution of values is not known beforehand, $p_{t+1}$ can only depend on the finite history  $\mathcal{H}'_t = \{p_1,d_1,\dots,p_{t},d_{t}\}$. The discounted bidder utility is $\sum_{t=1}^{T}  \gamma_t d_t (x_t - p_t)$, where $\gamma =(\gamma_t)_t$ is a sequence of non-negative weights. In this section, we shall assume for simplicity that values are uniformly bounded by 1.

The objective of the seller is to choose a  dynamic selling mechanism $\mathcal{DM}$, that will maximize her revenue,  against buyers that know  $\mathcal{DM}$ and  respond optimally for them, in the objective of maximizing their discounted and expected utilities. Let us denote by $d_t^*(\mathcal{DM})$ the optimal strategy of the bidder and by $p_t(\mathcal{DM})$ the price posted.  The performance of a dynamic mechanism will be measured in terms of ``regret'', whose definition is slightly different than in the previous section. 

\begin{definition2}%[Regret of a dynamic mechanism]
Given a dynamic mechanism $\mathcal{DM}$, the discount sequence $\gamma$ and the value distribution $\mathcal{F}$, the regret of the seller is
$$
R(\mathcal{DM},\gamma,F,T)=\max_{\mathrm{DM}^*} \mathds{E} \sum_{t=1}^T d_t^*(\mathrm{DM}^*)p_t(\mathrm{DM}^*) - \sum_{t=1}^T d_t^*(\mathcal{DM})p_t(\mathcal{DM})
$$ 
\end{definition2}
In this setting, $\mathrm{DM}^*$ consists in posting the monopoly price corresponding to the value distribution $\mathcal{F}$ at each round. We emphasize here that the dependencies in $\gamma$ and $F$ in the regret definition are hidden in the best responses $d_t^*(\cdot)$.

\begin{theorem2}[\cite{amin2013learning}]%[lower bound]
Let $\gamma_t$  be any positive non-increasing sequence and $\mathcal{D}\mathcal{M}$ be any dynamic selling mechanism. Then, there exists a buyer value distribution $F$ such that the regret $R(\mathcal{D}\mathcal{M},\gamma,F,T)  \geq \frac{1}{12} \sum_{t=1}^T \gamma_t$. In particular, sublinear regret is impossible to achieve if  $\sum_{t=1}^T \gamma_t = \Theta(T)$.
\end{theorem2}
This theorem states that if the buyer is patient enough, the seller can not learn the monopoly price soon enough to reach a sublinear regret.  However, when the sequence $\gamma_t$ decreases geometrically, i.e., $\gamma_t=\gamma^{t}$ for some $\gamma \in (0,1]$ which means that the buyer is relatively quite impatient, reaching sublinear regret is possible as $\sum \gamma_t = o(T)$. This can be achieved with a simple two-phased dynamic mechanism \citep{amin2014repeated}.

\begin{enumerate}
\item Phase  1 (of length: $\alpha T$) : offer a random price, uniformly in $[0,1]$
\item  Phase 2 (of length: $(1-\alpha) T$) : compute the optimal price corresponding to the bids of the first stage and offer this price until the end.
\end{enumerate}
\begin{theorem2}[\cite{amin2014repeated}]%[upper bound]
Choosing $\alpha=T^{-1/3}$  in the above mechanism ensures that for all  discount sequence  $\gamma_t=\gamma^{t}$, for some $\gamma \in (0,1]$, the regret is bounded as $\mathcal{O}(T^{\frac{2}{3}}\sqrt{\frac{\log(T)}{\log(1/\gamma)}})$.
\end{theorem2}
To reach this regret, the former algorithm  is actually run on several stages. On each stage, the seller has an explore phase (Phase 1) and an exploit phase (Phase 2). The length of each stage is growing with time (a length equal to $2^i$ steps where $i$ corresponds to the stage number). This technique is called \emph{peeling} and used to reach asymptotical bounds. 

To bound the regret, the main idea is to upper-bound the number of times the buyer can \emph{lie} by not being truthful.  Indeed, lying during the learning phase, could end up in a better price at phase 2. However, the total weight of that second phase is of order $\gamma^{T\alpha}$ for the bidder, so the future possible gain in lying becomes arbitrarily small as $T\alpha$ increases. On the contrary, lying during the first stage has a small, but non-negligible cost. As a consequence, it can be proved that the buyer is actually truthful at almost each stage (all but a finite number of them, independent of $T$). 

From the point of view of the seller, the first phase has a cost of $\alpha T$ and then, roughly speaking, optimal price can be computed up to $1/\sqrt{\alpha T}$, leading to a total cost of $\sqrt{T/\alpha}$ during the second phase. Balancing those terms gives the choice of $\alpha = T^{-1/3}$

This simple algorithm was then refined in \citep{mohri2015revenue} and extended to the case of K bidders in \citep{golrezaei2018dynamic}.

\begin{remark2}
Once again, this surplus extraction is possible only because there is an (artificial) asymmetry between the seller and the buyer preventing him to be too strategic. 
 This can also be enforced through another approach, yet it is valid only with several (almost) symmetric bidders -- leading to another type of asymmetry between the seller and buyers. The idea is quite simple: make the computations required (e.g., to determine a reserve price) not as a function of the buyer bids, but as a function of his competitors' bid \citep{ashlagi2016sequential,KanNaz14,epasto2018incentive}.  Unfortunately, this approach cannot handle the existence of any dominant buyer, i.e., a buyer with much higher values than the other bidders \citep{epasto2018incentive}. Therefore the impact of this technique is quite limited since revenue-optimizing mechanisms are mostly important when the buyers are heterogenous. Moreover, in the main real-world application of online advertising, with asymmetric bidders and no specific asymmetry between seller and buyers on future utilities, none of these mechanisms ends up being able to enforce truthful bidding.
\end{remark2}


\section{Reversing the asymmetry: Strategic buyer vs.\ myopic seller}
In the previous sections, the asymmetry between the seller and the buyers was always in favor of the former. On the other hand, there are many cases where the converse happens: the seller has her hand tied, while the buyers can and try to exploit this. For instance, the seller must sometimes disclose (and commit to) the learning algorithm she is using to devise her mechanism - for instance, a second price auction with  reserve price, or more generally the Myerson revenue-maximizing auction, based on the distribution of bids received. Let us denote by $\mathcal{M}(F_{B_i})$ the mechanism induced by the past distribution of bids $F_{B_i}$; for instance, $\mathcal{M}(F_{B_1},\ldots,F_{B_n})$ is a second price auction with personalized reserve price computed from $F_{B_i}$ (and not from the $F_i$ that are not known beforehand).

\subsection{A Stackelberg view}
The objective of \textit{a long-term strategic bidder} is to choose his bidding strategy $\beta_i \in \mathds{B}_i$ (a mapping from values to bids) to maximize his expected long-term utility. Because of this long-term aspect, we can assume that an arbitrarily large number of bids (it was denoted by $T$ previously) are sent, thus we will consider the following steady state analysis of the general dynamic game.  

 We recall that the strategy $\beta$ is defined so that when his value is $x_i \sim F_i$, the associated bid is $\beta_i(x_i)$; the (pushforward) distributions of such bids are denoted by $F_{B_i}= \beta_i\#F_i$ and they induce denoted by . 
 This steady-state  objective is particularly relevant in modern applications as most of the data-driven selling mechanisms are using large batches of bids as examples to update their mechanism. We consider that bidders are maximizing their expected utility since we assume the number of auctions to be sufficiently large in modern applications. 

\medskip

%We will also assume that the seller is myopic (but with respect to a batch of $m$ auctions): her learning algorithm is defined such that she maximizes her myopic revenue in a certain class of mechanism. 

%{\color{red} On a pas déjà dit ça ?? In terms of game theory, these interactions are a Stackelberg game between the seller - whose strategy is to pick a mechanism design that  maps bid distributions to reserve prices - and the bidders - who chose bidding strategies. The bidders are the leader of this game because we assume that bidders choose their strategy knowing the mechanism used by the seller.} Our overarching objective is to derive the best-response, for a given bidder $i$,  to  the strategy of the seller (i.e., a given learning algorithm) and the strategies of the other bidders (i.e., their bid distributions).

%\begin{definition2}[Bidder/Seller Stackelberg game] Stackelberg game in which strategic bidders assume the existence of a seller's learning algorithm $\mathcal{M}$. Each strategic bidder $i$ chooses a strategy $\beta_i$ that induces a (pushforward) bid distribution $F_{B_i} = \beta_i\#F_i$ used as input by the seller's algorithm. The goal of the strategic bidder is to optimize$$\argmax_{\beta_i} {U_i(\mathcal{M}(F_{B_i}),\beta_{i})}\;.$$ \end{definition2}

This problem has been tackled under the assumption of perfect knowledge of the optimization algorithm used by the seller \citep{KanNaz14,tang2016manipulate,nedelec2018thresholding}.  It exploits a conceptual opening in most automatic mechanism design works, i.e. the breakdown  of incentive compatibility for the buyer when the seller optimizes over incentive compatible auctions. In some sense, the computation of  bid distributions $F_{B_i}$ instead of value distributions $F_i$ can be seen as an ``attack'' of the optimization algorithm of the seller (possibly based on deep learning for complex auction systems \citep{dutting2017optimal}). However, we point out now that those attacks  differ from the celebrated adversarial attacks in computer vision. Indeed, the latter generally rely on the lack of local robustness of a classifier. Two other major differences are also quite important: these ``attacks'' do not necessarily yield lower revenues for the seller \citep{nedelec2018thresholding}; and they are also part of a dynamic game between buyers and seller and as such have a dynamic component that is absent from classical and static machine learning frameworks, such as image classification. 

If the buyer knows that the seller is going to find an \textbf{optimal} mechanism, and hence will optimize the auction based on the information given by the buyer's bid distribution, the buyer can anticipate this optimization to increase their utility. The order of the Stackelberg game is then reversed. The buyer becomes the leader and the seller the follower. The buyer reveals their bid distribution knowing the optimization problem that the seller will solve. In second price auctions with reserve prices, the buyer has an incentive to disclose a bid distribution that may be different from their value distribution as they then will be facing a more favorable reserve price by doing so. Our paper is focused on this version of the Stackelberg game, as we focus on the bidder standpoint. 

More formally, the timing of the game we consider is the following :
\begin{enumerate}
\item the seller chooses a mapping $\mathcal{M}$ from $F_{B_i}$ to a specific auction mechanism $\mathcal{M}(F_{B_i})$,
\item based on this mapping, each buyer chooses a bidding strategy $\beta_i$,
\item the payoff of the buyers is their utility under $(F_i, \mathcal{M}(F_{B_i}), \beta_i)$ and the seller's payoff is the revenue under this mechanism.
\end{enumerate}


This objective is particularly relevant in modern applications as most of the data-driven selling mechanisms are using large batches of bids as examples to update their mechanism.

We first consider the posted price setting where $K=1$ bidder plays against one seller. We assume, for simplicity of this introductory example, that bidder's value distributions $F_{X_i}$ is $\mathfrak{U}[0,1]$, i.e. uniform on the interval [0,1]. Let us initially consider that the bidder is bidding truthfully, i.e, $\beta_i = Id$. In this case, $F_{B_i} = F_{X_i}$ and the seller will set as reserve price the monopoly price by maximizing the monopoly revenue $r(1-F_{X_i}(r))$. This monopoly price is equal to 0.5 in the case of $\mathfrak{U}[0,1]$.  Note that this maximization problem is computationally simple as the monopoly revenue is a concave function if the value distribution is regular. The bidder can obviously do better. If he bids all the time zero  (or $\varepsilon$ arbitrarily close to zero), $F_{B_i}$ will be equal to a point mass at zero. Through computing the optimal reserve price corresponding to $F_{B_i}$, the seller chooses zero, obviously maximizing bidder's utility. The problem we consider derives from a simple extension of this example to the case of K bidders. In a lazy second price auction, the optimal reserve price for each bidder is still the monopoly price. Yet, as soon as there is some competition, bidders can not bid zero as they get zero utility in this case.  They have to tradeoff between beating the competition and decreasing their reserve price. 
\subsection{Improving the truthful strategy for any distributions of the competition}
\label{subsec:strat_bidder_any_distrib}
\citep{nedelec2018thresholding} derives a simple strategy which guarantees to the bidder an increase in utility compared to the truthful strategy for any distributions of the competition. This increase depends on the distribution of the competition. Yet, by playing this strategy, the bidder is sure to do better than by bidding truthfully. This is an important practical result as in many ad platforms, bidders have to bid without knowing the distribution of the competition. This strategy, that they call \textit{thresholding at the monopoly price}, has also the key property of making simple the optimization problem of the seller, i.e. if $F_{X_i}$ is regular, the bid distribution $F_{B_i}$ induced by
this strategy on  $F_{X_i}$ is also regular. 

\begin{table}[]
\centering
\small
\begin{tabular}{c|c|c|c|c|c|c|c|c}  
& \multicolumn{4}{c|}{Optimal reserve price} & \multicolumn{4}{c}{Utility} \\ \cline{2-9}
&K=1 &K=2&K=3&K=4  &K=1 &K=2&K=3&K=4\\ \hline
\multirow{2}{*}{Truthful bidding} & \multirow{2}{*}{0.5}& \multirow{2}{*}{0.5}& \multirow{2}{*}{0.5}&  \multirow{2}{*}{0.5}& \multirow{2}{*}{1/8} & \multirow{2}{*}{1/12} & \multirow{2}{*}{11/192}& \multirow{2}{*}{13/320} \\ 
 & &  &  & &&&& \\ \hline
\multirow{2}{*}{Zero bidding} &\multirow{2}{*}{0.0}&\multirow{2}{*}{0.0}&\multirow{2}{*}{0.0}& \multirow{2}{*}{0.0}  & 1/2 & 0.0 &  0.0 & 0.0\\ 
 &&&&  & (+400\%)  & (-100\%)  & (-100\%) & (-100\%) \\ \hline
 \multirow{2}{*}{Divide values by 2} &\multirow{2}{*}{0.25}&\multirow{2}{*}{0.25}&\multirow{2}{*}{0.25}& \multirow{2}{*}{0.25}  & 1/4 & $\approx 0.094$ &  $\approx 0.036$& $\approx 0.015$\\ 
 &&&&  & (+100\%)  & (+13\%)  & (-37\%) & (-63\%) \\ \hline
Thresholded at & \multirow{3}{*}{0.25}& \multirow{3}{*}{0.25}& \multirow{3}{*}{0.25}& \multirow{3}{*}{0.25}  & \multirow{2}{*}{1/4} &  \multirow{2}{*}{$\approx 0.132$}  & \multirow{2}{*}{$ \approx 0.076$}  & \multirow{2}{*}{$\approx 0.048$}\\
the monopoly price & &&&&&&&\\
(Theorem \ref{thm:settingReserveValToZeroImprovesPerformance}) &  &&&& (+100\%)  & (+57\%)  & (+33\%) & (+20\%) \\ \hlineB{4.0}
Optimal  regularity-& \multirow{2}{*}{0.0}& \multirow{2}{*}{0.162}& \multirow{2}{*}{0.204}& \multirow{2}{*}{0.22}  & \multirow{2}{*}{1/2} & \multirow{2}{*}{$\approx 0.147$}  & \multirow{2}{*}{$\approx 0.079$}  & \multirow{2}{*}{$\approx 0.049$}\\
preserving strategies&&&&  &  & &  & \\ 
(Theorem \ref{thm:quantificationOptimalThresholding})&&&&  & (+400\%)  & (+76\%)  & (+38\%) & (+21\%) \\ 
\hline
\end{tabular}
\caption{Comparison of the utility of the strategic bidder between the truthful strategy, the strategy corresponding to bidding zero for any values, the linear strategy dividing values by two, the strategy introduced in Theorem \ref{thm:settingReserveValToZeroImprovesPerformance} and the optimal regularity-preserving strategies for each number of competitors (derived from Theorem \ref{thm:quantificationOptimalThresholding}). The first four strategies are fixed and do not require knowledge of the competition to be computed. The last one is competition-specific and exact knowledge of the distribution followed by the highest bid of the competition is needed to compute it. For this example, bidders' value distributions are $\mathfrak{U}[0,1]$ and  opponents are assumed to bid truthfully.}
\label{table_intro}
\end{table}



\begin{definition}[Regularity-preserving strategy] Consider a bidder with a regular value distribution $F_{X_i}$. We say that a bidding strategy $\beta_i$ is regularity-preserving, if the bid distribution $F_{B_i}$ induced by $\beta_i$ on $F_{X_i}$ is a regular distribution.
\label{def:RP}
\end{definition}

When the reserve price is computed from $F_{B_i}$ -  the bid distribution induced by using $\beta$ on $F_{X_i}$ -  we have to make a distinction between the reserve price $r_\beta$ and the reserve value $x_\beta$.

\begin{definition}[Reserve value]
Consider a non-decreasing strategy $\beta$. We call reserve value $x_\beta$  the smallest value above which the seller accepts bids. 
\end{definition}
If the bidder bids truthfully, their reserve value is equal to their reserve price. If $\beta$ is increasing and $r_\beta$ is the reserve price associated with the strategy $\beta$, we have $x_\beta = \beta^{-1}(r_\beta)$. If $F_X = \mathfrak{U}[0,1]$, if we consider $\beta(x) = x/2$, we have $r_\beta = 0.25$ and $x_{\beta} = 0.5$. By dividing bids by two, the strategic bidder decreases their reserve price but does not change the reserve value~: it is the same as if they were  bidding truthfully.

\begin{theorem2}\label{thm:settingReserveValToZeroImprovesPerformance}
Let $\beta_r$ be an increasing strategy with associated reserve value $r>0$ in a lazy second price auction. Suppose the value distribution $F$ has a density $f$, with $f>0$ on the support of $F$ and that the left-end point of its support is 0. Suppose the bid distribution associated with $\beta_r$ has a virtual value. Assume that the other bidders' strategies are fixed. Then there exists another bidding strategy $\tilde{\beta}_r$ such that for any distributions of the highest bid of the competition: 
\begin{enumerate}
\item A reserve value associated with $\tilde{\beta}_r$ is 0. $\tilde{\beta}_r$ is increasing.
\item $\mathcal{U}_i(\tilde{\beta}_r)\geq \mathcal{U}_i(\beta_r)$, i.e., the utility of bidder $i$ is higher;
\item $P_i(\tilde{\beta}_r)\geq P_i(\beta_r)$, i.e., the payment of bidder $i$ to the seller is also higher,
\end{enumerate}
The following continuous function fulfills these conditions:
$$
\tilde{\beta}_r(x)=\left(\frac{\beta_r(r)(1-F_{X_i}(r))}{1-F_{X_i}(x)}\right)\mathds{1}\{x<r\}+\beta_r(x)\mathds{1}\{x\geq r\}
$$
\end{theorem2}
Having reserve value equal to zero means that the seller accepts all bids of the strategic bidder. It also means that the reserve price is equal to the minimum bid of the strategic bidder. This result can be applied to improve any preexisting shading strategy. A most important case is to apply this theorem to the truthful strategy, showing that there exists a strategy improving the truthful strategy regardless of the competition distribution. 
We now explain why we can improve any strategy in this setting without knowing the distribution of the competition.  Myerson's Lemma is a key element in this understanding.

In this setting, it is optimal for the seller to choose as reserve price for bidder $i$ the monopoly price corresponding to her bid distribution, and Myerson lemma implies that the expected payment of bidder $i$ in the optimized lazy second price auction is equal to 
\begin{equation*}
M_i(\beta_i) = \mathbb{E}_{B\sim F_{B_i}}\bigg(\psi_{F_{B_i}}(B)G_i(B)\textbf{1}(B \geq \psi_{B_i}^{-1}(0))\bigg)\;.
\end{equation*}
In order to simplify the computation of the expectation and remove the dependence on $B_i$, we rewrite this expected payment in the space of values using the fact that the strategic bidder is using an increasing strategy $\beta_i$. We will only consider increasing strategies in the rest of the paper. To do so, we define:
\begin{equation*}
h_{\beta_i}(x) \triangleq \psi_{F_{B_i}}(\beta_i(x))  
\end{equation*}
With this new notation, we can rewrite the expected payment of the strategic bidder $i$
\begin{equation*}
M_i(\beta_i) = \mathbb{E}_{X_i \sim F_{i}}\bigg(h_{\beta_i}(X_i)G_i(\beta_i(X_i))\textbf{1}(X_i \geq x_\beta)\bigg)\;.
\end{equation*}
and derive her expected utility as a function of $\beta_i$ as
\begin{equation}\label{equ:utility}
U(\beta_i) = \mathbb{E}_{X_i \sim F_{i}}\bigg((X_i-h_{\beta_i}(X_i))G_i(\beta_i(X_i))\textbf{1}(X_i \geq x_\beta)\bigg)\;.
\end{equation}
where $x_\beta$ is \emph{the reserve value}. If $h_{\beta_i}$ crosses 0 exactly once and is positive beyond that crossing point,  $x_\beta =  h_{\beta_i}^{-1}(0)$.  If we call $r_i=\psi_{F_{B_i}}^{-1}(0)$ the \emph{reserve price} of bidder $i$ and $\beta_i$  increasing , the \emph{reserve value} is equal to $\beta_i^{-1}(r_i)$. 

If we consider only increasing differentiable strategies, and we denote by  $\mathcal{I}$ the class of  such functions, the problem of the strategic bidder is therefore to solve  $ \sup_{\beta \in \mathcal{I}} U(\beta) $ with $U$ defined in Equation \eqref{equ:utility}. This equation is crucial, as it indicates that optimizing over bidding strategies can be reduced to finding a distribution with a well-specified  $h_\beta(\cdot)$. Our results extend to the case where the strategies are increasing and differentiable except at finitely many points, as we only need $bF_B(b)$ to be absolutely continuous for the previous result to go through.

A crucial difference between the long term vision and the classical, myopic (or one-shot)  auction theory is that in this setup bidders maximize expected utility globally over the full support of the value distribution. In the classical myopic setting, bidders determine their bids so as to maximize their expected utility at each value. In our setup, the strategic bidder also accounts for the computation of the reserve price, a function of her global bid distribution. He might therefore be willing to sometimes over-bid (incurring a negative utility at some specific auctions/values) or underbid (lose some auctions that he would have won otherwise) if this reduces her reserve price. Indeed, having a lower reserve price increases the utility of other auctions. Lose small to win big. In other words, the strategy trades-off ex-post individual rationality (IR) for higher utility (of course ex-ante IR still holds). This reasoning makes sense only with multiple interactions between bidders and seller.

\subsubsection{Thresholding the virtual value}
\label{subsec:thresholding_virtual_value}
A truthful bidding strategy can easily be improved by a strategic bidder, as illustrated by the following elementary example. Consider that the value distribution of the bidder is  $\mathfrak{U}([0,1])$, uniformly  between 0 and 1. With a truthful bidding, the associated virtual value is negative below $1/2$ and positive above, so that the optimal reserve price is $1/2$, so that no auction is won if the value is smaller than $1/2$.  On the other hand, if the strategic bidder was able to send bids so that the virtual value (of bids) below $1/2$ is exactly 0, then  the seller would not have any incentives to choose a reserve price, because of Myerson lemma. In particular, the latter also implies that since the virtual value is zero below $1/2$, the seller receives exactly the same expected payment as with a truthful bidder. 

This technique is called \textbf{thresholding the virtual value}. We now show formally how to find a bidding strategy such that the virtual value of the induced bid distribution is equal to zero below a certain threshold.
\begin{figure}[t]
\centering
\begin{tabular}{cc}
\includegraphics[width=.40\linewidth]{images/virt_value_truth.pdf} &
\includegraphics[width=.40\linewidth]{images/virt_value_thresh.pdf}
\end{tabular}
\caption{\textbf{Virtual value of truthful bidder vs. strategic bidder.} The value distribution of the bidder is $\mathfrak{U}[0,1]$, the standard textbook example used for the sake of illustration. Her virtual value is therefore equal to $\psi(x) = 2x -1$, and is represented by the blue line. The dashed red vertical line corresponds to the current reserve price. The green area corresponds to the bidder's payment if we picked $G=1$, i.e. no competition, for the sake of clarity of the plot. The left-hand side corresponds to truthful bidding, the right-hand side to strategic behavior. In both cases, the blue line corresponds to $\psi_{B}$.}
\label{fig:fig1vValueTruthvsStrat} % I can do without the label too
\end{figure}
Before carrying on with reasoning on the virtual value, such as in our motivating example, we need to ensure we can find the corresponding strategy $\beta_i$ that will expose a bid distribution $F_{B_i}$ with the corresponding virtual value to the seller. The two following technical lemmas show how to deduce $\beta_i$ from a given $h_{\beta_i}$.
%To derive the corresponding bidding strategy, we present two important technical lemmas. 
\begin{lemma2}\label{definition_psi}
Suppose $B_i=\beta_i(X_i)$, where $\beta_i$ is increasing and differentiable and $X_i$ is a random variable with cdf $F_i$ and pdf $f_i$ satisfying \textbf{A2}. Then 
\begin{equation}\label{eq:ODEPhiG}
h_{\beta_i}(x_i)\triangleq \beta_i(x)-\beta_i'(x)\frac{1-F_{i}(x)}{f_{i}(x)} = \psi_{F_{B_i}}(\beta_i(x)) \;.
\end{equation}
\end{lemma2}
\begin{proof}
We have $\psi_{F_{B_i}}(b) = b - \frac{1 - F_{B_i}(b)}{f_{B_i}(b)}$ with $F_{B_i}(b) = F_{i}(\beta_i^{-1}(b))$ and $f_{B_i}(b) = f_{i}(\beta_i^{-1}(b)/\beta_i'(\beta_i^{-1}(b))$.
Then, 
$h_{\beta_i}(x) = \psi_{B_i}(\beta_i(x)) = \beta_i(x) - \beta_i'(x)\frac{1-F_{i}(x)}{f_{i}(x)}\;.$
\end{proof}
The above results holds when $\beta$ is increasing, continuous, and differentiable except at finitely many points. The second lemma shows that for any function $g$ we can find a function $\beta$ such that $h_\beta = g$.

\begin{lemma2}\label{lemma:keyODEs}
Let $X$ be a random variable with cdf $F$ and pdf $f$ satisfying \textbf{A2}. Let $x_0$ be in the support of $X$, $C\in\mathbb{R}$ and $g:\mathbb{R} \rightarrow \mathbb{R}$. We call 
\begin{equation}\label{eq:gAsConditionalExpectation}
\beta_g(x)=\frac{C(1-F(x_0))-\int_{x_0}^{x} g(u) f(u) du}{1-F(x)}\;.
\end{equation}

% \begin{equation}\label{eq:gAsConditionalExpectation}
% \beta_g(x)=\frac{\int_x^{\mathfrak{u}} g(t) f(t) dt}{1-F(x)}=\mathbb{E}(g(X)|X\geq x)
% \end{equation}
% is increasing and differentiable on the support of $X$.

Then, if $B=\beta_g(X)$, 
$$
h_{\beta_g}(x) = g(x) \text{ and } \beta_g(x_0)=C\;.
$$ 
If for some $t$, $x_0\leq t$ and $g$ is non-decreasing on $[x_0,t]$,  $\beta_g'(x)\geq (C-g(x))(1-F(x_0))f(x)/(1-F(x))$ for $x\in[x_0,t]$. Hence $\beta_g$ is increasing on $[x_0,t]$ if $g$ is non-decreasing and $g<C$.
\end{lemma2}

\begin{proof}
The result follows by simply differentiating the expression for $\beta_g$, and plugging-in the expression for $h_{\beta_g}$ obtained in Lemma \ref{definition_psi}. The result on the derivative is simple algebra.
\end{proof}
The two technical lemmas \ref{definition_psi} and \ref{lemma:keyODEs} show that for any non-decreasing function $g$, we can find a strategy $\beta_i$ such that the bid distribution induced by using $\beta_i$ on $F_{X_i}$ verifies $\psi_{B_i}(\beta_i(x)) = g(x)$ for all $x$ in the support of $F_{X_i}$.

%
% In Section \ref{subsec:thresholding_virtual_value}, we explained why sending a virtual value equal to zero when the initial one was negative increases the bidder's expected utility. To go from this virtual value to the corresponding bidding strategy $\beta$, we need to solve the simple ODE defined in Lemma \ref{definition_psi}. More formally, the following theorem shows how to improve any strategy assuming the bidder knows the current reserve price or value. This theorem works for non-regular value distributions and in the asymmetric case when the bidders have different value distributions.\nek{Conditions on $\psi$? This looks like an impossible result and will trigger referee backlash}
We explained why sending to the seller a virtual value equal to zero when the initial one was negative increases the bidder's expected utility. To derive the corresponding bidding strategy $\beta$ from the virtual value, the strategic bidder only needs to solve the simple ODE defined in Lemma \ref{definition_psi}. 


\begin{figure}[t!]
\centering
\begin{tabular}{ccc}
\includegraphics[width=.40\linewidth]{images/truthfulvsthresh.pdf} &
\includegraphics[width=.40\linewidth]{images/virtual_value_bid_distribution.pdf}&

\end{tabular}	
\caption{\textbf{The value distribution is $\mathfrak{U}[0,1]$. Left: Thresholded strategy $\tilde{\beta}_{0.5}^{(0)}$ compared to the traditional truthful strategy. Right: virtual value of the bid distribution induced by the thresholded strategy.} The optimal reserve price of the thresholded strategy is equal to 0.25 (corresponding to a reserve value of 0) whereas the reserve price of the truthful strategy is equal to 0.5. (corresponding to a reserve value of 0.5). The green area represents the expected payment corresponding to the thresholded strategy (we assumed $G = 1$ for the sake of clarity).}
\label{fig:fig2} % I can do without the label too
\end{figure}
This improvement of bidder's utility does not depend of the estimation of the competition and thus can easily be implemented in practice. 
%This technique is called thresholding the virtual value at the monopoly price.
We plot in Figure \ref{fig:fig3}, the bidding strategy $\tilde{\beta}_{0.5}^{(0)}$ when the initial value distribution is $\mathfrak{U}[0,1]$ and the virtual value of the bid distribution induced by $\tilde{\beta}_{0.5}^{(0)}$ on $\mathfrak{U}[0,1]$. We recall that the monopoly price corresponding to $\mathfrak{U}[0,1]$ is equal to $0.5$. We remark that the strategy consists in overbidding below the monopoly price of the initial value distribution. The strategic bidder is ready to increase pointwise her payment when she wins auctions with low values in order to get a large decrease of the reserve price (going from $0.5$ to $0.25$). Globally, the payment of the bidder remains unchanged compared to when the bidder was bidding truthfully with a reserve price equal to 0.5. Thresholding the virtual value at the monopoly price amounts to overbidding below the monopoly price, effectively providing over the course of the auctions an extra payment to the seller in exchange for lowering the reserve price/value faced by the strategic bidder. This strategy unlocks a very substantial utility gain for the bidder. 

Naturally, a key question is to understand the impact of this new strategy on the utility of the strategic bidder. We compare the situation with two bidders bidding truthfully against an optimal reserve price and the new situation with one bidder using the thresholded strategy and the second one bidding truthfully. We assume, as is standard in many textbooks and research papers numerical examples, that their value distribution is $\mathfrak{U}[0,1]$. 

Then, elementary computation show that in this specific illustrative example, the strategic bidder utility increases from $1/12$ to $1/12 + (\log(2) - 1/2) / 4 \approx 0.132$ (\textbf{a 57\% increase}) and the welfare increases from 7/12 to $7/12 + (\log(2) - 1/2) / 4 \approx 0.632$. (\textbf{a 8\% increase}).
\subsection{Best response for a known distribution of the competition}
\label{sec:best_response_with_competition_knowledge}
%\section{Strategic improvements with increased side information}
We now show, for a specific given distribution of the competition, what is the optimal increasing and regularity-preserving (RP) strategy (Definition \ref{def:RP})). 

We presented in Subsection \ref{subsec:strat_bidder_any_distrib} a direct way to compute the expected utility of a bidding strategy $\beta_i$ when the seller is using a second price auction with personalized reserve price and the other bidders are bidding truthfully:
\begin{equation}\label{equ:utility_v2}
U(\beta_i) = \mathbb{E}_{X \sim F_{i}}\bigg((X-h_{\beta_i}(X))G_i(\beta(X))\textbf{1}(X \geq x_{\beta_i})\bigg)\;.
\end{equation}
with 
$h_{\beta_i}(x) = \beta_i(x) - \beta_i'(x)\frac{1-F_{X_i}(x)}{f_{X_i}(x)}\;$ and $x_{\beta_i} = h_{\beta_i}^{-1}(0)$.
In this section, we assume that the bidder has now access to the distribution of the highest bid of the competition that we denote by $G_i$ ($g_i$ being the associated pdf). 
% This form can be computed in many different settings and offers a way to compute optimal bidding strategies in some parametric class of functions by finding zeros of the directional derivatives.


In the following, unless otherwise stated, the expectation is taken according to the value distribution of the bidder. In order to be able to derive optimal strategies, we make use  of the previous expression and obtain the following lemma (we remove the subscript $i$ as it is now clear we consider bidder $i$).


We can optimize among the strategies with thresholded virtual values that we introduced in Subsection \ref{subsec:strat_bidder_any_distrib}.

\begin{definition2}[Thresholded bidding strategies]\label{definition_thresholded_strategies}
 A bidding strategy $\beta$ is called a thresholded bidding strategy if and only if there exists $r>0$ such that for all $x < r, h_{\beta}(x) = \psi_B(\beta(x)) = 0$. This family of functions can be parametrized with
\begin{equation*}
\beta_r^\gamma(x)=\frac{\gamma(r)(1-F(r))}{1-F(x)}\indicator{x< r}+\gamma(x)\indicator{x\geq r}\;,
\end{equation*}
with $r \in \mathbb{R}$ and $\gamma: \mathbb{R} \rightarrow \mathbb{R}$ continuous and increasing.
\end{definition2}

This class of continuous bidding strategies has two degrees of freedom : the threshold $r$ such that for all $x < r, h_{\beta}(x) = 0$ and the strategy $\gamma$ used beyond the threshold. We do not restrict the functions  $\gamma$ that can be used beyond the threshold (beside being continuous and increasing). All the strategies defined in this class have the property that their reserve value is equal to zero, i.e. their reserve price is equal to their minimum bid, when the seller is welfare benevolent and the virtual value of $\gamma$ is positive beyond $r$. We can prove that the optimal regularity-preserving strategy belongs to the class of thresholded strategies.

We now show that there exists an optimal threshold $r$ for the strategic bidder that depends on the competition and that the optimal strategy to use for $x > r$ is to be truthful. We derive this result by computing the directional derivatives of the utility function defined in Equation \eqref{equ:utility_v2}.

\begin{theorem2}\label{thm:quantificationOptimalThresholding}
Assume $F_i$ is regular, a best response in the class of increasing and regularity-preserving strategies consists in thresholding at $r^*$ and bidding truthfully beyond $r^*$, where $r^*$ satisfies the equation, if $G$ is the distribution of the largest bid of the competition, 
\begin{equation*}\label{eq:keyEqThreshStratOneStrategic2}
G(r^*)=\mathbb{E}\bigg(\frac{X}{1-F(X)}g\left(\frac{r^*(1-F(r^*))}{1-F(X)}\right)\indicator{X\leq r^*}\bigg)\;.
\end{equation*}
\label{theorem2}
\end{theorem2}
%This lemma is useful when searching for the optimal shading strategies in various class of shading functions. It can also be used to improve bidding strategies by performing gradient ascent for $\beta$ expanded in a dictionary of functions, such as splines. We ran some of these experiments and got interesting results but do not report on them in this paper.\redtext{is this paragraph needed?}

%When bidder $i$ knows the distribution of the maximum bid of the competition denoted by $G_i$, she can optimize her strategy over various class of functions. 
\begin{figure}[t]
\centering
\begin{tabular}{ccc}
\includegraphics[width=.33\linewidth]{images/Optimal_strategies2.pdf} &
\includegraphics[width=.33\linewidth]{images/virtual_value_bid_distribution2.pdf}&
\includegraphics[width=.33\linewidth]{images/bidder_paiment2.pdf} 

\end{tabular}	
\caption{\textbf{The value distribution is $\mathfrak{U}[0,1]$. Left: Thresholded strategy compared to the traditional truthful strategy. Middle: virtual value of the bid distribution induced by the thresholded strategy. Right: monopoly revenue of the induced bid distribution as function of the reserve price.}  }
\label{fig:fig3} % I can do without the label too
\end{figure}

In Theorem \ref{thm:settingReserveValToZeroImprovesPerformance}, we proved that when the strategic bidder does not know the distribution of the highest bid of the competition, he can use the thresholded strategy at his monopoly price and increases his utility compared to truthful bidding. Theorem \ref{thm:quantificationOptimalThresholding} gives the optimal threshold when the strategic bidder knows $G$. 

\textbf{Some numerical results} We consider the situation where we have 1 strategic bidder, and 1 non-strategic one, both wit in Subsection \ref{subsec:strat_bidder_any_distrib} was to bid truthfully beyond the monopoly price ($r=.5$ here) and using Theorem \ref{thm:settingReserveValToZeroImprovesPerformance} before.  This strategy yields a utility of $0.1316$, a $57\%$ increase over the standard truthful bidding revenue. The optimal strategy coming out of Theorem \ref{theorem2} consists in bidding truthfully beyond $r\simeq .8$ and using the thresholding completion before. The utility is then around 0.1468, a 76\% percent increase in bidder utility compared to bidding truthfully (truthful bidding yields a utility of $1/12\simeq .083$). This second strategy yields a higher utility for the strategic bidder but requires some knowledge of the competition. The optimal strategy in Theorem \ref{thm:quantificationOptimalThresholding} overbids on small values, underbids on intermediate values and is truthful on high values. We also recover that with no competition, the optimal strategy is to bid zero for any possible valuations. In Table \ref{table_intro}, we also notice that the difference in utility is decreasing with the number of players since, with increasing  competition, the strategic bidder can not lower his bid for values above his monopoly price. 


\subsection{Nash equilibrium}
In the previous section, only one bidder was strategic and the other bidders did not directly react to this strategy. It could be  a reasonable assumption in practice since the number of bidders able to implement sophisticated bidding strategies appears to be limited, but we still investigate the case where all bidders are strategic. For simplicity, we shall assume that they are symmetric, with  the same value distribution $F_X$. We consider a  large class of admissible bidders strategies: the large set of all thresholded bidding strategies introduced in Definition \ref{definition_thresholded_strategies}. If bidders only use strategies from this set, then there exists a unique Nash equilibrium, and  their  utility is the same as in a  second price auction without reserve price.

\begin{theorem2}[\cite{tang2016manipulate,nedelec2018thresholding}]
\label{thm:nashEquiThresholded} 
Assume that bidders are symmetric, with a  valuations distribution  supported on $[0,1]$, with a continuous positive  density at $0$ and $1$, and such that the virtual value  equals 0 exactly once and is positive beyond. Then there exists a unique symmetric Nash equilibrium in the class of thresholded bidding strategies that can be computed by solving 
\begin{equation}\label{eq:keyEqThreshStratAllStrategic}
\frac{n-1}{r^*(1-F(r^*))}\mathds{E}\Big[XF^{n-2}(X)(1-F(X))\indicator{X\leq r^*}\Big] = F^{n-1}(r^*)\;
\end{equation}
 to determine the common reserve price $r^*$. Moreover, at this Nash equilibrium, the revenue of the seller and the utilities of the buyers are the same as in a second price auction without reserve prices. 	
\end{theorem2}
With appropriate shading functions, the bidders can recover the utility they would get when the seller was not optimizing her mechanism to maximize her revenue. The fact that at symmetric equilibrium bidders recover the same utility as in a second price auction with no reserves arguably makes it an even more natural class of bidding strategies to consider from the bidder standpoint. 
\subsection{Perturbation analysis for the Myerson auction}
These precedent results can be extended beyond the lazy second price, and to the Myerson auction (see, e.g.,  \citep{nedelec2019learning}. for more details). The Nash equilibrium has a relatively simple form given in the following Theorem \ref{thm:shadingInSymmMyerson}. 

\begin{theorem2}[\cite{tang2016manipulate,abeille2018explicit}]\label{thm:shadingInSymmMyerson}
%Consider an auction with $K$ independent and symmetric bidders, having value distribution represented by the random variable $X$. 
In the Myerson auction, the symmetric equilibrium strategy   $\shadingFunc_{eq}$  satisfies 
$$
\shadingFunc_{eq}(x)+\shadingFunc_{eq}'(x)(\vValue_X(x)-x)=\beta^{I}(x)\;,
$$
where $\beta^{I}(x)$ is the symmetric equilibrium strategy in a first price auction with no reserve price.  A solution of this equation is $$\shadingFunc_{eq}(x)=\mathds{E}[\beta^{I}(X)|X\geq x]\;.$$
At the equilibrium, the bidders' expected utilities are the same as  in a first price auction without reserve price; in particular, it is strictly greater than their expected payoffs had they bid truthfully. 
\end{theorem2}
\paragraph{\textbf{Discussion}} The intuition behind this result is quite clear. In the Myerson auction, the expected utility of a bidder is the same as in a first price auction where her bids have been transformed through his virtual value function. We call the corresponding pseudo-bids ``virtualized'' bids. Hence, if the bidders can bid in such a way that their virtualized bids are equal to their symmetric equilibrium first price bids, the situation is completely equivalent to a first price auction. And hence their equilibrium strategy in virtualized bid space should be the strategy they use in a standard first price auction with no reserve price. 
\iffalse
Our theorem shows that by adopting such a strategy symmetric bidders can avoid facing a non-zero reserve price. Furthermore, Lemmas \ref{definition_thresholded_strategies} and \ref{lemma:makingSureGIncreasing} show that it is easy for bidders to shade in such a way that their virtualized bids are equal to any increasing function of their value they choose. Also, this shading is specific to each bidder: the corresponding ordinary differential equations do not involve the other bidders. As such it is also quite easy to implement. 
\fi
\subsection{Approximations of the Myerson auction via numerical methods}
This new variational approach unlocks, through numerical optimization, a method to find best-responses to most of the approximated Myerson auction, such as boosted second price auctions \citep{nedelec2019learning}.  
 A straightforward optimization can fail because the objective is  discontinuous as a function of the bidding strategy.  To circumvent this issue,  a new relaxation of the problem which is stable to local perturbations of the objective function and computationally tractable and efficient has been introduced.  This new objective can be  numerically optimized through a simple neural network, with very significant improvements in bidder utility compared to truthful bidding. This simple approach can be plugged in any modern bidding algorithms learning distribution of the highest bid of the competition and we test it on other classes of mechanism without any known closed form optimal bidding strategies. 
 
The major and prohibitive drawback of these approaches is that they require that strategic bidders perfectly know the underlying mechanism design problem (i.e. the revenue maximization problem) solved by the seller, leading to a strong asymmetry between the bidders and the seller, this time in favor of the former.

It is nonetheless possible to remove the prior knowledge on  the exact algorithmic procedure used by the seller to optimize her mechanism by a classical exploration/exploitation trade-off, inspired by reinforcement learning techniques, thus reducing this asymmetry \citep{nedelec2019adversarial}.


\section{A general dynamic game and multi-agent reinforcement learning}

%Recently, \citep{bravo2018bandit} studied some convergence properties in concave-N-person games. They prove that if all the players are using a no-regret algorithm to learn how to play, this converges to a Nash equilibrium. 

Probably more practical and realistic interactions between the seller and the bidders would be described as follows.

During the first stage of the game, the seller, as she has no information on bidders' value distribution, runs a batch of $T_0$ second-price auctions without reserve price (mechanism $M_0$). The strategic bidder is using the strategy $\beta_{i,0}$ for this first batch of auctions. The seller has then access to a dataset of $m$ bids $S_{T_0}^0 = \{b_1^0,...,b_{T_0}^0\}$ corresponding to these first $m$ auctions. She can then use a learning algorithm $\mathcal{M}_1$ to compute a new mechanism $\mathcal{M}_1(S_{T_0}^0)$   that would be used for the second stage. In full generality, at each stage, the bidder can change of bidding strategy and the seller can change of learning algorithm.  We only show one strategic bidder but there could exist multiple strategic bidders on the seller's platform.

\begin{figure*}[h!]
\begin{tikzpicture}[
    block/.style={rectangle, draw, text centered, rounded corners,     minimum
    height=4em,text width=5.5em}
]
\small
	
	\node[thick] (z) {Strategic bidders};
	\node[above=of z, thick] (xinit) {Dynamic game};
	%\node[left=of xinit] (lxinit) {};
	%\draw[-stealth, thick] (lxinit) -- node[above] {$F$} (xinit);
	[
	\node[above=of xinit, thick] (xinit2) {Strategic seller};
	%\node[left=of xinit2] (lxinit2) {};
	%\draw[-stealth, thick] (lxinit2) -- node[above] {$F$} (xinit2);
	

	
	%\node[left=of z] (i) {};
	%\draw[-stealth, thick] (i) -- node[above] {$F$} (z);
	\node[rectangle, draw, thick, right=1.0em of xinit, text width=1.8cm] (bidderbox) {$T_0$ auctions of type $M_0$} ;
	
	\node[circle, draw, thick, right=1.5em of bidderbox, text width=0.6cm] (dataset) {$S_m^0$} ;
	
	\node[rectangle, draw, thick, right=2.0em of dataset, text width=1.8cm] (mech1) {$T_1$ auctions of type $\mathcal{M}_1(S_{T_0}^0)$} ;

	\node[circle, draw, thick, right=2.0em of mech1, text width=0.6cm] (dataset2)  {$S_{T_1}^1$} ;

	\node[rectangle, draw, thick, right=2.0em of dataset2, text width=1.8cm] (mech2) {$T_2$ auctions of type $\mathcal{M}_2(S_{T_2}^1)$} ;

	\node[ thick, right=1.0em of mech2, text width=1.5cm] (end) {$\dots$} ;
	
	\draw[-stealth] (bidderbox) --  (dataset);
	\draw[-stealth] (dataset) --  (mech1);
	\draw[-stealth] (mech1) --  (dataset2);
	\draw[-stealth] (dataset2) --  (mech2);
	\draw[-stealth] (mech2) --  (end);

	%\node[right=0.5em of bidderbox, circle, fill, inner sep=0.15em] (pt1) {};
	\node[right=0.5em of dataset, circle, fill, inner sep=0.15em] (pt2) {};
	%\node[right=0.5em of mech1, circle, fill, inner sep=0.15em] (pt3) {};
	\node[right=0.5em of dataset2, circle, fill, inner sep=0.15em] (pt4) {};
	%\node[right=0.5em of mech2, circle, fill, inner sep=0.15em] (pt5) {};
	
	\node[rectangle, draw, thick, below= of bidderbox] (bidderstrat1) {$\beta_{i,0}$} ;
	\node[rectangle, draw, thick, above= of pt2] (seller1) {$\mathcal{M}_1$} ;
	\node[rectangle, draw, thick, above= of pt4] (seller2) {$\mathcal{M}_2$} ;
	\node[rectangle, draw, thick, below= of mech1] (bidderstrat2) {$\beta_{i,1}$} ;
	\node[rectangle, draw, thick, below= of mech2] (bidderstrat3) {$\beta_{i,2}$} ;

	\draw[-stealth] (bidderstrat1) --  (bidderbox);
	\draw[-stealth] (bidderstrat2) --  (mech1);
	\draw[-stealth] (bidderstrat3) --  (mech2);

	\draw[-stealth] (seller1) --  (pt2);
	\draw[-stealth] (seller2) --  (pt4);
			
	%\draw[thick] (pt1) edge (pt2);
			
	%\node[circle, draw, thick, fill=white, inner sep=0.15em] at ([xshift=-0.9em, yshift=4em]pt1.north) (pt3) {};
			
	%\draw[-stealth, thick] (x) -- (pt1);
	%\draw[-stealth, thick] (xt) -- (pt2);
	%\draw[-stealth, thick] (pt3) -- (D);

\end{tikzpicture}
\caption{\textbf{A general dynamic game for the batch auction setting.}
} 
 \label{dynamic_game}
\end{figure*}

One natural extension would be to understand what would happen, in terms of convergence, if players are using more complex algorithms. Instead of no-regret algorithm, they could be long-term strategic with anticipating other agent's decisions. Work at the frontier between these fields will be key to address concerns on the use of automatic decision processes in most economical problems.







==> chapters/sept2Chap2BackupIncase/chapter2_some_classical_results.tex <==
%!TEX root = ../main.tex
\chapter{Bayesian mechanism design}
\label{Chapter:Bayes}

Auctions mechanisms involve many different agents, sellers and/or buyers, with possibly different and conflicting objectives as they all seek to optimize of their own utility functions. These interactions can be modeled using game-theoretic concepts. More specifically, we are going to focus on a specific types of games with \emph{incomplete information} that are called \textit{mechanisms}. In those games, each player has some private information (i.e. unknown from everyone else), and send a \emph{message} to a central authority.  Based on those gathered messages, the latter decides on the final outcome.  The utility of each player then solely depends on it \nek{the set of messages sent +mechanism?}. 

Mechanisms model appropriately  many practical situations such as the celebrated  problems of assigning students to schools, or matchings in organ-transplant applications.  In these problems, a central authority forms pairs between school and students or donors and recipients. In selling mechanisms, the central authority is the seller of a specific item and the players are the buyers.  \emph{Auctions} are mechanisms used to sell a particular item. In the case of a sale of a single non-divisible item, they have the following specific features. 


%\clem{The notation defined here is not used later on and even conflicts with later notation.}{\color{red}VP : agreed !}
%A \textit{normal-form game} is defined by a set of of players $\mathcal{N}$ of cardinality $N$, the set of actions  $\mathcal{A}_i$ and the payoff function  of player $i \in \mathcal{N}$
%$u_i:\mathcal{A}_1 \times \dots \times \mathcal{A}_N \rightarrow \mathds{R}.$ 
%
%In such a game, each player chooses independently an action $a_i \in \mathcal{A}_i$ and gets a utility of $u_i(a_1,\ldots,a_N)=u_i(a_i,a_{-i})$
%that depends on both the action $a_i \in   \mathcal{A}_i$ of the player and the profile of actions of other players, denoted by $a_{-i} := (a_1,\ldots, a_{i-1}, a_{i+1},a_N) \in \prod_{j \neq i} \mathcal{A}_j$.
%
% 
%\begin{definition2}[Normal-form game]
%A normal-form game is:
%\begin{itemize}
%\item a set of players $\mathcal{N}$ of cardinality $N$.
%\item for each player $i \in [1,N]$, a set of possible actions $\mathcal{A}_i$.
%\item a set of payoff functions which gives for each player her payoff corresponding to her action and actions of other players
%$$u_i:\mathcal{A}_1 \times \dots \times \mathcal{A}_N \rightarrow \mathds{R}\;.$$
%\end{itemize}
%In a normal-form game of complete information, actions, outcomes and payoff functions are common knowledge to all players. In a game of incomplete information, every player's payoff function depends on a variable $X$ called private information and which is only known to each specific player. If we denote by $\mathcal{X}$ the set of private information, the payoff function of player $i$ is defined as $u_i:\mathcal{A}^{N} \times \mathcal{X} \rightarrow \mathds{R}$.
%\end{definition2}


%In the different settings we are going to consider,  players have some private information that actually impacts their payoff functions. Formally, let us denote by  $\mathcal{X}$ the set of private information, so that the payoff function of player $i$ rewrites as  $u_i:\prod_{j \in \mathcal{N}} \mathcal{A}_j \times \mathcal{X} \rightarrow \mathds{R}$. Those games are called with \textit{incomplete information}.


\medskip


%and decides each player's outcome according to these messages. In these games, players' actions correspond to the message they send to the central authority. 

%In a game of incomplete information, every player's payoff function depends on a variable $X$ called private information and which is only known to each specific player. If we denote by, the payoff function of player $i$ is defined as 

%In this survey, we are focusing on a certain type of games with incomplete information where there exists a central authority which gathers messages from the different players and decides each player's outcome according to these messages. In these games, players' actions correspond to the message they send to the central authority. This type of centralized gamed is called mechanism. 
%\begin{definition2}[Mechanism]
%A mechanism is a game of incomplete information where players send a message to a central authority who does not know the private information of each player. The central authority decides based on messages it receives and some predefined rules every player's outcome.  
%\end{definition2}

Auctions are games of incomplete information as each buyer has some private valuation for the item to be sold, i.e. the highest price they are willing to  pay to acquire  this item. This valuation might be different from one buyer to another. We denote by $\mathcal{N}$ the set of buyers, of cardinality $n \in \mathbb{N}$, by  $x_i \in \mathcal{X}_i$ the  private value of bidder $i \in \mathcal{N}$, $\mathcal{X}_i $ the set of private values of bidder $i$, and by  $x = (x_1,\dots,x_n)\in \mathbb{R}^n$, the so-called profile of private values. 
The possible messages (or actions) of buyer $i\in \mathcal{N}$ are called ``bids'' and the set of bids of buyer $i$ is denoted by $\mathcal{B}_i$. The outcome of an auction mechanism is defined by two different rules~:
\begin{enumerate}
\item an \textit{allocation rule} $q:\mathcal{B}_1 \times \dots \times  \mathcal{B}_n \rightarrow \Delta_n$ where $\Delta_n$ is the set of probability distributions over the set of $n$ buyers. It specifies the probability that each player gets the item.
\item a \textit{payment rule} $p: \mathcal{B}_1 \times \dots \times  \mathcal{B}_n \rightarrow \mathds{R}^{n}$. It specifies the expected payment of each player, whether or not they get the item.
\end{enumerate}

We also denote by $b = (b_1,\dots,b_n)$ the vector of bids of the bidders.  With these notations, the expected utility of bidder $i \in \mathcal{N}$ is then defined as
$$u_i(b,x_i) = q_i(b)\big(x_i -p_i(b)\big)\;;$$
on the other hand, the seller aims at maximizing her expected revenue
$$\sum_{i=1}^n q_i(b)p_i(b)\;.$$

%\begin{definition2}[Auction mechanism]
%An auction mechanism is a mechanism defined by three features: 
%\begin{itemize}
%\item a set of possible messages $\mathcal{B}_i$ for each buyer (bids in most cases). 
%\item an allocation rule $q:\mathcal{B}_1 \times \dots \times  \mathcal{B}_N \rightarrow \Delta_N$ where $\Delta_N$ is the set of probability distributions over the set of $N$ buyers. It gives the probability that each player gets the object.
%\item a payment rule $p: \mathcal{B}_1 \times \dots \times  \mathcal{B}_N \rightarrow \mathds{R}^{N}$. It defines the expected payment of each player whether he got or not the object.
%\end{itemize}
%A selling mechanism is nothing more than a set of rules explaining how a group of buyers and a seller interact. 
%
%The private information owned by each buyer which conditions their payoff function is their own value for the item, i.e., the highest price they are ready to pay to own the item. We denote by $\mathcal{X}_i$ the set of all possible values for one item for bidder $i$.  The value vector which contains the values of all the different players is denoted by $x = (x_1,\dots,x_N)$. The \textit{messages} sent to the seller are called \textit{bids}.  We denote by $b = (b_1,\dots,b_N)$ the corresponding bid vector. 
%
%Depending on the information they have on the mechanism and the other bidders, the ultimate goal of the bidders is to maximize their utility 
%$$u_i(x_i, (b_1,...,b_N)) = q_i(b_1,...,b_N)(x_i -p_i(b_1,...,b_N))\;,$$
%and the objective of the seller is to maximize her revenue
%$$\sum_{i=1}^N q_i(b_1,...,b_N)p_i(b_1,...,b_N))\;.$$
%\end{definition2}
\section{The Bayesian setting}
The auction literature has often considered  a Bayesian setting where the value $x_i$ of bidder $i \in \mathcal{N}$ is random, drawn according to the \emph{value distribution} that ``represents the seller assessment of the probability of bidder $i$ having a value estimate of $x_i$ or less''  \citep{Myerson81}. The value distribution quantifies the uncertainty of the seller on the maximum price that one buyer is willing to pay for the item and is represented as a Bayesian prior on the private information of each buyer. 


A widely made assumption is that value distributions are common knowledge among bidders and seller.  As a consequence, we denote by $F_i$ the value distribution - i.e. the cumulative distribution function of the value -  of buyer $i \in \mathcal{N}$ and by $f_i$ its corresponding density function, assuming it exists, an assumption we are going to make repeatedly (removing this assumption is almost always a matter of technicalities and little to no impact on conceptual matters). We implicitly identify the distribution $F_i$ with its cumulative distribution function (cdf) and use both terms exchangeably. We are also going to assume that values $x_i \in {\mathcal X}_i$ are non-negative, i.e. the support of $F_i$ is included in (but not necessarily equal to)  $\mathds{R}_+ = [0,\infty)$. Unless otherwise noted, we assume that $\mathds{E}_{x_i \sim F_i} [x_i] < +\infty$ to get optimality results (and not just $\varepsilon$-optimality). A crucial assumption throughout this survey is that, unless otherwise noted, the values $x_i$ are drawn independently for different $i$'s and hence they are statistically independent as random variables. We shall  denote by $\mathcal{F} = \mathcal{F}^{(n)} =  F_1\otimes \ldots\otimes F_n$ the joint - and hence - product distribution of $x=(x_1,\ldots,x_n)$, the vector of values. 


\medskip

\paragraph{Examples} Typical examples of value distributions are the \emph{uniform} distribution, which is widely used in textbook examples due to its simplicity,  the \emph{exponential} and the \emph{log-normal} distributions as they are similar to some empirical distributions encountered on modern internet platforms. Power law distributions (also known as \emph{Pareto} distributions) are also widely used, as they capture the idea that the value in real time bidding and online advertising comes from few matches of very high quality, such as consumers who recently viewed a product \citep{arnosti2016adverse} (this situation where 20\% of individuals own/generate 80\% of wealth is also referred as the Pareto principle in economics). \emph{Generalized Pareto} distributions are also often used as examples because their virtual value - an important concept we will define later - is linear. 
\begin{definition}[Symmetric setting]
The auction setting will be called \textit{symmetric} if all bidders have the same value distribution.
\end{definition} 

For the sake of clarity, we use pronouns her/she for the seller and he/his for one specific bidder.

\subsubsection*{Assumptions and Notations}
If $v$ is a vector (of scalars or functions) in $\mathbb{R}^n$, we call $v_{-i}$ the vector in $\mathbb{R}^{n-1}$ that contains all entries of $v$ except the $i$-th one, $v_i$. 
In other words, $v_{-i}=(v_1,\ldots,v_{i-1},v_{i+1},\ldots,v_n)$. 

We use the notation $v_{-i}(j)$ to denote the $j$-th entry of $v_{i}$

Similarly, the notation  $F_{-i}$ will denote the product distribution of values of all bidders except $i$ and $b_{-i}$ is the vector of all bids except bidder's $i$. 

\begin{definition2}[Key Default Assumption on distributions]
Unless otherwise noted, we assume that $F_{i}$ is supported on a subset of $[0,b]$, with $b$ being possibly infinite. $F_i$ is assumed to be continuous. We, quite importantly, assume unless otherwise noted that $f_i>0$ on $(0,b)$, except possibly on a set of Lebesgue measure 0. 
\end{definition2}
Note that if ${\cal G}_i$ is the cdf of the largest value of a vector $x_{-i}$ drawn according to $F_{-i}$, ${\cal G}_i(t)=\prod_{j\neq i}F_j(t)$. In particular, with our key default assumption on distributions, ${\cal G}_i$ is differentiable and its density is strictly positive except possibly on a set of measure zero. 

When we say that a function $\beta$ is increasing, we use the standard convention that it means that if $l>u$, $\beta(l)>\beta(u)$. A non-decreasing function is such that if $l>u$, $\beta(l)\geq \beta(u)$.

We use $\partial f$ to denote the subdifferential of a convex function $f$ (see \cite{HULLbook01}, Chapter D). 

\nek{this is ongoing and needs to be completed}

%{\color{red} VP: Je pense qu'il faut elaborer un peu sur le "typical". Ca veut dire quoi exactement ? Soit on met des refs, soit on vire}

%The notion of information owned by the seller and value distribution have progressively changed with several new applications of auction systems. One of the goal of this thesis is to clarify this change and show how sellers and bidders can adapt to this new information structure of the game. For instance, in a repeated setting, where multiple different items are sold successively, the value distribution could also represent the variety of values that a specific buyer can give to one item. 

\subsection{Properties of auction systems}
\label{subsec_prop_auction}
A bidder's \textit{strategy} is the mapping indicating which bids he sends to the seller to buy one specific item, conditional on his private information, a.k.a his value. Stated otherwise, a strategy is a mapping $\beta: \mathcal{X} \rightarrow \mathcal{B}$ that maps private values to bids. %\nek{technical detail: is this mapping possibly random? or is it a function?}

%Bidders have the choice on the bids they send to the seller to get one specific item. A strategy defines how these bids depend on buyer's original private value.
%\begin{definition2}[Strategy]
%A strategy is a function $\beta: \mathcal{X} \rightarrow \mathcal{B}$ that maps private values to bids.
%\end{definition2}

We will denote by $\mathds{B}_i$ the set of all strategies of player $i$, $\beta_i$ the strategy chosen by $i$ and $\beta_{-i}$ the profile of strategies corresponding to all bidders except bidder $i$. Similarly, the notation  $F_{-i}$ will denote the product distribution of values of all bidders except $i$ and $b_{-i}$ is the vector of all bids except bidder's $i$. 

In Bayesian games, it is important to differentiate between \textit{ex ante}, \textit{interim} and \textit{ex post} properties \citep{hartline2013bayesian}. These notions depend on the information available to buyers when they decide to participate in the game and choose their strategy.  
\begin{itemize}
\item For  \emph{ex-ante} properties, bidders do not know yet their own value for the item; i.e. they only know $F_i$ and $F_{-i}$.
\item For \emph{interim} properties, bidders know their valuation but do not know the values of other players, i.e. they know $x_i$ and $F_{-i}$.
\item For \emph{ex-post} properties, bidders know their valuations and the other players', i.e. they know  $x_i$ and $x_{-i}$.
\end{itemize}
In the next sections, we will mostly focus on  interim properties. It is the starting point of most of the auction literature ~: we assume that value distributions are common knowledge and that exact valuations are private information to each bidder.  

We are also assuming that bidders are risk-neutral. In other words, they seek to maximize their expected utility and use utility-maximizing strategies. %over all other bidders' possible valuations and with respect to their strategies\nek{awkward; need to rephrase; need to def for interim and ex-ante. review that.}.  
Stated otherwise, assuming the other bidders are using the strategy $\beta_{-i}$, the  expected utility  of the strategy $\beta_i$  given bidder $i$'s value $x_i$ is denoted by
$$
U_{i}(\beta_i,\beta_{-i},x_i) = \mathds{E}_{x_{-i} \sim F_{-i}}\Big[u_{i}\big((\beta_1(x_1), \dots,\beta_{i-1}(x_{i-1}),\beta_i(x_i),\beta_{i+1}(x_{i+1}),\beta_n(x_n)), x_i\big)\Big]\;.
$$
%\nek{this is awkward as interim doesn't mean we know other people's strategies... and a strategy is a mapping but technically here we just need to know $\beta_i(x_i)$; also if $\beta_i(x_i)$ included in the stuff?}


\textbf{Optimality and characterization of strategies} Maybe one of the most central concept in game theory is \emph{(Bayesian) Nash equilibrium}. It is a characteristic of the vector of strategies $(\beta_1,\ldots,\beta_n)$ and the valuation distributions $F_1,\ldots,F_n$.  At a Bayesian Nash Equilibrium, for any bidder $i$, strategy $\beta_i$ maximizes the expected utility of bidder $i$, given his valuation distribution $F_i$, and given the strategies of his opponents and their valuation distributions, i.e. $\beta_{-i}$ and $F_{-i}$. A stronger concept is that of \emph{weak dominance}.  $\beta_i$ is weakly dominant when it is optimal in terms of expected utility of bidder $i$ against any strategies used in $\beta_{-i}$ and not only ones constituting a Bayesian Nash Equilibrium. The strongest concept is ex-post dominance, where optimality is achieved at any possible profile of valuations.
\begin{definition2}

\textbf{Nash equilibrium} 
A profile of strategies $(\beta_{1},\dots,\beta_{n})$ is \textit{a Bayesian Nash equilibrium} if for all players $i \in \mathcal{N}$, 
\begin{equation*}
\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \quad U_{i}(\beta_i,\beta_{-i},x_i)  \geq U_{i}(\beta,\beta_{-i},x_i) \;.
\end{equation*} 

\noindent \textbf{Weak dominance} A strategy $\beta_i$ is  weakly dominant for player $i \in \mathcal{N}$ if
\begin{equation*}
\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \forall \beta_{-i} \in  \mathds{B}_{-i}, \quad U_{i}(\beta_i,\beta_{-i},x_i)  \geq U_{i}(\beta,\beta_{-i},x_i) \;.
\end{equation*}

\noindent \textbf{Ex-Post Weak dominance} A strategy $\beta_i$ is  ex-post weakly dominant for player $i \in \mathcal{N}$ if
\begin{equation*}
%\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \forall \beta_{-i} \in  \mathds{B}_{-i}, \forall x_{-i} \in \mathcal{X}^{N-1},\quad u_{i}((\beta_1(x_1),\dots,\beta_i(x_i),\dots,\beta_N(x_N)),x_i)  \geq u_{i}((\beta_1(x_1),\dots,\beta(x_i),\dots,\beta_N(x_N)),x_i) \;.
\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \forall \beta_{-i} \in  \mathds{B}_{-i}, \forall x_{-i} \in \mathcal{X}^{N-1},\quad u_{i}((\beta_i(x_i),\beta_{-i}(x_{-i})),x_i)  \geq u_{i}((\beta(x_i),\beta_{-i}(x_{-i})),x_i) \;.
\end{equation*}
\end{definition2}

%
%
%A strategy which is optimising the expected utility of one bidder for any valuation and for any strategies of the other bidders is said dominant. 
%\begin{definition2}[(Weakly) dominant strategy]
%A strategy $\beta^{*}$ is  ex-post weakly dominant for player $i$ if for all $\beta_{-i} \in  \mathds{B}^{N-1}$, for all $\beta \in \mathds{B}$ and for all $x \in X^{N}$:
%
%\end{definition2}

\nek{Maybe say that this is all formulated in interim} Those properties of strategies are classical concepts in game theory. On the other hand, it is also possible to introduce and study different properties of mechanisms. Some of them require the concept of \emph{``truthful bidding''} which correspond to the specific strategy $\beta_i(x)= x$. We will denote by $\beta_{tr}$ this truthful strategy.


\textbf{Characterization of mechanisms}
\begin{definition2} A mechanism is
\begin{description}
\item[(BIC)] Bayesian Incentive-Compatible:  if all bidders bidding truthfully is a Bayesian Nash equilibrium.
\item[(DSIC)] Dominant Strategy Incentive-Compatible:  if bidding truthfully is a weakly dominant strategy for all bidders.
\item[(Standard)] if it allocates the item to the buyer with the highest bid.
\item[(Efficient)] if it allocates the item to the buyer with the highest valuation (at least for some equilibrium).
\item[(IR)]  interim Individually-Rational: if 
\begin{equation*}
\forall \, i \; \forall x_i \in \mathcal{X}_i, \quad U_{i}((\beta_i=\beta_{tr}, \beta_{-i}=\beta_{tr}),x_i) \geq 0\;.
 \end{equation*}
 and ex-post Individually-Rational: if 
 \begin{equation*}
 \forall x_i \in \mathcal{X}_i,  \forall x_{-i} \in \mathcal{X}_{-i}, \quad u_{i}\big((x_i, x_{-i}), x_i\big) \geq 0\;.
\end{equation*}
\end{description}
\end{definition2}

A DSIC mechanism is obviously a BIC mechanism. More generally,  Incentive Compatible (IC) auctions have the nice property of being ``simple'' for the buyers from a strategic standpoint:  bidding their (known in the interim setting) valuation is optimal for them. Notice  that this unfortunately does not ensure the uniqueness of the equilibrium where each bidder bids truthfully (we will call this equilibrium the  \textsl{truthful equilibrium}). See Section \ref{sec:NashIsDifficult} for more details. \nek{move that to section \ref{sec:NashIsDifficult}} Indeed, there exist many other equilibria such as the following one: every bidder always bids 0 except one of them bidding arbitrarily high\nek{this is unclear; this is really an example with unif[0,1], one bids zero one bids one. given the strategy of the other, second price is dsic. but obviously non-uniqueness of equilibrium.Probably give this example later after intro 2nd price; and point to it now}. Those are pathological equilibria and will be discarded in the following. As we will see later on, being DSIC is one of the main reasons explaining the tremendous success of second-price auctions in practice. Another reason is that if bidders are bidding truthfully, then the seller can, in a first step, elicit their value distributions through a DSIC mechanism and then  move to another  mechanism that maximizes her revenue (this is detailed in Section \ref{Section:RevenueMax}).

% - even if it is at the cost of efficiency\nek{efficiency as in what?}.


 
\medskip
Finally, before presenting and analyzing two classical types of auction, we indicate that individual rationality simply ensures that bidders have an interest in taking part in these auctions.

\section{Sealed-bid auctions}
In a sealed-bid auction bidders privately send their bid to the seller. We present below two of the most well-known sealed-bid auctions, the second-price and the first-price auctions. This class of auctions does not include the well-known - in popular culture -  ascending auction, a.k.a English auction, where bidders can observe bids from other bidders and progressively choose to increase their bids until only one bidder remains. On the other hand,  if bidders' valuations are independent, there exists a strategic-equivalence between the ascending auction and a classical sealed-bid auction which is called the \emph{second-price auction}. % \nek{cut remaining, introduced below along with another classical sealed bid auction, the \emph{first-price auction}}. \nek{Dutch or English auction? look in krishna and specify; one is ascending the other descending}
\subsection{The sealed-bid second-price auction}
The second-price auction allocates the item to the highest bidder who pays the highest bid among other bidders, i.e. the second highest bid. A key property of this auction is the following result \citep{vickrey1961counterspeculation}, which does not require any assumption on bidders' value distributions. 

\begin{theorem2}
The second-price auction is DSIC. In other words, bidding truthfully is weakly dominant. 
\end{theorem2}
\begin{proof}
Let us denote by $x_i$ the private value of bidder $i$ and by $b^*_{-i}$ the highest bid of the competition. We are going to compare the utility of bidding  $b$ instead of $x_i$.
\begin{itemize}
\item Case $b > x_i$. The only case where his (ex-post) utility is changed is when $x_i < b^*_{-i} < b$. With a bid $b$, he now wins the auction but his utility is negative since $x_i - b^*_{-i} < 0 $.
\item  Case $b < x_i$. The only case where his (ex-post) utility is changed is when $x_i > b^*_{-i} > b$. With a bid $b$, he now loses a profitable  (i.e. with a positive utility) auction.
\end{itemize}
Hence, bidder $i$ has no incentive to deviate  from truthful bidding. 
\end{proof}
The classical second-price auction was used until recently \citep{feng2020reserve} by most of the biggest online platforms to sell ad placements on publishers' websites. Another widely used and studied sealed-bid auction is the first-price auction.
\subsection{The sealed-bid first-price auction} 
\label{first-price-auction}
The first-price auction allocates the item to the highest bidder who pays his own bid.

\medskip

Before studying Nash equilibria of symmetric first-price auction, we derive the general best reply of player $i$ to the bid distribution of the competition, specifically the distribution of the maximum bid of the competition. This result is of increasing interest to practitioners as many online auctions are now first price auctions.

\begin{proposition2}\label{Prop:BestReply1st}
	Call $G_i$ the cdf of the highest bid of the competition of bidder $i$, i.e. $\max_{j\neq i} b_j$. 
In a sealed-bid first price auction, a best response of bidder $i$  to $G_i$ is 
\begin{equation*}\label{eq:bestresponsefirstpriceSemiAbstract}
\beta(x_i):  \beta(x_i)=b(x_i) \text{ where } b(x_i)\in \argmax_{b \in \mathbb{R}} G_i(b)(x_i-b)\;.	
\end{equation*}
When $G_i$ is log-concave and $G_i(x_i)>0$, the best response is unique. 

Suppose further that $G_i$ has a pdf $g_i$. Call $a_i=\max_{t \in \mathbb{R}}\{t: G_i(t)=0\}$ 
First order conditions, also give, if $G_i(x_i)>0$, 
\begin{equation*} \label{eq:bestresponsefirstprice}
\beta_i(x_i)=b(x_i), \text{ where } b \text{ is a solution of } b + \frac{G_{i}(b)}{g_{i}(b)}= x_i \text{ on } [a_i,x_i]\,.
\end{equation*}
If $G_i(x_i)=0$ a best response is $\beta_i(x_i)=x_i$.

 \end{proposition2}
Calling $Y_{-i}$ a random variable with cdf $G_i$, it can also be shown that under mild technical conditions that $\beta_i$ is increasing and satisfies the equation $\beta_i(x)=\Exp{\beta_i^{-1}(Y_{-i})|Y_{-i}\leq \beta_i(x)}$. We also have the following interesting corollary.

\begin{corollary2}\label{coro:1stPriceNotBIC}
Proposition \ref{Prop:BestReply1st} implies that the first price auction is in general not BIC.	
\end{corollary2}
The corollary follows by simply showing that the best response of bidder $i$ when all other bidders bid truthfully (and hence the top bid of the competition is the largest value of the other bidders) consists in bidding something else than $x_i$. If $G_i(x_i)>0$ it follows immediately than they are better strategies than bidding $b_i=x_i$~: for instance, take any $\tilde{b}_i$ such that $G_i(\tilde{b}_i)=G_i(x_i)/2$ ($\tilde{b}_i$ exists by continuity of $G_i$ and $G_i(a_i)=0$). The utility of bidder $i$ is strictly positive at $\tilde{b}_i$ and is 0 at $x_i$. 
\begin{proof}
Let us denote by $B_{-i}$ the random variable corresponding to the maximum bid of the competition of bidder $i$, so that its cdf and pdf are $G_i$ and $g_i$. Note that $a_i$ is a max as $G_i$ is continuous and non-decreasing. 

When bidder $i$ has private value is $x_i$ and bids $b_i$, the utility he derives from the auction is $u_i(b_i,x_i)=(x_i-b_i)\mathds{1}\{b_i>B_{-i}\}$; in other words, it is his value minus his cost when he wins the auction and zero otherwise. 

We denote by $\mathcal{U}_i(b_i,x_{i}):\mathds{R}^{+}\times\mathds{R}^{+}\rightarrow \mathds{R}$ the associated expected utility of bidder $i$ when his private value is $x_i$ and he bids $b_i$. We have 
$$
\mathcal{U}_i(b_i,x_i) = \mathds{E}_{B_{-i}}\Big[(x_i-b_i)\mathds{1}\{b_i>B_{-i}\}\Big] = G_i(b_i)(x_i-b_i)\;.
$$
A best response is therefore any $b(x_i)\in \argmax_{b\in \mathds{R}^+}G_i(b)(x_i-b)$. Note that when $G_i$ is log-concave and $G_i(x_i)>0$, we can verify by inspection that $\mathcal{U}_i(b_i,x_i)$ is strictly log-concave in $b_i$ on $[a_i,x_i]$  and therefore it has a unique maximum on this interval \citep{boydvandenberghe04}. (This property follows also immediately from the definition of a strictly concave function.)

Note that since $G_i$ has a pdf, it is continuous and differentiable and therefore so is $\mathcal{U}_i(b_i,x_i)$ as a function of $b_i$. 
The derivative with respect to $b_i$ is then equal to 
$$
\frac{\partial \mathcal{U}_i}{\partial b_i}(b_i,x_i) = g_i(b_i)(x_i-b_i) - G_i(b_i).
$$
Let us assume that $G_i(x_i) >0$, then $\mathcal{U}_i(x_i,x_i)=0$ but $\left.\frac{\partial \mathcal{U}_i(b_i,x_i)}{\partial b_i}\right|_{b=x_i} <0$. This first implies by continuity that there exists  bids where the utility is positive. Rolle's theorem applied to $t\mapsto G_i(t)(x_i-t)$ also gives the existence of a stationary point $b_i^* \in  [a_i,x_i]$ where  $\frac{\partial \mathcal{U}_i}{\partial b_i}(b^*_i,x_i) =0$, as $\mathcal{U}_i(a_i,x_i)=0$, too. Note that $ \mathcal{U}_i(b_i,x_i)\geq 0$ on $[a_i,x_i]$.
Since our argument above shows that $\mathcal{U}_i(b_i,x_i)$ is positive in a neighborhood of $x_i$, we can assume that $b_i^*$ is chosen so that $\mathcal{U}_i(b_i^*,x_i)>0$. If $g_i(b^*_i)=0$ then necessarily $G_i(b^*_i)$ is also equal to 0 and $\mathcal{U}_i(b_i^*,x_i)$ would be equal to 0. This contradicts the fact that $b^*_i$ maximizes the utility, as we have shown that there exists points of positive utility.

The case where $G_i(x_i)=0$ is trivial as bidder $i$ cannot have a positive utility (recall that $G_i$ is a non-decreasing and non-negative function, so $0\leq G_i(b_i)\leq G_i(x_i)$ if $b_i\leq x_i$). Bidding $x_i$ is then optimal.
\end{proof}


There is a very rich line of work focusing on deriving Nash equilibria in first-price auctions when bidders have different value distributions. This involves solving complex systems of coupled first-order differential equations (at least with continuous value distributions, see \cite{krishna2009auction}, Section 4.3; see also p. \pageref{thm:SystemEquiAsymetricFirstPrice}). On the other hand, with symmetric bidders, i.e. with identical value distributions, it is possible to solve explicitly this system of equations and to derive the unique symmetric  Nash equilibrium with increasing strategy. From now on, we will call an Nash equilibrium  \emph{increasing} if the  strategies  are all increasing mappings. 
\begin{theorem2}%[Nash equilibrium in a first-price auction]
We assume that $n$ bidders are symmetric, independent and have a differentiable cdf, $F$, whose pdf $f$ is such that $f(x)>0$ except possibly on a set of Lebesgue measure 0 within the support of $F$. Then there exists a symmetric increasing Nash-equilibrium whose strategy is described by:  
\begin{equation*}
\beta(x) = \mathds{E}[X^{(1)}_{-i} | X^{(1)}_{-i} < x]\;.
\end{equation*}
where $X^{(1)}_{-i}$ the highest value among bidders except bidder $i$.
\end{theorem2}
% \nek{tech question: if we assume $f>0$ then $\beta$ is increasing and we have zero problems below. If $f\geq 0$, $\beta$ is only non-decreasing; then we have to deal with possible ties, how to break them and make sure that the PWin is $G_i(x)$. when they all bid $\beta(x_j)$ I haven't done this. this minor tech stuff would preferably done in an appendix; probably need to replace $x_j$ by $x_j^-$, i.e. the $inf_x F(x)=t$. I leave the proof with non-decreasing but worth a check}.
\textbf{Interpretation~:} the bidding strategy can be interpreted as saying that bidder $i$ should be bidding the expectation of the largest value of the competition, conditional on the fact that this value is smaller than bidder $i$'s value. 

\textbf{Technical note~:} We note that this bidding strategy can be derived from the proof of the revenue-equivalence Theorem \ref{Th:RevEquivalence}, and specifically the expected payment formula. This is another common method for finding equilibrium bidding strategies. We chose the proof presented below as we think it leads more directly to the solution.  
\begin{proof}
We assume that $n\geq 2$ otherwise there is nothing to show. Let us assume that all bidders are using the function $\beta$ described above. As we will show below, this function is increasing on the support of $F$ under our assumptions. Note furthermore that when all bidders are using the same \emph{increasing} strategy on the union of the support of their value distributions, the probability that bidder $i$ wins the auction is the same as the probability that he has the highest value. (Note that this latter statement would not always be true if the strategy were only non-decreasing.) 

Note furthermore that elementary properties of conditional expectations give, if $G_i$ and $g_i$ are the cdf and pdf of $X_{-i}^{(1)}$,
$$
\beta(x)=\beta_i(x)=\frac{\int_{0}^{x} y g_i(y) dy}{G_i(x)}=x-\frac{\int_0^x G_i(u)du}{G_i(x)}\;, \text{ whenever } G_i(x)>0\;.
$$
Under our assumptions, $G_i=F^{n-1}$ and hence $g_i(x)=(n-1)f(x)F^{n-2}(x)$. Note that under our assumptions $g_i(x)>0$ on the support of $F$ except possibly on a set of Lebesgue measure 0.  $\beta'(x)=\frac{g_i(x)\int_0^x G_i(u)du}{[G_i(x)]^2}$. Hence, restricted to the support of $F$, $\beta$ is a non-decreasing function whose derivative is 0 on a set of Lebesgue measure 0 . We conclude that $\beta$ is actually increasing on the support of $F$ under our assumptions. 

We denote by $x_i$ the private value of bidder $i$, by $b_i$ his bid and by $H$ the supremum of the support of $F$. Bidder $i$ has no incentive to bid higher than $\beta(H)$~: suppose he did bid $b>\beta(H)$. Clearly since the other bidders bid according to $\beta$, their maximum bid is lower than $\beta(H)$. Then, bidding $b$, bidder $i$'s probability of winning the auction would be 1 and his cost $x-b$. He could achieve the same probability of winning by bidding $\beta(H)$ - here we use the fact that $F_i$ is continuous for all $i$ so there are no point masses at $H$ - but his cost would be lower~: $x-\beta(H)$. Then, any other bid $b$ will satisfy $b \in [0,\beta(H)]$ and since $\beta(0) =0$ and $\beta$ continuous (because $F$ is and because of properties of conditional expectation), there exists $z \in [0,H]$ such that $b = \beta(z)$. Finally, note that the probability that bidder $i$ wins the auction when bidding $\beta(z)$ is just $G_i(z)$, since $\beta$ is increasing on the support of $F$. Therefore,
\begin{align*}
\mathcal{U}_i(\beta(x),x) - \mathcal{U}_i(b,x) &= \mathcal{U}_i(\beta(x),x) - \mathcal{U}_i(\beta(z),x)
\\&= G_i(x)\left(x - \frac{\int_{0}^{x} y g_i(y) dy}{G_i(x)}\right) - G_i(z)\left(x - \frac{\int_{0}^{z} y g_i(y) dy}{G_i(z)}\right)
\\&= x(G_i(x) - G_i(z)) + \int_{x}^{z} y g_i(y) dy = 
\int_x^z(y-x)g_i(y)dy 
\geq 0\;.
\end{align*}
This shows that the best response that bidder $i$ can use is $\beta$. Therefore, $(\beta,\dots,\beta)$ is a symmetric (increasing) Nash equilibrium.   We will prove unicity of this increasing differentiable symmetric Nash equilibrium in symmetric first-price auctions in Section \ref{sec_rev_equi}. 
\end{proof}

Unlike second-price auctions, first price auctions are not incentive compatible (see e.g. Corollary \ref{coro:1stPriceNotBIC}). As a consequence, the strategy of a bidder at an equilibrium  depends on the bidding strategy of the other bidders, and ultimately on other bidders' valuation distributions (see Proposition \ref{Prop:BestReply1st}). So in practice, computing a good or optimal bidding strategy would require estimating the distribution of the highest bid of the competition, which can be very challenging. Nevertheless, because of their relative transparency for bidders (who know ahead of time what they might pay if they win), first-price auctions are increasingly used in online advertising auctions\nek{Thomas: tu peux mettre une ref \`a Lahaie ou Feng?}. However, optimal bidding becomes much more complex for bidders than it is in second price or other BIC/DSIC/``truthful'' auctions.
\paragraph{Nash equilibrium in the asymmetric case}

Asymmetric first price auctions are much more intricate than symmetric ones as  the equilibrium strategy of each  bidder depends in a very subtle manner of the other bidders' strategies  \citep{LebrunFirstPriceAsymmetric1999}. Indeed, let us assume that the distributions $F_1,\ldots,F_n$ are supported on $[h,H]$, have a density  bounded away from 0 on $(h,H)$ and possibly have a point mass  at $h$. 
%This assumption comes from practical  -- as many auctions have 0 value to online advertisers -- and technical -- if a common reserve price is set at $r>h$, then distributions can be assumed to be  supported on $[r,H]$ with a point mass at $r$  \citep{LebrunFirstPriceAsymmetric1999}. 
\begin{theorem2}[\citep{LebrunFirstPriceAsymmetric1999}]\label{thm:SystemEquiAsymetricFirstPrice}
Under these  assumptions, there exist deterministic Nash equilibrium strategies that are increasing. Let us denote them by $\beta_i$ and by $x_i(b)=\beta_i^{-1}(b)\geq b$ their inverse, i.e. the value inducing the bid $b$. Then the increasing functions $b\rightarrow x_i(b)$ solve  the system of differential equations : 
\begin{equation}\label{eq:equilibrium1stPriceAsymmetric}
\forall \, i \;, 1\leq i \leq n\;, \frac{\partial}{\partial b}\log(F_i(x_i(b)))=\frac{-1}{x_i(b)-b}+\frac{1}{n-1}\sum_{j=1}^n \frac{1}{x_j(b)-b}\;. 
\end{equation}	
When the distributions are without atoms, the boundary conditions are 
$x_i(h)=h$ for all $i \in \mathcal{N}$, and there exists $\eta>0$ such that for all $i$, $\beta_i(H)=\eta$. 
\end{theorem2}
The boundary conditions mean that bidders bid their value at $h$ and have a common maximal bid \citep{FibichGaviousAsymmetricFirstPricePerturbApproach2003}.
\paragraph{Numerical issues in computing Nash equilibrium}
Finding the solution to the differential system \eqref{eq:equilibrium1stPriceAsymmetric} is considered hard essentially because the solutions are unstable near the boundary \citep{MarshallNumericalAnalysis1stPrice94}. The case of $n=2$ bidders has received a fair amount of attention both from both theoretical and numerical perspectives \citep{FibichGaviousDynamicalSystem2012}. Another approach finds yet another form of the differential system of equations and expands the functions appearing in it in a fixed polynomial basis.  \citep{NumericalSolutionsFirstPriceGayle2008}. 
\section{A revenue equivalence theorem}
\label{sec_rev_equi}
Revenue equivalence theorems are general results showing that different auction systems  -- sharing nonetheless some properties -- are equivalent in terms of expected revenue \emph{at a specific equilibrium}.  The first revenue equivalence theorem showed that the sealed-bid second-price auction and the ascending/English auction lead to the same revenue for the seller \citep{vickrey1961counterspeculation}. This result was later extended to all standard auctions - under rather minimal assumptions. 



\begin{theorem2}%[Revenue equivalence]
\label{Th:RevEquivalence}
Consider the family of auctions that are both

 i) \textsl{standard} (i.e. the winner is the bidder with the highest bid)

 ii) \textsl{0-rational} (i.e. winning the auction with a bid of 0 induces a payment of 0).

\noindent When all bidders have the same value distribution and their bids are statistically independent, i.e. in the symmetric case, the seller's expected revenue and bidders' expected utilities at a symmetric increasing Nash equilibrium are independent of the  specific payment rule. 
\end{theorem2}
\begin{remark2} The revenue equivalence Theorem \ref{Th:RevEquivalence} applies in particular to first and second price auctions, in the symmetric case where all bidders have the same value distribution \citep{Myerson81} and use an increasing strategy at equilibrium. The revenue equivalence theorem assumes that bidders have all the same value distributions. There exists asymmetric cases where the first-price auction brings more revenue than the second-price auction and vice-versa (\cite{krishna2009auction}, Section 4.3.2). 
\end{remark2}
\begin{proof} 
Given a specific standard auction, let $\beta$  be a  strategy at an increasing symmetric Nash equilibrium. Let us denote by $P(t)$ the corresponding expected payment of player $i$ when he bids $\beta(t)$ and the other bidders are using the same strategy $\beta$. As before, we  denote by $G_i$ the distribution of $X^{(1)}_{-i}$, the highest value among all the bidders except bidder $i$. Using the fact that $\beta$ is increasing, that all players use this strategy - we are at a Nash equilibrium -  and the fact that the auction is standard, the probability that bidder $i$ wins when he bids $\beta(t)$ is $G_i(t)$.

We can still assume that a deviation of bidder $i$ consists in  bidding $\beta(z)$ instead of $\beta(x_i)$ (because the auction is standard and $\beta$ is increasing).  In particular, the expected utility for bidder $i$ of this deviation can be written as
\begin{align*}
\mathcal{U}_i(z,x_i) = x_iG_{i}(z) - P_i(z)\;.
\end{align*}
% If $p_i(t,x_{-i})$ is the payment of bidder $i$ when bidding $\beta(t)$ and the other players have value $x_{-i}$,
% $$P_{i}(t) =  \mathds{E}_{F_{-i}}\Big[p_i(t_i,x_{-i})\Big] = \int_{\mathcal{X}_{-i}} p_i(t,x_{-i})f_{-i}(x_{-i})dx_{-i} \;.$$

Since $\beta$ is a strategy corresponding to a Nash equilibrium, bidder $i$'s expected utility is maximized when he bids $\beta(x_i)$ and hence 
$$
\mathcal{U}_i(x_i,x_i) =\max_{z} \mathcal{U}_i(z,x_i) =\max_{z}  \, x_iG_i(z) - P_i(z)  \;.
$$
We denote ${\mathcal V}(x_i)=\mathcal{U}_i(x_i,x_i)$. 
Clearly $x_i \mapsto \mathcal{V}_i(x_i)$ is convex - as a max of linear and hence convex functions - and hence almost everywhere differentiable \citep{HULLbook01}, p. 115). Recall also that (Lemma 4.4.1 in \citep{HULLbook01}, p. 188) the subdifferential at a point $x$ of a supremum of convex functions contains the convex hull of the subdifferentials of the functions achieving this supremum (and is empty if the supremum is not achieved). Here the functions we consider have a very simple differential in $x$: it is simply $G_i(z)$. This suggests informally that when $\mathcal{V}$ is differentiable, ``${\mathcal V}'(x)=G_i(z^*(x))$", where $z^*(x)=\argmax_z \mathcal{U}_i(z,x)$. In particular in our case it suggests that ``${\mathcal V}'(x)=G_i(x)$". The envelope theorem allows us to make this intuition formal. 

The envelope Theorem in its Theorem 2 form in \citep{MilgromSegal2002} applies because $\mathcal{U}_i(z,\cdot)$ is linear for all $z$ and hence differentiable and therefore absolutely continuous. Furthermore $\frac{\partial \mathcal{U}_i(z,x)}{\partial x} =G_i(z)\in[0,1]$ for all $z$. Since the max of $z\mapsto \mathcal{U}_i(z,x_i)$ is attained for $z=x_i$ because we are at a Nash equilibrium, the envelope theorem then gives 
$$
{\mathcal V}(x)-{\mathcal V}(0)=\int_0^{x}G_i(u)du\;.
$$
However, almost by definition, ${\mathcal V}(x)-{\mathcal V}(0)=xG_i(x)-P_i(x)+P_i(0)$. 
Thus, since $P_i(0)=0$ because of 0-rationality, we finally get that
$$
P_i(x)=P_i(0)+xG_i(x)-\int_0^x G_i(u)du = \int_0^x tdG_i(t) dt=G_i(x)\mathds{E}[X^{(1)}_{-i}|X^{(1)}_{-i} < x]\;.
$$
Note that the second equality comes from integration by parts. 
\iffalse
\nek{I changed the argument to above}
Assuming differentiability, it  holds that, since $\mathcal{U}_i(z,x_i)$ attains its maximum at $x_i$, 
\begin{equation*}
\left.\frac{\partial \mathcal{U}_i}{\partial z} (\cdot,x_i)\right|_{z=x_i} = x_ig_i(x_i) - P_i'(x_i) = 0\;.  
\end{equation*}
Thus, since $P_i(0)=0$ because of 0-rationality, we finally get that
\begin{equation*}
P_i(x) = P_i(0) + \int_{0}^{x} sg_i(s)ds = G_i(x)\mathds{E}[X^{(1)}_{-i}|X^{(1)}_{-i} < x]\;.
\end{equation*}
In the case where $\mathcal{U}_i$ is not everywhere differentiable, the same argument holds using standard mean-value theorems for the subdifferential \citep{HULLbook01}, pp.178-180. \nek{check with Thomas, Vianney, Clem} \nek{note to thomas: there's a slight confusion around the function of the first variable and the function $\gamma(x_i)=\mathcal{U}_i(x_i,x_i)$}
\nek{keep below}
\fi
Hence the expected payment of bidder $i$ is independent of the specific auction format. As a consequence, so are  the expected seller's revenue and the expected utility of bidder $i$, because the auction is standard.
\iffalse
Finally, we assumed in the proof that $P$ is  differentiable (for the sake of simplifying the exposition). This assumption is not necessary and can be removed using the convexity of $x_i \mapsto \mathcal{U}_i(x_i,x_i)$ in a way that is similar to the proof of the more general Theorem \ref{Th:MyersonLemma}. \nek{je pense qu'il faut faire très gaffe; l'exemple d'Hartline a un payoff discontinu (a l'equilibre je sais pas parce que son contre example est faux)}
\fi

\textbf{Remark:} a more informal but perhaps more intuitive derivation of this result is the following. Assuming differentiability of $P_i(z)$ and $G_i(z)$, it holds that, since $\mathcal{U}_i(z,x_i)$ attains its maximum at $x_i$, 
\begin{equation*}
\left.\frac{\partial \mathcal{U}_i}{\partial z} (\cdot,x_i)\right|_{z=x_i} = x_ig_i(x_i) - P_i'(x_i) = 0\;.  
\end{equation*}
Thus, since $P_i(0)=0$ because of 0-rationality, we get 
\begin{equation*}
P_i(x) = P_i(0) + \int_{0}^{x} sg_i(s)ds = G_i(x)\mathds{E}[X^{(1)}_{-i}|X^{(1)}_{-i} < x]\;.
\end{equation*}
\end{proof}

\begin{remark2} This proof shows a principled way to get necessary conditions on bidding strategies forming an increasing Nash equilibrium, through the payment formula derived above.  \end{remark2}

\subsubsection{Informal derivation of symmetric first-price auction equilibrium strategy} Denote by $\beta$ the common strategy of an increasing Nash equilibrium of the first-price auction, postulated at this point for this informal derivation to exist. Note that by symmetry, we have $G_j=G_i=G$ for all $i,j$ and similarly for the pdfs. So we use the notations $G$ and $g$ for cdf and pdf below. Conducting the same computations as in the proof of Theorem \ref{Th:RevEquivalence}, assume that all bidders  but $i$  follow $\beta$ and that bidder $i$ is bidding $\beta(z)$ instead of $\beta(x_i)$. Then his utility rewrites in the specific case of first price auction as 
\begin{equation*}
\mathcal{U}_i(\beta(z),x_i) = (x_i - \beta(z))G(z)\;. 
\end{equation*}
$\beta$  is a  symmetric increasing Nash equilibrium, and hence the maximum utility is attained by bidding $b=\beta(x_i)$. Differentiating with respect to $z$, temporarily assuming that $\beta$ is differentiable, then yields 
\begin{equation*}
0=\left.\frac{\partial \mathcal{U}_i}{\partial z} (\beta(z),x_i)\right|_{z=x_i} = (x_i-\beta(x_i))g(x_i) - \beta'(x_i)G(x_i)\;.
\end{equation*}
Notice that the above equation can be rewritten in the more compact form
\begin{equation*}
(\beta(x)G(x))' = xg(x)\;.
\end{equation*}
Integrating the above equation and using the fact that $G(0)=0$, we can compute explicitly the symmetric equilibrium strategy
\begin{equation*}
\beta(x) = \frac{\int_{s=0}^{x}sg(s)ds}{G(x)}= \mathds{E}[X^{(1)}_{-1}|X^{(1)}_{-1}<x]\;.
\end{equation*}
We can verify as posteriori that $\beta$ is differentiable and increasing when $g>0$. 

This also proves the uniqueness of  increasing differentiable Nash equilibria  in a symmetric first-price auction. 



% \begin{remark2} The system of equations corresponding to the Nash Equilibrium in the asymmetric setting presented in Theorem \ref{thm:SystemEquiAsymetricFirstPrice} can actually be easily deduced by applying the same perturbative approach.\nek{this is very unclear; we should drop it I think or do it} \end{remark2}

\section{Deriving revenue-maximizing auctions}
\label{Section:RevenueMax}
We now focus on how the seller can design her auction system to maximize her revenue. A large part of the recent literature on auctions have focused on this objective since most of the auctioneers have a choice in designing the rules of their respective auction platforms.

To compute the optimal revenue-maximizing auction, we assume that the seller has prior knowledge on the distribution $F_i$ on each bidders' valuations.  These value distributions quantify the information that the seller has on each bidder. 

\subsection{The role of reserve prices}
Setting reserve prices is a crucial tool used to improve or maximize seller's revenue in classical auctions. To illustrate its role, we focus on  second-price auctions. 
\begin{definition2}
The reserve price is the minimum price a bidder must pay to acquire an  item. The reserve price is  \textit{anonymous} (respectively \emph{personalized}) if it is the same for all bidders (if it is different from one bidder to the other).
\end{definition2}
In a second-price auction with reserve prices the buyer that wins the auction must have bid above his reserve price. He then pays the maximum between his reserve price and the second highest bid. A crucial and perhaps surprising point  is that, in expectation,  it can be beneficial for the seller to sometimes not allocate the item. However, whenever the item is sold, the payment is higher because of the reserve price than it would have been without reserve price. 

To illustrate this point, we quickly recall a historical example, the New-Zealand radio spectrum rights auction \citep{milgrom2004putting}. In 1990, the NZ government decided to sell some radio spectrum rights through multiple simultaneous sealed-bid second-price auctions without reserve prices for the corresponding licenses. These auctions were expected to raise around NZ\$250 million. Instead, the government revenue was around NZ\$36 million. On many licenses, there was a huge discrepancy between the first and the second bid. For instance, a firm bid NZ\$100 000 and the second price was only NZ\$36\dots If reserve prices had been set beforehand, it would have ensured to the government that the firm who made a bid of NZ\$100 000 would have paid a price sufficiently high. 

This example illustrates the importance of reserve prices. A first way to set a reserve price would be to assume that the seller can compute an intrinsic value for keeping the item. This could be a reasonable assumption for housing or wine auctions. However, in many other situations (TV rights, radio spectrum rights auctions..), the seller does not have any intrinsic value for the item. To give an example, we compute the optimal reserve price in the simple case of a single buyer. As before, we denote by $F$ the cdf of the buyer valuation, and for the sake of simplicity, we assume it has a density $f$ (again, all the following results generalize to arbitrary distributions, but at the cost of technicalities) and has finite expectation.


%\iffalse and the need for a careful modelisation of the different incentives of the system. {\color{red}VP: la phrase suivante est moche, et il faut une reference et/ou plus d'explications} For instance, in the recent sell of French football TV rights, in 2017, the auctioneer was very careful on its definition of the reserve prices by setting very specific reserve prices for every TV rights packages. 
%\fi
\subsection{The posted price setting: monopoly pricing}
\label{monopoly-pricing}
In this  particularly simple through practically very common setting, designing an auction simply reduces to  a \textit{take-it-or-leave-it} offer. In other words, a fixed selling price is offered and a rational bidder will accept to pay it to acquire the item if and only if the price is smaller than his valuation. 
\begin{lemma2}\label{TH:Monopoly}
In a posted price setting, the seller's expected revenue is 
\begin{equation} \label{eq:defPiOfr}
\Pi(r) = r(1-F(r))\;.
\end{equation}
In the same setting, when $F$ is differentiable and has one moment/finite expectation, the optimal reserve price, called \emph{the monopoly price}, is a solution of :
\begin{equation*}
0=-[r(1-F(r))]'=rf(r) - (1-F(r)) = f(r)\Big(r- \frac{1-F(r)}{f(r)}\Big)\;. 
\end{equation*}
\end{lemma2}
\begin{proof}
The seller's revenue can be written as a function of $r$ as: in expectation, the seller's revenue is just the fixed price $r$ multiplied by the probability that the buyer buys the item. This latter probability is just the probability that the value of the buyer is above $r$. Formally, if $x$ is the value of the item for the buyer, the revenue of the seller $\Pi(r)$ when selling at the fixed price $r$ is 
\begin{equation*} 
\Pi(r) = r P(x\geq r)=r \int_{r}^{+\infty} f(x)dx = r(1-F(r))\;.
\end{equation*}
The result on the monopoly price follows from differentiating the previous relation, since
\begin{equation*} 
\frac{d\Pi(r)}{dr} = (1-F(r)) - rf(r) \;.
\end{equation*}
Furthermore choosing $r=0$ or $r$ arbitrarily high gives 0 revenue, the latter because $F$ is assumed to have one moment, which then implies that $\lim_{t\tendsto \infty} t(1-F(t))=0$ by the dominated convergence theorem. Indeed, if $x$ has distribution $F$, $t(1-F(t))\leq \mathds{E}_{x\sim F}[x\indicator{x\geq t}]\leq \mathds{E}_{x\sim F}[x]<\infty$.  Hence a maximum of the function $\Pi$ exists among its stationary points, finishing the proof. 
\end{proof}
%\iffalse
%\begin{figure}[H]
%\includegraphics[width=.5\linewidth]{images/monopolistic_revenue}
%\caption{Seller's revenue as a function of the reserve price. The revenue is computed based on $r(1-F(r))$ with $F = \mathcal{U}([0,1])$.}
%\end{figure}
%{\color{red} VP: Quel est l'interet du paragraphe suivant ?} 
%The setting of posted price is very related to the setting where a monopolistic firm sells a service to different customers. She must define a single price for all her clients. She will choose the monopoly price corresponding to the distribution of values representing her customers. Sometimes, the firm prefers not to sell the item and sacrifies a bit of short-term revenue to insure that in most other cases, buyers will pay a price sufficiently high.  
%\fi
\bigskip
Notice that without the assumption that $F$ has a finite expectation, the optimal reserve price could be arbitrarily high: take for instance $F(r)=1-r^{-\alpha}$ with $0<\alpha<1$.
Such an example is relevant in markets for luxury items.
 
One of the purpose of discussing the single bidder case was to introduce organically the crucial concept of \textit{virtual value} introduced in \citep{Myerson81}. 
\begin{definition2}%[Virtual value]
The virtual value function $\psi : \mathcal{X} \to \mathds{R}$ of a distribution $F$ (with pdf $f$) is: 
\begin{equation} \label{eq:defVirtualValue}
\boxed{
\psi(x) = \psi_F(x) = x - \frac{1-F(x)}{f(x)}\;.
}
\end{equation}
\end{definition2}
The virtual value function can be either positive or negative, irrespective of the support of the value distribution. The expectation  under $F$ of the virtual value,  i.e. $\mathds{E}_{X \sim F} [ \psi(X)]$, is actually equal to the infimum of the support of $F$, when $F$ has one moment. In particular, it is equal to 0 if the support of $F$ ``starts" at 0. 
%\nek{maybe stop here; afterwards it kind of implies that $\psi_F$ is increasing...} and in that case, the virtual value is necessarily sometimes negative (at least around $x=0$) and sometimes positive (at least around the supremum of the support of $F$) \nek{latter is false unless virtual value is assumed to be increasing}.

The virtual value $\psi(x)$ is a crucial concept that can be interpreted as  \emph{virtual payment}, as we explain now. If the bidder has value $x$ and decides to buy the item, so $x\geq r$, his (virtual) payment can be thought of as $\psi(x)$,  \textsl{independently} of the price $r$ set by the seller. Indeed, the revenue generated by such a price $r$ is
\begin{gather*}
\mathds{E}_{X \sim F} [ \psi(X) \mathds{1}\{X \geq r\}]=
\int_r^\infty \psi(x) f(x)dx= \int_r^\infty xf(x) - (1-F(x)) dx \\
= -\int_r^\infty (x(1-F(x)))' dx=
r(1-F(r))=\Pi(r)\;.
\end{gather*}
The last equality comes from the definition of $\Pi(r)$, see Equation \eqref{eq:defPiOfr}. As a consequence, even though it is traditionally called virtual value, $\psi(x)$ could rather be understood as a virtual \textsl{payment}~: the buyer pays on average $\psi(x)$ when his value is $x$ and he buys/wins the item, i.e. $x\geq r$. See also Proposition \ref{prop:virtualValueIsVirtualPaymentGeneralCase} for an explanation of why this interpretation holds for general auction systems and buyers optimizing their expected utility.

\subsubsection{Examples of virtual value functions:} 
\begin{itemize}
\item if $x\sim\mathfrak{U}([0,1))$, the uniform distribution over $[0,1]$, then $\psi(x)=2x-1$ for $x \in [0,1]$.
\item if $x\sim \mathfrak{E}\mathrm{xp}(\lambda)$, the exponential distribution, then  $\psi(x)=x-\lambda$ for $x \in \mathds{R}_+$ ($F(x)=1-\exp(-x/\lambda)$).
\item Generalized Pareto (GP) distributions, parametrized by $(\mu,\sigma,\xi)$ where $\sigma >0$ and $\xi\leq 0$, have cdf 
\begin{equation*}
F_{\mu,\xi,\sigma}(x)   = \begin{cases} 1-(1 +\frac{\xi (x-\mu)}{\sigma})^{-1/\xi} & \text{for } \xi < 0 \\
1-e^{-(x-\mu)/\sigma} & \text{for } \xi= 0\end{cases}\;.
\end{equation*} 
Their virtual value is affine \citep{balseiro2020multistage}
$$\psi_{\mu,\xi,\sigma}(x) = (1-\xi)x+\xi\mu-\sigma$$
\end{itemize}
%\begin{remark2}
%With $\xi = -1 , \mu = 0, \sigma = 1 $, we recover the uniform distribution. With $\xi = 0 , \mu = 0 , \sigma = 1$, we recover the exponential distribution. With  $ \mu = 1, \sigma = \xi$ , this corresponds the power law (a.k.a the Pareto distribution) with parameter $\alpha = 1/\xi$. Hence, the generalized Pareto distribution are widely used in auction theory due to their flexibility (they model a large spectrum of distributions) and the fact that their virtual value is easy to compute (the virtual value is affine).
%\end{remark2}
\subsubsection{Relationship between  monopoly price and virtual value/payment}
Lemma \ref{TH:Monopoly} states that the optimal reserve price against  a single bidder (which was called the monopoly price)  is, in the case where the virtual value/payment function  $\psi$ is increasing and changes sign, necessarily the root of $\psi$ (or the point where the sign changes if $\psi$ is not continuous). If $\psi$ is strictly positive everywhere, which can happen if the  infimum of the support of $F_i$ is positive, then the optimal reserve price is that specific point (or equivalently 0). Note that if $\Pi(t)$ is the expected revenue of the seller at reserve price $t$ (see Equation \eqref{eq:defPiOfr}), $\Pi'(t)=-f(t)\psi(t)$.  Quite interestingly, even with multiple other bidders, the optimal reserve price for bidder $i$ is still $i$'s monopoly price, i.e. the same as if he were the only bidder. This is illustrated in the following Section \ref{optimal_reserve_for_lazy} under the same assumptions of $\psi$ being increasing and/or changing sign once. 

As a consequence, in the following,  our main focus will be on these distributions which are called \textsl{regular}. The results we will prove can be generalized to non-regular distribution with a technique called \textsl{ironing}, see Section \ref{Se:Ironing}.  
 \begin{definition2} 
The distribution $F$ is  regular if the corresponding virtual value $\psi$ is increasing.
\end{definition2}

\textbf{Examples }The uniform, exponential and generalized Pareto distributions with $\xi <1$, are all regular distributions. % 
%\begin{proposition2}
%If $\psi$ increasing and crossing zero exactly once and F is defined over its full support, then r is the monopoly price if and only if
%$$\psi(r) = 0$$ 
%\end{proposition2}
%\begin{proof}
%The monopoly price r is defined as $$\argmax_r R(r) = r(1-F(r)).$$
%Then, 
%$$
%\frac{dR(r)}{dr} = -f(r)\psi(r)\;.
%$$
%Since $\psi$ increasing, R is concave and $\psi(r)=0$.
%\end{proof}
%If $\psi$ is crossing zero multiple times, the monopoly price also verifies $\psi(r)=0$. 
%One of the beauty of auction theory is that this notion of monopoly price can be extended to auctions with multiple buyers.
\subsection{Optimal reserve prices in second-price auctions}
\label{optimal_reserve_for_lazy}
We  focus in this section on second-price auctions with reserve prices \citep{riley1981optimal} where  $n$ buyers are asymmetric, i.e. their value distribution can be different. As a consequence, the seller might also set different, personalized, reserve prices so as to increase her revenue. When introducing the concept of reserve price, we mentioned that a bidder can only win the auction if his bid was higher than his reserve price and that the latter is the minimal payment that bidder might pay. There however remains some ambiguity on how the auction unfolds (depending on which condition ``highest bidders" or ``bid above reserve price" is checked first). As a consequence, there exist at least two different types of second-price auction with reserve prices.

\begin{description}
\item[``Lazy" 2nd-price auction:] The winner can only be the highest bidder. He gets the item only if he  clears his reserve price (i.e. he bids above it), and pays the maximum between his reserve price and the second highest bid overall (regardless of whether the second highest bid cleared its reserve).
\item[``Eager" 2nd-price auction:] Bidders that have not cleared their respective reserve price are  disregarded. Thus the winner is the highest bidder amongst those that have cleared their reserve price and he pays the maximum between his reserve price and the second highest cleared bid.
\end{description}


First of all, notice that if the reserve prices are anonymous, i.e. the same for all bidders, as they should be in the symmetric case for instance, both types of auctions coincide.  Optimal reserve prices are easy to compute in lazy auctions, as they have an explicit form. They are on the other hand hard to compute for eager auctions. Moreover, the eager 2nd-price auction is also not the revenue-maximizing auction for the seller. So this concept is neither simple (as is the lazy auction) nor optimal (as is the Myerson auction, see Section \ref{emp_Myerson}). As a consequence, we will not put too much emphasis on eager auctions. In practice, if one wishes to implement eager 2nd-price auctions, a good idea would be to use the reserve prices of the corresponding lazy 2nd-price auction.



\medskip

It is quite immediate to see that lazy and eager second price auctions are still DSIC mechanism (the proof follows the exact same lines as that without reserve prices), hence we shall again only consider the truthful equilibrium. We now derive the expected payment of a bidder at this equilibrium.
%\begin{theorem2}[Expected payment in a lazy second-price auction]\label{myerson_for_second_price}
%Consider bidder $i$ with virtual value $\psi_i$ and reserve price $r_i$. We denote by $G_i$ the cdf of $Y_{-i} = max_{j\neq i} X_j$. The expected payment $P_i(\beta_{tr})$ of bidder $i$ in a lazy second-price auction when all bidders are bidding truthfully is equal to:
%\begin{equation*}
%P_i(\beta_{tr}) = \mathds{E}_{x_i\sim F_{i}}\bigg(\psi_i(x_i)G_i(x_i)\textbf{1}_{x_i\geq r_i}\bigg)\;.
%\end{equation*}
%\end{theorem2}
\begin{theorem2}\label{myerson_for_second_price}
Let   $P_i$ be the expected payment of bidder $i$ facing reserve price $r_i$ at the truthful equilibrium of a lazy second-price auction. Assume the bidders are statistically independent. Then 
\begin{equation*}
P_i = \mathds{E}_{x_i\sim F_{i}}\Big[\psi_i(x_i)G_i(x_i)\mathds{1}\{x_i\geq r_i\|\Big]\;,
\end{equation*} 
where $G_i$ the cdf of $\max_{j\neq i} X_j$ and $r_i$ is the personalized reserve price of bidder $i$.

\end{theorem2}
\begin{proof} 
Let us introduce the notation $y_{-i}= \max_{j\neq i} x_j$ so that the pointwise payment of bidder $i$, when he has value $x_i$, given all the values $x_j$ is equal to: 
\begin{equation*}
\max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x_i\geq r_i\}\;,
\end{equation*}
We note that 
$$
\max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x_i\geq r_i\}=
\mathds{1}\{x_i\geq r_i\}(r_i\mathds{1}\{y_{-i}\leq r_i\}+\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{ y_{-i}\geq r_i\}y_{-i})\;.
$$
As a consequence,
\allowdisplaybreaks
\begin{align*}
P_i&= \mathds{E}_{F_1,\dots,F_n}\Big[\max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x\geq r_i\}\Big]
\\& = \int_{x_i} \int_{y_{-i}} \max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x_i\geq r_i\}f_i(x_i)g_i(y_{-i})dy_{-i}dx_i
\\& =\Big(1-F_i(r_i)\Big)G_i(r_i)r_i + \int_{x_i=r_i}^{+\infty}\int_{y_{-i}=r_i}^{+\infty}y_{-i}g_i(y_{-i})f_i(x_i)\textbf{1}(x_i \geq y_{-i})dy_{-i}dx_i
\\& = \Big(1-F_i(r_i)\Big)G_i(r_i)r_i + \int_{y_{-i} = r_i}^{+\infty}y_{-i}g_i(y_{-i})\int_{x_i=y_{-i}}^{+\infty}f_i(x_i)dy_{-i}dx_i \hspace{2cm} \text{ (by Fubini)}
\\& = \Big(1-F_i(r_i)\Big)G_i(r_i)r_i + \int_{y_{-i} = r_i}^{+\infty}y_{-i}g_i(y_{-i})(1-F_i(y_{-i}))dy_{-i} 
\\& = \int_{y_{-i} = r_i}^{+\infty} \Big(f(y_{-i})y_{-i} - (1-F_i(y_{-i}))\Big)G_i(y_{-i})dy_{-i} \hspace{2.5cm} \text{(by integration by parts)}
\\& = \mathds{E}_{F_i}\Big[\psi_i(x)G_i(x)\mathds{1}\{x\geq r_i\}\Big]\;.
\end{align*}
\end{proof}
We can therefore easily derive the optimal reserve prices, as a function of $\psi_i$ at least for regular distributions.%\begin{definition2} 
%The distribution F  is said regular if its corresponding virtual value $\psi$ is increasing.
%\end{definition2}
%\redtext{changement}
%{\color{red} VP: est-ce qu'on a besoin de ce graphique ? En plus celui en haut a droite deconne, le vert n'est pas aligne avec le trait pointille rouge}
%\begin{figure}[h!]
%\begin{tabular}{cc}
%\includegraphics[width=.50\linewidth]{images/r025}&
%\includegraphics[width=.50\linewidth]{images/r075}\\
%\multicolumn{2}{c}{\includegraphics[width=.50\linewidth]{images/r05}}
%\end{tabular}
%\caption{\textbf{Change in bidder payment as a function of the reserve price.} The value distribution of the bidder is uniform [0,1] with $\psi(x) = 2x -1$, and is represented by the blue line. The dashed red vertical line corresponds to the current reserve price. We picked $G=1$, i.e. no competition. The bidder payment is equal to the area under the curve. The seller has no incentive to set the reserve price lower than $\psi_i^{-1}(0)$ since it decreases her total expected payment (because of the negative contribution of the red area). It is also clear that $r \ge \psi_i^{-1}(0)$ is suboptimal since it results in lost revenue for the seller.}
%\label{fig:visualOptimalR} % I can do without the label too
%\end{figure}
\begin{theorem2}%[Optimal reserve price in lazy second-price auction]
If  $F_i$ are regular, the optimal reserve prices in a lazy second-price auction are:
\begin{equation*}
\bigg(r_1,\dots,r_n\bigg) = \bigg(\psi_1^{-1}(0),\dots,\psi_n^{-1}(0)\bigg)\;,
\end{equation*}
with the convention that $\psi_1^{-1}(0)$ is the minimum of the support of $F_i$ is $\psi_i$ is  positive everywhere and the point where $\psi_i$ changes its sign if it is discontinuous.
\end{theorem2}
\begin{proof} 
The seller maximizes the sum of expected payment: 
\begin{align*}
\mathds{E}_{F_1,\dots,F_N}\Big[\sum_{i=1}^{n} P_i\Big] &= \sum_{i=1}^{n}  \mathds{E}_{F_i}\Big[\psi_i(x_i)G_i(x_i)\mathds{1}\{x_i\geq r_i\}\Big]\;.
\end{align*}
Since $F_i$ is regular, $\psi_i$ has one zero and is negative before the zero and positive after. Thus, the optimal choice for $r_i$ is clearly $\psi_i^{-1}(0)$. Indeed, the function $t\rightarrow \mathds{E}_{F_i}\Big[\psi_i(x_i)G_i(x_i)\mathds{1}\{x_i\geq t\}\Big]$ is increasing before $\psi_i^{-1}(0)$ and decreasing afterwards, owing to the sign of the integrand on both sides of $\psi_i^{-1}(0)$.
\end{proof}
We see in the proof that in a lazy second-price auction, the seller can safely maximize the payment of each bidder one by one independently. Indeed, in a lazy second price auction, changing the reserve price of one specific bidder does not change the probability of winning and the payment of the other bidders. This is not the case for eager second-price auctions on the other hand, which explains the complexity of computing the optimal reserve prices in them. Finally, the optimal reserve prices in a lazy second-price auction correspond to the monopoly prices of each bidder.



\begin{corollary2}The optimal reserve price for a bidder in a lazy second-price auction is independent of the presence, or not, of other bidders. In particular, it is the same as in the situation where he is the only bidder.
\end{corollary2}

\begin{figure}[H]
\includegraphics[width=.6\linewidth]{images/optimalmonopolyprice.pdf}
\caption{Bidder's payment as a function of the reserve price depending on the number of players in second-price auction with bidders all having a uniform value distribution $\mathfrak{U}([0,1])$.}
\end{figure}
%The proof also shows that when the distribution is not regular, the optimal reserve prices for each bidder verifies: $r_i \in \argmax(\mathds{E}_{F_i}(\psi_i(x)G(x)\textbf{1}_{x\geq r_i}))$.

The seller's revenue increases through the use of personalized reserve prices when bidders have very different value distributions. Intuitively, it is in the seller's best interest to set a high reserve price to bidders who have high values most of the time  (or very high values some of the time) and low reserve prices to bidders who have  low values most the time.

So far, we have only focused on the seller's revenue when designing auctions. An alternative objective can be the maximization of the  \textsl{global welfare} of the system, which is the sum of the seller's revenue and all bidders' utility. 

\bigskip


Even though reserve prices largely increase the seller's revenue, they actually significantly decrease the expected total welfare, as the item will sometimes not be allocated. This happens when all bidders (or at least the highest one in lazy auctions) have values below their reserve prices.

\begin{example2}
To illustrate this decrease in welfare, we are going to consider a simple example.  There are $n=2$ symmetric bidders with a value drawn uniformly over $[0,1]$. Because of the  symmetry, the optimal reserve price is the same for both bidders hence lazy and eager auctions coincide (and we do not need to specify the rule).  In this simple case, $r^* = \psi^{-1}(0) = 1/2$. As a consequence, the item is allocated as soon as one  bidder bids above 1/2, which happens with probability $3/4$. Otherwise, the item is not sold (which obviously happens with probability $1/4$). Simple computations show that changing the design from a second-price auction without reserve price to a second-price auction with optimal reserve price yields 
\begin{itemize}
\item a \textbf{12,5 \% decrease} of the global welfare (from $2/3$ to $7/12$).
\item a \textbf{50 \% decrease} of every single  bidder's utility  (from $1/6$ to $1/12$).
\item a \textbf{25 \%  increase} of the seller's revenue (from $1/3$ to $5/12$).
\end{itemize}
\end{example2}
\subsection{Myerson's lemma and characterization of BIC and DSIC auctions}
We mentioned before that the virtual value could (and maybe should) be understood as a virtual payment in a single bidder auction and/or in lazy second price auctions. The following lemma (that will be referred to as the ``Myerson Lemma'') is a crucial result \citep{Myerson81}. It states that virtual payment of a bidder is the correct quantity to study in any  incentive-compatible auctions, and not just lazy second-price ones. The proof, while conceptually profound, is not very hard technically and requires integration by part and Fubini's theorem as we used in the case of the lazy second-price auction. This result holds for any Bayesian Incentive Compatible auction (if bidding truthfully is weakly dominant) that is 0-rational (if bidding 0 ensures a payment of 0). The latter assumption can be weakened, at the cost of an additive constant in the payment formula. 
\begin{theorem2}%[Myerson lemma]
\label{Th:MyersonLemma}
For any BIC and 0-rational auction, the expected payment of bidder $i$ at the truthful equilibrium is 
\begin{equation*} 
\mathds{E}_{x_i\sim F_i}[P_i(x_i)] = \mathds{E}_{x_i \sim F_{i}}[\psi_i(x_i)Q_i(x_i)] = \mathds{E}_{x \sim \mathcal{F}^{(n)}}[\psi_i(x_i)q_i(x)]\;.
\end{equation*}
Here $Q_i(x_i)$ is the winning probability  of bidder $i$  at the truthful equilibrium given his value  $x_i$ and $q_i(x)$ is the probability that the item is attributed to bidder $i$ when the values are $x=(x_1,\ldots,x_n)$. 
\label{myerson_lemma}
\end{theorem2}
\begin{proof}
We consider the case where we are at the truthful equilibrium of the BIC auction. In particular, we assume that all bidders except possibly $i$ bid their values, i.e. they bid truthful. Let us call $Q_i(z)$ the probability that bidder $i$ bidding $z$ wins the auction (when all other bidders bid truthful) and $P_i(z)$ his expected payment (when all other bidders bid truthful). The expected utility of bidder $i$ when he has value $x_i$ and bids $z$ is simply $Q_i(z)x_i - P_i(z)$. 
By definition of Bayesian incentive-compatibility, at the truthful equilibrium the auction must verify: 
\begin{equation*}
\forall z \in \mathds{R}^{+}, \forall x_i \in \mathds{R}^{+}, Q_i(x_i)x_i - P_i(x_i) \geq Q_i(z)x_i - P_i(z)\;,
\end{equation*}
since at the truthful equilibrium bidder $i$ gets maximum utility by bidding his value. 
Thus, if we denote by $\mathcal{U}_i(x_i)$ the expected utility of bidder $i$ when he has value $x_i$, 
\begin{equation*}
\mathcal{U}_i(x_i) = \max_{z} Q_i(z)x_i - P_i(z) = x_i Q_i(x_i)-P_i(x_i)\;.
\end{equation*}
As a consequence, $\mathcal{U}_i$ is a  convex mapping (the maximum of affine mappings) and therefore is differentiable almost everywhere and absolutely continuous (i.e. it is equal to the integral of its derivative).

Bayesian-incentive compatibility also implies that
\begin{equation*}
\forall z \in \mathds{R}^{+}, \mathcal{U}_i(z) =\max_t zQ_i(t)-P_i(t)\geq z Q_i(x_i)-P_i(x_i)= \mathcal{U}_i(x_i) + Q_i(x_i)(z-x_i)\;.
\end{equation*}
Since $\mathcal{U}_i$ is convex, this means that $Q_i(x_i)$ belongs to the subdifferential of $\mathcal{U}_i$ at $x_i$, i.e.
\begin{equation*}
Q_i(x_i) \in \partial \mathcal{U}_i(x_i)\;,
\end{equation*}
and  $\nabla \mathcal{U}_{i}(x_i) = Q_i(x_i)$  if  $\mathcal{U}_i$ differentiable at  $x_i$. Therefore, using Theorem  D.2.3.4 in \citep{HULLbook01}, 
$$
\mathcal{U}_i(x_i)-\mathcal{U}_i(0)=\int_0^{x_i}Q_i(z)dz\;,
$$
and since $\mathcal{U}_i(x_i)=x_i Q_i(x_i)-P_i(x_i)$, 
\begin{equation*}
P_i(x_i) = P_i(0) + Q_i(x_i)x_i - \int_{0}^{x_i}Q_i(z)dz\;.
\end{equation*}
Taking expectation over $x_i$ now gives~: 
\begin{align*}
 \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] &= \int_{x_i}P_i(x_i)f_i(x_i)dx_i 
\\&=  P_i(0) + \int_{x_i} \Big(Q_i(x_i)x_i - \int_{0}^{x_i}Q_i(z)dz\Big)f_i(x_i)dx_i
\\& = P_i(0) + \int_{x_i} Q_i(x_i)x_if_i(x_i)dx_i - \int_{z}Q_i(z)\Big(\int_{z}^\infty f_i(x_i)dx_i\Big)dz \qquad \text{ (Fubini) }
\\& = P_i(0) + \int_{x_i} \Big(x_i - \frac{1-F_i(x_i)}{f_i(x_i)}\Big)Q_i(x_i)f_i(x_i)dx_i 
%\\&= P_i(0) + \int_{x} \Big(x_i - \frac{1-F_i(x_i)}{f_i(x_i)}\Big)q_i(x)f(x)dx
\\& =  
 P_i(0) + \mathds{E}_{x_i \sim F_i}[\psi_i(x_i)Q_i(x_i)]\;.
% P_i(0) + \mathds{E}_{x \sim \mathcal{F}}[\psi_i(x_i)q_i(x)] =
\end{align*}
The result follows from the fact that $P_i(0) =0$ since the auction is 0-rational.

The last equality comes from the fact that $Q_i(x_i)= \mathds{E}_{x \sim \mathcal{F}^{(n)}}[q_i(x)|x_i]$ and the tower property of conditional expectations.
\end{proof}
\begin{remark2}
Notice that Theorem \ref{myerson_for_second_price} is a direct consequence  of this result with the specific choice of $Q_i(x_i) = G_i(x_i)\mathds{1}\{x_i\geq r_i\}$.
\end{remark2}
Myerson's lemma indicates that the expected payment of a 0-rational BIC auction only depends on the allocation rule and the virtual value; the proof actually gives a characterization of any incentive-compatible auction.  However, this characterization is slightly different for  BIC and DSIC auctions. 
\nek{Thomas: in coro below, do we need the auction to be 0-rational? }
\begin{corollary2}%[characterization of BIC auctions]
[\cite{Myerson81}]
\label{characterization_inc_comp}
Using the notations of Theorem \ref{Th:MyersonLemma}, an auction is BIC if and only if
\begin{itemize}
\item[i)] the allocation rule is monotone, i.e.  the probability of winning, as a function of the bid, is non-decreasing (for any fixed bids of others bidders)  and
\item[ii)] the expected payment verifies 
$$P_i(x_i) = Q_{i}(x_i)x_i - \int_{0}^{x_i} Q_{i}(z)dz.$$
\end{itemize}
\end{corollary2}
\begin{proof} 
The proof of Theorem \ref{myerson_lemma} gives the first implication. For the reverse, 
let us assume that all bidders except $i$ bid truthfully; and let us show that $i$ has an incentive to also bid truthfully. This will show that truthful bidding constitutes a Nash equilibrium and hence the auction is BIC. 

Note that because we have assumed that all other bidders bid truthfully, if bidder $i$ bids $z$, the probability that he wins is $Q_i(z)$. Hence, the expected utility derived by bidder $i$ when bidding $z$ and his value is $x_i$ is 
$$
\mathcal{U}_i(z,x_i)=x_i Q_i(z)-P_i(z)=(x_i-z)Q_i(z)+\int_0^z Q_i(t) dt\;.
$$
The second equality comes from assumption ii). 
Let us call $b_i^*$, the optimal bid of bidder $i$. 
% \nek{version 1}
% $b_i^*$ satisfies
% $$
% b_i^*=\argmax_z (x_i-z)Q_i(z)+\int_0^z Q_i(t) dt\;.
% $$
% Let us now show that $b_i^*=x_i$, which would conclude the proof.
% Consider the function $H: y\mapsto \int_0^y Q_i(t) dt$\;. This function is differentiable, with derivative $H'(y)=Q_i(y)$; as a consequence of assumption i) it is convex, since $Q_i(y)$ is non-decreasing in $y$. Therefore it is above all of its tangents, i.e~:
% $$
% \forall z\;, H(x_i)\geq H(z)+(x_i-z)H'(z)=H(z)+(x_i-z)Q_i(z)\;.
% $$
% In other words,
% $$
% \forall z\;, \mathcal{U}_i(x_i,x_i)=\int_0^{x_i}Q_i(t)dt\geq (x_i-z)Q_i(z)+\int_0^z Q_i(t) dt=\mathcal{U}_i(z,x_i)\;.
% $$
% This shows that $b_i^*=x_i$ and the auction is BIC.
%
% \nek{alternative}
Let us now show that $b_i^*=x_i$. To do so, we simply need to establish that 
$$
\forall z\;, \mathcal{U}_i(x_i,x_i)=\int_0^{x_i} Q_i(t) dt \geq (x_i-z)Q_i(z)+\int_0^z Q_i(t) dt\;.
$$
This is equivalent to showing that 
$$
\forall z\;, \int_z^{x_i} Q_i(t) dt \geq (x_i-z)Q_i(z)\;.
$$
If $z\leq x_i$, since $Q_i$ is non-decreasing, $Q_i(t)\geq Q_i(z)$ on $[z,x_i]$ and hence 
$$
\int_z^{x_i} Q_i(t) dt \geq (x_i-z)Q_i(z)\;.
$$
If $z\geq x_i$, since $Q_i$ is non-decreasing, $Q_i(t)\leq Q_i(z)$ on $[z,x_i]$ and hence
$$
\int_{x_i}^z Q_i(t) dt \leq (z-x_i) Q_i(z)\;.
$$
Multiplying the previous inequality by $(-1)$ on both sides shows that if $z\leq x_i$, we also have 
$$
\int_z^{x_i} Q_i(t) dt \geq (x_i-z)Q_i(z)\;.
$$
So we have shown that 
$$
\forall z\;, \mathcal{U}_i(x_i,x_i)\geq \mathcal{U}_i(z,x_i)\;.
$$
Therefore, bidding truthfully is an optimal strategy for bidder $i$ and the auction is BIC. (Note that the inequalities needed also follow from realizing that the function $H: y\mapsto \int_0^y Q_i(t) dt$ is convex.)
%
% if the auction verifies
% $$P_i(x_i) = Q_{i}(x_i)x_i - \int_{0}^{x_i} Q_{i}(z)dz\;,$$
% then it implies that the auction verifies  $\nabla \mathcal{U}_i(x_i) = Q_{i}(x_i)$.\nek{do you mean this with subdifferentials?}
% \nek{I don't understand below}
% Since the probability of winning is increasing as a function of the bid, $$\mathcal{U}_i(x_i) - \mathcal{U}_i(z) = \int_{x_i}^{z}Q_{i}(s)ds \geq Q_i(x_i)(z - x_i)$$ which entails that $$\mathcal{U}_{i}(x)\geq Q_i(z)x - P(z).$$ This is the definition of bayesian incentive-compatibility (BIC).
%
%
% \nek{alternative}
% not clear yet that we know the gradient of $U_i$.
%
% Increasing allocation+others are truthful means $PWin(z)=Q_i(z)$ if we use $z$ instead of $x_i$ in $\beta(z)$.
%
% Now optimal strategy means $U_i(x_i)=\max_z x_iQ_i(z)-P(z)$. use convexity.
%
% see krishna pp.64-65 and possibly 69.
%
% Since the probability of winning is increasing as a function of the bid, the function
% $\mathcal{U}_i(x_i)$ is convex since its derivative is increasing. It is in particular above all of its tangents, hence
% $$
% \forall z\;,\mathcal{U}_i(x_i)\geq \mathcal{U}_i(z)+\mathcal{Q}_i(z)(x_i-z)\;.
% $$
% Since $\mathcal{U}_i(z)=z\mathcal{Q}_i(z)-P(z)$, we have
% $$
% \forall z\;,\mathcal{U}_i(x_i)\geq x_i \mathcal{Q}_i(z)-P(z)\;.
% $$
% This is the definition of bayesian incentive-compatibility (BIC).


\end{proof}
\begin{corollary2}%[characterization of DSIC auctions]
[\cite{Myerson81}]
\label{corollary_charect_DSIC}
An auction is DSIC if and only if
\begin{itemize}
\item[i)] the allocation rule is monotone and
\item[ii)]  the payment  of the winning bidder is the minimum bid guaranteeing that he would still have won the auction.\end{itemize}
 Given a monotone allocation rule and assuming 0-rationality, the payment rule is unique. 
\end{corollary2}
\begin{proof} 
The proof is almost identical, one just needs to make the various computations pointwise (for any vector $x_{-i}$) instead of in expectation.
\end{proof}
This characterization can be extended to very general mechanisms~: see \citep{archer2001truthful}.
\subsection{The Myerson auction : revenue maximization for BIC auctions}
After having established the Myerson lemma, it is now possible to derive the  revenue-maximizing auction among all BIC auctions. 
\begin{definition2}%[Myerson auction]
The Myerson auction is defined by the two following rules~: suppose bidder $i$ has value distribution $F_i$'s with associated virtual value (see Equation \eqref{eq:defVirtualValue}) $\psi_i$. Assume $F_i$ are regular, i.e. $\psi_i$ are increasing. 
\begin{description}
\item[Allocation rule:] Given the bids $b=(b_1,\ldots,b_n)$, the winner is the bidder with the highest non-negative virtual value $\psi_i(b_i)$, i.e.
$$
q(b) = \indicator{\arg\max \big\{ \psi_i(b_i) \, ; \, i \text{ s.t. } \psi_i(b_i) \geq 0 \big\} }
$$
with the convention that if the set is empty (when all virtual values are negative), then the item is not allocated and $q(b) = 0$. Ties are broken arbitrarily.
\item[Payment rule:] If bidder $i$ wins the auction, he pays
$$p_i(b)=\max \Big\{ \psi_i^{-1}(0), \psi_i^{-1}\Big(\max_{j\neq i} \big\{\psi_j(b_j)\big\}\Big) \Big\}$$
\end{description}
\end{definition2}
\textbf{Interpretation ~: } this auction amounts to running a second price auction with reserve 0 among the \emph{virtualized bids} $\psi_k(b_k)$ and converting back this ``virtual cost" in the original bid space of the winner $i$ through the function $\psi_{i}^{-1}$\;.
\begin{theorem2} \label{theorem_regular_distributions}
If $F_1,\dots,F_n$ are regular, the Myerson auction maximizes seller's revenue among all BIC and  interim-IR  auctions.
\end{theorem2}
\begin{proof}
The Myerson auction is BIC (for regular distributions)~: this can be verified in an elementary fashion - as we did for the second price auction earlier -  by comparing $\psi_i(x_i)$ to $\max_{j\neq i}\psi_j(b_j)$ and checking that in all situations it is optimal for bidder $i$ to bid his value. Indeed, bidding $b_i>x_i$ or $b_i<x_i$ never results in improvement of bidder $i$'s utility.


To show individual-rationality, we remark that since the auction is BIC, $$\mathcal{U}_{i}(x_i) = \mathcal{U}_{i}(0) + \int_{0}^{x_i}Q_i(s_i)ds_i = -P_{i}(0) + \int_{0}^{x_i}Q_i(s_i)ds_i \geq 0,$$ because $P_i(0) = 0$.  Thanks to  Myerson's lemma, Theorem \ref{Th:MyersonLemma}, the payment of each BIC auction is equal to 
$$
 P_i(0) + \mathds{E}_{x_i \sim F_{i}}(\psi_i(x_i)Q_i(x_i))\;. 
$$
The Myerson auction maximizes the two terms of this expression since for any rational auction, $P_i(0)\leq 0$.  Since the winner in the Myerson auction is the bidder who verifies
\begin{equation*} 
\psi_i(x_i) = \max_{j \in S}(\psi_j(x_j))\;,
\end{equation*}
and the item is not allocated when all $\psi_i$ are negative, the second term, is also maximized pointwise. 
Indeed, note that we can rewrite this second term
$$
\mathds{E}_{x_i \sim F_{i}}(\psi_i(x_i)Q_i(x_i))=\mathds{E}_{x \sim \mathcal{F}^{(n)}}[<\psi(x),q(x)>]\;,
$$
where $<a,b>$ is the scalar product between vectors $a$ and $b$. 
\end{proof}
\begin{corollary2} In the symmetric case, the second-price auction with reserve prices set to  monopoly prices is the revenue-maximizing auction.
\end{corollary2}
\nek{should we move this remark to the ``difficult things" section?}
\begin{remark2} 
The seller can do better if the mechanism is  only required to satisfy ex-ante rationality instead of interim rationality, as shown in 	
\citep{cremer1988full}. Indeed, there exists a BIC auction that is ex ante individually rational that accomplishes full-surplus extraction for the seller. In other words, the utility of bidders in this auction is equal to zero. This auction is not interim individually-rational since the expected utility when the bidder's value is zero is strictly negative. This setting of ex-ante individual rationality only makes sense when bidders have to decide to take part in the auction before understanding their value for the item. We come back in more details to this setting in Section \ref{sub_full_surplus_extraction}.
\end{remark2}
\subsection{Generalization of optimality result}
\label{SE:General_OptimalityResults}
\subsubsection{Non Incentive-Compatible mechanism: the revelation principle}
Myerson's optimality result can be extended to any incentive-compatible auctions, as long as there is a Nash equilibrium between bidders.
\begin{theorem2}%[Revelation principle]
Given a mechanism and a specific Nash equilibrium for this mechanism, there exists another BIC mechanism where the bidders' expected utility and seller's revenue at the truthful equilibrium are equal to the ones at the original Nash equilibrium. 
\end{theorem2}
\begin{proof}
Consider a mechanism and  $\beta = (\beta_1,\dots,\beta_n)$ a profile of strategies that is a Nash equilibrium. This mechanism is defined by an allocation rule $q:\mathcal{B}^{n}\rightarrow \mathds{R}^{n}$ and a payment rule  $p:\mathcal{B}^n\rightarrow \mathds{R}^{n}$. The mechanism $(q \circ \beta, p \circ \beta)$ is then clearly BIC and bidding truthful generate the same bids distributions, allocation and paiement as in the original mechanism; hence utilities and revenue are unchanged.
\end{proof}
\begin{corollary2} 
The Myerson auction is the revenue-maximizing mechanism among all individually-rational mechanisms which have a Nash equilibrium.
\end{corollary2} 
\begin{proof}
This is a direct application of the revelation principle.
\end{proof}
\nek{it's still unclear how to do it. And what about non-regular distributions? Then Myerson not defined at this point...}
We now extend the Myerson auction to cases where value distributions are not regular. 
\subsubsection{Non-regular distributions and the ironing technique}\label{Se:Ironing}

If $F_i$'s are not regular, the Myerson auction is poorly defined as $\psi_i$'s may not be invertible. From an allocation standpoint, since $\psi_i$ is not necessarily increasing,  the allocation rule may not be monotone. Hence a bidder might have incentive to ``shade" (or lower) his bid to increase his virtual bid and his probability of winning. Non-regular distributions are not uncommon, as a mixture of two distributions typically is not regular (for instance the mixture of two uniforms, Gaussians, etc...). It is therefore crucial to adapt the Myerson mechanism to non-regular distributions. The canonical way is to define a slightly different allocation rule based on a modified virtual value \citep{Myerson81} called the \textit{ironed virtual value}. 

Recall that one key consequence of having a non-decreasing virtual value is that the monopoly revenue $\Pi(r) = r(1-F(r)) = \int_r^\infty \psi(v)f(v)dv$ is ``almost''  concave, in the sense that $\Pi\circ F^{-1}$ is concave with derivative  $-\psi\circ F^{-1}(\cdot)$. As a consequence, optimizing the monopoly revenue boils down to finding the root of $\psi$.  The ironing technique consists in replacing $\Pi\circ F^{-1}$, which is not necessarily concave, by its concavification. 

\begin{definition2}[$\mathrm{cav}$ notation]\label{def:Concavification}
For a function $h$, we call 
$$
\mathrm{cav}(h) \text{ the concavification of the  function } h.
$$
We recall that , $\mathrm{cav}(h)$ is its smallest concave majorant of $h$, i.e. the smallest concave function above it~: its hypograph is the convex hull of the hypograph of $h$.
\end{definition2}
We can now define the ironed virtual value. 
\begin{definition2}[Ironed virtual value] \label{def:IronedVirtualValue}
For any non-regular distribution $F$, the \emph{ironed virtual value} of $\psi$, denoted by $\tilde{\psi}$ is defined by
$$
 \tilde{\psi}(x)= \partial \Big(-\mathrm{cav}(\Pi\circ F^{-1})\Big)(F(x))\;, \text{ where } \partial \text{ denotes subdifferential}. 
$$
\end{definition2}

In general, the concavification of a function $g$ is either equal to $g$ at some point or linear on some interval otherwise. Luckily enough, the ironed virtual value has a closed form on intervals where it is not equal to the virtual value.


\begin{lemma2}%[Expression of ironed virtual value on [a,b]] 
Assume that for some $a<b$, it holds that \begin{itemize}
\item[--] $\mathrm{cav}(\Pi\circ F^{-1})(F(a))=\Pi (a)$,  
\item[--]$\mathrm{cav}({\Pi}\circ F^{-1})(F(b))=\Pi(b)$
\item[--] $\mathrm{cav}({\Pi}\circ F^{-1})(F(x)) > \Pi (x)$ for $x \in(a,b)$ 
\end{itemize}then
the ironed virtual value  of $\psi$ on $(a,b)$ is constant and equal to
$$
\tilde{\psi}(x)= \frac{\int_{a}^b \psi(t) f(t) \mathrm{d} t}{F(b)-F(a)}$$
\end{lemma2}
\begin{proof}
By definition of the concavification, $\mathrm{cav}(\Pi\circ F^{-1})$ is linear on $[F(a),F(b)]$ and the results comes from linear interpolation.
\end{proof}
%Typically, non-increasing virtual value function are ironed on an interval where it is non-increasing. On the other hand, if the ironing is limited to the smallest interval  where the virtual value is non-increasing, this might not guarantee that the ironed virtual value is increasing. To insure that the ironed virtual value is non-decreasing, the ironing should be extended a larger interval. The final minimal interval $[a_{opt},b_{opt}]$ where the virtual value is ironed should verify the following conditions:
%$$\psi(a_{opt}) \leq \psi([a_{opt},b_{opt}]) \leq \psi(b) \text{ and } \forall c,d \in [a_{opt},b_{opt}], \psi(c) \geq \psi([c,d]) \geq \psi(d)$$
%A good way to visualize how to set $a_{opt}$ and $b_{opt}$ is to plot $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$ as a function of $F(t)$.  We recall that $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t = -b(1-F(b))$, the opposite of the monopoly revenue. The intervals where the virtual value should be ironed are the ones where the convex envelop of $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$ is different from $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$.
%
%\begin{definition2}[Ironed virtual value] Consider a value distribuion F with corresponding virtual value $\phi$. Let $[a_1,b_1],...,[a_k,b_k]$ be the intervals that are straightened out when one takes the convex hull for the plot of the cumulative virtual value $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$ against F(b). The ironed virtual value  of $\psi_i$ denoted by $\tilde{\psi}_i$ is defined as 
%$$
%\tilde{\psi}_i(x)=\left\{\begin{array}{ll}{\psi([a,b]) = \frac{\int_{a}^{b} \psi(t) f(t) \mathrm{d} t}{F\left(b\right)-F\left(a\right)},} & {x \in\left[a_i, b_i\right]} \\ {\psi(x),} & {\text { otherwise }}\end{array}\right.
%$$
%\end{definition2}
We refer to \citep{note_ironings} for more technical details. In particular, the ironed virtual value, since  it is defined as a sub-differential, is not a function but a multi-valued mapping, a.k.a a multifunction. On the other hand, selecting the aforementioned $\tilde{\psi}(x)$ as $\psi(x)$ when the sub-differential is not reduced to a singleton is also perfectly valid and implicitly used as convention from now on.  With this latter expression, either $\tilde{\psi}$ is equal to $\psi$ or it is constant on some interval around $x$. It is  non-decreasing everywhere and intervals where $\psi$ is  decreasing are ``flattened'', as illustrated in Figure \ref{Ironed}.



Recall that the purpose of ironing is to replace the - possibly somewhere decreasing - virtual value function $\psi$ in the Myerson auction (that might then not be BIC) by $\tilde{\psi}$. We now show that ironing the virtual value does not decrease the revenue of the Myerson auction.

\begin{figure}[h!]
\centering
\begin{tabular}{cc}
\includegraphics[width=.5\linewidth]{images/convex_hull.pdf}&
\includegraphics[width=.5\linewidth]{images/virtual_value_ironing.pdf}
\end{tabular}
\includegraphics[width=.55\linewidth]{images/ironed_revenue_curve.pdf}

\caption{\textbf{Left:} Concavification of $\Pi\circ F^{-1}$ for a  mixture of $\mathfrak{U}(0,0.5)$ and $\mathfrak{U}(0,1)$. \textbf{Right:} Associated virtual value (plain black) and ironed one (dashed orange).
\textbf{Center:} Original (plain black) and ironed (dashed orange) monopoly revenue.}
\label{Ironed}
\end{figure}
\begin{lemma2} 
The payment of bidder $i$ at the truthful equilibrium of any BIC auction satisfies 
$$ \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] \leq P_i(0) + \mathbf{E}_{x_{i} \sim F_{i}}\left[Q_{i}\left(x_{i}\right) \tilde{\psi}_{i}\left(x_{i}\right)\right]\;,$$
where $\tilde{\psi}_i$ is his ironed virtual value.\end{lemma2} 
\begin{proof} 
The proof is based on  the Harris inequality \citep{harris1960lower}, a direct application of Chebyschev' sum inequality. 
\begin{lemma2}[Harris inequality]
For any  non-decreasing mapping $\rho$ and  non-increasing mapping $\gamma$, the following holds for any random variable $X$, 
$$\mathds{E}[\rho(X)\gamma(X)] \leq \mathds{E}[\rho(X)]\mathds{E}[\gamma(X)]\;.$$
\end{lemma2}
Consider a BIC auction. According to Theorem \ref{Th:MyersonLemma}, 
$$
\mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] = P_i(0) + \mathbf{E}_{x_{i} \sim F_{i}}\left[Q_{i}\left(x_{i}\right) \psi_{i}\left(x_{i}\right)\right]\;.
$$
Furthemore, since the auction is BIC, Corollary \ref{characterization_inc_comp} $Q_i$ must be non-decreasing. 

Let assume there exists $[c,d]$ where $\psi_i$ requires ironing (otherwise there is nothing to show); we now call $[a,b]$ the largest interval that contains $[c,d]$ over which $\psi(x)\neq \tilde{\psi}(x)$. In other words, $[a,b]$ is the whole interval over which we have ironed $\psi$. We consider the function $\tilde{\psi}$ defined above on the corresponding $[a,b]$ interval. Furthermore, note that $f_i(x)/(F_i(b)-F_i(a))$ is a valid probability density on $[a,b]$. We then have
\begin{align*}
&\int_{a}^{b}Q_i(x)\psi_{i}(x)f_i(x)dx =(F_i(b) - F_i(a)) \int_{a}^{b}Q_i(x)\psi_{i}(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx
\\&\leq (F_i(b) - F_i(a)) \int_{a}^{b}Q_i(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx\int_{a}^{b}\psi_i(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx
\\&=\int_{a}^{b}Q_i(x)\tilde{\psi}_{i}(x)f_i(x)dx\;.
\end{align*}
from where the result follows. The first inequality comes from applying Harris' inequality. \nek{c'est faux non? $\psi$ est justement pas monotone sur l'interval, donc pourquoi appliquer Harris?} The last equality comes from the definition of $\tilde{\psi}$ which is a constant and equal to $\int_{a}^{b}\psi_i(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx$ on the interval $[a,b]$ by definition. Here it is important that we use the whole ironing interval for $[a,b]$. The same argument applies on all intervals where $\psi$ requires ironing.  
The statement of the Lemma is shown by applying Theorem \ref{Th:MyersonLemma} to compute expected revenue. 
\end{proof}
We now generalize Theorem \ref{theorem_regular_distributions} to the case of non-regular value distributions. \nek{the theorem below doesn't make sense. Are we doing BIC auctions with non-regular value distribution?}
 \begin{theorem2}[\cite{Myerson81}]%[Optimal auctions for general value distribution]
  In a single item auction, with general value distribution, a revenue-maximing auction \nek{in what class?} is an auction where the seller allocates the item to the bidder with the highest non-negative ironed virtual value. The payment rule is defined such that the auction is incentive compatible - see Corollary \ref{characterization_inc_comp}.
 \end{theorem2}
 
 \subsection{Reserve prices in first price auctions}
%\nek{need to read his assumptions carefully and state them} 
We start with an abstract result that we then apply to first price auctions. 

\begin{proposition2}\label{prop:virtualValueIsVirtualPaymentGeneralCase}
Suppose bidder $i$ participates in an auction such that the probability of winning the auction when bidding $b$ is $G_i(b)$ and the corresponding expected payment is $P_i(b)$. Call $\beta_i$ an optimal strategy for bidder $i$ in this setup, i.e. one that maximizes their utility. 	
Then the seller revenue coming from bidder $i$ is 
\begin{equation}\label{eq:RevSellerGeneralPriceWithVValue}
 \mathds{E}_{x_i\sim F_{i}}[P_i(\beta_i(x_i))]-P_i(\beta_i(0)) =\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;,
\end{equation}
where $\psi_i$ is the virtual value (see Equation \eqref{eq:defVirtualValue}) associated with the value distribution of $x_i$. 
\end{proposition2}
\begin{remark2}
This proposition helps explain how our interpretation of the $\psi_i(x_i)$ as a virtual payment makes sense for utility-maximizing bidders in general and not only in the case of BIC or DSIC auctions we encountered previously. It can also be seen as a more quantitative version of the revelation principle. 
\end{remark2}
\begin{proof}
Note that since bidder $i$ tries to maximize his utility, 
$$
\beta_i(x_i)=\argmax_b x_iG_i(b)-P_i(b)\;. 
$$
Let us call 
$$
W(x)=x G_i(\beta_i(x))-P_i(\beta_i(x))
$$
The envelope theorem in the form of Theorem 2 of \cite{MilgromSegal2002} applies since $0\leq G_i(t)\leq 1$ for all $t$ and hence 
$$
W(x)-W(0)=\int_0^x G_i(\beta_i(t)) dt\;.
$$
Therefore, the expected payment satisfies
$$
P_i(\beta_i(x))-P_i(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(t)) dt\;.
$$
Taking expectation with respect to $x_i$ with cdf $F_i$ in the previous equation gives
\begin{align*}
\mathds{E}_{x_i\sim F_{i}}[P_i(\beta_i(x_i))]-P_i(\beta_i(0))&=\int_0^{\infty} xG_i(\beta_i(x)) f_i(x)dx-\int_0^{\infty}\int_0^{\infty} f_i(x)\indicator{t\leq x}G_i(\beta_i(t))dt\, dx\;,\\
&=\int_0^{\infty} xG_i(\beta_i(x)) f_i(x)dx-\int_0^{\infty} (1-F_i(t))G_i(\beta_i(t))dt\;,\\
&=\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
\end{align*}
% $$
% \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
% $$

% This is not limited to first price... as long as $P(\beta_i(0))=0$\\
% En gros,  1st order conditions give $xG_i'(\beta_i(x))=P'(\beta_i(x))$. Multiply both sides by $\beta'_i(x)$ and integrate to get $P(\beta_i(x))-P(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(u))du\;.$ Then doing the same as below, we get that
% $$
% \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)]-P(\beta_i(0))=\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
% $$
% Ou: envelope theorem says that if $W_i(x)=\max_b xG_i(b)-P(b)$, and $\beta_i$ is an optimal strategy, $W_i'(x)=G(\beta_i(x))$. Hence, $W_i(x)-W_i(0)=\int_0^x G_i(\beta_i(u))du=xG_i(\beta_i(x))-P(\beta_i(x))+P(\beta_i(0))$. We conclude that
% $P(\beta_i(x))-P(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(u))du\;.$ And the result follows as above.

	
	
\end{proof}




In the case of first price auctions, we have $P_i(\beta_i(x_i))=\beta_i(x_i)G_i(\beta_i(x_i))$, since the probability of winning is $G_i(\beta_i(x_i))$. 
So the arguments given in the proof above allow us to recover a result from \citep{KirkegaardAsymmetricFirstPrice2009}~: the optimal strategy for bidder $i$ when the top bid of the competition has cdf $G_i$ and $P_i(\beta_i(0))=0$ satisfies 
\begin{equation}\label{eq:OptStrat1stPriceEnvelope}
\beta_{i}(x)=x-\frac{\int_0^x G_i(\beta_i(t))dt}{G_i(\beta_i(x))}\;.
\end{equation}

%Because of the the envelope theorem and arguments similar to those used to derived the revenue maximizing auctions, the equilibrium strategy must satisfy 
\iffalse
Using the envelope theorem, one can show \citep{KirkegaardAsymmetricFirstPrice2009} that the optimal strategy for bidder $i$ when the top bid of the competition has cdf $G_i$ satisfies 
\begin{equation}\label{eq:OptStrat1stPriceEnvelope}
\beta_{i}(x)=x-\frac{\int_0^x G_i(\beta_i(t))dt}{G_i(\beta_i(x))}\;.
\end{equation}
\fi
The expected payoff of player $i$ at $x$ is then equal to $u_i(x,\beta_{i}(x))=\int_0^x G_i(\beta_i(t))dt$ and in particular it holds  that $\mathds{E} U_i (\beta,x_i)=\ \mathds{E}_{x_i\sim F_{i}}\big[G_i(\beta_i(x_i))(x_i-\psi(x_i))\big]$. 
\iffalse
\nek{I think with the envelope theorem we can show that if I'm a utility maximizer, i.e. I pick 
$$
\beta(x)=\argmax_b xG(b)-P(b)\;,
$$
regardless of the payment rule, then 
$$
\mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
$$
This is not limited to first price... as long as $P(\beta_i(0))=0$\\
En gros,  1st order conditions give $xG_i'(\beta_i(x))=P'(\beta_i(x))$. Multiply both sides by $\beta'_i(x)$ and integrate to get $P(\beta_i(x))-P(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(u))du\;.$ Then doing the same as below, we get that 
$$ 
\mathds{E}_{x_i\sim F_{i}}[P_i(x_i)]-P(\beta_i(0))=\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
$$
Ou: envelope theorem says that if $W_i(x)=\max_b xG_i(b)-P(b)$, and $\beta_i$ is an optimal strategy, $W_i'(x)=G(\beta_i(x))$. Hence, $W_i(x)-W_i(0)=\int_0^x G_i(\beta_i(u))du=xG_i(\beta_i(x))-P(\beta_i(x))+P(\beta_i(0))$. We conclude that 
$P(\beta_i(x))-P(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(u))du\;.$ And the result follows as above. 
}
\fi
\begin{corollary2}\label{coro:RevSeller1stPriceWithVValue}
In a first price auction, when bidder $i$ uses the strategy implicitly defined in Equation \eqref{eq:OptStrat1stPriceEnvelope}, the seller revenue coming from bidder $i$ is 
\begin{equation}\label{eq:RevSeller1stPriceWithVValue}
 \mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;,
\end{equation}
where $\psi_i$ is the virtual value associated with the value distribution of $x_i$. 
\end{corollary2}
The corollary follows from Proposition \ref{prop:virtualValueIsVirtualPaymentGeneralCase} after noticing that $P_i(\beta_i(0))=\beta_i(0)G_i(\beta_i(0))=0$ when bidder $i$ uses $\beta_i$ defined in Equation \eqref{eq:OptStrat1stPriceEnvelope}.

\iffalse
\begin{proof}
We note that 
$$
 \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\int_0^{\infty}\beta_{i}(x) G_i(\beta_i(x)) f_i(x) dx =\int_0^{\infty} xG_i(\beta_i(x))f_i(x)dx - \int_0^{\infty}f_i(x)\int_0^x G_i(\beta_i(t))dt dx\;.
$$	
Using Fubini's theorem, we have 
$$
\int_0^{\infty}f_i(x)\int_0^x G_i(\beta_i(t)))dt dx=\int_0^{\infty}f_i(x)G_i(\beta_i(t))dt \indicator{t\leq x} dx dt=\int_0^{\infty}(1-F_i(t))G_i(\beta_i(t))) dt\;.
$$
We conclude that 
$$
 \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\int_0^\infty G_i(\beta_i(x))\left[x-\frac{1-F_i(x)}{f_i(x)}\right]f_i(x) dx = \mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi(x_i)\big]\;.
$$
\end{proof}
\fi

\paragraph{Good or optimal reserve prices} Proposition \ref{prop:virtualValueIsVirtualPaymentGeneralCase} and Corollary \ref{coro:RevSeller1stPriceWithVValue} suggest that from a seller revenue standpoint it would be good to avoid bids corresponding to values that have negative virtual values. In other words, setting individual reserve values at $\psi_i^{-1}(0)$ for bidders may have positive impact for seller revenue. However, this interpretation ignores the impact of setting such reserve values on the strategic response of the bidder that is optimizing his utility. 


Finding optimal reserve prices for first price auctions is much more complicated than finding them for the second price auctions, even with $n=2$ symmetric bidders \citep{KotowskiAsymmetricReserves2018} for the following two reasons. First, if the distribution $F$ is not regular and its density is discontinuous at the monopoly price, giving two different reserve prices to the two symmetric buyers actually increases the seller revenue at equilibrium, at least when $r_1$ and $r_2$ are close.
Second, in the specific case where those two reserve prices $r_1$ and $r_2$ are sufficiently close,  the equilibrium bid distribution of the player with the lower reserve price becomes discontinuous.


Many further difficulties arise when the seller tries to learn good reserve prices for first price auctions from data and does not have access to the bidders' value distributions. We further detail them in Section \ref{learning_reserve_prices_first_price}.

\section{Prior-independent optimal auctions} 
\label{sec-Bulow}
In the previous section, we  derived the revenue-maximizing auction given the prior of the seller on the possible valuations of the different bidders. In some cases, the seller does not have access to a reliable prior and she has to choose an auction without this information. An associated challenge is to understand what auctions are robust to a lack of knowledge about (or some mis-specification in) the bidders' value distributions.

The following theorem shows that a basic second-price auction without reserve price -  referred to henceforth as the Vickrey auction - with just one extra bidder, leads to a higher revenue than the optimal Myerson auction \citep{bulow1996auction}. Only the symmetric case is considered, so that the comparison of two auctions with different set of bidders is possible.
\begin{theorem2}[\cite{bulow1996auction}]%[Bulow-Klemperer Theorem]
In the symmetric setting and with regular distributions, the revenue of the Myerson auction with $n$ bidders is lower than the revenue of the Vickrey auction with $n+1$ bidders. 
\end{theorem2}
\begin{figure}[H]
\includegraphics[width=.5\linewidth]{images/BulowKlemperer.pdf}
\caption{Illustration of the Bulow-Klemperer theorem for the case with value distributions  $\mathfrak{U}([0,1])$.}
%{\color{red} Ca ne devrait pas etre $K$ bidders mais $n$ bidders ; choix des couleurs discutables ; on ne dit pas Nb bidders en Anglais }}
\label{fig:BK}
\end{figure}
Before proving the Bulow-Klemperer theorem, we introduce a useful lemma.
\begin{lemma2}\label{second_price_without_reserve}
In the symmetric case and with regular distributions, the Vickrey auction is revenue-maximizing in the class of individually-rational auctions where the item is always attributed. 
\end{lemma2}
\begin{proof}
Based on the revelation principle, we shall only consider incentive-compatible auctions. Theorem \ref{Th:MyersonLemma} then applies. Since the item must always be attributed, in order to maximize the seller's revenue it should be allocated to the bidder with the highest virtual value, regardless of whether the highest virtual value is non-negative or not. This is a consequence of the proof of Theorem \ref{Th:MyersonLemma}. Since the distributions are regular and identical, the bidder with the highest virtual value is also the bidder with the highest value. As a consequence, the mechanism we just described is exactly the Vickrey auction.
\end{proof}
The proof of the Bulow-Klemperer theorem can now be derived from the previous lemma.
\begin{proof} 
Let us assume that there are $n+1$ bidders, and consider the following mechanism. First, the seller runs a Myerson auction on  $n$ bidders (chosen arbitrarily). If the item is not allocated by the Myerson auction, it is allocated for free (i.e. without any payment) the $(n+1)$-th bidder. The revenue of this auction is equal to the revenue of the Myerson auction with $n$ bidder, yet it is  an auction that always allocate an item amongst $n+1$ bidders. Lemma \ref{second_price_without_reserve} implies that the revenue of this auction is smaller than the one of the Vickrey auction. 
This gives the result.
\end{proof}

As a consequence, it is more interesting,  from a seller revenue maximization standpoint to have one more bidder in the auction than to implement a complex mechanism. This is the reason why one of the first recommendations of most economists dealing with institutions organizing auctions is to maximize the competition  before implementing complex mechanisms \citep{bulow1996auction,milgrom2004putting}. This is sometimes referred to as the Wilson doctrine.

\bigskip

Nonetheless, let us assume that a specific mechanism has been chosen, independently of the value distributions (which are unknown in this setup). A crucial  question that remains is the evaluation of this specific choice of mechanism in the worst-case analysis. We will restrict ourselves to DSIC auctions. We will use the notion of \textsl{competitive ratio} defined as the infimum, over all possible value distributions, of the revenue of this auction divided by the optimal revenue of the Myerson auction for these distributions. 

The competitive ratio is obviously smaller than 1, and the bigger the better. Unfortunately, if the class of value distributions is not restricted when computing this infimum, there does not exist any auction with a positive competitive ratio \citep{allouah2018prior}. As a consequence, we will use different types of restrictions to achieve non-trivial approximation results. Based on the Bulow-Klemperer theorem, we can derive some revenue guarantees on the second price auction without reserve price. 
\begin{corollary2} \label{compet-ratio}
The Vickrey auction  with $n$ symmetric bidders and regular value distributions is at least a $\left(\frac{n-1}{n}\right)$-approximation of the Myerson auction. 
\end{corollary2}
\begin{proof}
We denote  respectively by $R(\mathrm{Vickrey}_n)$ and $R(\mathrm{Myerson}_n)$ the expected revenue of the seller  in the Vickrey or  Myerson auction with $n$ bidders and by $P_i(\mathrm{Vickrey}_n)$ and $P_i(\mathrm{Myerson}_n)$ the expected payment of the bidder $i$ in those auctions (so that $R(\cdot) = \sum_{i=1}^n P_i(\cdot)$).


Let us first prove that $P_i(\mathrm{Myerson}_n)\geq P_i(\mathrm{Myerson}_{n+1})$.

By symmetry and with regular distributions, their exists a unique monopoly price $r^*$ which is independent of the number of players. Note that $\psi(x)\geq 0$ when $x\geq r^*$. Furthermore, in the symmetric case, the probability that bidder $i$ wins the auction when facing $k$ competitors is just $F^k(x)$. Hence, 
\begin{align*}
	P_i(\mathrm{Myerson}_{n})&= \int  \psi(x) F^{n-1}(x)f(x)\mathds{1}\{x\geq r^*\} dx\\&\geq \int \psi(x) F^{n}(x)f(x)\mathds{1}\{x\geq r^*\}dx\\&=P_i(\mathrm{Myerson}_{n+1}),\end{align*}
which proves the inequality.



Then, based on the Bulow-Klemperer theorem, 
$$R(\mathrm{Vickrey}_n)\geq R(\mathrm{Myerson}_{n-1}) = (n-1)  P_i(\mathrm{Myerson}_{n-1}) \geq (1-\frac{1}{n})  R(\mathrm{Myerson}_{n})$$
which gives the result. \end{proof}
We proved in Corollary \ref{compet-ratio}, through the Bulow-Klemperer theorem that the competitive ratio of the Vickrey auction is at least 0.5, when the distributions are restricted to regular ones. Interestingly, it is possible to do better with a slightly different auction. 
\begin{theorem2}[\cite{fu2015randomization}]
There exists an incentive-compatible auction with a competitive ratio of 0.512 against regular value distributions. 
\end{theorem2}
The mechanism considered was the first  with a higher competitive ratio than 0.5  against regular distributions. It is a slight modification  of the Vickrey auction where the seller inflates the second highest bid. Formally, the mechanism is the following: with probability $1-\varepsilon$,  a second price auction without reserve price is run. With the  probability $\varepsilon$, the mechanism allocates the object to the bidder with the highest valuation, but only if his valuation is greater than $1+\delta$  times the valuation of the second highest bidder and pays  $(1+\delta)$ the second highest bid. Otherwise, the mechanism does not allocate the item. 

The idea behind this theorem is the following. The Bulow-Klemperer bound of $0.5$ on the competitive ratio is rather tight for regular distributions that would induce a high optimal reserve price. On the other hand, it is rather loose for regular distribution with a low associated reserve price. Inflating the second highest bid has a positive effect for the former type of distribution (as it somehow emulates a high reserve price) and a negative effect for the later type (because it induces some reserve price, bigger than what it should be). As a consequence, the ratio of revenues increase in the first case, and decreases in the second one; but thanks to the looseness in the Bulow-Klemperer bound of $0.5$, the infimum globally increases. 

On the other hand, when restricted to MHR distributions, the ratio is equal to 0.7153 and this result is tight. 

For regular distribution, this result was then improved up to 0.519 \citep{allouah2018prior}  and further improved in \citep{hartline2020benchmark} which identified the optimal prior-independent mechanism. The optimal mechanism is a mixture between a second price auction and the same auction where the prices are scaled up by a factor of about 2.5. The authors find the worst-case family of distributions and use these distributions to derive the optimal mechanism and solve the problem. 

\section{Further reading: non-unicity of Nash equilibria and related complications}
\label{sec:NashIsDifficult}
\nek{Add the two counter examples here...}


==> chapters/sept2Chap2BackupIncase/chapter2_some_classical_results_vPreCopyVianney.tex <==
%!TEX root = ../main.tex
\chapter{Bayesian mechanism design}
\label{Chapter:Bayes}

Auctions mechanisms involve many different agents, sellers and/or buyers, with possibly different and conflicting objectives as they all seek to optimize of their own utility functions. These interactions can be modeled using game-theoretic concepts. More specifically, we are going to focus on a specific types of games with \emph{incomplete information} that are called \textit{mechanisms}. In those games, each player has some private information (i.e. unknown from everyone else), and send a \emph{message} to a central authority.  Based on those gathered messages, the latter decides on the final outcome.  The utility of each player then solely depends on it \nek{the set of messages sent +mechanism?}. 

Mechanisms model appropriately  many practical situations such as the celebrated  problems of assigning students to schools, or matchings in organ-transplant applications.  In these problems, a central authority forms pairs between school and students or donors and recipients. In selling mechanisms, the central authority is the seller of a specific item and the players are the buyers.  \emph{Auctions} are mechanisms used to sell a particular item. In the case of a sale of a single non-divisible item, they have the following specific features. 


%\clem{The notation defined here is not used later on and even conflicts with later notation.}{\color{red}VP : agreed !}
%A \textit{normal-form game} is defined by a set of of players $\mathcal{N}$ of cardinality $N$, the set of actions  $\mathcal{A}_i$ and the payoff function  of player $i \in \mathcal{N}$
%$u_i:\mathcal{A}_1 \times \dots \times \mathcal{A}_N \rightarrow \mathds{R}.$ 
%
%In such a game, each player chooses independently an action $a_i \in \mathcal{A}_i$ and gets a utility of $u_i(a_1,\ldots,a_N)=u_i(a_i,a_{-i})$
%that depends on both the action $a_i \in   \mathcal{A}_i$ of the player and the profile of actions of other players, denoted by $a_{-i} := (a_1,\ldots, a_{i-1}, a_{i+1},a_N) \in \prod_{j \neq i} \mathcal{A}_j$.
%
% 
%\begin{definition2}[Normal-form game]
%A normal-form game is:
%\begin{itemize}
%\item a set of players $\mathcal{N}$ of cardinality $N$.
%\item for each player $i \in [1,N]$, a set of possible actions $\mathcal{A}_i$.
%\item a set of payoff functions which gives for each player her payoff corresponding to her action and actions of other players
%$$u_i:\mathcal{A}_1 \times \dots \times \mathcal{A}_N \rightarrow \mathds{R}\;.$$
%\end{itemize}
%In a normal-form game of complete information, actions, outcomes and payoff functions are common knowledge to all players. In a game of incomplete information, every player's payoff function depends on a variable $X$ called private information and which is only known to each specific player. If we denote by $\mathcal{X}$ the set of private information, the payoff function of player $i$ is defined as $u_i:\mathcal{A}^{N} \times \mathcal{X} \rightarrow \mathds{R}$.
%\end{definition2}


%In the different settings we are going to consider,  players have some private information that actually impacts their payoff functions. Formally, let us denote by  $\mathcal{X}$ the set of private information, so that the payoff function of player $i$ rewrites as  $u_i:\prod_{j \in \mathcal{N}} \mathcal{A}_j \times \mathcal{X} \rightarrow \mathds{R}$. Those games are called with \textit{incomplete information}.


\medskip


%and decides each player's outcome according to these messages. In these games, players' actions correspond to the message they send to the central authority. 

%In a game of incomplete information, every player's payoff function depends on a variable $X$ called private information and which is only known to each specific player. If we denote by, the payoff function of player $i$ is defined as 

%In this survey, we are focusing on a certain type of games with incomplete information where there exists a central authority which gathers messages from the different players and decides each player's outcome according to these messages. In these games, players' actions correspond to the message they send to the central authority. This type of centralized gamed is called mechanism. 
%\begin{definition2}[Mechanism]
%A mechanism is a game of incomplete information where players send a message to a central authority who does not know the private information of each player. The central authority decides based on messages it receives and some predefined rules every player's outcome.  
%\end{definition2}

Auctions are games of incomplete information as each buyer has some private valuation for the item to be sold, i.e. the highest price they are willing to  pay to acquire  this item. This valuation might be different from one buyer to another. We denote by $\mathcal{N}$ the set of buyers, of cardinality $n \in \mathbb{N}$, by  $x_i \in \mathcal{X}_i$ the  private value of bidder $i \in \mathcal{N}$, $\mathcal{X}_i $ the set of private values of bidder $i$, and by  $x = (x_1,\dots,x_n)\in \mathbb{R}^n$, the so-called profile of private values. 
The possible messages (or actions) of buyer $i\in \mathcal{N}$ are called ``bids'' and the set of bids of buyer $i$ is denoted by $\mathcal{B}_i$. The outcome of an auction mechanism is defined by two different rules~:
\begin{enumerate}
\item an \textit{allocation rule} $q:\mathcal{B}_1 \times \dots \times  \mathcal{B}_n \rightarrow \Delta_n$ where $\Delta_n$ is the set of probability distributions over the set of $n$ buyers. It specifies the probability that each player gets the item.
\item a \textit{payment rule} $p: \mathcal{B}_1 \times \dots \times  \mathcal{B}_n \rightarrow \mathds{R}^{n}$. It specifies the expected payment of each player, whether or not they get the item.
\end{enumerate}

We also denote by $b = (b_1,\dots,b_n)$ the vector of bids of the bidders.  With these notations, the expected utility of bidder $i \in \mathcal{N}$ is then defined as
$$u_i(b,x_i) = q_i(b)\big(x_i -p_i(b)\big)\;;$$
on the other hand, the seller aims at maximizing her expected revenue
$$\sum_{i=1}^n q_i(b)p_i(b)\;.$$

%\begin{definition2}[Auction mechanism]
%An auction mechanism is a mechanism defined by three features: 
%\begin{itemize}
%\item a set of possible messages $\mathcal{B}_i$ for each buyer (bids in most cases). 
%\item an allocation rule $q:\mathcal{B}_1 \times \dots \times  \mathcal{B}_N \rightarrow \Delta_N$ where $\Delta_N$ is the set of probability distributions over the set of $N$ buyers. It gives the probability that each player gets the object.
%\item a payment rule $p: \mathcal{B}_1 \times \dots \times  \mathcal{B}_N \rightarrow \mathds{R}^{N}$. It defines the expected payment of each player whether he got or not the object.
%\end{itemize}
%A selling mechanism is nothing more than a set of rules explaining how a group of buyers and a seller interact. 
%
%The private information owned by each buyer which conditions their payoff function is their own value for the item, i.e., the highest price they are ready to pay to own the item. We denote by $\mathcal{X}_i$ the set of all possible values for one item for bidder $i$.  The value vector which contains the values of all the different players is denoted by $x = (x_1,\dots,x_N)$. The \textit{messages} sent to the seller are called \textit{bids}.  We denote by $b = (b_1,\dots,b_N)$ the corresponding bid vector. 
%
%Depending on the information they have on the mechanism and the other bidders, the ultimate goal of the bidders is to maximize their utility 
%$$u_i(x_i, (b_1,...,b_N)) = q_i(b_1,...,b_N)(x_i -p_i(b_1,...,b_N))\;,$$
%and the objective of the seller is to maximize her revenue
%$$\sum_{i=1}^N q_i(b_1,...,b_N)p_i(b_1,...,b_N))\;.$$
%\end{definition2}
\section{The Bayesian setting}
The auction literature has often considered  a Bayesian setting where the value $x_i$ of bidder $i \in \mathcal{N}$ is random, drawn according to the \emph{value distribution} that ``represents the seller assessment of the probability of bidder $i$ having a value estimate of $x_i$ or less''  \citep{Myerson81}. The value distribution quantifies the uncertainty of the seller on the maximum price that one buyer is willing to pay for the item and is represented as a Bayesian prior on the private information of each buyer. 


A widely made assumption is that value distributions are common knowledge among bidders and seller.  As a consequence, we denote by $F_i$ the value distribution - i.e. the cumulative distribution function of the value -  of buyer $i \in \mathcal{N}$ and by $f_i$ its corresponding density function, assuming it exists, an assumption we are going to make repeatedly (removing this assumption is almost always a matter of technicalities and little to no impact on conceptual matters). We implicitly identify the distribution $F_i$ with its cumulative distribution function (cdf) and use both terms exchangeably. We are also going to assume that values $x_i \in {\mathcal X}_i$ are non-negative, i.e. the support of $F_i$ is included in (but not necessarily equal to)  $\mathds{R}_+ = [0,\infty)$. Unless otherwise noted, we assume that $\mathds{E}_{x_i \sim F_i} [x_i] < +\infty$ to get optimality results (and not just $\varepsilon$-optimality). A crucial assumption throughout this survey is that, unless otherwise noted, the values $x_i$ are drawn independently for different $i$'s and hence they are statistically independent as random variables. We shall  denote by $\mathcal{F} = \mathcal{F}^{(n)} =  F_1\otimes \ldots\otimes F_n$ the joint - and hence - product distribution of $x=(x_1,\ldots,x_n)$, the vector of values. 


\medskip

\paragraph{Examples} Typical examples of value distributions are the \emph{uniform} distribution, which is widely used in textbook examples due to its simplicity,  the \emph{exponential} and the \emph{log-normal} distributions as they are similar to some empirical distributions encountered on modern internet platforms. Power law distributions (also known as \emph{Pareto} distributions) are also widely used, as they capture the idea that the value in real time bidding and online advertising comes from few matches of very high quality, such as consumers who recently viewed a product \citep{arnosti2016adverse} (this situation where 20\% of individuals own/generate 80\% of wealth is also referred as the Pareto principle in economics). \emph{Generalized Pareto} distributions are also often used as examples because their virtual value - an important concept we will define later - is linear. 
\begin{definition}[Symmetric setting]
The auction setting will be called \textit{symmetric} if all bidders have the same value distribution.
\end{definition} 

For the sake of clarity, we use pronouns her/she for the seller and he/his for one specific bidder.

\subsubsection*{Assumptions and Notations}
If $v$ is a vector (of scalars or functions) in $\mathbb{R}^n$, we call $v_{-i}$ the vector in $\mathbb{R}^{n-1}$ that contains all entries of $v$ except the $i$-th one, $v_i$. 
In other words, $v_{-i}=(v_1,\ldots,v_{i-1},v_{i+1},\ldots,v_n)$. 

We use the notation $v_{-i}(j)$ to denote the $j$-th entry of $v_{i}$

Similarly, the notation  $F_{-i}$ will denote the product distribution of values of all bidders except $i$ and $b_{-i}$ is the vector of all bids except bidder's $i$. 

\begin{definition2}[Key Default Assumption on distributions]
Unless otherwise noted, we assume that $F_{i}$ is supported on a subset of $[0,b]$, with $b$ being possibly infinite. $F_i$ is assumed to be continuous. We, quite importantly, assume unless otherwise noted that $f_i>0$ on $(0,b)$, except possibly on a set of Lebesgue measure 0. 
\end{definition2}
Note that if ${\cal G}_i$ is the cdf of the largest value of a vector $x_{-i}$ drawn according to $F_{-i}$, ${\cal G}_i(t)=\prod_{j\neq i}F_j(t)$. In particular, with our key default assumption on distributions, ${\cal G}_i$ is differentiable and its density is strictly positive except possibly on a set of measure zero. 

When we say that a function $\beta$ is increasing, we use the standard convention that it means that if $l>u$, $\beta(l)>\beta(u)$. A non-decreasing function is such that if $l>u$, $\beta(l)\geq \beta(u)$.

We use $\partial f$ to denote the subdifferential of a convex function $f$ (see \cite{HULLbook01}, Chapter D). 

\nek{this is ongoing and needs to be completed}

%{\color{red} VP: Je pense qu'il faut elaborer un peu sur le "typical". Ca veut dire quoi exactement ? Soit on met des refs, soit on vire}

%The notion of information owned by the seller and value distribution have progressively changed with several new applications of auction systems. One of the goal of this thesis is to clarify this change and show how sellers and bidders can adapt to this new information structure of the game. For instance, in a repeated setting, where multiple different items are sold successively, the value distribution could also represent the variety of values that a specific buyer can give to one item. 

\subsection{Properties of auction systems}
\label{subsec_prop_auction}
A bidder's \textit{strategy} is the mapping indicating which bids he sends to the seller to buy one specific item, conditional on his private information, a.k.a his value. Stated otherwise, a strategy is a mapping $\beta: \mathcal{X} \rightarrow \mathcal{B}$ that maps private values to bids. %\nek{technical detail: is this mapping possibly random? or is it a function?}

%Bidders have the choice on the bids they send to the seller to get one specific item. A strategy defines how these bids depend on buyer's original private value.
%\begin{definition2}[Strategy]
%A strategy is a function $\beta: \mathcal{X} \rightarrow \mathcal{B}$ that maps private values to bids.
%\end{definition2}

We will denote by $\mathds{B}_i$ the set of all strategies of player $i$, $\beta_i$ the strategy chosen by $i$ and $\beta_{-i}$ the profile of strategies corresponding to all bidders except bidder $i$. Similarly, the notation  $F_{-i}$ will denote the product distribution of values of all bidders except $i$ and $b_{-i}$ is the vector of all bids except bidder's $i$. 

In Bayesian games, it is important to differentiate between \textit{ex ante}, \textit{interim} and \textit{ex post} properties \citep{hartline2013bayesian}. These notions depend on the information available to buyers when they decide to participate in the game and choose their strategy.  
\begin{itemize}
\item For  \emph{ex-ante} properties, bidders do not know yet their own value for the item; i.e. they only know $F_i$ and $F_{-i}$.
\item For \emph{interim} properties, bidders know their valuation but do not know the values of other players, i.e. they know $x_i$ and $F_{-i}$.
\item For \emph{ex-post} properties, bidders know their valuations and the other players', i.e. they know  $x_i$ and $x_{-i}$.
\end{itemize}
In the next sections, we will mostly focus on  interim properties. It is the starting point of most of the auction literature ~: we assume that value distributions are common knowledge and that exact valuations are private information to each bidder.  

We are also assuming that bidders are risk-neutral. In other words, they seek to maximize their expected utility and use utility-maximizing strategies. %over all other bidders' possible valuations and with respect to their strategies\nek{awkward; need to rephrase; need to def for interim and ex-ante. review that.}.  
Stated otherwise, assuming the other bidders are using the strategy $\beta_{-i}$, the  expected utility  of the strategy $\beta_i$  given bidder $i$'s value $x_i$ is denoted by
$$
U_{i}(\beta_i,\beta_{-i},x_i) = \mathds{E}_{x_{-i} \sim F_{-i}}\Big[u_{i}\big((\beta_1(x_1), \dots,\beta_{i-1}(x_{i-1}),\beta_i(x_i),\beta_{i+1}(x_{i+1}),\beta_n(x_n)), x_i\big)\Big]\;.
$$
%\nek{this is awkward as interim doesn't mean we know other people's strategies... and a strategy is a mapping but technically here we just need to know $\beta_i(x_i)$; also if $\beta_i(x_i)$ included in the stuff?}


\textbf{Optimality and characterization of strategies} Maybe one of the most central concept in game theory is \emph{(Bayesian) Nash equilibrium}. It is a characteristic of the vector of strategies $(\beta_1,\ldots,\beta_n)$ and the valuation distributions $F_1,\ldots,F_n$.  At a Bayesian Nash Equilibrium, for any bidder $i$, strategy $\beta_i$ maximizes the expected utility of bidder $i$, given his valuation distribution $F_i$, and given the strategies of his opponents and their valuation distributions, i.e. $\beta_{-i}$ and $F_{-i}$. A stronger concept is that of \emph{weak dominance}.  $\beta_i$ is weakly dominant when it is optimal in terms of expected utility of bidder $i$ against any strategies used in $\beta_{-i}$ and not only ones constituting a Bayesian Nash Equilibrium. The strongest concept is ex-post dominance, where optimality is achieved at any possible profile of valuations.
\begin{definition2}

\textbf{Nash equilibrium} 
A profile of strategies $(\beta_{1},\dots,\beta_{n})$ is \textit{a Bayesian Nash equilibrium} if for all players $i \in \mathcal{N}$, 
\begin{equation*}
\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \quad U_{i}(\beta_i,\beta_{-i},x_i)  \geq U_{i}(\beta,\beta_{-i},x_i) \;.
\end{equation*} 

\noindent \textbf{Weak dominance} A strategy $\beta_i$ is  weakly dominant for player $i \in \mathcal{N}$ if
\begin{equation*}
\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \forall \beta_{-i} \in  \mathds{B}_{-i}, \quad U_{i}(\beta_i,\beta_{-i},x_i)  \geq U_{i}(\beta,\beta_{-i},x_i) \;.
\end{equation*}

\noindent \textbf{Ex-Post Weak dominance} A strategy $\beta_i$ is  ex-post weakly dominant for player $i \in \mathcal{N}$ if
\begin{equation*}
%\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \forall \beta_{-i} \in  \mathds{B}_{-i}, \forall x_{-i} \in \mathcal{X}^{N-1},\quad u_{i}((\beta_1(x_1),\dots,\beta_i(x_i),\dots,\beta_N(x_N)),x_i)  \geq u_{i}((\beta_1(x_1),\dots,\beta(x_i),\dots,\beta_N(x_N)),x_i) \;.
\forall \beta \in \mathds{B}_i, \forall x_i \in \mathcal{X}, \forall \beta_{-i} \in  \mathds{B}_{-i}, \forall x_{-i} \in \mathcal{X}^{N-1},\quad u_{i}((\beta_i(x_i),\beta_{-i}(x_{-i})),x_i)  \geq u_{i}((\beta(x_i),\beta_{-i}(x_{-i})),x_i) \;.
\end{equation*}
\end{definition2}

%
%
%A strategy which is optimising the expected utility of one bidder for any valuation and for any strategies of the other bidders is said dominant. 
%\begin{definition2}[(Weakly) dominant strategy]
%A strategy $\beta^{*}$ is  ex-post weakly dominant for player $i$ if for all $\beta_{-i} \in  \mathds{B}^{N-1}$, for all $\beta \in \mathds{B}$ and for all $x \in X^{N}$:
%
%\end{definition2}

\nek{Maybe say that this is all formulated in interim} Those properties of strategies are classical concepts in game theory. On the other hand, it is also possible to introduce and study different properties of mechanisms. Some of them require the concept of \emph{``truthful bidding''} which correspond to the specific strategy $\beta_i(x)= x$. We will denote by $\beta_{tr}$ this truthful strategy.


\textbf{Characterization of mechanisms}
\begin{definition2} A mechanism is
\begin{description}
\item[(BIC)] Bayesian Incentive-Compatible:  if all bidders bidding truthfully is a Bayesian Nash equilibrium.
\item[(DSIC)] Dominant Strategy Incentive-Compatible:  if bidding truthfully is a weakly dominant strategy for all bidders.
\item[(Standard)] if it allocates the item to the buyer with the highest bid.
\item[(Efficient)] if it allocates the item to the buyer with the highest valuation (at least for some equilibrium).
\item[(IR)]  interim Individually-Rational: if 
\begin{equation*}
\forall \, i \; \forall x_i \in \mathcal{X}_i, \quad U_{i}((\beta_i=\beta_{tr}, \beta_{-i}=\beta_{tr}),x_i) \geq 0\;.
 \end{equation*}
 and ex-post Individually-Rational: if 
 \begin{equation*}
 \forall x_i \in \mathcal{X}_i,  \forall x_{-i} \in \mathcal{X}_{-i}, \quad u_{i}\big((x_i, x_{-i}), x_i\big) \geq 0\;.
\end{equation*}
\end{description}
\end{definition2}

A DSIC mechanism is obviously a BIC mechanism. More generally,  Incentive Compatible (IC) auctions have the nice property of being ``simple'' for the buyers from a strategic standpoint:  bidding their (known in the interim setting) valuation is optimal for them. Notice  that this unfortunately does not ensure the uniqueness of the equilibrium where each bidder bids truthfully (we will call this equilibrium the  \textsl{truthful equilibrium}). See Section \ref{sec:NashIsDifficult} for more details. \nek{move that to section \ref{sec:NashIsDifficult}} Indeed, there exist many other equilibria such as the following one: every bidder always bids 0 except one of them bidding arbitrarily high\nek{this is unclear; this is really an example with unif[0,1], one bids zero one bids one. given the strategy of the other, second price is dsic. but obviously non-uniqueness of equilibrium.Probably give this example later after intro 2nd price; and point to it now}. Those are pathological equilibria and will be discarded in the following. As we will see later on, being DSIC is one of the main reasons explaining the tremendous success of second-price auctions in practice. Another reason is that if bidders are bidding truthfully, then the seller can, in a first step, elicit their value distributions through a DSIC mechanism and then  move to another  mechanism that maximizes her revenue (this is detailed in Section \ref{Section:RevenueMax}).

% - even if it is at the cost of efficiency\nek{efficiency as in what?}.


 
\medskip
Finally, before presenting and analyzing two classical types of auction, we indicate that individual rationality simply ensures that bidders have an interest in taking part in these auctions.

\section{Sealed-bid auctions}
In a sealed-bid auction bidders privately send their bid to the seller. We present below two of the most well-known sealed-bid auctions, the second-price and the first-price auctions. This class of auctions does not include the well-known - in popular culture -  ascending auction, a.k.a English auction, where bidders can observe bids from other bidders and progressively choose to increase their bids until only one bidder remains. On the other hand,  if bidders' valuations are independent, there exists a strategic-equivalence between the ascending auction and a classical sealed-bid auction which is called the \emph{second-price auction}. % \nek{cut remaining, introduced below along with another classical sealed bid auction, the \emph{first-price auction}}. \nek{Dutch or English auction? look in krishna and specify; one is ascending the other descending}
\subsection{The sealed-bid second-price auction}
The second-price auction allocates the item to the highest bidder who pays the highest bid among other bidders, i.e. the second highest bid. A key property of this auction is the following result \citep{vickrey1961counterspeculation}, which does not require any assumption on bidders' value distributions. 

\begin{theorem2}
The second-price auction is DSIC. In other words, bidding truthfully is weakly dominant. 
\end{theorem2}
\begin{proof}
Let us denote by $x_i$ the private value of bidder $i$ and by $b^*_{-i}$ the highest bid of the competition. We are going to compare the utility of bidding  $b$ instead of $x_i$.
\begin{itemize}
\item Case $b > x_i$. The only case where his (ex-post) utility is changed is when $x_i < b^*_{-i} < b$. With a bid $b$, he now wins the auction but his utility is negative since $x_i - b^*_{-i} < 0 $.
\item  Case $b < x_i$. The only case where his (ex-post) utility is changed is when $x_i > b^*_{-i} > b$. With a bid $b$, he now loses a profitable  (i.e. with a positive utility) auction.
\end{itemize}
Hence, bidder $i$ has no incentive to deviate  from truthful bidding. 
\end{proof}
The classical second-price auction was used until recently \citep{feng2020reserve} by most of the biggest online platforms to sell ad placements on publishers' websites. Another widely used and studied sealed-bid auction is the first-price auction.
\subsection{The sealed-bid first-price auction} 
\label{first-price-auction}
The first-price auction allocates the item to the highest bidder who pays his own bid.

\medskip

Before studying Nash equilibria of symmetric first-price auction, we derive the general best reply of player $i$ to the bid distribution of the competition, specifically the distribution of the maximum bid of the competition. This result is of increasing interest to practitioners as many online auctions are now first price auctions.

\begin{proposition2}\label{Prop:BestReply1st}
	Call $G_i$ the cdf of the highest bid of the competition of bidder $i$, i.e. $\max_{j\neq i} b_j$. 
In a sealed-bid first price auction, a best response of bidder $i$  to $G_i$ is 
\begin{equation*}\label{eq:bestresponsefirstpriceSemiAbstract}
\beta(x_i):  \beta(x_i)=b(x_i) \text{ where } b(x_i)\in \argmax_{b \in \mathbb{R}} G_i(b)(x_i-b)\;.	
\end{equation*}
When $G_i$ is log-concave and $G_i(x_i)>0$, the best response is unique. 

Suppose further that $G_i$ has a pdf $g_i$. Call $a_i=\max_{t \in \mathbb{R}}\{t: G_i(t)=0\}$ 
First order conditions, also give, if $G_i(x_i)>0$, 
\begin{equation*} \label{eq:bestresponsefirstprice}
\beta_i(x_i)=b(x_i), \text{ where } b \text{ is a solution of } b + \frac{G_{i}(b)}{g_{i}(b)}= x_i \text{ on } [a_i,x_i]\,.
\end{equation*}
If $G_i(x_i)=0$ a best response is $\beta_i(x_i)=x_i$.

 \end{proposition2}
Calling $Y_{-i}$ a random variable with cdf $G_i$, it can also be shown that under mild technical conditions that $\beta_i$ is increasing and satisfies the equation $\beta_i(x)=\Exp{\beta_i^{-1}(Y_{-i})|Y_{-i}\leq \beta_i(x)}$. We also have the following interesting corollary.

\begin{corollary2}\label{coro:1stPriceNotBIC}
Proposition \ref{Prop:BestReply1st} implies that the first price auction is in general not BIC.	
\end{corollary2}
The corollary follows by simply showing that the best response of bidder $i$ when all other bidders bid truthfully (and hence the top bid of the competition is the largest value of the other bidders) consists in bidding something else than $x_i$. If $G_i(x_i)>0$ it follows immediately than they are better strategies than bidding $b_i=x_i$~: for instance, take any $\tilde{b}_i$ such that $G_i(\tilde{b}_i)=G_i(x_i)/2$ ($\tilde{b}_i$ exists by continuity of $G_i$ and $G_i(a_i)=0$). The utility of bidder $i$ is strictly positive at $\tilde{b}_i$ and is 0 at $x_i$. 
\begin{proof}
Let us denote by $B_{-i}$ the random variable corresponding to the maximum bid of the competition of bidder $i$, so that its cdf and pdf are $G_i$ and $g_i$. Note that $a_i$ is a max as $G_i$ is continuous and non-decreasing. 

When bidder $i$ has private value is $x_i$ and bids $b_i$, the utility he derives from the auction is $u_i(b_i,x_i)=(x_i-b_i)\mathds{1}\{b_i>B_{-i}\}$; in other words, it is his value minus his cost when he wins the auction and zero otherwise. 

We denote by $\mathcal{U}_i(b_i,x_{i}):\mathds{R}^{+}\times\mathds{R}^{+}\rightarrow \mathds{R}$ the associated expected utility of bidder $i$ when his private value is $x_i$ and he bids $b_i$. We have 
$$
\mathcal{U}_i(b_i,x_i) = \mathds{E}_{B_{-i}}\Big[(x_i-b_i)\mathds{1}\{b_i>B_{-i}\}\Big] = G_i(b_i)(x_i-b_i)\;.
$$
A best response is therefore any $b(x_i)\in \argmax_{b\in \mathds{R}^+}G_i(b)(x_i-b)$. Note that when $G_i$ is log-concave and $G_i(x_i)>0$, we can verify by inspection that $\mathcal{U}_i(b_i,x_i)$ is strictly log-concave in $b_i$ on $[a_i,x_i]$  and therefore it has a unique maximum on this interval \citep{boydvandenberghe04}. (This property follows also immediately from the definition of a strictly concave function.)

Note that since $G_i$ has a pdf, it is continuous and differentiable and therefore so is $\mathcal{U}_i(b_i,x_i)$ as a function of $b_i$. 
The derivative with respect to $b_i$ is then equal to 
$$
\frac{\partial \mathcal{U}_i}{\partial b_i}(b_i,x_i) = g_i(b_i)(x_i-b_i) - G_i(b_i).
$$
Let us assume that $G_i(x_i) >0$, then $\mathcal{U}_i(x_i,x_i)=0$ but $\left.\frac{\partial \mathcal{U}_i(b_i,x_i)}{\partial b_i}\right|_{b=x_i} <0$. This first implies by continuity that there exists  bids where the utility is positive. Rolle's theorem applied to $t\mapsto G_i(t)(x_i-t)$ also gives the existence of a stationary point $b_i^* \in  [a_i,x_i]$ where  $\frac{\partial \mathcal{U}_i}{\partial b_i}(b^*_i,x_i) =0$, as $\mathcal{U}_i(a_i,x_i)=0$, too. Note that $ \mathcal{U}_i(b_i,x_i)\geq 0$ on $[a_i,x_i]$.
Since our argument above shows that $\mathcal{U}_i(b_i,x_i)$ is positive in a neighborhood of $x_i$, we can assume that $b_i^*$ is chosen so that $\mathcal{U}_i(b_i^*,x_i)>0$. If $g_i(b^*_i)=0$ then necessarily $G_i(b^*_i)$ is also equal to 0 and $\mathcal{U}_i(b_i^*,x_i)$ would be equal to 0. This contradicts the fact that $b^*_i$ maximizes the utility, as we have shown that there exists points of positive utility.

The case where $G_i(x_i)=0$ is trivial as bidder $i$ cannot have a positive utility (recall that $G_i$ is a non-decreasing and non-negative function, so $0\leq G_i(b_i)\leq G_i(x_i)$ if $b_i\leq x_i$). Bidding $x_i$ is then optimal.
\end{proof}


There is a very rich line of work focusing on deriving Nash equilibria in first-price auctions when bidders have different value distributions. This involves solving complex systems of coupled first-order differential equations (at least with continuous value distributions, see \cite{krishna2009auction}, Section 4.3; see also p. \pageref{thm:SystemEquiAsymetricFirstPrice}). On the other hand, with symmetric bidders, i.e. with identical value distributions, it is possible to solve explicitly this system of equations and to derive the unique symmetric  Nash equilibrium with increasing strategy. From now on, we will call an Nash equilibrium  \emph{increasing} if the  strategies  are all increasing mappings. 
\begin{theorem2}%[Nash equilibrium in a first-price auction]
We assume that $n$ bidders are symmetric, independent and have a differentiable cdf, $F$, whose pdf $f$ is such that $f(x)>0$ except possibly on a set of Lebesgue measure 0 within the support of $F$. Then there exists a symmetric increasing Nash-equilibrium whose strategy is described by:  
\begin{equation*}
\beta(x) = \mathds{E}[X^{(1)}_{-i} | X^{(1)}_{-i} < x]\;.
\end{equation*}
where $X^{(1)}_{-i}$ the highest value among bidders except bidder $i$.
\end{theorem2}
% \nek{tech question: if we assume $f>0$ then $\beta$ is increasing and we have zero problems below. If $f\geq 0$, $\beta$ is only non-decreasing; then we have to deal with possible ties, how to break them and make sure that the PWin is $G_i(x)$. when they all bid $\beta(x_j)$ I haven't done this. this minor tech stuff would preferably done in an appendix; probably need to replace $x_j$ by $x_j^-$, i.e. the $inf_x F(x)=t$. I leave the proof with non-decreasing but worth a check}.
\textbf{Interpretation~:} the bidding strategy can be interpreted as saying that bidder $i$ should be bidding the expectation of the largest value of the competition, conditional on the fact that this value is smaller than bidder $i$'s value. 

\textbf{Technical note~:} We note that this bidding strategy can be derived from the proof of the revenue-equivalence Theorem \ref{Th:RevEquivalence}, and specifically the expected payment formula. This is another common method for finding equilibrium bidding strategies. We chose the proof presented below as we think it leads more directly to the solution.  
\begin{proof}
We assume that $n\geq 2$ otherwise there is nothing to show. Let us assume that all bidders are using the function $\beta$ described above. As we will show below, this function is increasing on the support of $F$ under our assumptions. Note furthermore that when all bidders are using the same \emph{increasing} strategy on the union of the support of their value distributions, the probability that bidder $i$ wins the auction is the same as the probability that he has the highest value. (Note that this latter statement would not always be true if the strategy were only non-decreasing.) 

Note furthermore that elementary properties of conditional expectations give, if $G_i$ and $g_i$ are the cdf and pdf of $X_{-i}^{(1)}$,
$$
\beta(x)=\beta_i(x)=\frac{\int_{0}^{x} y g_i(y) dy}{G_i(x)}=x-\frac{\int_0^x G_i(u)du}{G_i(x)}\;, \text{ whenever } G_i(x)>0\;.
$$
Under our assumptions, $G_i=F^{n-1}$ and hence $g_i(x)=(n-1)f(x)F^{n-2}(x)$. Note that under our assumptions $g_i(x)>0$ on the support of $F$ except possibly on a set of Lebesgue measure 0.  $\beta'(x)=\frac{g_i(x)\int_0^x G_i(u)du}{[G_i(x)]^2}$. Hence, restricted to the support of $F$, $\beta$ is a non-decreasing function whose derivative is 0 on a set of Lebesgue measure 0 . We conclude that $\beta$ is actually increasing on the support of $F$ under our assumptions. 

We denote by $x_i$ the private value of bidder $i$, by $b_i$ his bid and by $H$ the supremum of the support of $F$. Bidder $i$ has no incentive to bid higher than $\beta(H)$~: suppose he did bid $b>\beta(H)$. Clearly since the other bidders bid according to $\beta$, their maximum bid is lower than $\beta(H)$. Then, bidding $b$, bidder $i$'s probability of winning the auction would be 1 and his cost $x-b$. He could achieve the same probability of winning by bidding $\beta(H)$ - here we use the fact that $F_i$ is continuous for all $i$ so there are no point masses at $H$ - but his cost would be lower~: $x-\beta(H)$. Then, any other bid $b$ will satisfy $b \in [0,\beta(H)]$ and since $\beta(0) =0$ and $\beta$ continuous (because $F$ is and because of properties of conditional expectation), there exists $z \in [0,H]$ such that $b = \beta(z)$. Finally, note that the probability that bidder $i$ wins the auction when bidding $\beta(z)$ is just $G_i(z)$, since $\beta$ is increasing on the support of $F$. Therefore,
\begin{align*}
\mathcal{U}_i(\beta(x),x) - \mathcal{U}_i(b,x) &= \mathcal{U}_i(\beta(x),x) - \mathcal{U}_i(\beta(z),x)
\\&= G_i(x)\left(x - \frac{\int_{0}^{x} y g_i(y) dy}{G_i(x)}\right) - G_i(z)\left(x - \frac{\int_{0}^{z} y g_i(y) dy}{G_i(z)}\right)
\\&= x(G_i(x) - G_i(z)) + \int_{x}^{z} y g_i(y) dy = 
\int_x^z(y-x)g_i(y)dy 
\geq 0\;.
\end{align*}
This shows that the best response that bidder $i$ can use is $\beta$. Therefore, $(\beta,\dots,\beta)$ is a symmetric (increasing) Nash equilibrium.   We will prove unicity of this increasing differentiable symmetric Nash equilibrium in symmetric first-price auctions in Section \ref{sec_rev_equi}. 
\end{proof}

Unlike second-price auctions, first price auctions are not incentive compatible (see e.g. Corollary \ref{coro:1stPriceNotBIC}). As a consequence, the strategy of a bidder at an equilibrium  depends on the bidding strategy of the other bidders, and ultimately on other bidders' valuation distributions (see Proposition \ref{Prop:BestReply1st}). So in practice, computing a good or optimal bidding strategy would require estimating the distribution of the highest bid of the competition, which can be very challenging. Nevertheless, because of their relative transparency for bidders (who know ahead of time what they might pay if they win), first-price auctions are increasingly used in online advertising auctions\nek{Thomas: tu peux mettre une ref \`a Lahaie ou Feng?}. However, optimal bidding becomes much more complex for bidders than it is in second price or other BIC/DSIC/``truthful'' auctions.
\paragraph{Nash equilibrium in the asymmetric case}

Asymmetric first price auctions are much more intricate than symmetric ones as  the equilibrium strategy of each  bidder depends in a very subtle manner of the other bidders' strategies  \citep{LebrunFirstPriceAsymmetric1999}. Indeed, let us assume that the distributions $F_1,\ldots,F_n$ are supported on $[h,H]$, have a density  bounded away from 0 on $(h,H)$ and possibly have a point mass  at $h$. 
%This assumption comes from practical  -- as many auctions have 0 value to online advertisers -- and technical -- if a common reserve price is set at $r>h$, then distributions can be assumed to be  supported on $[r,H]$ with a point mass at $r$  \citep{LebrunFirstPriceAsymmetric1999}. 
\begin{theorem2}[\citep{LebrunFirstPriceAsymmetric1999}]\label{thm:SystemEquiAsymetricFirstPrice}
Under these  assumptions, there exist deterministic Nash equilibrium strategies that are increasing. Let us denote them by $\beta_i$ and by $x_i(b)=\beta_i^{-1}(b)\geq b$ their inverse, i.e. the value inducing the bid $b$. Then the increasing functions $b\rightarrow x_i(b)$ solve  the system of differential equations : 
\begin{equation}\label{eq:equilibrium1stPriceAsymmetric}
\forall \, i \;, 1\leq i \leq n\;, \frac{\partial}{\partial b}\log(F_i(x_i(b)))=\frac{-1}{x_i(b)-b}+\frac{1}{n-1}\sum_{j=1}^n \frac{1}{x_j(b)-b}\;. 
\end{equation}	
When the distributions are without atoms, the boundary conditions are 
$x_i(h)=h$ for all $i \in \mathcal{N}$, and there exists $\eta>0$ such that for all $i$, $\beta_i(H)=\eta$. 
\end{theorem2}
The boundary conditions mean that bidders bid their value at $h$ and have a common maximal bid \citep{FibichGaviousAsymmetricFirstPricePerturbApproach2003}.
\paragraph{Numerical issues in computing Nash equilibrium}
Finding the solution to the differential system \eqref{eq:equilibrium1stPriceAsymmetric} is considered hard essentially because the solutions are unstable near the boundary \citep{MarshallNumericalAnalysis1stPrice94}. The case of $n=2$ bidders has received a fair amount of attention both from both theoretical and numerical perspectives \citep{FibichGaviousDynamicalSystem2012}. Another approach finds yet another form of the differential system of equations and expands the functions appearing in it in a fixed polynomial basis.  \citep{NumericalSolutionsFirstPriceGayle2008}. 
\section{A revenue equivalence theorem}
\label{sec_rev_equi}
Revenue equivalence theorems are general results showing that different auction systems  -- sharing nonetheless some properties -- are equivalent in terms of expected revenue \emph{at a specific equilibrium}.  The first revenue equivalence theorem showed that the sealed-bid second-price auction and the ascending/English auction lead to the same revenue for the seller \citep{vickrey1961counterspeculation}. This result was later extended to all standard auctions - under rather minimal assumptions. 



\begin{theorem2}%[Revenue equivalence]
\label{Th:RevEquivalence}
Consider the family of auctions that are both

 i) \textsl{standard} (i.e. the winner is the bidder with the highest bid)

 ii) \textsl{0-rational} (i.e. winning the auction with a bid of 0 induces a payment of 0).

\noindent When all bidders have the same value distribution and their bids are statistically independent, i.e. in the symmetric case, the seller's expected revenue and bidders' expected utilities at a symmetric increasing Nash equilibrium are independent of the  specific payment rule. 
\end{theorem2}
\begin{remark2} The revenue equivalence Theorem \ref{Th:RevEquivalence} applies in particular to first and second price auctions, in the symmetric case where all bidders have the same value distribution \citep{Myerson81} and use an increasing strategy at equilibrium. The revenue equivalence theorem assumes that bidders have all the same value distributions. There exists asymmetric cases where the first-price auction brings more revenue than the second-price auction and vice-versa (\cite{krishna2009auction}, Section 4.3.2). 
\end{remark2}
\begin{proof} 
Given a specific standard auction, let $\beta$  be a  strategy at an increasing symmetric Nash equilibrium. Let us denote by $P(t)$ the corresponding expected payment of player $i$ when he bids $\beta(t)$ and the other bidders are using the same strategy $\beta$. As before, we  denote by $G_i$ the distribution of $X^{(1)}_{-i}$, the highest value among all the bidders except bidder $i$. Using the fact that $\beta$ is increasing, that all players use this strategy - we are at a Nash equilibrium -  and the fact that the auction is standard, the probability that bidder $i$ wins when he bids $\beta(t)$ is $G_i(t)$.

We can still assume that a deviation of bidder $i$ consists in  bidding $\beta(z)$ instead of $\beta(x_i)$ (because the auction is standard and $\beta$ is increasing).  In particular, the expected utility for bidder $i$ of this deviation can be written as
\begin{align*}
\mathcal{U}_i(z,x_i) = x_iG_{i}(z) - P_i(z)\;.
\end{align*}
% If $p_i(t,x_{-i})$ is the payment of bidder $i$ when bidding $\beta(t)$ and the other players have value $x_{-i}$,
% $$P_{i}(t) =  \mathds{E}_{F_{-i}}\Big[p_i(t_i,x_{-i})\Big] = \int_{\mathcal{X}_{-i}} p_i(t,x_{-i})f_{-i}(x_{-i})dx_{-i} \;.$$

Since $\beta$ is a strategy corresponding to a Nash equilibrium, bidder $i$'s expected utility is maximized when he bids $\beta(x_i)$ and hence 
$$
\mathcal{U}_i(x_i,x_i) =\max_{z} \mathcal{U}_i(z,x_i) =\max_{z}  \, x_iG_i(z) - P_i(z)  \;.
$$
We denote ${\mathcal V}(x_i)=\mathcal{U}_i(x_i,x_i)$. 
Clearly $x_i \mapsto \mathcal{V}_i(x_i)$ is convex - as a max of linear and hence convex functions - and hence almost everywhere differentiable \citep{HULLbook01}, p. 115). Recall also that (Lemma 4.4.1 in \citep{HULLbook01}, p. 188) the subdifferential at a point $x$ of a supremum of convex functions contains the convex hull of the subdifferentials of the functions achieving this supremum (and is empty if the supremum is not achieved). Here the functions we consider have a very simple differential in $x$: it is simply $G_i(z)$. This suggests informally that when $\mathcal{V}$ is differentiable, ``${\mathcal V}'(x)=G_i(z^*(x))$", where $z^*(x)=\argmax_z \mathcal{U}_i(z,x)$. In particular in our case it suggests that ``${\mathcal V}'(x)=G_i(x)$". The envelope theorem allows us to make this intuition formal. 

The envelope Theorem in its Theorem 2 form in \citep{MilgromSegal2002} applies because $\mathcal{U}_i(z,\cdot)$ is linear for all $z$ and hence differentiable and therefore absolutely continuous. Furthermore $\frac{\partial \mathcal{U}_i(z,x)}{\partial x} =G_i(z)\in[0,1]$ for all $z$. Since the max of $z\mapsto \mathcal{U}_i(z,x_i)$ is attained for $z=x_i$ because we are at a Nash equilibrium, the envelope theorem then gives 
$$
{\mathcal V}(x)-{\mathcal V}(0)=\int_0^{x}G_i(u)du\;.
$$
However, almost by definition, ${\mathcal V}(x)-{\mathcal V}(0)=xG_i(x)-P_i(x)+P_i(0)$. 
Thus, since $P_i(0)=0$ because of 0-rationality, we finally get that
$$
P_i(x)=P_i(0)+xG_i(x)-\int_0^x G_i(u)du = \int_0^x tdG_i(t) dt=G_i(x)\mathds{E}[X^{(1)}_{-i}|X^{(1)}_{-i} < x]\;.
$$
Note that the second equality comes from integration by parts. 
\iffalse
\nek{I changed the argument to above}
Assuming differentiability, it  holds that, since $\mathcal{U}_i(z,x_i)$ attains its maximum at $x_i$, 
\begin{equation*}
\left.\frac{\partial \mathcal{U}_i}{\partial z} (\cdot,x_i)\right|_{z=x_i} = x_ig_i(x_i) - P_i'(x_i) = 0\;.  
\end{equation*}
Thus, since $P_i(0)=0$ because of 0-rationality, we finally get that
\begin{equation*}
P_i(x) = P_i(0) + \int_{0}^{x} sg_i(s)ds = G_i(x)\mathds{E}[X^{(1)}_{-i}|X^{(1)}_{-i} < x]\;.
\end{equation*}
In the case where $\mathcal{U}_i$ is not everywhere differentiable, the same argument holds using standard mean-value theorems for the subdifferential \citep{HULLbook01}, pp.178-180. \nek{check with Thomas, Vianney, Clem} \nek{note to thomas: there's a slight confusion around the function of the first variable and the function $\gamma(x_i)=\mathcal{U}_i(x_i,x_i)$}
\nek{keep below}
\fi
Hence the expected payment of bidder $i$ is independent of the specific auction format. As a consequence, so are  the expected seller's revenue and the expected utility of bidder $i$, because the auction is standard.
\iffalse
Finally, we assumed in the proof that $P$ is  differentiable (for the sake of simplifying the exposition). This assumption is not necessary and can be removed using the convexity of $x_i \mapsto \mathcal{U}_i(x_i,x_i)$ in a way that is similar to the proof of the more general Theorem \ref{Th:MyersonLemma}. \nek{je pense qu'il faut faire très gaffe; l'exemple d'Hartline a un payoff discontinu (a l'equilibre je sais pas parce que son contre example est faux)}
\fi

\textbf{Remark:} a more informal but perhaps more intuitive derivation of this result is the following. Assuming differentiability of $P_i(z)$ and $G_i(z)$, it holds that, since $\mathcal{U}_i(z,x_i)$ attains its maximum at $x_i$, 
\begin{equation*}
\left.\frac{\partial \mathcal{U}_i}{\partial z} (\cdot,x_i)\right|_{z=x_i} = x_ig_i(x_i) - P_i'(x_i) = 0\;.  
\end{equation*}
Thus, since $P_i(0)=0$ because of 0-rationality, we get 
\begin{equation*}
P_i(x) = P_i(0) + \int_{0}^{x} sg_i(s)ds = G_i(x)\mathds{E}[X^{(1)}_{-i}|X^{(1)}_{-i} < x]\;.
\end{equation*}
\end{proof}

\begin{remark2} This proof shows a principled way to get necessary conditions on bidding strategies forming an increasing Nash equilibrium, through the payment formula derived above.  \end{remark2}

\subsubsection{Informal derivation of symmetric first-price auction equilibrium strategy} Denote by $\beta$ the common strategy of an increasing Nash equilibrium of the first-price auction, postulated at this point for this informal derivation to exist. Note that by symmetry, we have $G_j=G_i=G$ for all $i,j$ and similarly for the pdfs. So we use the notations $G$ and $g$ for cdf and pdf below. Conducting the same computations as in the proof of Theorem \ref{Th:RevEquivalence}, assume that all bidders  but $i$  follow $\beta$ and that bidder $i$ is bidding $\beta(z)$ instead of $\beta(x_i)$. Then his utility rewrites in the specific case of first price auction as 
\begin{equation*}
\mathcal{U}_i(\beta(z),x_i) = (x_i - \beta(z))G(z)\;. 
\end{equation*}
$\beta$  is a  symmetric increasing Nash equilibrium, and hence the maximum utility is attained by bidding $b=\beta(x_i)$. Differentiating with respect to $z$, temporarily assuming that $\beta$ is differentiable, then yields 
\begin{equation*}
0=\left.\frac{\partial \mathcal{U}_i}{\partial z} (\beta(z),x_i)\right|_{z=x_i} = (x_i-\beta(x_i))g(x_i) - \beta'(x_i)G(x_i)\;.
\end{equation*}
Notice that the above equation can be rewritten in the more compact form
\begin{equation*}
(\beta(x)G(x))' = xg(x)\;.
\end{equation*}
Integrating the above equation and using the fact that $G(0)=0$, we can compute explicitly the symmetric equilibrium strategy
\begin{equation*}
\beta(x) = \frac{\int_{s=0}^{x}sg(s)ds}{G(x)}= \mathds{E}[X^{(1)}_{-1}|X^{(1)}_{-1}<x]\;.
\end{equation*}
We can verify as posteriori that $\beta$ is differentiable and increasing when $g>0$. 

This also proves the uniqueness of  increasing differentiable Nash equilibria  in a symmetric first-price auction. 



% \begin{remark2} The system of equations corresponding to the Nash Equilibrium in the asymmetric setting presented in Theorem \ref{thm:SystemEquiAsymetricFirstPrice} can actually be easily deduced by applying the same perturbative approach.\nek{this is very unclear; we should drop it I think or do it} \end{remark2}

\section{Deriving revenue-maximizing auctions}
\label{Section:RevenueMax}
We now focus on how the seller can design her auction system to maximize her revenue. A large part of the recent literature on auctions have focused on this objective since most of the auctioneers have a choice in designing the rules of their respective auction platforms.

To compute the optimal revenue-maximizing auction, we assume that the seller has prior knowledge on the distribution $F_i$ on each bidders' valuations.  These value distributions quantify the information that the seller has on each bidder. 

\subsection{The role of reserve prices}
Setting reserve prices is a crucial tool used to improve or maximize seller's revenue in classical auctions. To illustrate its role, we focus on  second-price auctions. 
\begin{definition2}
The reserve price is the minimum price a bidder must pay to acquire an  item. The reserve price is  \textit{anonymous} (respectively \emph{personalized}) if it is the same for all bidders (if it is different from one bidder to the other).
\end{definition2}
In a second-price auction with reserve prices the buyer that wins the auction must have bid above his reserve price. He then pays the maximum between his reserve price and the second highest bid. A crucial and perhaps surprising point  is that, in expectation,  it can be beneficial for the seller to sometimes not allocate the item. However, whenever the item is sold, the payment is higher because of the reserve price than it would have been without reserve price. 

To illustrate this point, we quickly recall a historical example, the New-Zealand radio spectrum rights auction \citep{milgrom2004putting}. In 1990, the NZ government decided to sell some radio spectrum rights through multiple simultaneous sealed-bid second-price auctions without reserve prices for the corresponding licenses. These auctions were expected to raise around NZ\$250 million. Instead, the government revenue was around NZ\$36 million. On many licenses, there was a huge discrepancy between the first and the second bid. For instance, a firm bid NZ\$100 000 and the second price was only NZ\$36\dots If reserve prices had been set beforehand, it would have ensured to the government that the firm who made a bid of NZ\$100 000 would have paid a price sufficiently high. 

This example illustrates the importance of reserve prices. A first way to set a reserve price would be to assume that the seller can compute an intrinsic value for keeping the item. This could be a reasonable assumption for housing or wine auctions. However, in many other situations (TV rights, radio spectrum rights auctions..), the seller does not have any intrinsic value for the item. To give an example, we compute the optimal reserve price in the simple case of a single buyer. As before, we denote by $F$ the cdf of the buyer valuation, and for the sake of simplicity, we assume it has a density $f$ (again, all the following results generalize to arbitrary distributions, but at the cost of technicalities) and has finite expectation.


%\iffalse and the need for a careful modelisation of the different incentives of the system. {\color{red}VP: la phrase suivante est moche, et il faut une reference et/ou plus d'explications} For instance, in the recent sell of French football TV rights, in 2017, the auctioneer was very careful on its definition of the reserve prices by setting very specific reserve prices for every TV rights packages. 
%\fi
\subsection{The posted price setting: monopoly pricing}
\label{monopoly-pricing}
In this  particularly simple through practically very common setting, designing an auction simply reduces to  a \textit{take-it-or-leave-it} offer. In other words, a fixed selling price is offered and a rational bidder will accept to pay it to acquire the item if and only if the price is smaller than his valuation. 
\begin{lemma2}\label{TH:Monopoly}
In a posted price setting, the seller's expected revenue is 
\begin{equation} \label{eq:defPiOfr}
\Pi(r) = r(1-F(r))\;.
\end{equation}
In the same setting, when $F$ is differentiable and has one moment/finite expectation, the optimal reserve price, called \emph{the monopoly price}, is a solution of :
\begin{equation*}
0=-[r(1-F(r))]'=rf(r) - (1-F(r)) = f(r)\Big(r- \frac{1-F(r)}{f(r)}\Big)\;. 
\end{equation*}
\end{lemma2}
\begin{proof}
The seller's revenue can be written as a function of $r$ as: in expectation, the seller's revenue is just the fixed price $r$ multiplied by the probability that the buyer buys the item. This latter probability is just the probability that the value of the buyer is above $r$. Formally, if $x$ is the value of the item for the buyer, the revenue of the seller $\Pi(r)$ when selling at the fixed price $r$ is 
\begin{equation*} 
\Pi(r) = r P(x\geq r)=r \int_{r}^{+\infty} f(x)dx = r(1-F(r))\;.
\end{equation*}
The result on the monopoly price follows from differentiating the previous relation, since
\begin{equation*} 
\frac{d\Pi(r)}{dr} = (1-F(r)) - rf(r) \;.
\end{equation*}
Furthermore choosing $r=0$ or $r$ arbitrarily high gives 0 revenue, the latter because $F$ is assumed to have one moment, which then implies that $\lim_{t\tendsto \infty} t(1-F(t))=0$ by the dominated convergence theorem. Indeed, if $x$ has distribution $F$, $t(1-F(t))\leq \mathds{E}_{x\sim F}[x\indicator{x\geq t}]\leq \mathds{E}_{x\sim F}[x]<\infty$.  Hence a maximum of the function $\Pi$ exists among its stationary points, finishing the proof. 
\end{proof}
%\iffalse
%\begin{figure}[H]
%\includegraphics[width=.5\linewidth]{images/monopolistic_revenue}
%\caption{Seller's revenue as a function of the reserve price. The revenue is computed based on $r(1-F(r))$ with $F = \mathcal{U}([0,1])$.}
%\end{figure}
%{\color{red} VP: Quel est l'interet du paragraphe suivant ?} 
%The setting of posted price is very related to the setting where a monopolistic firm sells a service to different customers. She must define a single price for all her clients. She will choose the monopoly price corresponding to the distribution of values representing her customers. Sometimes, the firm prefers not to sell the item and sacrifies a bit of short-term revenue to insure that in most other cases, buyers will pay a price sufficiently high.  
%\fi
\bigskip
Notice that without the assumption that $F$ has a finite expectation, the optimal reserve price could be arbitrarily high: take for instance $F(r)=1-r^{-\alpha}$ with $0<\alpha<1$.
Such an example is relevant in markets for luxury items.
 
One of the purpose of discussing the single bidder case was to introduce organically the crucial concept of \textit{virtual value} introduced in \citep{Myerson81}. 
\begin{definition2}%[Virtual value]
The virtual value function $\psi : \mathcal{X} \to \mathds{R}$ of a distribution $F$ (with pdf $f$) is: 
\begin{equation} \label{eq:defVirtualValue}
\boxed{
\psi(x) = \psi_F(x) = x - \frac{1-F(x)}{f(x)}\;.
}
\end{equation}
\end{definition2}
The virtual value function can be either positive or negative, irrespective of the support of the value distribution. The expectation  under $F$ of the virtual value,  i.e. $\mathds{E}_{X \sim F} [ \psi(X)]$, is actually equal to the infimum of the support of $F$, when $F$ has one moment. In particular, it is equal to 0 if the support of $F$ ``starts" at 0. 
%\nek{maybe stop here; afterwards it kind of implies that $\psi_F$ is increasing...} and in that case, the virtual value is necessarily sometimes negative (at least around $x=0$) and sometimes positive (at least around the supremum of the support of $F$) \nek{latter is false unless virtual value is assumed to be increasing}.

The virtual value $\psi(x)$ is a crucial concept that can be interpreted as  \emph{virtual payment}, as we explain now. If the bidder has value $x$ and decides to buy the item, so $x\geq r$, his (virtual) payment can be thought of as $\psi(x)$,  \textsl{independently} of the price $r$ set by the seller. Indeed, the revenue generated by such a price $r$ is
\begin{gather*}
\mathds{E}_{X \sim F} [ \psi(X) \mathds{1}\{X \geq r\}]=
\int_r^\infty \psi(x) f(x)dx= \int_r^\infty xf(x) - (1-F(x)) dx \\
= -\int_r^\infty (x(1-F(x)))' dx=
r(1-F(r))=\Pi(r)\;.
\end{gather*}
The last equality comes from the definition of $\Pi(r)$, see Equation \eqref{eq:defPiOfr}. As a consequence, even though it is traditionally called virtual value, $\psi(x)$ could rather be understood as a virtual \textsl{payment}~: the buyer pays on average $\psi(x)$ when his value is $x$ and he buys/wins the item, i.e. $x\geq r$. See also Proposition \ref{prop:virtualValueIsVirtualPaymentGeneralCase} for an explanation of why this interpretation holds for general auction systems and buyers optimizing their expected utility.

\subsubsection{Examples of virtual value functions:} 
\begin{itemize}
\item if $x\sim\mathfrak{U}([0,1))$, the uniform distribution over $[0,1]$, then $\psi(x)=2x-1$ for $x \in [0,1]$.
\item if $x\sim \mathfrak{E}\mathrm{xp}(\lambda)$, the exponential distribution, then  $\psi(x)=x-\lambda$ for $x \in \mathds{R}_+$ ($F(x)=1-\exp(-x/\lambda)$).
\item Generalized Pareto (GP) distributions, parametrized by $(\mu,\sigma,\xi)$ where $\sigma >0$ and $\xi\leq 0$, have cdf 
\begin{equation*}
F_{\mu,\xi,\sigma}(x)   = \begin{cases} 1-(1 +\frac{\xi (x-\mu)}{\sigma})^{-1/\xi} & \text{for } \xi < 0 \\
1-e^{-(x-\mu)/\sigma} & \text{for } \xi= 0\end{cases}\;.
\end{equation*} 
Their virtual value is affine \citep{balseiro2020multistage}
$$\psi_{\mu,\xi,\sigma}(x) = (1-\xi)x+\xi\mu-\sigma$$
\end{itemize}
%\begin{remark2}
%With $\xi = -1 , \mu = 0, \sigma = 1 $, we recover the uniform distribution. With $\xi = 0 , \mu = 0 , \sigma = 1$, we recover the exponential distribution. With  $ \mu = 1, \sigma = \xi$ , this corresponds the power law (a.k.a the Pareto distribution) with parameter $\alpha = 1/\xi$. Hence, the generalized Pareto distribution are widely used in auction theory due to their flexibility (they model a large spectrum of distributions) and the fact that their virtual value is easy to compute (the virtual value is affine).
%\end{remark2}
\subsubsection{Relationship between  monopoly price and virtual value/payment}
Lemma \ref{TH:Monopoly} states that the optimal reserve price against  a single bidder (which was called the monopoly price)  is, in the case where the virtual value/payment function  $\psi$ is increasing and changes sign, necessarily the root of $\psi$ (or the point where the sign changes if $\psi$ is not continuous). If $\psi$ is strictly positive everywhere, which can happen if the  infimum of the support of $F_i$ is positive, then the optimal reserve price is that specific point (or equivalently 0). Note that if $\Pi(t)$ is the expected revenue of the seller at reserve price $t$ (see Equation \eqref{eq:defPiOfr}), $\Pi'(t)=-f(t)\psi(t)$.  Quite interestingly, even with multiple other bidders, the optimal reserve price for bidder $i$ is still $i$'s monopoly price, i.e. the same as if he were the only bidder. This is illustrated in the following Section \ref{optimal_reserve_for_lazy} under the same assumptions of $\psi$ being increasing and/or changing sign once. 

As a consequence, in the following,  our main focus will be on these distributions which are called \textsl{regular}. The results we will prove can be generalized to non-regular distribution with a technique called \textsl{ironing}, see Section \ref{Se:Ironing}.  
 \begin{definition2} 
The distribution $F$ is  regular if the corresponding virtual value $\psi$ is increasing.
\end{definition2}

\textbf{Examples }The uniform, exponential and generalized Pareto distributions with $\xi <1$, are all regular distributions. % 
%\begin{proposition2}
%If $\psi$ increasing and crossing zero exactly once and F is defined over its full support, then r is the monopoly price if and only if
%$$\psi(r) = 0$$ 
%\end{proposition2}
%\begin{proof}
%The monopoly price r is defined as $$\argmax_r R(r) = r(1-F(r)).$$
%Then, 
%$$
%\frac{dR(r)}{dr} = -f(r)\psi(r)\;.
%$$
%Since $\psi$ increasing, R is concave and $\psi(r)=0$.
%\end{proof}
%If $\psi$ is crossing zero multiple times, the monopoly price also verifies $\psi(r)=0$. 
%One of the beauty of auction theory is that this notion of monopoly price can be extended to auctions with multiple buyers.
\subsection{Optimal reserve prices in second-price auctions}
\label{optimal_reserve_for_lazy}
We  focus in this section on second-price auctions with reserve prices \citep{riley1981optimal} where  $n$ buyers are asymmetric, i.e. their value distribution can be different. As a consequence, the seller might also set different, personalized, reserve prices so as to increase her revenue. When introducing the concept of reserve price, we mentioned that a bidder can only win the auction if his bid was higher than his reserve price and that the latter is the minimal payment that bidder might pay. There however remains some ambiguity on how the auction unfolds (depending on which condition ``highest bidders" or ``bid above reserve price" is checked first). As a consequence, there exist at least two different types of second-price auction with reserve prices.

\begin{description}
\item[``Lazy" 2nd-price auction:] The winner can only be the highest bidder. He gets the item only if he  clears his reserve price (i.e. he bids above it), and pays the maximum between his reserve price and the second highest bid overall (regardless of whether the second highest bid cleared its reserve).
\item[``Eager" 2nd-price auction:] Bidders that have not cleared their respective reserve price are  disregarded. Thus the winner is the highest bidder amongst those that have cleared their reserve price and he pays the maximum between his reserve price and the second highest cleared bid.
\end{description}


First of all, notice that if the reserve prices are anonymous, i.e. the same for all bidders, as they should be in the symmetric case for instance, both types of auctions coincide.  Optimal reserve prices are easy to compute in lazy auctions, as they have an explicit form. They are on the other hand hard to compute for eager auctions. Moreover, the eager 2nd-price auction is also not the revenue-maximizing auction for the seller. So this concept is neither simple (as is the lazy auction) nor optimal (as is the Myerson auction, see Section \ref{emp_Myerson}). As a consequence, we will not put too much emphasis on eager auctions. In practice, if one wishes to implement eager 2nd-price auctions, a good idea would be to use the reserve prices of the corresponding lazy 2nd-price auction.



\medskip

It is quite immediate to see that lazy and eager second price auctions are still DSIC mechanism (the proof follows the exact same lines as that without reserve prices), hence we shall again only consider the truthful equilibrium. We now derive the expected payment of a bidder at this equilibrium.
%\begin{theorem2}[Expected payment in a lazy second-price auction]\label{myerson_for_second_price}
%Consider bidder $i$ with virtual value $\psi_i$ and reserve price $r_i$. We denote by $G_i$ the cdf of $Y_{-i} = max_{j\neq i} X_j$. The expected payment $P_i(\beta_{tr})$ of bidder $i$ in a lazy second-price auction when all bidders are bidding truthfully is equal to:
%\begin{equation*}
%P_i(\beta_{tr}) = \mathds{E}_{x_i\sim F_{i}}\bigg(\psi_i(x_i)G_i(x_i)\textbf{1}_{x_i\geq r_i}\bigg)\;.
%\end{equation*}
%\end{theorem2}
\begin{theorem2}\label{myerson_for_second_price}
Let   $P_i$ be the expected payment of bidder $i$ facing reserve price $r_i$ at the truthful equilibrium of a lazy second-price auction. Assume the bidders are statistically independent. Then 
\begin{equation*}
P_i = \mathds{E}_{x_i\sim F_{i}}\Big[\psi_i(x_i)G_i(x_i)\mathds{1}\{x_i\geq r_i\|\Big]\;,
\end{equation*} 
where $G_i$ the cdf of $\max_{j\neq i} X_j$ and $r_i$ is the personalized reserve price of bidder $i$.

\end{theorem2}
\begin{proof} 
Let us introduce the notation $y_{-i}= \max_{j\neq i} x_j$ so that the pointwise payment of bidder $i$, when he has value $x_i$, given all the values $x_j$ is equal to: 
\begin{equation*}
\max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x_i\geq r_i\}\;,
\end{equation*}
We note that 
$$
\max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x_i\geq r_i\}=
\mathds{1}\{x_i\geq r_i\}(r_i\mathds{1}\{y_{-i}\leq r_i\}+\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{ y_{-i}\geq r_i\}y_{-i})\;.
$$
As a consequence,
\allowdisplaybreaks
\begin{align*}
P_i&= \mathds{E}_{F_1,\dots,F_n}\Big[\max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x\geq r_i\}\Big]
\\& = \int_{x_i} \int_{y_{-i}} \max(r_i,y_{-i})\mathds{1}\{x_i\geq y_{-i}\}\mathds{1}\{x_i\geq r_i\}f_i(x_i)g_i(y_{-i})dy_{-i}dx_i
\\& =\Big(1-F_i(r_i)\Big)G_i(r_i)r_i + \int_{x_i=r_i}^{+\infty}\int_{y_{-i}=r_i}^{+\infty}y_{-i}g_i(y_{-i})f_i(x_i)\textbf{1}(x_i \geq y_{-i})dy_{-i}dx_i
\\& = \Big(1-F_i(r_i)\Big)G_i(r_i)r_i + \int_{y_{-i} = r_i}^{+\infty}y_{-i}g_i(y_{-i})\int_{x_i=y_{-i}}^{+\infty}f_i(x_i)dy_{-i}dx_i \hspace{2cm} \text{ (by Fubini)}
\\& = \Big(1-F_i(r_i)\Big)G_i(r_i)r_i + \int_{y_{-i} = r_i}^{+\infty}y_{-i}g_i(y_{-i})(1-F_i(y_{-i}))dy_{-i} 
\\& = \int_{y_{-i} = r_i}^{+\infty} \Big(f(y_{-i})y_{-i} - (1-F_i(y_{-i}))\Big)G_i(y_{-i})dy_{-i} \hspace{2.5cm} \text{(by integration by parts)}
\\& = \mathds{E}_{F_i}\Big[\psi_i(x)G_i(x)\mathds{1}\{x\geq r_i\}\Big]\;.
\end{align*}
\end{proof}
We can therefore easily derive the optimal reserve prices, as a function of $\psi_i$ at least for regular distributions.%\begin{definition2} 
%The distribution F  is said regular if its corresponding virtual value $\psi$ is increasing.
%\end{definition2}
%\redtext{changement}
%{\color{red} VP: est-ce qu'on a besoin de ce graphique ? En plus celui en haut a droite deconne, le vert n'est pas aligne avec le trait pointille rouge}
%\begin{figure}[h!]
%\begin{tabular}{cc}
%\includegraphics[width=.50\linewidth]{images/r025}&
%\includegraphics[width=.50\linewidth]{images/r075}\\
%\multicolumn{2}{c}{\includegraphics[width=.50\linewidth]{images/r05}}
%\end{tabular}
%\caption{\textbf{Change in bidder payment as a function of the reserve price.} The value distribution of the bidder is uniform [0,1] with $\psi(x) = 2x -1$, and is represented by the blue line. The dashed red vertical line corresponds to the current reserve price. We picked $G=1$, i.e. no competition. The bidder payment is equal to the area under the curve. The seller has no incentive to set the reserve price lower than $\psi_i^{-1}(0)$ since it decreases her total expected payment (because of the negative contribution of the red area). It is also clear that $r \ge \psi_i^{-1}(0)$ is suboptimal since it results in lost revenue for the seller.}
%\label{fig:visualOptimalR} % I can do without the label too
%\end{figure}
\begin{theorem2}%[Optimal reserve price in lazy second-price auction]
If  $F_i$ are regular, the optimal reserve prices in a lazy second-price auction are:
\begin{equation*}
\bigg(r_1,\dots,r_n\bigg) = \bigg(\psi_1^{-1}(0),\dots,\psi_n^{-1}(0)\bigg)\;,
\end{equation*}
with the convention that $\psi_1^{-1}(0)$ is the minimum of the support of $F_i$ is $\psi_i$ is  positive everywhere and the point where $\psi_i$ changes its sign if it is discontinuous.
\end{theorem2}
\begin{proof} 
The seller maximizes the sum of expected payment: 
\begin{align*}
\mathds{E}_{F_1,\dots,F_N}\Big[\sum_{i=1}^{n} P_i\Big] &= \sum_{i=1}^{n}  \mathds{E}_{F_i}\Big[\psi_i(x_i)G_i(x_i)\mathds{1}\{x_i\geq r_i\}\Big]\;.
\end{align*}
Since $F_i$ is regular, $\psi_i$ has one zero and is negative before the zero and positive after. Thus, the optimal choice for $r_i$ is clearly $\psi_i^{-1}(0)$. Indeed, the function $t\rightarrow \mathds{E}_{F_i}\Big[\psi_i(x_i)G_i(x_i)\mathds{1}\{x_i\geq t\}\Big]$ is increasing before $\psi_i^{-1}(0)$ and decreasing afterwards, owing to the sign of the integrand on both sides of $\psi_i^{-1}(0)$.
\end{proof}
We see in the proof that in a lazy second-price auction, the seller can safely maximize the payment of each bidder one by one independently. Indeed, in a lazy second price auction, changing the reserve price of one specific bidder does not change the probability of winning and the payment of the other bidders. This is not the case for eager second-price auctions on the other hand, which explains the complexity of computing the optimal reserve prices in them. Finally, the optimal reserve prices in a lazy second-price auction correspond to the monopoly prices of each bidder.



\begin{corollary2}The optimal reserve price for a bidder in a lazy second-price auction is independent of the presence, or not, of other bidders. In particular, it is the same as in the situation where he is the only bidder.
\end{corollary2}

\begin{figure}[H]
\includegraphics[width=.6\linewidth]{images/optimalmonopolyprice.pdf}
\caption{Bidder's payment as a function of the reserve price depending on the number of players in second-price auction with bidders all having a uniform value distribution $\mathfrak{U}([0,1])$.}
\end{figure}
%The proof also shows that when the distribution is not regular, the optimal reserve prices for each bidder verifies: $r_i \in \argmax(\mathds{E}_{F_i}(\psi_i(x)G(x)\textbf{1}_{x\geq r_i}))$.

The seller's revenue increases through the use of personalized reserve prices when bidders have very different value distributions. Intuitively, it is in the seller's best interest to set a high reserve price to bidders who have high values most of the time  (or very high values some of the time) and low reserve prices to bidders who have  low values most the time.

So far, we have only focused on the seller's revenue when designing auctions. An alternative objective can be the maximization of the  \textsl{global welfare} of the system, which is the sum of the seller's revenue and all bidders' utility. 

\bigskip


Even though reserve prices largely increase the seller's revenue, they actually significantly decrease the expected total welfare, as the item will sometimes not be allocated. This happens when all bidders (or at least the highest one in lazy auctions) have values below their reserve prices.

\begin{example2}
To illustrate this decrease in welfare, we are going to consider a simple example.  There are $n=2$ symmetric bidders with a value drawn uniformly over $[0,1]$. Because of the  symmetry, the optimal reserve price is the same for both bidders hence lazy and eager auctions coincide (and we do not need to specify the rule).  In this simple case, $r^* = \psi^{-1}(0) = 1/2$. As a consequence, the item is allocated as soon as one  bidder bids above 1/2, which happens with probability $3/4$. Otherwise, the item is not sold (which obviously happens with probability $1/4$). Simple computations show that changing the design from a second-price auction without reserve price to a second-price auction with optimal reserve price yields 
\begin{itemize}
\item a \textbf{12,5 \% decrease} of the global welfare (from $2/3$ to $7/12$).
\item a \textbf{50 \% decrease} of every single  bidder's utility  (from $1/6$ to $1/12$).
\item a \textbf{25 \%  increase} of the seller's revenue (from $1/3$ to $5/12$).
\end{itemize}
\end{example2}
\subsection{Myerson's lemma and characterization of BIC and DSIC auctions}
We mentioned before that the virtual value could (and maybe should) be understood as a virtual payment in a single bidder auction and/or in lazy second price auctions. The following lemma (that will be referred to as the ``Myerson Lemma'') is a crucial result \citep{Myerson81}. It states that virtual payment of a bidder is the correct quantity to study in any  incentive-compatible auctions, and not just lazy second-price ones. The proof, while conceptually profound, is not very hard technically and requires integration by part and Fubini's theorem as we used in the case of the lazy second-price auction. This result holds for any Bayesian Incentive Compatible auction (if bidding truthfully is weakly dominant) that is 0-rational (if bidding 0 ensures a payment of 0). The latter assumption can be weakened, at the cost of an additive constant in the payment formula. 
\begin{theorem2}%[Myerson lemma]
\label{Th:MyersonLemma}
For any BIC and 0-rational auction, the expected payment of bidder $i$ at the truthful equilibrium is 
\begin{equation*} 
\mathds{E}_{x_i\sim F_i}[P_i(x_i)] = \mathds{E}_{x_i \sim F_{i}}[\psi_i(x_i)Q_i(x_i)] = \mathds{E}_{x \sim \mathcal{F}^{(n)}}[\psi_i(x_i)q_i(x)]\;.
\end{equation*}
Here $Q_i(x_i)$ is the winning probability  of bidder $i$  at the truthful equilibrium given his value  $x_i$ and $q_i(x)$ is the probability that the item is attributed to bidder $i$ when the values are $x=(x_1,\ldots,x_n)$. 
\label{myerson_lemma}
\end{theorem2}
\begin{proof}
We consider the case where we are at the truthful equilibrium of the BIC auction. In particular, we assume that all bidders except possibly $i$ bid their values, i.e. they bid truthful. Let us call $Q_i(z)$ the probability that bidder $i$ bidding $z$ wins the auction (when all other bidders bid truthful) and $P_i(z)$ his expected payment (when all other bidders bid truthful). The expected utility of bidder $i$ when he has value $x_i$ and bids $z$ is simply $Q_i(z)x_i - P_i(z)$. 
By definition of Bayesian incentive-compatibility, at the truthful equilibrium the auction must verify: 
\begin{equation*}
\forall z \in \mathds{R}^{+}, \forall x_i \in \mathds{R}^{+}, Q_i(x_i)x_i - P_i(x_i) \geq Q_i(z)x_i - P_i(z)\;,
\end{equation*}
since at the truthful equilibrium bidder $i$ gets maximum utility by bidding his value. 
Thus, if we denote by $\mathcal{U}_i(x_i)$ the expected utility of bidder $i$ when he has value $x_i$, 
\begin{equation*}
\mathcal{U}_i(x_i) = \max_{z} Q_i(z)x_i - P_i(z) = x_i Q_i(x_i)-P_i(x_i)\;.
\end{equation*}
As a consequence, $\mathcal{U}_i$ is a  convex mapping (the maximum of affine mappings) and therefore is differentiable almost everywhere and absolutely continuous (i.e. it is equal to the integral of its derivative).

Bayesian-incentive compatibility also implies that
\begin{equation*}
\forall z \in \mathds{R}^{+}, \mathcal{U}_i(z) =\max_t zQ_i(t)-P_i(t)\geq z Q_i(x_i)-P_i(x_i)= \mathcal{U}_i(x_i) + Q_i(x_i)(z-x_i)\;.
\end{equation*}
Since $\mathcal{U}_i$ is convex, this means that $Q_i(x_i)$ belongs to the subdifferential of $\mathcal{U}_i$ at $x_i$, i.e.
\begin{equation*}
Q_i(x_i) \in \partial \mathcal{U}_i(x_i)\;,
\end{equation*}
and  $\nabla \mathcal{U}_{i}(x_i) = Q_i(x_i)$  if  $\mathcal{U}_i$ differentiable at  $x_i$. Therefore, using Theorem  D.2.3.4 in \citep{HULLbook01}, 
$$
\mathcal{U}_i(x_i)-\mathcal{U}_i(0)=\int_0^{x_i}Q_i(z)dz\;,
$$
and since $\mathcal{U}_i(x_i)=x_i Q_i(x_i)-P_i(x_i)$, 
\begin{equation*}
P_i(x_i) = P_i(0) + Q_i(x_i)x_i - \int_{0}^{x_i}Q_i(z)dz\;.
\end{equation*}
Taking expectation over $x_i$ now gives~: 
\begin{align*}
 \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] &= \int_{x_i}P_i(x_i)f_i(x_i)dx_i 
\\&=  P_i(0) + \int_{x_i} \Big(Q_i(x_i)x_i - \int_{0}^{x_i}Q_i(z)dz\Big)f_i(x_i)dx_i
\\& = P_i(0) + \int_{x_i} Q_i(x_i)x_if_i(x_i)dx_i - \int_{z}Q_i(z)\Big(\int_{z}^\infty f_i(x_i)dx_i\Big)dz \qquad \text{ (Fubini) }
\\& = P_i(0) + \int_{x_i} \Big(x_i - \frac{1-F_i(x_i)}{f_i(x_i)}\Big)Q_i(x_i)f_i(x_i)dx_i 
%\\&= P_i(0) + \int_{x} \Big(x_i - \frac{1-F_i(x_i)}{f_i(x_i)}\Big)q_i(x)f(x)dx
\\& =  
 P_i(0) + \mathds{E}_{x_i \sim F_i}[\psi_i(x_i)Q_i(x_i)]\;.
% P_i(0) + \mathds{E}_{x \sim \mathcal{F}}[\psi_i(x_i)q_i(x)] =
\end{align*}
The result follows from the fact that $P_i(0) =0$ since the auction is 0-rational.

The last equality comes from the fact that $Q_i(x_i)= \mathds{E}_{x \sim \mathcal{F}^{(n)}}[q_i(x)|x_i]$ and the tower property of conditional expectations.
\end{proof}
\begin{remark2}
Notice that Theorem \ref{myerson_for_second_price} is a direct consequence  of this result with the specific choice of $Q_i(x_i) = G_i(x_i)\mathds{1}\{x_i\geq r_i\}$.
\end{remark2}
Myerson's lemma indicates that the expected payment of a 0-rational BIC auction only depends on the allocation rule and the virtual value; the proof actually gives a characterization of any incentive-compatible auction.  However, this characterization is slightly different for  BIC and DSIC auctions. 
\nek{Thomas: in coro below, do we need the auction to be 0-rational? }
\begin{corollary2}%[characterization of BIC auctions]
[\cite{Myerson81}]
\label{characterization_inc_comp}
Using the notations of Theorem \ref{Th:MyersonLemma}, an auction is BIC if and only if
\begin{itemize}
\item[i)] the allocation rule is monotone, i.e.  the probability of winning, as a function of the bid, is non-decreasing (for any fixed bids of others bidders)  and
\item[ii)] the expected payment verifies 
$$P_i(x_i) = Q_{i}(x_i)x_i - \int_{0}^{x_i} Q_{i}(z)dz.$$
\end{itemize}
\end{corollary2}
\begin{proof} 
The proof of Theorem \ref{myerson_lemma} gives the first implication. For the reverse, 
let us assume that all bidders except $i$ bid truthfully; and let us show that $i$ has an incentive to also bid truthfully. This will show that truthful bidding constitutes a Nash equilibrium and hence the auction is BIC. 

Note that because we have assumed that all other bidders bid truthfully, if bidder $i$ bids $z$, the probability that he wins is $Q_i(z)$. Hence, the expected utility derived by bidder $i$ when bidding $z$ and his value is $x_i$ is 
$$
\mathcal{U}_i(z,x_i)=x_i Q_i(z)-P_i(z)=(x_i-z)Q_i(z)+\int_0^z Q_i(t) dt\;.
$$
The second equality comes from assumption ii). 
Let us call $b_i^*$, the optimal bid of bidder $i$. 
% \nek{version 1}
% $b_i^*$ satisfies
% $$
% b_i^*=\argmax_z (x_i-z)Q_i(z)+\int_0^z Q_i(t) dt\;.
% $$
% Let us now show that $b_i^*=x_i$, which would conclude the proof.
% Consider the function $H: y\mapsto \int_0^y Q_i(t) dt$\;. This function is differentiable, with derivative $H'(y)=Q_i(y)$; as a consequence of assumption i) it is convex, since $Q_i(y)$ is non-decreasing in $y$. Therefore it is above all of its tangents, i.e~:
% $$
% \forall z\;, H(x_i)\geq H(z)+(x_i-z)H'(z)=H(z)+(x_i-z)Q_i(z)\;.
% $$
% In other words,
% $$
% \forall z\;, \mathcal{U}_i(x_i,x_i)=\int_0^{x_i}Q_i(t)dt\geq (x_i-z)Q_i(z)+\int_0^z Q_i(t) dt=\mathcal{U}_i(z,x_i)\;.
% $$
% This shows that $b_i^*=x_i$ and the auction is BIC.
%
% \nek{alternative}
Let us now show that $b_i^*=x_i$. To do so, we simply need to establish that 
$$
\forall z\;, \mathcal{U}_i(x_i,x_i)=\int_0^{x_i} Q_i(t) dt \geq (x_i-z)Q_i(z)+\int_0^z Q_i(t) dt\;.
$$
This is equivalent to showing that 
$$
\forall z\;, \int_z^{x_i} Q_i(t) dt \geq (x_i-z)Q_i(z)\;.
$$
If $z\leq x_i$, since $Q_i$ is non-decreasing, $Q_i(t)\geq Q_i(z)$ on $[z,x_i]$ and hence 
$$
\int_z^{x_i} Q_i(t) dt \geq (x_i-z)Q_i(z)\;.
$$
If $z\geq x_i$, since $Q_i$ is non-decreasing, $Q_i(t)\leq Q_i(z)$ on $[z,x_i]$ and hence
$$
\int_{x_i}^z Q_i(t) dt \leq (z-x_i) Q_i(z)\;.
$$
Multiplying the previous inequality by $(-1)$ on both sides shows that if $z\leq x_i$, we also have 
$$
\int_z^{x_i} Q_i(t) dt \geq (x_i-z)Q_i(z)\;.
$$
So we have shown that 
$$
\forall z\;, \mathcal{U}_i(x_i,x_i)\geq \mathcal{U}_i(z,x_i)\;.
$$
Therefore, bidding truthfully is an optimal strategy for bidder $i$ and the auction is BIC. (Note that the inequalities needed also follow from realizing that the function $H: y\mapsto \int_0^y Q_i(t) dt$ is convex.)
%
% if the auction verifies
% $$P_i(x_i) = Q_{i}(x_i)x_i - \int_{0}^{x_i} Q_{i}(z)dz\;,$$
% then it implies that the auction verifies  $\nabla \mathcal{U}_i(x_i) = Q_{i}(x_i)$.\nek{do you mean this with subdifferentials?}
% \nek{I don't understand below}
% Since the probability of winning is increasing as a function of the bid, $$\mathcal{U}_i(x_i) - \mathcal{U}_i(z) = \int_{x_i}^{z}Q_{i}(s)ds \geq Q_i(x_i)(z - x_i)$$ which entails that $$\mathcal{U}_{i}(x)\geq Q_i(z)x - P(z).$$ This is the definition of bayesian incentive-compatibility (BIC).
%
%
% \nek{alternative}
% not clear yet that we know the gradient of $U_i$.
%
% Increasing allocation+others are truthful means $PWin(z)=Q_i(z)$ if we use $z$ instead of $x_i$ in $\beta(z)$.
%
% Now optimal strategy means $U_i(x_i)=\max_z x_iQ_i(z)-P(z)$. use convexity.
%
% see krishna pp.64-65 and possibly 69.
%
% Since the probability of winning is increasing as a function of the bid, the function
% $\mathcal{U}_i(x_i)$ is convex since its derivative is increasing. It is in particular above all of its tangents, hence
% $$
% \forall z\;,\mathcal{U}_i(x_i)\geq \mathcal{U}_i(z)+\mathcal{Q}_i(z)(x_i-z)\;.
% $$
% Since $\mathcal{U}_i(z)=z\mathcal{Q}_i(z)-P(z)$, we have
% $$
% \forall z\;,\mathcal{U}_i(x_i)\geq x_i \mathcal{Q}_i(z)-P(z)\;.
% $$
% This is the definition of bayesian incentive-compatibility (BIC).


\end{proof}
\begin{corollary2}%[characterization of DSIC auctions]
[\cite{Myerson81}]
\label{corollary_charect_DSIC}
An auction is DSIC if and only if
\begin{itemize}
\item[i)] the allocation rule is monotone and
\item[ii)]  the payment  of the winning bidder is the minimum bid guaranteeing that he would still have won the auction.\end{itemize}
 Given a monotone allocation rule and assuming 0-rationality, the payment rule is unique. 
\end{corollary2}
\begin{proof} 
The proof is almost identical, one just needs to make the various computations pointwise (for any vector $x_{-i}$) instead of in expectation.
\end{proof}
This characterization can be extended to very general mechanisms~: see \citep{archer2001truthful}.
\subsection{The Myerson auction : revenue maximization for BIC auctions}
After having established the Myerson lemma, it is now possible to derive the  revenue-maximizing auction among all BIC auctions. 
\begin{definition2}%[Myerson auction]
The Myerson auction is defined by the two following rules~: suppose bidder $i$ has value distribution $F_i$'s with associated virtual value (see Equation \eqref{eq:defVirtualValue}) $\psi_i$. Assume $F_i$ are regular, i.e. $\psi_i$ are increasing. 
\begin{description}
\item[Allocation rule:] Given the bids $b=(b_1,\ldots,b_n)$, the winner is the bidder with the highest non-negative virtual value $\psi_i(b_i)$, i.e.
$$
q(b) = \indicator{\arg\max \big\{ \psi_i(b_i) \, ; \, i \text{ s.t. } \psi_i(b_i) \geq 0 \big\} }
$$
with the convention that if the set is empty (when all virtual values are negative), then the item is not allocated and $q(b) = 0$. Ties are broken arbitrarily.
\item[Payment rule:] If bidder $i$ wins the auction, he pays
$$p_i(b)=\max \Big\{ \psi_i^{-1}(0), \psi_i^{-1}\Big(\max_{j\neq i} \big\{\psi_j(b_j)\big\}\Big) \Big\}$$
\end{description}
\end{definition2}
\textbf{Interpretation ~: } this auction amounts to running a second price auction with reserve 0 among the \emph{virtualized bids} $\psi_k(b_k)$ and converting back this ``virtual cost" in the original bid space of the winner $i$ through the function $\psi_{i}^{-1}$\;.
\begin{theorem2} \label{theorem_regular_distributions}
If $F_1,\dots,F_n$ are regular, the Myerson auction maximizes seller's revenue among all BIC and  interim-IR  auctions.
\end{theorem2}
\begin{proof}
The Myerson auction is BIC (for regular distributions)~: this can be verified in an elementary fashion - as we did for the second price auction earlier -  by comparing $\psi_i(x_i)$ to $\max_{j\neq i}\psi_j(b_j)$ and checking that in all situations it is optimal for bidder $i$ to bid his value. Indeed, bidding $b_i>x_i$ or $b_i<x_i$ never results in improvement of bidder $i$'s utility.


To show individual-rationality, we remark that since the auction is BIC, $$\mathcal{U}_{i}(x_i) = \mathcal{U}_{i}(0) + \int_{0}^{x_i}Q_i(s_i)ds_i = -P_{i}(0) + \int_{0}^{x_i}Q_i(s_i)ds_i \geq 0,$$ because $P_i(0) = 0$.  Thanks to  Myerson's lemma, Theorem \ref{Th:MyersonLemma}, the payment of each BIC auction is equal to 
$$
 P_i(0) + \mathds{E}_{x_i \sim F_{i}}(\psi_i(x_i)Q_i(x_i))\;. 
$$
The Myerson auction maximizes the two terms of this expression since for any rational auction, $P_i(0)\leq 0$.  Since the winner in the Myerson auction is the bidder who verifies
\begin{equation*} 
\psi_i(x_i) = \max_{j \in S}(\psi_j(x_j))\;,
\end{equation*}
and the item is not allocated when all $\psi_i$ are negative, the second term, is also maximized pointwise. 
Indeed, note that we can rewrite this second term
$$
\mathds{E}_{x_i \sim F_{i}}(\psi_i(x_i)Q_i(x_i))=\mathds{E}_{x \sim \mathcal{F}^{(n)}}[<\psi(x),q(x)>]\;,
$$
where $<a,b>$ is the scalar product between vectors $a$ and $b$. 
\end{proof}
\begin{corollary2} In the symmetric case, the second-price auction with reserve prices set to  monopoly prices is the revenue-maximizing auction.
\end{corollary2}
\nek{should we move this remark to the ``difficult things" section?}
\begin{remark2} 
The seller can do better if the mechanism is  only required to satisfy ex-ante rationality instead of interim rationality, as shown in 	
\citep{cremer1988full}. Indeed, there exists a BIC auction that is ex ante individually rational that accomplishes full-surplus extraction for the seller. In other words, the utility of bidders in this auction is equal to zero. This auction is not interim individually-rational since the expected utility when the bidder's value is zero is strictly negative. This setting of ex-ante individual rationality only makes sense when bidders have to decide to take part in the auction before understanding their value for the item. We come back in more details to this setting in Section \ref{sub_full_surplus_extraction}.
\end{remark2}
\subsection{Generalization of optimality result}
\label{SE:General_OptimalityResults}
\subsubsection{Non Incentive-Compatible mechanism: the revelation principle}
Myerson's optimality result can be extended to any incentive-compatible auctions, as long as there is a Nash equilibrium between bidders.
\begin{theorem2}%[Revelation principle]
Given a mechanism and a specific Nash equilibrium for this mechanism, there exists another BIC mechanism where the bidders' expected utility and seller's revenue at the truthful equilibrium are equal to the ones at the original Nash equilibrium. 
\end{theorem2}
\begin{proof}
Consider a mechanism and  $\beta = (\beta_1,\dots,\beta_n)$ a profile of strategies that is a Nash equilibrium. This mechanism is defined by an allocation rule $q:\mathcal{B}^{n}\rightarrow \mathds{R}^{n}$ and a payment rule  $p:\mathcal{B}^n\rightarrow \mathds{R}^{n}$. The mechanism $(q \circ \beta, p \circ \beta)$ is then clearly BIC and bidding truthful generate the same bids distributions, allocation and paiement as in the original mechanism; hence utilities and revenue are unchanged.
\end{proof}
\begin{corollary2} 
The Myerson auction is the revenue-maximizing mechanism among all individually-rational mechanisms which have a Nash equilibrium.
\end{corollary2} 
\begin{proof}
This is a direct application of the revelation principle.
\end{proof}
\nek{it's still unclear how to do it. And what about non-regular distributions? Then Myerson not defined at this point...}
We now extend the Myerson auction to cases where value distributions are not regular. 
\subsubsection{Non-regular distributions and the ironing technique}\label{Se:Ironing}

If $F_i$'s are not regular, the Myerson auction is poorly defined as $\psi_i$'s may not be invertible. From an allocation standpoint, since $\psi_i$ is not necessarily increasing,  the allocation rule may not be monotone. Hence a bidder might have incentive to ``shade" (or lower) his bid to increase his virtual bid and his probability of winning. Non-regular distributions are not uncommon, as a mixture of two distributions typically is not regular (for instance the mixture of two uniforms, Gaussians, etc...). It is therefore crucial to adapt the Myerson mechanism to non-regular distributions. The canonical way is to define a slightly different allocation rule based on a modified virtual value \citep{Myerson81} called the \textit{ironed virtual value}. 

Recall that one key consequence of having a non-decreasing virtual value is that the monopoly revenue $\Pi(r) = r(1-F(r)) = \int_r^\infty \psi(v)f(v)dv$ is ``almost''  concave, in the sense that $\Pi\circ F^{-1}$ is concave with derivative  $-\psi\circ F^{-1}(\cdot)$. As a consequence, optimizing the monopoly revenue boils down to finding the root of $\psi$.  The ironing technique consists in replacing $\Pi\circ F^{-1}$, which is not necessarily concave, by its concavification. 

\begin{definition2}[$\mathrm{cav}$ notation]\label{def:Concavification}
For a function $h$, we call 
$$
\mathrm{cav}(h) \text{ the concavification of the  function } h.
$$
We recall that , $\mathrm{cav}(h)$ is its smallest concave majorant of $h$, i.e. the smallest concave function above it~: its hypograph is the convex hull of the hypograph of $h$.
\end{definition2}
We can now define the ironed virtual value. 
\begin{definition2}[Ironed virtual value] \label{def:IronedVirtualValue}
For any non-regular distribution $F$, the \emph{ironed virtual value} of $\psi$, denoted by $\tilde{\psi}$ is defined by
$$
 \tilde{\psi}(x)= \partial \Big(-\mathrm{cav}(\Pi\circ F^{-1})\Big)(F(x))\;, \text{ where } \partial \text{ denotes subdifferential}. 
$$
\end{definition2}

In general, the concavification of a function $g$ is either equal to $g$ at some point or linear on some interval otherwise. Luckily enough, the ironed virtual value has a closed form on intervals where it is not equal to the virtual value.


\begin{lemma2}%[Expression of ironed virtual value on [a,b]] 
Assume that for some $a<b$, it holds that \begin{itemize}
\item[--] $\mathrm{cav}(\Pi\circ F^{-1})(F(a))=\Pi (a)$,  
\item[--]$\mathrm{cav}({\Pi}\circ F^{-1})(F(b))=\Pi(b)$
\item[--] $\mathrm{cav}({\Pi}\circ F^{-1})(F(x)) > \Pi (x)$ for $x \in(a,b)$ 
\end{itemize}then
the ironed virtual value  of $\psi$ on $(a,b)$ is constant and equal to
$$
\tilde{\psi}(x)= \frac{\int_{a}^b \psi(t) f(t) \mathrm{d} t}{F(b)-F(a)}$$
\end{lemma2}
\begin{proof}
By definition of the concavification, $\mathrm{cav}(\Pi\circ F^{-1})$ is linear on $[F(a),F(b)]$ and the results comes from linear interpolation.
\end{proof}
%Typically, non-increasing virtual value function are ironed on an interval where it is non-increasing. On the other hand, if the ironing is limited to the smallest interval  where the virtual value is non-increasing, this might not guarantee that the ironed virtual value is increasing. To insure that the ironed virtual value is non-decreasing, the ironing should be extended a larger interval. The final minimal interval $[a_{opt},b_{opt}]$ where the virtual value is ironed should verify the following conditions:
%$$\psi(a_{opt}) \leq \psi([a_{opt},b_{opt}]) \leq \psi(b) \text{ and } \forall c,d \in [a_{opt},b_{opt}], \psi(c) \geq \psi([c,d]) \geq \psi(d)$$
%A good way to visualize how to set $a_{opt}$ and $b_{opt}$ is to plot $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$ as a function of $F(t)$.  We recall that $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t = -b(1-F(b))$, the opposite of the monopoly revenue. The intervals where the virtual value should be ironed are the ones where the convex envelop of $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$ is different from $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$.
%
%\begin{definition2}[Ironed virtual value] Consider a value distribuion F with corresponding virtual value $\phi$. Let $[a_1,b_1],...,[a_k,b_k]$ be the intervals that are straightened out when one takes the convex hull for the plot of the cumulative virtual value $\int_{0}^{b} \psi(t) f(t) \mathrm{d} t$ against F(b). The ironed virtual value  of $\psi_i$ denoted by $\tilde{\psi}_i$ is defined as 
%$$
%\tilde{\psi}_i(x)=\left\{\begin{array}{ll}{\psi([a,b]) = \frac{\int_{a}^{b} \psi(t) f(t) \mathrm{d} t}{F\left(b\right)-F\left(a\right)},} & {x \in\left[a_i, b_i\right]} \\ {\psi(x),} & {\text { otherwise }}\end{array}\right.
%$$
%\end{definition2}
We refer to \citep{note_ironings} for more technical details. In particular, the ironed virtual value, since  it is defined as a sub-differential, is not a function but a multi-valued mapping, a.k.a a multifunction. On the other hand, selecting the aforementioned $\tilde{\psi}(x)$ as $\psi(x)$ when the sub-differential is not reduced to a singleton is also perfectly valid and implicitly used as convention from now on.  With this latter expression, either $\tilde{\psi}$ is equal to $\psi$ or it is constant on some interval around $x$. It is  non-decreasing everywhere and intervals where $\psi$ is  decreasing are ``flattened'', as illustrated in Figure \ref{Ironed}.



Recall that the purpose of ironing is to replace the - possibly somewhere decreasing - virtual value function $\psi$ in the Myerson auction (that might then not be BIC) by $\tilde{\psi}$. We now show that ironing the virtual value does not decrease the revenue of the Myerson auction.

\begin{figure}[h!]
\centering
\begin{tabular}{cc}
\includegraphics[width=.5\linewidth]{images/convex_hull.pdf}&
\includegraphics[width=.5\linewidth]{images/virtual_value_ironing.pdf}
\end{tabular}
\includegraphics[width=.55\linewidth]{images/ironed_revenue_curve.pdf}

\caption{\textbf{Left:} Concavification of $\Pi\circ F^{-1}$ for a  mixture of $\mathfrak{U}(0,0.5)$ and $\mathfrak{U}(0,1)$. \textbf{Right:} Associated virtual value (plain black) and ironed one (dashed orange).
\textbf{Center:} Original (plain black) and ironed (dashed orange) monopoly revenue.}
\label{Ironed}
\end{figure}
\begin{lemma2} 
The payment of bidder $i$ at the truthful equilibrium of any BIC auction satisfies 
$$ \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] \leq P_i(0) + \mathbf{E}_{x_{i} \sim F_{i}}\left[Q_{i}\left(x_{i}\right) \tilde{\psi}_{i}\left(x_{i}\right)\right]\;,$$
where $\tilde{\psi}_i$ is his ironed virtual value.\end{lemma2} 
\begin{proof} 
Consider a BIC auction. According to Theorem \ref{Th:MyersonLemma}, 
$$
\mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] = P_i(0) + \mathbf{E}_{x_{i} \sim F_{i}}\left[Q_{i}\left(x_{i}\right) \psi_{i}\left(x_{i}\right)\right]\;.
$$
Furthemore, since the auction is BIC, Corollary \ref{characterization_inc_comp} $Q_i$ must be non-decreasing. 
So we just need to show that 
$$
\mathbf{E}_{x_{i} \sim F_{i}}\left[Q_{i}\left(x_{i}\right) \psi_{i}\left(x_{i}\right)\right]\leq 
\mathbf{E}_{x_{i} \sim F_{i}}\left[Q_{i}\left(x_{i}\right) \tilde{\psi}_{i}\left(x_{i}\right)\right]
$$
We split the 






The proof is based on  the Harris inequality \citep{harris1960lower}, a direct application of Chebyschev' sum inequality. 
\begin{lemma2}[Harris inequality]
For any  non-decreasing mapping $\rho$ and  non-increasing mapping $\gamma$, the following holds for any random variable $X$, 
$$\mathds{E}[\rho(X)\gamma(X)] \leq \mathds{E}[\rho(X)]\mathds{E}[\gamma(X)]\;.$$
\end{lemma2}
Consider a BIC auction. According to Theorem \ref{Th:MyersonLemma}, 
$$
\mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] = P_i(0) + \mathbf{E}_{x_{i} \sim F_{i}}\left[Q_{i}\left(x_{i}\right) \psi_{i}\left(x_{i}\right)\right]\;.
$$
Furthemore, since the auction is BIC, Corollary \ref{characterization_inc_comp} $Q_i$ must be non-decreasing. 

Let assume there exists $[c,d]$ where $\psi_i$ requires ironing (otherwise there is nothing to show); we now call $[a,b]$ the largest interval that contains $[c,d]$ over which $\psi(x)\neq \tilde{\psi}(x)$. In other words, $[a,b]$ is the whole interval over which we have ironed $\psi$. We consider the function $\tilde{\psi}$ defined above on the corresponding $[a,b]$ interval. Furthermore, note that $f_i(x)/(F_i(b)-F_i(a))$ is a valid probability density on $[a,b]$. We then have
\begin{align*}
&\int_{a}^{b}Q_i(x)\psi_{i}(x)f_i(x)dx =(F_i(b) - F_i(a)) \int_{a}^{b}Q_i(x)\psi_{i}(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx
\\&\leq (F_i(b) - F_i(a)) \int_{a}^{b}Q_i(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx\int_{a}^{b}\psi_i(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx
\\&=\int_{a}^{b}Q_i(x)\tilde{\psi}_{i}(x)f_i(x)dx\;.
\end{align*}
from where the result follows. The first inequality comes from applying Harris' inequality. \nek{c'est faux non? $\psi$ est justement pas monotone sur l'interval, donc pourquoi appliquer Harris?} The last equality comes from the definition of $\tilde{\psi}$ which is a constant and equal to $\int_{a}^{b}\psi_i(x)\frac{f_i(x)}{F_i(b)-F_i(a)}dx$ on the interval $[a,b]$ by definition. Here it is important that we use the whole ironing interval for $[a,b]$. The same argument applies on all intervals where $\psi$ requires ironing.  
The statement of the Lemma is shown by applying Theorem \ref{Th:MyersonLemma} to compute expected revenue. 
\end{proof}
We now generalize Theorem \ref{theorem_regular_distributions} to the case of non-regular value distributions. \nek{the theorem below doesn't make sense. Are we doing BIC auctions with non-regular value distribution?}
 \begin{theorem2}[\cite{Myerson81}]%[Optimal auctions for general value distribution]
  In a single item auction, with general value distribution, a revenue-maximing auction \nek{in what class?} is an auction where the seller allocates the item to the bidder with the highest non-negative ironed virtual value. The payment rule is defined such that the auction is incentive compatible - see Corollary \ref{characterization_inc_comp}.
 \end{theorem2}
 
 \subsection{Reserve prices in first price auctions}
%\nek{need to read his assumptions carefully and state them} 
We start with an abstract result that we then apply to first price auctions. 

\begin{proposition2}\label{prop:virtualValueIsVirtualPaymentGeneralCase}
Suppose bidder $i$ participates in an auction such that the probability of winning the auction when bidding $b$ is $G_i(b)$ and the corresponding expected payment is $P_i(b)$. Call $\beta_i$ an optimal strategy for bidder $i$ in this setup, i.e. one that maximizes their utility. 	
Then the seller revenue coming from bidder $i$ is 
\begin{equation}\label{eq:RevSellerGeneralPriceWithVValue}
 \mathds{E}_{x_i\sim F_{i}}[P_i(\beta_i(x_i))]-P_i(\beta_i(0)) =\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;,
\end{equation}
where $\psi_i$ is the virtual value (see Equation \eqref{eq:defVirtualValue}) associated with the value distribution of $x_i$. 
\end{proposition2}
\begin{remark2}
This proposition helps explain how our interpretation of the $\psi_i(x_i)$ as a virtual payment makes sense for utility-maximizing bidders in general and not only in the case of BIC or DSIC auctions we encountered previously. It can also be seen as a more quantitative version of the revelation principle. 
\end{remark2}
\begin{proof}
Note that since bidder $i$ tries to maximize his utility, 
$$
\beta_i(x_i)=\argmax_b x_iG_i(b)-P_i(b)\;. 
$$
Let us call 
$$
W(x)=x G_i(\beta_i(x))-P_i(\beta_i(x))
$$
The envelope theorem in the form of Theorem 2 of \cite{MilgromSegal2002} applies since $0\leq G_i(t)\leq 1$ for all $t$ and hence 
$$
W(x)-W(0)=\int_0^x G_i(\beta_i(t)) dt\;.
$$
Therefore, the expected payment satisfies
$$
P_i(\beta_i(x))-P_i(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(t)) dt\;.
$$
Taking expectation with respect to $x_i$ with cdf $F_i$ in the previous equation gives
\begin{align*}
\mathds{E}_{x_i\sim F_{i}}[P_i(\beta_i(x_i))]-P_i(\beta_i(0))&=\int_0^{\infty} xG_i(\beta_i(x)) f_i(x)dx-\int_0^{\infty}\int_0^{\infty} f_i(x)\indicator{t\leq x}G_i(\beta_i(t))dt\, dx\;,\\
&=\int_0^{\infty} xG_i(\beta_i(x)) f_i(x)dx-\int_0^{\infty} (1-F_i(t))G_i(\beta_i(t))dt\;,\\
&=\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
\end{align*}
% $$
% \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
% $$

% This is not limited to first price... as long as $P(\beta_i(0))=0$\\
% En gros,  1st order conditions give $xG_i'(\beta_i(x))=P'(\beta_i(x))$. Multiply both sides by $\beta'_i(x)$ and integrate to get $P(\beta_i(x))-P(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(u))du\;.$ Then doing the same as below, we get that
% $$
% \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)]-P(\beta_i(0))=\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
% $$
% Ou: envelope theorem says that if $W_i(x)=\max_b xG_i(b)-P(b)$, and $\beta_i$ is an optimal strategy, $W_i'(x)=G(\beta_i(x))$. Hence, $W_i(x)-W_i(0)=\int_0^x G_i(\beta_i(u))du=xG_i(\beta_i(x))-P(\beta_i(x))+P(\beta_i(0))$. We conclude that
% $P(\beta_i(x))-P(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(u))du\;.$ And the result follows as above.

	
	
\end{proof}




In the case of first price auctions, we have $P_i(\beta_i(x_i))=\beta_i(x_i)G_i(\beta_i(x_i))$, since the probability of winning is $G_i(\beta_i(x_i))$. 
So the arguments given in the proof above allow us to recover a result from \citep{KirkegaardAsymmetricFirstPrice2009}~: the optimal strategy for bidder $i$ when the top bid of the competition has cdf $G_i$ and $P_i(\beta_i(0))=0$ satisfies 
\begin{equation}\label{eq:OptStrat1stPriceEnvelope}
\beta_{i}(x)=x-\frac{\int_0^x G_i(\beta_i(t))dt}{G_i(\beta_i(x))}\;.
\end{equation}

%Because of the the envelope theorem and arguments similar to those used to derived the revenue maximizing auctions, the equilibrium strategy must satisfy 
\iffalse
Using the envelope theorem, one can show \citep{KirkegaardAsymmetricFirstPrice2009} that the optimal strategy for bidder $i$ when the top bid of the competition has cdf $G_i$ satisfies 
\begin{equation}\label{eq:OptStrat1stPriceEnvelope}
\beta_{i}(x)=x-\frac{\int_0^x G_i(\beta_i(t))dt}{G_i(\beta_i(x))}\;.
\end{equation}
\fi
The expected payoff of player $i$ at $x$ is then equal to $u_i(x,\beta_{i}(x))=\int_0^x G_i(\beta_i(t))dt$ and in particular it holds  that $\mathds{E} U_i (\beta,x_i)=\ \mathds{E}_{x_i\sim F_{i}}\big[G_i(\beta_i(x_i))(x_i-\psi(x_i))\big]$. 
\iffalse
\nek{I think with the envelope theorem we can show that if I'm a utility maximizer, i.e. I pick 
$$
\beta(x)=\argmax_b xG(b)-P(b)\;,
$$
regardless of the payment rule, then 
$$
\mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
$$
This is not limited to first price... as long as $P(\beta_i(0))=0$\\
En gros,  1st order conditions give $xG_i'(\beta_i(x))=P'(\beta_i(x))$. Multiply both sides by $\beta'_i(x)$ and integrate to get $P(\beta_i(x))-P(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(u))du\;.$ Then doing the same as below, we get that 
$$ 
\mathds{E}_{x_i\sim F_{i}}[P_i(x_i)]-P(\beta_i(0))=\mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;.
$$
Ou: envelope theorem says that if $W_i(x)=\max_b xG_i(b)-P(b)$, and $\beta_i$ is an optimal strategy, $W_i'(x)=G(\beta_i(x))$. Hence, $W_i(x)-W_i(0)=\int_0^x G_i(\beta_i(u))du=xG_i(\beta_i(x))-P(\beta_i(x))+P(\beta_i(0))$. We conclude that 
$P(\beta_i(x))-P(\beta_i(0))=xG_i(\beta_i(x))-\int_0^x G_i(\beta_i(u))du\;.$ And the result follows as above. 
}
\fi
\begin{corollary2}\label{coro:RevSeller1stPriceWithVValue}
In a first price auction, when bidder $i$ uses the strategy implicitly defined in Equation \eqref{eq:OptStrat1stPriceEnvelope}, the seller revenue coming from bidder $i$ is 
\begin{equation}\label{eq:RevSeller1stPriceWithVValue}
 \mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi_i(x_i)\big]\;,
\end{equation}
where $\psi_i$ is the virtual value associated with the value distribution of $x_i$. 
\end{corollary2}
The corollary follows from Proposition \ref{prop:virtualValueIsVirtualPaymentGeneralCase} after noticing that $P_i(\beta_i(0))=\beta_i(0)G_i(\beta_i(0))=0$ when bidder $i$ uses $\beta_i$ defined in Equation \eqref{eq:OptStrat1stPriceEnvelope}.

\iffalse
\begin{proof}
We note that 
$$
 \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\int_0^{\infty}\beta_{i}(x) G_i(\beta_i(x)) f_i(x) dx =\int_0^{\infty} xG_i(\beta_i(x))f_i(x)dx - \int_0^{\infty}f_i(x)\int_0^x G_i(\beta_i(t))dt dx\;.
$$	
Using Fubini's theorem, we have 
$$
\int_0^{\infty}f_i(x)\int_0^x G_i(\beta_i(t)))dt dx=\int_0^{\infty}f_i(x)G_i(\beta_i(t))dt \indicator{t\leq x} dx dt=\int_0^{\infty}(1-F_i(t))G_i(\beta_i(t))) dt\;.
$$
We conclude that 
$$
 \mathds{E}_{x_i\sim F_{i}}[P_i(x_i)] =\int_0^\infty G_i(\beta_i(x))\left[x-\frac{1-F_i(x)}{f_i(x)}\right]f_i(x) dx = \mathds{E}_{x_i\sim F_{i}} \big[G_i(\beta_i(x_i))\psi(x_i)\big]\;.
$$
\end{proof}
\fi

\paragraph{Good or optimal reserve prices} Proposition \ref{prop:virtualValueIsVirtualPaymentGeneralCase} and Corollary \ref{coro:RevSeller1stPriceWithVValue} suggest that from a seller revenue standpoint it would be good to avoid bids corresponding to values that have negative virtual values. In other words, setting individual reserve values at $\psi_i^{-1}(0)$ for bidders may have positive impact for seller revenue. However, this interpretation ignores the impact of setting such reserve values on the strategic response of the bidder that is optimizing his utility. 


Finding optimal reserve prices for first price auctions is much more complicated than finding them for the second price auctions, even with $n=2$ symmetric bidders \citep{KotowskiAsymmetricReserves2018} for the following two reasons. First, if the distribution $F$ is not regular and its density is discontinuous at the monopoly price, giving two different reserve prices to the two symmetric buyers actually increases the seller revenue at equilibrium, at least when $r_1$ and $r_2$ are close.
Second, in the specific case where those two reserve prices $r_1$ and $r_2$ are sufficiently close,  the equilibrium bid distribution of the player with the lower reserve price becomes discontinuous.


Many further difficulties arise when the seller tries to learn good reserve prices for first price auctions from data and does not have access to the bidders' value distributions. We further detail them in Section \ref{learning_reserve_prices_first_price}.

\section{Prior-independent optimal auctions} 
\label{sec-Bulow}
In the previous section, we  derived the revenue-maximizing auction given the prior of the seller on the possible valuations of the different bidders. In some cases, the seller does not have access to a reliable prior and she has to choose an auction without this information. An associated challenge is to understand what auctions are robust to a lack of knowledge about (or some mis-specification in) the bidders' value distributions.

The following theorem shows that a basic second-price auction without reserve price -  referred to henceforth as the Vickrey auction - with just one extra bidder, leads to a higher revenue than the optimal Myerson auction \citep{bulow1996auction}. Only the symmetric case is considered, so that the comparison of two auctions with different set of bidders is possible.
\begin{theorem2}[\cite{bulow1996auction}]%[Bulow-Klemperer Theorem]
In the symmetric setting and with regular distributions, the revenue of the Myerson auction with $n$ bidders is lower than the revenue of the Vickrey auction with $n+1$ bidders. 
\end{theorem2}
\begin{figure}[H]
\includegraphics[width=.5\linewidth]{images/BulowKlemperer.pdf}
\caption{Illustration of the Bulow-Klemperer theorem for the case with value distributions  $\mathfrak{U}([0,1])$.}
%{\color{red} Ca ne devrait pas etre $K$ bidders mais $n$ bidders ; choix des couleurs discutables ; on ne dit pas Nb bidders en Anglais }}
\label{fig:BK}
\end{figure}
Before proving the Bulow-Klemperer theorem, we introduce a useful lemma.
\begin{lemma2}\label{second_price_without_reserve}
In the symmetric case and with regular distributions, the Vickrey auction is revenue-maximizing in the class of individually-rational auctions where the item is always attributed. 
\end{lemma2}
\begin{proof}
Based on the revelation principle, we shall only consider incentive-compatible auctions. Theorem \ref{Th:MyersonLemma} then applies. Since the item must always be attributed, in order to maximize the seller's revenue it should be allocated to the bidder with the highest virtual value, regardless of whether the highest virtual value is non-negative or not. This is a consequence of the proof of Theorem \ref{Th:MyersonLemma}. Since the distributions are regular and identical, the bidder with the highest virtual value is also the bidder with the highest value. As a consequence, the mechanism we just described is exactly the Vickrey auction.
\end{proof}
The proof of the Bulow-Klemperer theorem can now be derived from the previous lemma.
\begin{proof} 
Let us assume that there are $n+1$ bidders, and consider the following mechanism. First, the seller runs a Myerson auction on  $n$ bidders (chosen arbitrarily). If the item is not allocated by the Myerson auction, it is allocated for free (i.e. without any payment) the $(n+1)$-th bidder. The revenue of this auction is equal to the revenue of the Myerson auction with $n$ bidder, yet it is  an auction that always allocate an item amongst $n+1$ bidders. Lemma \ref{second_price_without_reserve} implies that the revenue of this auction is smaller than the one of the Vickrey auction. 
This gives the result.
\end{proof}

As a consequence, it is more interesting,  from a seller revenue maximization standpoint to have one more bidder in the auction than to implement a complex mechanism. This is the reason why one of the first recommendations of most economists dealing with institutions organizing auctions is to maximize the competition  before implementing complex mechanisms \citep{bulow1996auction,milgrom2004putting}. This is sometimes referred to as the Wilson doctrine.

\bigskip

Nonetheless, let us assume that a specific mechanism has been chosen, independently of the value distributions (which are unknown in this setup). A crucial  question that remains is the evaluation of this specific choice of mechanism in the worst-case analysis. We will restrict ourselves to DSIC auctions. We will use the notion of \textsl{competitive ratio} defined as the infimum, over all possible value distributions, of the revenue of this auction divided by the optimal revenue of the Myerson auction for these distributions. 

The competitive ratio is obviously smaller than 1, and the bigger the better. Unfortunately, if the class of value distributions is not restricted when computing this infimum, there does not exist any auction with a positive competitive ratio \citep{allouah2018prior}. As a consequence, we will use different types of restrictions to achieve non-trivial approximation results. Based on the Bulow-Klemperer theorem, we can derive some revenue guarantees on the second price auction without reserve price. 
\begin{corollary2} \label{compet-ratio}
The Vickrey auction  with $n$ symmetric bidders and regular value distributions is at least a $\left(\frac{n-1}{n}\right)$-approximation of the Myerson auction. 
\end{corollary2}
\begin{proof}
We denote  respectively by $R(\mathrm{Vickrey}_n)$ and $R(\mathrm{Myerson}_n)$ the expected revenue of the seller  in the Vickrey or  Myerson auction with $n$ bidders and by $P_i(\mathrm{Vickrey}_n)$ and $P_i(\mathrm{Myerson}_n)$ the expected payment of the bidder $i$ in those auctions (so that $R(\cdot) = \sum_{i=1}^n P_i(\cdot)$).


Let us first prove that $P_i(\mathrm{Myerson}_n)\geq P_i(\mathrm{Myerson}_{n+1})$.

By symmetry and with regular distributions, their exists a unique monopoly price $r^*$ which is independent of the number of players. Note that $\psi(x)\geq 0$ when $x\geq r^*$. Furthermore, in the symmetric case, the probability that bidder $i$ wins the auction when facing $k$ competitors is just $F^k(x)$. Hence, 
\begin{align*}
	P_i(\mathrm{Myerson}_{n})&= \int  \psi(x) F^{n-1}(x)f(x)\mathds{1}\{x\geq r^*\} dx\\&\geq \int \psi(x) F^{n}(x)f(x)\mathds{1}\{x\geq r^*\}dx\\&=P_i(\mathrm{Myerson}_{n+1}),\end{align*}
which proves the inequality.



Then, based on the Bulow-Klemperer theorem, 
$$R(\mathrm{Vickrey}_n)\geq R(\mathrm{Myerson}_{n-1}) = (n-1)  P_i(\mathrm{Myerson}_{n-1}) \geq (1-\frac{1}{n})  R(\mathrm{Myerson}_{n})$$
which gives the result. \end{proof}
We proved in Corollary \ref{compet-ratio}, through the Bulow-Klemperer theorem that the competitive ratio of the Vickrey auction is at least 0.5, when the distributions are restricted to regular ones. Interestingly, it is possible to do better with a slightly different auction. 
\begin{theorem2}[\cite{fu2015randomization}]
There exists an incentive-compatible auction with a competitive ratio of 0.512 against regular value distributions. 
\end{theorem2}
The mechanism considered was the first  with a higher competitive ratio than 0.5  against regular distributions. It is a slight modification  of the Vickrey auction where the seller inflates the second highest bid. Formally, the mechanism is the following: with probability $1-\varepsilon$,  a second price auction without reserve price is run. With the  probability $\varepsilon$, the mechanism allocates the object to the bidder with the highest valuation, but only if his valuation is greater than $1+\delta$  times the valuation of the second highest bidder and pays  $(1+\delta)$ the second highest bid. Otherwise, the mechanism does not allocate the item. 

The idea behind this theorem is the following. The Bulow-Klemperer bound of $0.5$ on the competitive ratio is rather tight for regular distributions that would induce a high optimal reserve price. On the other hand, it is rather loose for regular distribution with a low associated reserve price. Inflating the second highest bid has a positive effect for the former type of distribution (as it somehow emulates a high reserve price) and a negative effect for the later type (because it induces some reserve price, bigger than what it should be). As a consequence, the ratio of revenues increase in the first case, and decreases in the second one; but thanks to the looseness in the Bulow-Klemperer bound of $0.5$, the infimum globally increases. 

On the other hand, when restricted to MHR distributions, the ratio is equal to 0.7153 and this result is tight. 

For regular distribution, this result was then improved up to 0.519 \citep{allouah2018prior}  and further improved in \citep{hartline2020benchmark} which identified the optimal prior-independent mechanism. The optimal mechanism is a mixture between a second price auction and the same auction where the prices are scaled up by a factor of about 2.5. The authors find the worst-case family of distributions and use these distributions to derive the optimal mechanism and solve the problem. 

\section{Further reading: non-unicity of Nash equilibria and related complications}
\label{sec:NashIsDifficult}
\nek{Add the two counter examples here...}


==> journaldata/ACC-editorialboard.tex <==
%ACG-Editorialboard.

\begin{editorialboard}

%\subsection{Editor-in-Chief}

%\journalchiefeditor{Stefan J. Reichelstein}{Stanford University\\United States}



\subsection{Executive Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Robert Bushman}{The University of North Carolina at Chapel Hill}
\journaleditor{Sunil Dutta}{University of California at Berkeley}
\journaleditor{Stephen Penman}{Columbia University}
\journaleditor{Stefan J. Reichelstein, Managing editor}{Stanford University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ACC-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{ACCcolor}{officegreen}   %new color names can be defined before use
\journalcolor      {ACCcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Accounting}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ACC}
\journalurl        {http://www.nowpublishers.com/ACC}
\journalissnprint  {1554-0642}
\journalissnonline {1554-0650}
\journaldoi        {10.1561/14}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Accounting publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Auditing}
\item{Corporate Governance}
\item{Cost Management}
\item{Disclosure}
\item{Event Studies/Market Efficiency Studies}
\item{Executive Compensation}
\item{Financial Reporting}
\item{Management Control}
\item{Performance Measurement}
\item{Taxation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Accounting, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ACC-seriespage.tex <==
\vspace{12pt}
\noindent \textit{The Role of Stakeholders in Corporate Governance: A View from\\ Accounting Research}\\
Gaizka Ormazabal
\\ISBN: 978-1-68083-396-6
\\
\\
\noindent \textit{Financial Analysts and Their Contribution to Well-Functioning Capital Markets}\\
Mark Bradshaw, Yonca Ertimur and Patricia O'Brien
\\ISBN: 978-1-68083-354-6
\\
\\
\noindent \textit{Rethinking Financial Reporting: Standards, Norms and Institutions}\\
Shyam Sunder
\\ISBN: 978-1-68083-144-3


==> journaldata/ACG-editorialboard.tex <==
%ACG-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Douglas Cumming}{Florida Atlantic University\\USA}
\journalchiefeditor{Geoffrey Wood}{University of Essex\\UK}



\subsection{Associate Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Renee Adams}{University of New South Wales}
\journaleditor{Lucian Bebchuk}{Harvard University}
\journaleditor{William Judge}{Old Dominion University}
\journaleditor{Mark Roe}{Harvard University}
\journaleditor{Rene Stulz}{Ohio State University}
\journaleditor{James Westphal}{University of Michigan}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ACG-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ACGcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ACGcolor} %a color name. 
\journaltitle      {Annals of Corporate Governance}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ACG}
\journalurl        {http://www.nowpublishers.com/ACG}
\journalissnprint  {2381-6724}
\journalissnonline {2381-6732}
\journaldoi        {10.1561/109	}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
Annals of Corporate Governancepublishes
 articles in the following topics:
% \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Boards of Directors}
\item{Ownership}
\item{National Corporate Governance Mechanisms}
\item{Comparative Corporate Governance Systems}
\item{Self Governance}
\item{Teaching Corporate Governance}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
 Annals of Corporate Governance, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ACG-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Leveraged Buyouts: Motives and Sources of Value}\\
Luc Renneboog and Cara Vansteenkiste
\\ISBN: 978-1-68083-274-7
\\
\\
\noindent \textit{Microfinance: What Do We Know? Where Do We Go?}\\
Sugato Chakravarty and Mariya Pylypiv
\\ISBN: 978-1-68083-270-9
\\
\\
\noindent \textit{Board Involvement in the Strategic Decision Making Process:\\ A Comprehensive Review}\\
William Q. Judge and Till Talaulicar
\\ISBN: 978-1-68083-260-0
\\
\\
\noindent \textit{Understanding Boards of Directors: A Systems Perspective}\\
Jay W. Lorsch
\\ISBN: 978-1-68083-246-4


==> journaldata/ASTP-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Audretsch}{Indiana University}
\journaleditor{William Bonvillian}{MIT}
\journaleditor{Barry Bozeman}{Arizona State University}
\journaleditor{Kaye Husbands Fealing}{Georgia Institute of Technology}
\journaleditor{John Hardin}{North Carolina Board of Science and Technology}
\journaleditor{Mariagrazia Squicciarini}{OECD}
\journaleditor{Wolfgang Polt}{Joanneum Research Institute}
\journaleditor{Nicholas Vonortas}{The George Washington University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ASTP-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ASTPcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ASTPcolor} %a color name. 
\journaltitle      {Annals of Science and Technology Policy}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ASTP}
\journalurl        {http://www.nowpublishers.com/ASTP}
\journalissnprint  {2475-1820}
\journalissnonline {2475-1812}
\journaldoi        {10.1561/110}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Annals of Science and Technology Policy publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Literature reviews of technology and innovation policies}
\item{Historical case studies of technology development and implementation}
\item{Institutional histories of technology- and innovation-based organizations}
\item{Analyses of policies attendant to technology development and adoption and diffusion}
\item{Studies documenting the adoption and diffusion of technologies and subsequent consequences}
\item{Studies of public and private research partnerships (cross sectional, over time, or case based)}
\item{Assessments and evaluations of specific technology and innovation policies}
\item{Analyses of ecosystems associated with the technology and/or innovation development}
\item{Cross observational (e.g., cross-agency or cross-country) comparisons of technology and innovation policies}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Annals of Science and Technology Policy, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ASTP-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Policies for the Provision of Finance to Science-based Entrepreneurship}\\
Alice Civera, Michele Meoli and Silvio Vismara\\
ISBN: 978-1-68083-352-2\\
\\
\noindent \textit{The Roles and Impacts of Technical Standards on Economic Growth and Implications for Innovation Policy}\\
Gregory Tassey\\
ISBN: 978-1-68083-316-4\\
\\
\noindent \textit{Bureaucratization in Academic Research Policy: What Causes It?}\\
Barry Bozeman and Jiwon Jung\\
ISBN: 978-1-68083-262-4\\
\\
\noindent \textit{Advanced Manufacturing: A New Policy Challenge}\\
William B. Bonvillian\\
ISBN: 978-1-68083-240-2

==> journaldata/CGV-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols*}{2}\raggedcolumns
\journalchiefeditor{Brian Curless}{University of Washington}
\journalchiefeditor{William T. Freeman}{MIT}
\journalchiefeditor{Luc Van Gool}{KU Leuven and ETH Zurich}
%\end{multicols*}


\subsection{Editors} \scriptsize
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Marc Alexa}{TU Berlin}
\journaleditor{Kavita Bala}{Cornel}
\journaleditor{Ronen Basri}{Weizmann Institute of Science}
\journaleditor{Peter Belhumeur}{Columbia University}
\journaleditor{Andrew Blake}{Microsoft Research}
\journaleditor{Chris Bregler}{Facebook-Oculus}
\journaleditor{Joachim Buhmann}{ETH Zurich}
\journaleditor{Michael Cohen}{Microsoft Research}
\journaleditor{Paul Debevec}{USC Institute for Creative Technologies}
\journaleditor{Julie Dorsey}{Yale}
\journaleditor{Fredo Durand}{MIT}
\journaleditor{Olivier Faugeras}{INRIA}
\journaleditor{Rob Fergus}{NYU}
%\columnbreak
\journaleditor{Mike Gleicher}{University of Wisconsin}
\journaleditor{Richard Hartley}{Australian National University}
\journaleditor{Aaron Hertzmann}{Adobe Research}
\journaleditor{Hugues Hoppe}{Microsoft Research}
\journaleditor{C. Karen Liu}{Georgia Tech}
\journaleditor{David Lowe}{University of British Columbia}
\journaleditor{Jitendra Malik}{ Berkeley}
\journaleditor{Steve Marschner}{Cornell}
\journaleditor{Shree Nayar}{Columbia}
\journaleditor{James O'Brien}{Berkeley}
\journaleditor{Tomas Pajdla}{Czech Technical University}
\journaleditor{Pietro Perona}{California Institute of Technology}
\journaleditor{Marc Pollefeys}{ETH Zurich}
%\columnbreak
\journaleditor{Jean Ponce}{Ecole Normale Superieure}
\journaleditor{Long Quan}{HKUST}
\journaleditor{Cordelia Schmid}{INRIA}
\journaleditor{Steve Seitz}{University of Washington}
\journaleditor{Amnon Shashua}{Hebrew University}
\journaleditor{Peter Shirley}{University of Utah}
\journaleditor{Noah Snavely}{Cornell}
\journaleditor{Stefano Soatto}{UCLA}
\journaleditor{Richard Szeliski}{Microsoft Research}
\journaleditor{Joachim Weickert}{Saarland University}
\journaleditor{Song Chun Zhu}{UCLA}
\journaleditor{Andrew Zisserman}{Oxford}
\end{multicols*}
\end{editorialboard} 

==> journaldata/CGV-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{CGVcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {CGVcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Computer Graphics and Vision}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CGV}
\journalurl        {http://www.nowpublishers.com/CGV}
\journalissnprint  {1572-2740}
\journalissnonline {1572-2759}
\journaldoi        {10.1561/06}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Rendering}
\item{Shape}
\item{Mesh simplification}
\item{Animation}
\item{Sensors and sensing}
\item{Image restoration and enhancement}
\item{Segmentation and grouping}
\item{Feature detection and selection}
\item{Color processing}
\item{Texture analysis and synthesis}
\item{Illumination and reflectance modeling}
\item{Shape representation}
\item{Tracking}
\item{Calibration}
\item{Structure from motion}
\item{Motion estimation and registration}
\item{Stereo matching and reconstruction}
\item{3D reconstruction and image-based modeling}
\item{Learning and statistical methods}
\item{Appearance-based matching}
\item{Object and scene recognition}
\item{Face detection and recognition}
\item{Activity and gesture recognition}
\item{Image and video retrieval}
\item{Video analysis and event recognition}
\item{Medical image analysis}
\item{Robot localization and navigation}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Computer Graphics and Vision, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/CGV-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Crowdsourcing in Computer Vision}\\
Adriana Kovashka, Olga Russakovsky, Li Fei-Fei and Kristen Grauman\\
ISBN: 978-1-68083-212-9\\
\\
\noindent \textit{The Path to Path-Traced Movies}\\
Per H. Christensen and Wojciech Jarosz\\
ISBN: 978-1-68083-210-5\\
\\
\noindent \textit{(Hyper)-Graphs Inference through Convex Relaxations and Move Making Algorithms}\\
Nikos Komodakis, M. Pawan Kumar and Nikos Paragios\\
ISBN: 978-1-68083-138-2\\
\\
\noindent \textit{A Survey of Photometric Stereo Techniques}\\
Jens Ackermann and Michael Goesele\\
ISBN: 978-1-68083-078-1\\
\\
\noindent \textit{Multi-View Stereo: A Tutorial}\\
Yasutaka Furukawa and Carlos Hernandez\\
ISBN: 978-1-60198-836-2

==> journaldata/CIT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Helmut B\"{o}lcskei}{ETH Zurich\\Switzerland}



\subsection{Editors} \scriptsize
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Venkat Anantharam}{UC Berkeley}
\journaleditor{Giuseppe Caire}{TU Berlin}
\journaleditor{Daniel Costello}{University of Notre Dame}
\journaleditor{Anthony Ephremides}{University of Maryland}
\journaleditor{Andrea Goldsmith}{Stanford University}
\journaleditor{Albert Guillen i Fabregas}{Pompeu Fabra University}
\journaleditor{Dongning Guo}{Northwestern University}
\journaleditor{Dave Forney}{MIT}
\journaleditor{Te Sun Han}{University of Tokyo}
\journaleditor{Babak Hassibi}{Caltech}
\journaleditor{Michael Honig}{Northwestern University}
\journaleditor{Tara Javidi}{UC San Diego}
%\columnbreak
\journaleditor{Ioannis Kontoyiannis}{Cambridge University}
\journaleditor{Gerhard Kramer}{TU Munich}
\journaleditor{Amos Lapidoth}{ETH Zurich}
\journaleditor{Muriel Medard}{MIT}
\journaleditor{Neri Merhav}{Technion}
\journaleditor{David Neuhoff}{University of Michigan}
\journaleditor{Alon Orlitsky}{UC San Diego}
\journaleditor{Yury Polyanskiy}{MIT}
\journaleditor{Vincent Poor}{Princeton University}
\journaleditor{Maxim Raginsky}{UIUC}
\journaleditor{Kannan Ramchandran}{UC Berkeley}
\journaleditor{Igal Sason}{Technion}
%\columnbreak
\journaleditor{Shlomo Shamai}{Technion}
\journaleditor{Amin Shokrollahi}{EPF Lausanne}
\journaleditor{Yossef Steinberg}{Technion}
\journaleditor{Wojciech Szpankowski}{Purdue University}
\journaleditor{David Tse}{Stanford University}
\journaleditor{Antonia Tulino}{Bell Labs}
\journaleditor{R\"{u}diger Urbanke}{EPF Lausanne}
\journaleditor{Emanuele Viterbo}{Monash University}
\journaleditor{Frans Willems}{TU Eindhoven}
\journaleditor{Raymond Yeung}{CUHK}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> journaldata/CIT-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{CITcolor}{officegreen}   %new color names can be defined before use
\journalcolor      {CITcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Communications and Information Theory}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {CIT}
\journalurl        {http://www.nowpublishers.com/CIT}
\journalissnprint  {1567-2190}
\journalissnonline {1567-2328 }
\journaldoi        {10.1561/01}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Communications and Information Theory publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Coded modulation}
\item{Coding theory and practice}
\item{Communication complexity}
\item{Communication system design}
\item{Cryptology and data security}
\item{Data compression}
\item{Data networks}
\item{Demodulation and Equalization}
\item{Denoising}
\item{Detection and estimation}
\item{Information theory and statistics}
\item{Information theory and computer science}
\item{Joint source/channel coding}
\item{Modulation and signal design}
\item{Multiuser detection}
\item{Multiuser information theory}
\item{Optical communication channels}
\item{Pattern recognition and learning}
\item{Quantization}
\item{Quantum information processing}
\item{Rate-distortion theory}
\item{Shannon theory}
\item{Signal processing for communications}
\item{Source coding}
\item{Storage and recording codes}
\item{Speech and Image Compression}
\item{Wireless Communications}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Communications and Information Theory, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/CIT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Redundancy of Lossless Data Compression for Known Sources by\\ Analytic Methods}\\
Michael Drmota and Wojciech Szpankowski\\
ISBN: 978-1-68083-284-6\\
\\
\noindent \textit{Multiterminal Secrecy by Public Discussion}\\
Prakash Narayan and Himanshu Tyagi\\
ISBN: 978-1-68083-186-3\\
\\
\noindent \textit{Channel Coding Methods for Non-Volatile Memories}\\
Lara Dolecek and Frederic Sala\\
ISBN: 978-1-68083-042-2\\
\\
\noindent \textit{Multi-way Communications: An Information Theoretic Perspective}\\
Anas Chaaban and Aydin Sezgin\\
978-1-60198-788-4\\
\\
\noindent \textit{An Approximation Approach to Network Information Theory}\\
A. Salman Avestimehr, Suhas N. Diggavi, Chao Tian and\\ David N. C. Tse\\
978-1-68083-026-2

==> journaldata/DBS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Joseph M. Hellerstein}{University of California at Berkeley\\United States}



\subsection{Editors} %\scriptsize
%\begin{multicols*}{3}\raggedcolumns
\journaleditor{Anastasia Ailamaki}{EPFL}
\journaleditor{Peter Bailis}{Stanford University}
\journaleditor{Mike Cafarella}{University of Michigan}
\journaleditor{Michael Carey}{University of California, Irvine}
\journaleditor{Surajit Chaudhuri}{Microsoft Research}
\journaleditor{Minos Garofalakis}{Technical University Crete}
\journaleditor{Ihab Ilyas}{University of Waterloo}
\journaleditor{Christopher Olston}{Google}
\journaleditor{Jignesh Patel}{University of Wisconsin}
\journaleditor{Chris Re}{Stanford University}
\journaleditor{Gerhard Weikum}{Max Planck Institute Saarbr{\"u}cken}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/DBS-journaldata.tex <==
 	\definecolor{officegreen}{rgb}{0.0, 0.5, 0.0}
\colorlet{DBScolor}{officegreen}   %new color names can be defined before use
\journalcolor      {DBScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Databases}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {DBS}
\journalurl        {http://www.nowpublishers.com/DBS}
\journalissnprint  {1931-7883}
\journalissnonline {1931-7891}
\journaldoi        {10.1561/19}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Databases publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Data Models and Query Languages}
    \item{Query Processing and Optimization}
    \item{Storage, Access Methods, and Indexing}
    \item{Transaction Management, Concurrency Control and Recovery}
    \item{Deductive Databases}
    \item{Parallel and Distributed Database Systems}
    \item{Database Design and Tuning}
    \item{Metadata Management}
    \item{Object Management}
    \item{Trigger Processing and Active Databases}
    \item{Data Mining and OLAP}
    \item{Approximate and Interactive Query Processing}
    \item{Data Warehousing}
    \item{Adaptive Query Processing}
    \item{Data Stream Management}
    \item{Search and Query Integration}
    \item{XML and Semi-Structured Data}
    \item{Web Services and Middleware}
    \item{Data Integration and Exchange}
    \item{Private and Secure Data Management}
    \item{Peer-to-Peer, Sensornet and Mobile Data Management}
    \item{Scientific and Spatial Data Management}
    \item{Data Brokering and Publish/Subscribe}
    \item{Data Cleaning and Information Extraction}
    \item{Probabilistic Data Management}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Databases, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/DBS-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Data Infrastructure for Medical Research}\\
Thomas Heinis and Anastasia Ailamaki\\
ISBN: 978-1-68083-348-5\\
\\
\noindent \textit{Main Memory Database Systems}\\
Franz Faerber, Alfons Kemper, Per-Ake Larson, Justin Levandoski, Thomas Neumann and Andrew Pavlo\\
ISBN: 978-1-68083-324-9\\
\\
\noindent \textit{Query Processing on Probabilistic Data: A Survey}\\
Guy Van den Broeck and Dan Suciu\\
ISBN: 978-1-68083-314-0\\
\\
\noindent \textit{Big Graph Analytics Platforms}\\
Da Yan, Yingyi Bu, Yuanyuan Tian and Amol Deshpande\\
978-1-68083-242-6

==> journaldata/ECO-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{William H. Greene}{New York University\\United States}


\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Manuel Arellano}{CEMFI Spain}
\journaleditor{Wiji Arulampalam}{University of Warwick}
\journaleditor{Orley Ashenfelter}{Princeton University}
\journaleditor{Jushan Bai}{Columbia University}
\journaleditor{Badi Baltagi}{Syracuse University}
\journaleditor{Anil Bera}{University of Illinois}
\journaleditor{Tim Bollerslev}{Duke University}
\journaleditor{David Brownstone}{UC Irvine}
\journaleditor{Xiaohong Chen}{Yale University}
\journaleditor{Steven Durlauf}{University of Wisconsin}
\journaleditor{Amos Golan}{American University}
\journaleditor{Bill Griffiths}{University of Melbourne}
\journaleditor{James Heckman}{University of Chicago}
\journaleditor{Jan Kiviet}{University of Amsterdam}
\journaleditor{Gary Koop}{The University of Strathclyde}
\journaleditor{Michael Lechner}{University of St. Gallen}
\journaleditor{Lung-Fei Lee}{Ohio State University}
\journaleditor{Larry Marsh}{Notre Dame University}
\journaleditor{James MacKinnon}{Queens University}
\journaleditor{Bruce McCullough}{Drexel University}
\journaleditor{Jeff Simonoff}{New York University}
\journaleditor{Joseph Terza}{Purdue University}
\journaleditor{Ken Train}{UC Berkeley}
\journaleditor{Pravin Travedi}{Indiana University}
\journaleditor{Adonis Yatchew}{University of Toronto}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ECO-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{ECOcolor}{brickred}   %new color names can be defined before use
\journalcolor      {ECOcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Econometrics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ECO}
\journalurl        {http://www.nowpublishers.com/ECO}
\journalissnprint  {1551-3076}
\journalissnonline {1551-3084}
\journaldoi        {10.1561/08}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Econometrics publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Econometric Models}
    \item{Simultaneous Equation Models}
    \item{Estimation Frameworks}
    \item{Biased Estimation}
    \item{Computational Problems}
    \item{Microeconometrics}
    \item{Treatment Modeling}
    \item{Discrete Choice Modeling}
    \item{Models for Count Data}
    \item{Duration Models}
   \item{Limited Dependent Variables}
    \item{Panel Data}
    \item{Time Series Analysis}
    \item{Latent Variable Models}
    \item{Qualitative Response Models}
    \item{Hypothesis Testing}
    \item{Econometric Theory}
    \item{Financial Econometrics}
    \item{Measurement Error in Survey Data}
    \item{Productivity Measurement and Analysis}
    \item{Semiparametric and Nonparametric Estimation}
    \item{Bootstrap Methods}
    \item{Nonstationary Time Series}
    \item{Robust Estimation}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Econometrics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ECO-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Data Visualization and Health Econometrics}\\
Andrew M. Jones\\
ISBN: 978-1-68083-318-8\\
\\
\noindent \textit{Spatial Econometrics: A Broad View}\\
Giuseppe Arbia\\
ISBN: 978-1-68083-172-6\\
\\
\noindent \textit{Bifurcation of Macroeconometric Models and Robustness of\\ Dynamical Inferences}\\
William A. Barnett\\
ISBN: 978-1-68083-046-0

==> journaldata/EDA-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Radu Marculescu}{Carnegie Mellon University}


\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Robert K. Brayton}{University of California, Berkeley}
\journaleditor{Raul Camposano}{Sage Design Atomation}
\journaleditor{K.T. Tim Cheng}{HKUST}
\journaleditor{Jason Cong}{University of California, Los Angeles}
\journaleditor{Masahiro Fujita}{University of Tokyo}
\journaleditor{Georges Gielen}{KU Leuven}
\journaleditor{Tom Henzinger}{IST Austria}
\journaleditor{Andrew Kahng}{University of California, San Diego}
\columnbreak
\journaleditor{Andreas Kuehlmann}{Synopsys}
\journaleditor{Sharad Malik}{Princeton University}
\journaleditor{Joel Phillips}{Cadence Berkeley Labs}
\journaleditor{Jonathan Rose}{University of Toronto}
\journaleditor{Rob Rutenbar}{University of Pittsburgh}
\journaleditor{Alberto Sangiovanni-Vincentelli}{University of California, Berkeley}
\journaleditor{Leon Stok}{IBM Research}
\end{multicols*}
\end{editorialboard} 

==> journaldata/EDA-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{EDAcolor}{brickred}   %new color names can be defined before use
\journalcolor      {EDAcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Electronic Design Automation}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {EDA}
\journalurl        {http://www.nowpublishers.com/EDA}
\journalissnprint  {1551-3939}
\journalissnonline {1551-3947}
\journaldoi        {10.1561/10}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Electronic Design Automation publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{System Level Design}
    \item{Behavioral Synthesis}
    \item{Logic Design}
    \item{Verification}
    \item{Test}
    \item{Physical Design}
    \item{Circuit Level Design}
    \item{Reconfigurable Systems}
    \item{Analog Design}
    \item{Embedded software and parallel programming}
   \item{Multicore, GPU, FPGA, and heterogeneous systems}
    \item{Distributed, networked embedded systems}
    \item{Real-time and cyberphysical systems}
\end{itemize}
% \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Electronic Design Automation, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/EDA-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Error-Efficient Computing Systems}\\
Phillip Stanley-Marbell and Martin Rinard\\
ISBN: 978-1-68083-358-4\\
\\
\noindent \textit{Secure Processors Part II: Intel SGX Security Analysis\\ and MIT Sanctum Architecture}\\
Victor Costan, Ilia Lebedev and Srinivas Devadas\\
ISBN: 978-1-68083-302-7\\
\\
\noindent \textit{Secure Processors Part I: Background, Taxonomy for Secure Enclaves\\ and Intel SGX Architecture}\\
Victor Costan, Ilia Lebedev and Srinivas Devadas\\
ISBN: 978-1-68083-300-3

==> journaldata/EES-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Marija D. Ili\'c}{Carnegie Mellon University\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Istv\'an Erlich}{University of Duisburg-Essen}
\journaleditor{David Hill}{University of Hong Kong and University of Sydney}
\journaleditor{Daniel Kirschen}{University of Washington}
\journaleditor{J. Zico Kolter}{Carnegie Mellon University}
\journaleditor{Chao Lu}{Tsinghua University}
\journaleditor{Steven Low}{California Institute of Technology}
\journaleditor{Ram Rajagopa}{Stanford University}
\journaleditor{Lou van der Sluis}{TU Delft}
\journaleditor{Goran Strbac}{Imperial College London}
\journaleditor{Robert J. Thomas}{Cornell University}
\journaleditor{David Tse}{University of California, Berkeley}
\journaleditor{Le Xie}{Texas A\&M University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/EES-journaldata.tex <==
\definecolor{cinnabar}{rgb}{0.89, 0.26, 0.2}
\colorlet{EEScolor}{cinnabar}   %new color names can be defined before use
\journalcolor      {EEScolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Electric Energy Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {EES}
\journalurl        {http://www.nowpublishers.com/EES}
\journalissnprint  {2332-6557}
\journalissnonline {2332-6565}
\journaldoi        {10.1561/31}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Electric Energy Systems publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Advances in power dispatch}
\item{Demand-side and grid scale data analytics}
\item{Design and optimization of electric services}
\item{Distributed control and optimization of distribution networks}
\item{Distributed sensing for the grid}
\item{Distribution systems}
\item{Fault location and service restoration}
\item{Integration of physics-based and data-driven modeling of future electric energy systems}
\item{Integration of Power electronics, Networked FACTS}
\item{Integration of renewable energy sources}
\item{Interdependence of power system operations and planning and the electricity markets}
\item{Microgrids}
\item{Modern grid architecture}
\item{Power system analysis and computing}
\item{Power system dynamics}
\item{Power system operation}
\item{Power system planning}
\item{Power system reliability}
\item{Power system transients}
\item{Security and privacy}
\item{Stability and control for the whole multi-layer (granulated) network with new load models (to include storage, DR, EVs) and new generation}
\item{System protection and control}
\item{The new stability guidelines and control structures for supporting high penetration of renewables (>50\%)}
\item{Uncertainty quantification for the grid}
\item{System impacts of HVDC}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Electric Energy Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/EES-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Sustainable Transportation with Electric Vehicles}\\
Fanxin Kong and Xue Liu\\
ISBN: 978-1-68083-388-1\\
\\
\noindent \textit{Unit Commitment in Electric Energy Systems}\\
Miguel F. Anjos and Antonio J. Conejo\\
ISBN: 978-1-68083-370-6\\
\\
\noindent \textit{Reliability Standards for the Operation and Planning of Future\\ Electricity Networks}\\
Goran Strbac, Daniel Kirschen and Rodrigo Moreno\\
ISBN: 978-1-68083-182-5\\
\\
\noindent \textit{Toward a Unified Modeling and Control for Sustainable and Resilient Electric Energy Systems}\\
Marija D. Ilic\\
ISBN: 978-1-68083-226-6

==> journaldata/ENT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{1}
\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}
\journalchiefeditor{David B. Audretsch}{Indiana University\\United States}\\
\journalchiefeditor{Mike Wright}{Imperial College London\\United Kingdom}
\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Howard Aldrich}{University of North Carolina}
\journaleditor{Sharon Alvarez}{University of Denver}
\journaleditor{Per Davidsson}{Queensland University of Technology}
\journaleditor{Michael Frese}{National University of Singapore}
\journaleditor{William B. Gartner}{Copenhagen Business School}
\journaleditor{Magnus Henrekson}{IFN Stockholm}
\journaleditor{Michael A. Hitt}{Texas A\&M University}
\journaleditor{Joshua Lerner}{Harvard University}
\columnbreak
\journaleditor{Jeff McMullen}{Indiana University}
\journaleditor{P.R. Kumar}{Texas A\&M University}
\journaleditor{Maria Minniti}{Syracuse University}
\journaleditor{Simon Parker}{University of Western Ontario}
\journaleditor{Holger Patzelt}{TU Munich}
\journaleditor{Saras Sarasvathy}{University of Virginia}
\journaleditor{Roy Thurik}{Erasmus University}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ENT-journaldata.tex <==
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\colorlet{ENTcolor}{Cerulean}   %new color names can be defined before use
\journalcolor      {ENTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Entrepreneurship}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ENT}
\journalurl        {http://www.nowpublishers.com/ENT}
\journalissnprint  {1551-3114}
\journalissnonline {1551-3122}
\journaldoi        {10.1561/03}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Entrepreneurship publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Nascent and start-up entrepreneurs}
\item{Opportunity recognition}
\item{New venture creation process}
\item{Business formation}
\item{Firm ownership}
\item{Market value and firm growth}
\item{Franchising}
\item{Managerial characteristics and behavior of entrepreneurs}
\item{Strategic alliances and networks}
\item{Government programs and public policy}
\item{Gender and ethnicity}
\columnbreak
\item{New business financing:}
	\begin{itemize}
\item{Business angels}
\item{Bank financing, debt, and trade credit}
\item{Venture capital and private equity capital}
\item{Public equity and IPOs} 
\end{itemize}
\item{Family-owned firms}
\item{Management structure, governance and performance}
\item{Corporate entrepreneurship}
\item{High technology:}
	\begin{itemize}
        \item{Technology-based new firms}
        \item{High-tech clusters}
        \end{itemize}
\item{Small business and economic growth}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Entrepreneurship, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ENT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Corporate Entrepreneurship 2.0: Research Development and Future\\ Directions}\\
Donald F. Kuratko\\
ISBN: 978-1-68083-342-3\\
\\
\noindent \textit{Angel Investing: A Literature Review}\\
Linda F. Edelman, Tatiana S. Manolova and Candida G. Brush\\
ISBN: 978-1-68083-298-3\\
\\
\noindent \textit{Entrepreneurship and Institutions: A Bidirectional Relationship}\\
Niklas Elert and Magnus Henrekson\\
ISBN: 978-1-68083-320-1\\
\\
\noindent \textit{Households as a Site of Entrepreneurial Activity}\\
Sara Carter, Aniela Kuhl, Susan Marlow and Samuel Mwaura\\
ISBN: 978-1-68083-272-3\\
\\
\noindent \textit{Agglomeration, Industrial Districts and Industry Clusters:\\ Trends of the 21st Century Literature }\\
Brett Anitra Gilbert\\
ISBN: 978-1-68083-266-2\\

==> journaldata/FIN-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\begin{multicols}{1}
\journalchiefeditor{Sheridan Titman}{University of Texas at Austin\\United States}
\end{multicols}

\subsection{Associate Editors}
\begin{multicols}{1}
\journaleditor{Josef Zechner}{WU Vienna University of Economics and Finance}
\journaleditor{Chester Spatt}{Carnegie Mellon University}
\end{multicols}
\end{editorialboard} 

==> journaldata/FIN-journaldata.tex <==
\definecolor{ceruleanblue}{rgb}{0.16, 0.32, 0.75}
\colorlet{FINcolor}{ceruleanblue}   %new color names can be defined before use
\journalcolor      {FINcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Finance}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {FIN}
\journalurl        {http://www.nowpublishers.com/FIN}
\journalissnprint  {1567-2395}
\journalissnonline {1567-2409}
\journaldoi        {10.1561/05}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Finance publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Corporate Finance}
\begin{itemize}
\item{Corporate Governance}
\item{Corporate Financing}
\item{Dividend Policy and Capital Structure}
\item{Corporate Control}
\item{Investment Policy}
\item{Agency Theory and Information}
\end{itemize}
\end{itemize}
\columnbreak
\begin{itemize}
\item{Financial Markets}
\begin{itemize}
\item{Market Microstructure}
\item{Portfolio Theory}
\item{Financial Intermediation}
\item{Investment Banking}
\item{Market Efficiency}
\item{Security Issuance}
\item{Anomalies and Behavioral Finance}
\end{itemize}
\end{itemize}
\end{multicols}
%}
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
%\columnbreak
%\begin{itemize}
\item{Asset Pricing}
\begin{itemize}
\item{Asset-Pricing Theory}
\item{Asset-Pricing Models}
\item{Tax Effects}
\item{Liquidity} 
\item{Equity Risk Premium} 
\item{Pricing Models and Volatility} 
\item{Fixed Income Securities} 
\end{itemize}
\end{itemize}
\columnbreak
\begin{itemize}
\item{Derivatives}
\begin{itemize}
\item{Computational Finance}
\item{Futures Markets and Hedging}
\item{Financial Engineering}
\item{Interest Rate Derivatives}
\item{Credit Derivatives}
\item{Financial Econometrics}
\item{Estimating Volatilities and Correlations}
\end{itemize}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Finance, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/FIN-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Initial Public Offerings: A Synthesis of the Literature and Directions for Future Research}\\
Michelle Lowry, Roni Michaely and Ekaterina Volkova\\
ISBN: 978-1-68083-340-9\\

\noindent \textit{Privatization, State Capitalism, and State Ownership of Business in the 21st Century}\\
William L. Megginson\\
ISBN: 978-1-68083-338-6\\

\noindent \textit{Executive Compensation}\\
Raghavendra Rau\\
ISBN: 978-1-68083-296-9\\
\\
\noindent \textit{Three Branches of Theories of Financial Crises}\\
Itay Goldstein and Assaf Razin\\
ISBN: 978-1-68083-084-2\\
\\
\noindent \textit{The Economics and Finance of Hedge Funds: A Review of the\\ Academic Literature}\\
Vikas Agarwal, Kevin A. Mullally, and Narayan Y. Naik\\
ISBN: 978-1-68083-156-6\\

==> journaldata/HCI-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Desney S. Tan}{Microsoft Research}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Ben Bederson}{University of Maryland}
\journaleditor{Sheelagh Carpendale}{University of Calgary}
\journaleditor{Andy Cockburn}{University of Canterbury}
\journaleditor{Jon Froehlich}{University of Washington}
\journaleditor{Juan Pablo Hourcade}{University of Iowa}
\journaleditor{Karrie Karahalios}{University of Illinois at Urbana-Champaign}
\journaleditor{Youn-Kyung Lim}{Korea Advanced Institute of Science and Technology}
\journaleditor{Nuria Oliver}{Telefonica}
\journaleditor{Orit Shaer}{Wellesley College}
\journaleditor{Kentaro Toyama}{University of Michigan}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/HCI-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{HCIcolor}{pinegreen}   %new color names can be defined before use
\journalcolor      {HCIcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Human-Computer Interaction}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {HCI}
\journalurl        {http://www.nowpublishers.com/HCI}
\journalissnprint  {1551-3955}
\journalissnonline {1551-3963}
\journaldoi        {10.1561/11}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Human-Computer Interaction publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{History of the research community}
\item{Theory}
\item{Technology}
\item{Computer Supported Cooperative Work}
\item{Interdisciplinary influence}
\item{Advanced topics and trends}
\end{itemize}
%\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Human-Computer Interaction, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/HCI-seriespage.tex <==
\vspace{12pt}
\noindent \textit{HCIs Making Agendas}\\
Jeffrey Bardzell, Shaowen Bardzell, Cindy Lin, Silvia Lindtner and Austin Toombs\\
ISBN: 978-1-68083-372-0\\
\\
\noindent \textit{A Survey of Value Sensitive Design Methods}\\
Batya Friedman, David G. Hendry and Alan Borning\\
ISBN: 978-1-68083-290-7\\
\\
\noindent \textit{Communicating Personal Genomic Information to Non-experts:\\ A New Frontier for Human-Computer Interaction}\\
Orit Shaer, Oded Nov, Lauren Westendorf and Madeleine Ball\\
ISBN: 978-1-68083-254-9\\
\\
\noindent \textit{Personal Fabrication}\\
Patrick Baudisch and Stefanie Mueller \\
ISBN: 978-1-68083-258-7\\
\\
\noindent \textit{Canine-Centered Computing}\\
Larry Freil, Ceara Byrne, Giancarlo Valentin, Clint Zeagler,\\ David Roberts, Thad Starner and Melody Jackson\\
ISBN: 978-1-68083-244-0\\
\\
\noindent \textit{Exertion Games}\\
Florian Mueller, Rohit Ashok Khot, Kathrin Gerling and\\ Regan Mandryk\\
ISBN: 978-1-68083-202-0

==> journaldata/INR-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Maarten de Rijke}{University of Amsterdam\\The Netherlands}
\journalchiefeditor{Yiqun Liu}{Tsinghua University\\China}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Barbara Poblete}{University of Chile}
\journaleditor{Claudia Hauff}{Delft University of Technology}
\journaleditor{Diane Kelly}{University of Tennessee}
\journaleditor{Doug Oard}{University of Maryland}
\journaleditor{Ellen M. Voorhees}{National Institute of Standards and Technology}
\journaleditor{Fabrizio Sebastiani}{Consiglio Nazionale delle Ricerche, Italy}
\journaleditor{Hang Li}{Bytedance Technology}
\journaleditor{Helen Huang}{University of Queensland}
\journaleditor{Ian Ruthven}{University of Strathclyde, Glasgow}
\journaleditor{Jaap Kamps}{University of Amsterdam}
\journaleditor{Jian-Yun Nie}{Universit{\'e} de Montreal}
\columnbreak
\journaleditor{Jimmy Lin}{University of Maryland}
\journaleditor{Leif Azzopardi}{University of Glasgow}
\journaleditor{Lynda Tamine}{University of Toulouse}
\journaleditor{Rodrygo Luis Teodoro Santos}{Universidade Federal de Minas Gerais}
\journaleditor{Ryen White}{Microsoft Research}
\journaleditor{Shane Culpepper}{RMIT}
\journaleditor{Soumen Chakrabarti}{Indian Institute of Technology}
\journaleditor{Tie-Yan Liu}{Microsoft Research}
\journaleditor{Xuanjing Huang}{Fudan University}
\journaleditor{Zi Helen Huang}{University of Queensland}
\end{multicols*}
\end{editorialboard} 

==> journaldata/INR-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{INRcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {INRcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Information Retrieval}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {INR}
\journalurl        {http://www.nowpublishers.com/INR}
\journalissnprint  {1554-0669}
\journalissnonline {1554-0677}
\journaldoi        {10.1561/15}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Information Retrieval publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Applications of IR}
\item{Architectures for IR}
\item{Collaborative filtering and recommender systems}
\item{Cross-lingual and multilingual IR}
\item{Distributed IR and federated search}
\item{Evaluation issues and test collections for IR}
\item{Formal models and language models for IR}
\item{IR on mobile platforms}
\item{Indexing and retrieval of structured documents}
\item{Information categorization and clustering}
\item{Information extraction}
\item{Information filtering and routing}
\item{Metasearch, rank aggregation and data fusion}
\item{Natural language processing for IR}
\item{Performance issues for IR systems, including algorithms, data structures, optimization techniques, and scalability}
\item{Question answering}
\item{Summarization of single documents, multiple documents, and corpora}
\item{Text mining}
\item{Topic detection and tracking}
\item{Usability, interactivity, and visualization issues in IR}
\item{User modelling and user studies for IR}
\item{Web search}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Information Retrieval, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 5 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/INR-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Efficient Query Processing for Scalable Web Search}\\
Nicola Tonellotto, Craig Macdonald and Iadh Ounis\\
ISBN: 978-1-68083-542-7\\

\noindent \textit{Geographic Information Retrieval: Progress and Challenges in Spatial Search of Text}\\
Ross S. Purves, Paul Clough, Christopher B. Jones, Mark H. Hall and\\ Vanessa Murdock\\
ISBN: 978-1-68083-412-3\\

\noindent \textit{Web Forum Retrieval and Text Analytics: A Survey}\\
Doris Hoogeveen, Li Wang, Timothy Baldwin and Karin M. Verspoor\\
ISBN: 978-1-68083-350-8

==> journaldata/ISY-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

%\begin{multicols}{1}
\journalchiefeditor{Joey George}{Iowa State University\\United States}
%\end{multicols}

\subsection{Honorary Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Izak Benbasat}{University of British Columbia}
\journaleditor{Alan R. Dennis}{Kelley School of Business, Indiana University}
\journaleditor{Jacqueline Rees Ulmer}{Iowa State University}
\journaleditor{Veda Storey}{Georgia State University}
\journaleditor{Detmar Straub}{Georgia State University}
\journaleditor{Hugh Watson}{University of Georgia}
%\end{multicols*}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Alan Hevner}{University of South Florida}
\journaleditor{David Paradice}{Auburn University}
\journaleditor{Carol Saunders}{University of Central Florida}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/ISY-journaldata.tex <==
\definecolor{regalia}{rgb}{0.32, 0.18, 0.5}
\colorlet{ISYcolor}{regalia}   %new color names can be defined before use
\journalcolor      {ISYcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Information Systems}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ISY}
\journalurl        {http://www.nowpublishers.com/ISY}
\journalissnprint  {2331-1231}
\journalissnonline {2331-124X}
\journaldoi        {10.1561/29}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Information Systems publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{IS and Individuals}
\item{IS and Groups}
\item{IS and Organizations}
\item{IS and Industries}
\item{IS and Society}
\item{IS Development}
\item{IS Economics}
\item{IS Management}
\item{IS Research Methods}
\end{itemize}
% \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Information Systems, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ISY-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Longitudinal Author Cocitation Mapping: The Changing Structure\\ of Decision Support Systems Research (1969 - 2012)}\\
Sean Eom\\
ISBN: 978-1-68083-120-7\\
\\
\noindent \textit{Pondering the Fault Lines of Anywhere Working\\ (Telework, Telecommuting): A Literature Review}\\
Yvette Blount\\
ISBN: 978-1-60198-876-8\\
\\
\noindent \textit{Application of Dual-process Theory to Information Systems:\\ Current and Future Research Directions}\\
Stephanie Watts\\
ISBN: 978-1-68083-058-3\\
\\
\noindent \textit{E-business Value Creation from a Resource-Based Perspective:\\ 
A Review of the Last Decade of Empirical Research}\\
Orit Raphaeli, Sigal Berman and Lior Fink\\
ISBN: 978-1-60198-878-2\\

==> journaldata/MAL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Michael Jordan}{University of California, Berkeley\\United States}



\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Peter Bartlett}{UC Berkeley}
\journaleditor{Yoshua Bengio}{Universit{\'e} de Montr{\'e}al}
\journaleditor{Avrim Blum}{Toyota Technological Institute}
\journaleditor{Craig Boutilier}{University of Toronto}
\journaleditor{Stephen Boyd}{Stanford University}
\journaleditor{Carla Brodley}{Northeastern University}
\journaleditor{Inderjit Dhillon}{Texas at Austin}
\journaleditor{Jerome Friedman}{Stanford University}
\journaleditor{Kenji Fukumizu}{ISM}
\journaleditor{Zoubin Ghahramani}{Cambridge University}
\journaleditor{David Heckerman}{Amazon}
\journaleditor{Tom Heskes}{Radboud University}
\journaleditor{Geoffrey Hinton}{University of Toronto}
\journaleditor{Aapo Hyvarinen}{Helsinki IIT}
\journaleditor{Leslie Pack Kaelbling}{MIT}
\journaleditor{Michael Kearns}{UPenn}
\journaleditor{Daphne Koller}{Stanford University}
\journaleditor{John Lafferty}{Yale}
\journaleditor{Michael Littman}{Brown University}
\journaleditor{Gabor Lugosi}{Pompeu Fabra}
\journaleditor{David Madigan}{Columbia University}
\journaleditor{Pascal Massart}{Universit{\'e} de Paris-Sud}
\journaleditor{Andrew McCallum}{University of Massachusetts Amherst}
\journaleditor{Marina Meila}{University of Washington}
\journaleditor{Andrew Moore}{CMU}
\journaleditor{John Platt}{Microsoft Research}
\journaleditor{Luc de Raedt}{KU Leuven}
\journaleditor{Christian Robert}{Paris-Dauphine}
\journaleditor{Sunita Sarawagi}{IIT Bombay}
\journaleditor{Robert Schapire}{Microsoft Research}
\journaleditor{Bernhard Schoelkopf}{Max Planck Institute}
\journaleditor{Richard Sutton}{University of Alberta}
\journaleditor{Larry Wasserman}{CMU}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> journaldata/MAL-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MALcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MALcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Machine Learning}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MAL}
\journalurl        {http://www.nowpublishers.com/MAL}
\journalissnprint  {1935-8237}
\journalissnonline {1935-8245}
\journaldoi        {10.1561/22}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Machine Learning publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Adaptive control and signal processing}
\item{Applications and case studies}
\item{Behavioral, cognitive and neural learning}
\item{Bayesian learning}
\item{Classification and prediction}
\item{Clustering}
\item{Data mining}
\item{Dimensionality reduction}
\item{Evaluation}
\item{Game theoretic learning}
\item{Graphical models}
\item{Independent component analysis}
\item{Inductive logic programming}
\item{Kernel methods}
\item{Markov chain Monte Carlo}
\item{Model choice}
\item{Nonparametric methods}
\item{Online learning}
\item{Optimization}
\item{Reinforcement learning}
\item{Relational learning}
\item{Robustness}
\item{Spectral methods}
\item{Statistical learning theory}
\item{Variational inference}
\item{Visualization}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Machine Learning, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 6 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MAL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Non-convex Optimization for Machine Learningy}\\
Prateek Jain and Purushottam Ka\\
ISBN: 978-1-68083-368-3\\
\\
\noindent \textit{Kernel Mean Embedding of Distributions: A Review and Beyond}\\
Krikamol Muandet, Kenji Fukumizu, Bharath Sriperumbudur and\\ Bernhard Scholkopf\\
ISBN: 978-1-68083-288-4\\
\\
\noindent \textit{Tensor Networks for Dimensionality Reduction and Large-scale\\ Optimization: Part 1 Low-Rank Tensor Decompositions}\\
Andrzej Cichocki, Anh-Huy Phan, Qibin Zhao, Namgil Lee,\\ Ivan Oseledets, Masashi Sugiyama and Danilo P. Mandic\\
ISBN: 978-1-68083-222-8\\
\\
\noindent \textit{Tensor Networks for Dimensionality Reduction and Large-scale\\ Optimization: Part 2 Applications and Future Perspectives}\\
Andrzej Cichocki, Anh-Huy Phan, Qibin Zhao, Namgil Lee,\\ Ivan Oseledets, Masashi Sugiyama and Danilo P. Mandic\\
ISBN: 978-1-68083-276-1\\
\\
\noindent \textit{Patterns of Scalable Bayesian Inference}\\
Elaine Angelino, Matthew James Johnson and Ryan P. Adams \\
ISBN: 978-1-68083-218-1\\
\\
\noindent \textit{Generalized Low Rank Models}\\
Madeleine Udell, Corinne Horn, Reza Zadeh and Stephen Boyd \\
ISBN: 978-1-68083-140-5

==> journaldata/MGT-editorialboard.tex <==
%ACG-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{2}\raggedright
\journalchiefeditor{Nicholas S. Argyres}{Olin Business School, Washington University\\United States}
\journalchiefeditor{Timothy M. Devinney}{Leeds University Business School\\United Kingdom}
\journalchiefeditor{James Campbell Quick}{The University of Texas at Arlington\\United States}
\end{multicols}

\subsection{Editors}
\begin{multicols}{3}\raggedright \raggedcolumns
\renewcommand\journaleditor[2]{\par\textbf{#1}\\#2}%
\subsubsection{\footnotesize International Business}

\journaleditor{Gabriel R.G. Benito}{BI Norwegian School of Management}
\journaleditor{Allan Bird}{Northeastern University}
\journaleditor{Julian Birkinshaw}{London Business School}
\journaleditor{Peter Buckley}{University of Leeds}
\journaleditor{Saul Estrin}{London School of Economics}
\journaleditor{Sarianna Lundin}{University of Bremen}
\journaleditor{Xavier Martin}{Tilburg University} 
\journaleditor{Ram Mudambi}{Temple University}

\columnbreak

\subsubsection{\footnotesize Organizational Behavior}

\journaleditor{Myrtle Bell}{University of Texas at Arlington}
\journaleditor{Cary Cooper}{Lancaster University}
\journaleditor{Richard Griffin}{Texas A\&M University}
\journaleditor{Sean Hannah}{Wake Forest University}
\journaleditor{Debra Nelson}{Oklahoma State University}
\journaleditor{Pamela Perrewe}{Florida State University}

\columnbreak

\subsubsection{\footnotesize Strategy}

\journaleditor{Rajshree Agarwal}{University of Maryland}
\journaleditor{Marvin Lieberman}{UCLA}) 
\journaleditor{Michael Lenox}{University of Virginia}
\journaleditor{Joseph Mahoney}{University of Illinois at Urbana-Champaign}
\journaleditor{Jesper Sørensen}{Stanford University}
\journaleditor{Olav Sorenson}{Yale University}
\end{multicols}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MGT-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{MGTcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {MGTcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Management}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MGT}
\journalurl        {http://www.nowpublishers.com/MGT}
\journalissnprint  {2475-6946}
\journalissnonline {2475-6954}
\journaldoi        {10.1561/34}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Management publishes
 survey and tutorial articles in the following topics:
% \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{International Business}
\item{Organizational Behavior}
\item{Strategic Management}
\end{itemize}
 %\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Management, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MIC-editorialboard.tex <==
%MIC-Editorialboard.

\begin{editorialboard}

%\subsection{Editor-in-Chief}

\journalchiefeditor{W. Kip Viscusi}{Vanderbilt University Law School\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Richard Carson}{University of California, San Diego}
\journaleditor{William Gentry}{Williams College}
\journaleditor{Tom Kniesner}{Syracuse University}
\journaleditor{Mark V. Pauly}{University of Pennsylvania}
\journaleditor{Yossi Spiegel}{Tel Aviv University}
\journaleditor{William Zame}{University of California, Los Angeles}
\journaleditor{James Ziliak}{University of Kentucky}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MIC-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{MICcolor}{pinegreen}   %new color names can be defined before use   %new color names can be defined before use
\journalcolor      {MICcolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Microeconomics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MIC}
\journalurl        {http://www.nowpublishers.com/MIC}
\journalissnprint  {1547-9846}
\journalissnonline {1547-9854}
\journaldoi        {10.1561/07}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Microeconomics publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Environmental economics}
\item{Health economics}
\item{Industrial organization}
\item{Labor economics}
\item{Law and economics}
\item{Public economics}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Microeconomics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MIC-seriespage.tex <==
\vspace{12pt}
\vspace{12pt}
\noindent \textit{Natural Gas Pipeline Regulation in the United States: Past, Present, and Future}\\
Matthew E. Oliver
\\ISBN: 978-1-68083-452-9
\\
\\
\noindent \textit{The U.S. Market for Uranium: 70 Years of History}\\
Charles F. Mason
\\ISBN: 978-1-68083-382-9
\\
\\
\noindent \textit{Game Theory and Water Resources: Critical Review of its Contributions, Progress and Remaining Challenges}\\
Ariel Dinar and Margaret Hogarth
\\ISBN: 978-1-68083-016-3


==> journaldata/MKT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Jehoshua Eliashberg}{University of Pennsylvania}

\subsection{Associate Editors}

\journaleditor{Bernd Schmitt}{Columbia University}


\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Bell}{University of Pennsylvania}
\journaleditor{Gerrit van Bruggen}{Erasmus University}
\journaleditor{Christophe van den Bulte}{University of Pennsylvania}
\journaleditor{Amitava Chattopadhyay}{INSEAD}
\journaleditor{Pradeep Chintagunta}{University of Chicago}
\journaleditor{Dawn Iacobucci}{Vanderbilt University}
\journaleditor{Raj Ragunathan}{University of Texas, Austin}
\journaleditor{J. Miguel Villas-Boas}{University of California, Berkeley}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/MKT-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MKTcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MKTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Marketing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MKT}
\journalurl        {http://www.nowpublishers.com/MKT}
\journalissnprint  {1555-0753}
\journalissnonline {1555-0761}
\journaldoi        {10.1561/17}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Marketing publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{B2B Marketing}
\item{Bayesian Models}
\item{Behavioral Decision Making}
\item{Branding and Brand Equity}
\item{Channel Management}
\item{Choice Modeling}
\item{Comparative Market Structure}
\item{Competitive Marketing Strategy}
\item{Conjoint Analysis}
\item{Customer Equity}
\item{Customer Relationship Management}
\item{Game Theoretic Models}
\item{Group Choice and Negotiation}
\item{Discrete Choice Models}
\item{Individual Decision Making}
\item{Marketing Decisions Models}
\item{Market Forecasting}
\item{Marketing Information Systems}
\item{Market Response Models}
\item{Market Segmentation}
\item{Market Share Analysis}
\item{Multi-channel Marketing}
\item{New Product Diffusion}
\item{Pricing Models}
\item{Product Development}
\item{Product Innovation}
\item{Sales Forecasting}
\item{Sales Force Management}
\item{Sales Promotion}
\item{Services Marketing}
\item{Stochastic Model}
\end{itemize}
 \end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Marketing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/MKT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Modeling Dynamic Relations Among Marketing and Performance Metrics}\\
Koen H. Pauwels \\
ISBN:978-1-68083-490-1\\
\\
\noindent \textit{Sales Force Compensation: Trends and Research Opportunities}\\
Dominique Rouziès and Vincent Onyemah\\
ISBN: 978-1-68083-488-8\\
\\
\noindent \textit{From Doubt to Functionality: An Imagery Story}\\
Rashmi Adaval\\
ISBN:978-1-68083-458-1\\
\\
\noindent \textit{Consumer Informational Privacy}\\
Frank T. Beke, Felix Eggers and Peter C. Verhoef \\
ISBN: 978-1-68083-168-9


==> journaldata/NET-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Anthony Ephremides}{University of Maryland\\United States}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Fran\c{c}ois Baccelli}{University of Texas, Austin}
\journaleditor{Victor Bahl}{Microsoft Research}
\journaleditor{Helmut B\"{o}lcskei}{ETH Zurich}
\journaleditor{J.J. Garcia-Luna Aceves}{UC Santa Cruz}
\journaleditor{Andrea Goldsmith}{Stanford University}
\journaleditor{Roch Guerin}{Washington University in Saint Louis}
\journaleditor{Bruce Hajek}{UIUC}
\journaleditor{Jean-Pierre Hubaux}{EPFL}
\journaleditor{Frank Kelly}{University of Cambridge}
\journaleditor{P.R. Kumar}{Texas A\&M University}
\journaleditor{Steven Low}{Caltech}
\journaleditor{Eytan Modiano}{MIT}
\columnbreak
\journaleditor{Keith Ross}{Polytechnic Institute of NYU}
\journaleditor{Henning Schulzrinne}{Columbia University}
\journaleditor{Mani Srivastava}{UCLA}
\journaleditor{Leandros Tassiulas}{Yale University}
\journaleditor{Lang Tong}{Cornell University}
\journaleditor{Ozan Tonguz}{Carnegie Mellon University}
\journaleditor{Don Towsley}{University of Massachusetts, Amherst}
\journaleditor{Nitin Vaidya}{UIUC}
\journaleditor{Pravin Varaiya}{UC Berkeley}
\journaleditor{Roy Yates}{Rutgers University}
\journaleditor{Raymond Yeung}{Chinese University of Hong Kong}
\end{multicols*}
\end{editorialboard} 

==> journaldata/NET-journaldata.tex <==
\definecolor{cerise}{rgb}{0.87, 0.19, 0.39}
\colorlet{NETcolor}{cerise}   %new color names can be defined before use
\journalcolor      {NETcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Networking}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {NET}
\journalurl        {http://www.nowpublishers.com/NET}
\journalissnprint  {1554-057X}
\journalissnonline {1554-0588}
\journaldoi        {10.1561/13}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Networking publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Modeling and Analysis of:}
	\begin{itemize}
	\item{Ad Hoc Wireless Networks}
	\item{Sensor Networks}
	\item{Optical Networks}
	\item{Local Area Networks}
	\item{Satellite and Hybrid Networks}
	\item{Cellular Networks}
	\item{Internet and Web Services}
	\end{itemize}
\item{Protocols and Cross-Layer Design}
\item{Network Coding}
\item{Energy-Efficiency Incentives/Pricing/Utility-based}
\item{Games (co-operative or not)}
\item{Security}
\item{Scalability}
\item{Topology}
\item{Control/Graph-theoretic models}
\item{Dynamics and Asymptotic Behavior of Networks}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Networking, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/NET-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Age of Information: A New Concept, Metric, and Tool}\\
Antzela Kosta, Nikolaos Pappas and Vangelis Angelakis\\
ISBN: 978-1-68083-360-7\\
\\
\noindent \textit{Network and Protocol Architectures for Future Satellite Systems}\\
Tomaso de Cola, Alberto Ginesi, Giovanni Giambene,\\ George C. Polyzos, Vasilios A. Siris, Nikos Fotiou and Yiannis Thomas\\
ISBN: 978-1-68083-334-8\\
\\
\noindent \textit{Duality of the Max-Plus and Min-Plus Network Calculus}\\
Jorg Liebeherr\\
ISBN: 978-1-68083-294-5\\
\\
\noindent \textit{Opportunistic Routing in Wireless Networks}\\
Tara Javidi and Eric Van Buhler\\
ISBN: 978-1-68083-150-4

==> journaldata/NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> journaldata/OPT-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

%\begin{multicols}{1}
\journalchiefeditor{Stephen P. Boyd}{Stanford University, USA}
\journalchiefeditor{Yinyu Ye}{Stanford University, USA}
\journalchiefeditor{Garud Iyengar}{Columbia University, USA}
%\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Dimitris Bertsimas}{Massachusetts Institute of Technology}
\journaleditor{John R. Birge}{The University of Chicago}
\journaleditor{Robert E. Bixby}{Rice University}
\journaleditor{Emmanuel Candes}{Stanford University}
\journaleditor{David Donoho}{Stanford University}
\journaleditor{Laurent El Ghaoui}{University of California, Berkeley}
\journaleditor{Donald Goldfarb}{Columbia University}
\journaleditor{Michael I. Jordan}{University of California, Berkeley}
\journaleditor{Zhi-Quan (Tom) Luo}{University of Minnesota, Twin Cites}
\journaleditor{George L. Nemhauser}{Georgia Institute of Technology}
\journaleditor{Arkadi Nemirovski}{Georgia Institute of Technology}
\columnbreak
\journaleditor{Yurii Nesterov}{HSE University}
\journaleditor{Jorge Nocedal}{Northwestern University}
\journaleditor{Pablo A. Parrilo}{Massachusetts Institute of Technology}
\journaleditor{Boris T. Polyak}{Institute for Control Science, Moscow}
\journaleditor{Tam\'as Terlaky}{Lehigh University}
\journaleditor{Michael J. Todd}{Cornell University}
\journaleditor{Kim-Chuan Toh}{National University of Singapore}
\journaleditor{John N. Tsitsiklis}{Massachusetts Institute of Technology}
\journaleditor{Lieven Vandenberghe}{University of California, Los Angeles}
\journaleditor{Robert J. Vanderbei}{Princeton University}
\journaleditor{Stephen J. Wright}{University of Wisconsin}
\end{multicols*}
\end{editorialboard} 

==> journaldata/OPT-journaldata.tex <==
\definecolor{cerulean}{rgb}{0.0, 0.48, 0.65}
\colorlet{OPTcolor}{Cerulean}   %new color names can be defined before use
\journalcolor      {OPTcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Optimization}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {OPT}
\journalurl        {http://www.nowpublishers.com/OPT}
\journalissnprint  {2167-3888}
\journalissnonline {2167-3918}
\journaldoi        {10.1561/24}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Optimization publishes
 survey and tutorial articles in the following topics: 
%\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{algorithm design, analysis, and implementation (especially, on modern computing platforms}
\item{models and modeling systems, new optimization formulations for practical problems}
\item{applications of optimization in machine learning, statistics, and data analysis, signal and image processing, computational economics and finance, engineering design, scheduling and resource allocation, and other areas}
\end{itemize}
 %\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Optimization, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/OPT-seriespage.tex <==
\vspace{12pt}
\noindent \textit{The Many Faces of Degeneracy in Conic Optimization}\\
Dmitriy Drusvyatskiy and Henry Wolkowicz\\
ISBN: 978-1-68083-390-4\\
\\
\noindent \textit{Multi-Period Trading via Convex Optimization}\\
Stephen Boyd, Enzo Busseti, Steve Diamond, Ronald N. Kahn,\\ Kwangmoo Koh, Peter Nystrup and Jan Speth \\
ISBN: 978-1-68083-298-3\\
\\
\noindent \textit{Introduction to Online Convex Optimization}\\
Elad Hazan\\
ISBN: 978-1-68083-170-2\\
\\
\noindent \textit{Low-Rank Semidefinite Programming: Theory and Applications}\\
Alex Lemon, Anthony Man-Cho So and Yinyu Ye\\
ISBN: 978-1-68083-136-8

==> journaldata/PGL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Mooly Sagiv}{Tel-Aviv University, Israel}


\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Mart\'in Abadi}{Google and UC Santa Cruz}
\journaleditor{Anindya Banerjeei}{IMDEA Software Instituet}
\journaleditor{Patrick Cousoti}{ENS, Paris and NYU}
\journaleditor{Oege De Moori}{University of Oxford}
\journaleditor{Matthias Felleiseni}{Northeastern University}
\journaleditor{John Fieldi}{Google}
\journaleditor{Cormac Flanagani}{UC Santa Cruz}
\journaleditor{Philippa Gardneri}{Imperial College}
\journaleditor{Andrew Gordoni}{Microsoft Research and University of Edinburgh}
\journaleditor{Dan Grossmani}{University of Washington}
\journaleditor{Robert Harper}{CMU}
\journaleditor{Tim Harris}{Amazon}
\journaleditor{Fritz Hengleini}{University of Copenhagen}
\journaleditor{Rupak Majumdari}{MPI and UCLA}
\journaleditor{Kenneth McMillani}{Microsoft Research}
\journaleditor{J. Eliot B. Mossi}{University of Massachusetts, Amherst}
\journaleditor{Andrew C. Myersi}{Cornell University}
\journaleditor{Hanne Riis Nielsoni}{Technical University of Denmark}
\journaleditor{Peter O'Hearni}{University College London}
\journaleditor{Benjamin C. Piercei}{University of Pennsylvania}
\journaleditor{Andrew Pittsi}{University of Cambridge}
\journaleditor{Ganesan Ramalingami}{Microsoft Research}
\journaleditor{Mooly Sagivi}{Tel Aviv University}
\journaleditor{Davide Sangiorgii}{University of Bologna}
\journaleditor{David Schmidti}{Kansas State University}
\journaleditor{Peter Sewelli}{University of Cambridge}
\journaleditor{Scott Stolleri}{Stony Brook University}
\journaleditor{Peter Stuckeyi}{University of Melbourne}
\journaleditor{Jan Viteki}{Northeastern University}
\journaleditor{Philip Wadleri}{University of Edinburgh}
\journaleditor{David Walkeri}{Princeton University}
\journaleditor{Stephanie Weirici}{University of Pennsylvania}
\end{multicols*}
\end{editorialboard} 

==> journaldata/PGL-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{PGLcolor}{brickred}   %new color names can be defined before use
\journalcolor      {PGLcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Programming Languages}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {PGL}
\journalurl        {http://www.nowpublishers.com/PGL}
\journalissnprint  {2325-1107}
\journalissnonline {2325-1131}
\journaldoi        {10.1561/25}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Programming Languages publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Abstract Interpretation}
\item{Compilation and Interpretation Techniques}
\item{Domain Specific Languages}
\item{Formal Semantics, including Lambda Calculi, Process Calculi, and Process Algebra}
\item{Language Paradigms}
    \item{Mechanical Proof Checking}
    \item{Memory Management}
    \item{Partial Evaluation}
    \item{Program Logic}
    \item{Programming Language Implementation}
    \item{Programming Language Security}
    \item{Programming Languages for Concurrency}
    \item{Programming Languages for Parallelism}
    \item{Program Synthesis}
    \item{Program Transformations and Optimizations}
    \item{Program Verification}
    \item{Runtime Techniques for Programming Languages}
    \item{Software Model Checking}
    \item{Static and Dynamic Program Analysis}
    \item{Type Theory and Type Systems}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Programming Languages, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/PGL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Tutorial on Static Inference of Numeric Invariants by Abstract\\ Interpretation}\\
Antoine Min\'e\\
ISBN: 978-1-68083-386-7\\
\\
\noindent \textit{Program Synthesis}\\
Sumit Gulwani, Oleksandr Polozov and Rishabh Singh\\
ISBN: 978-1-68083-292-1\\
\\
\noindent \textit{Programming with Big Code}\\
Martin Vechev and Eran Yahav\\
ISBN: 978-1-68083-230-3
\\
\\
\noindent \textit{Behavioral Types in Programming Languages}\\
Davide Ancona et al.\\
ISBN: 978-1-68083-134-4
\\
\\
\noindent \textit{Computer-Assisted Query Formulation}\\
Alvin Cheung and Armando Solar-Lezama\\
ISBN: 978-1-68083-036-1

==> journaldata/ROB-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Henrik Christensen}{University of California, San Diego}
\journalchiefeditor{Roland Siegwart}{ETH Zurich}


\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Minoru Asada}{Osaka University}
\journaleditor{Antonio Bicchi}{University of Pisa}
\journaleditor{Aude Billard}{EPFL}
\journaleditor{Cynthia Breazeal}{Massachusetts Institute of Technology}
\journaleditor{Oliver Brock}{TU Berlin}
\journaleditor{Wolfram Burgard}{University of Freiburg}
\journaleditor{Udo Frese}{University of Bremen}
\journaleditor{Ken Goldberg}{University of California, Berkeley}
\journaleditor{Hiroshi Ishiguro}{Osaka University}
\journaleditor{Makoto Kaneko}{Osaka University}
\journaleditor{Danica Kragic}{KTH Stockholm}
\journaleditor{Vijay Kumar}{University of Pennsylvania}
\journaleditor{Simon Lacroix}{LAAS}
\journaleditor{Christian Laugier}{INRIA}
\journaleditor{Steve LaValle}{University of Illinois at Urbana-Champaign}
\journaleditor{Yoshihiko Nakamura}{The University of Tokyo}
\journaleditor{Brad Nelson}{ETH Zurich}
\journaleditor{Paul Newman}{University of Oxford}
\journaleditor{Daniela Rus}{Massachusetts Institute of Technology}
\journaleditor{Giulio Sandini}{University of Genova}
\journaleditor{Sebastian Thrun}{Stanford University}
\journaleditor{Manuela Veloso}{Carnegie Mellon University}
\journaleditor{Markus Vincze}{Vienna University}
\journaleditor{Alex Zelinsky}{DSTG}
\end{multicols*}
\end{editorialboard} 

==> journaldata/ROB-journaldata.tex <==
\definecolor{pinegreen}{rgb}{0.0, 0.47, 0.44}
\colorlet{ROBcolor}{pinegreen}   %new color names can be defined before use
\journalcolor      {ROBcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Robotics}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ROB}
\journalurl        {http://www.nowpublishers.com/ROB}
\journalissnprint  {1935-8253}
\journalissnonline {1935-8261}
\journaldoi        {10.1561/23}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Robotics publishes
 survey and tutorial articles in the following topics:
\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Mathematical modelling}
\item{Kinematics}
\item{Dynamics}
\item{Estimation Methods}
\item{Robot Control}
\item{Planning}
\item{Artificial Intelligence in Robotics}
\item{Software Systems and Architectures}
\item{Mechanisms and Actuators}
\item{Sensors and Estimation}
\item{Planning and Control}
\item{Human-Robot Interaction}
\item{Industrial Robotics}
\item{Service Robotics }
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Robotics, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/ROB-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Energy in Robotics}\\
Gerrit A. Folkertsma and Stefano Stramigioli\\
ISBN: 978-1-68083-312-6\\
\\
\noindent \textit{Factor Graphs for Robot Perception}\\
Frank Dellaert and Michael Kaess\\
ISBN: 978-1-68083-326-3\\
\\
\noindent \textit{A Survey of Methods for Safe Human-Robot Interaction}\\
Przemyslaw A. Lasota, Terrence Fong and Julie A. Shah\\
ISBN: 978-1-68083-278-5\\
\\
\noindent \textit{Soft-Material Robotics}\\
Sangbae Kim and Patrick M. Wensing \\
ISBN: 978-1-68083-256-3\\
\\
\noindent \textit{Cyber-Maritime Cycle: Autonomy of Marine Robots for Ocean Sensing}\\
Fumin Zhang\\
ISBN: 978-1-68083-232-7

==> journaldata/SEC-editorialboard.tex <==
%SEC-Editorialboard.

\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Anupam Datta}{Carnegie Mellon University, USA}
\journalchiefeditor{Jeannette Wing}{Columbia University, USA}


\subsection{Editors}
\begin{multicols}{2}\raggedcolumns
\journaleditor{Mart\'in Abadi}{Google and University of California, Santa Cruz}
\journaleditor{Michael Backes}{Saarland University}
\journaleditor{Dan Boneh}{Stanford University, USA}
\journaleditor{V\'eronique Cortier}{LORIA, CNRS, France}
\journaleditor{Lorrie Cranor}{Carnegie Mellon University}
\journaleditor{C\'edric Fournet}{Microsoft Research}
\journaleditor{Virgil Gligor}{Carnegie Mellon University}
\journaleditor{Jean-Pierre Hubaux}{EPFL}
\journaleditor{Deirdre Mulligan}{University of California, Berkeley}
\journaleditor{Andrew Myers}{Cornell University}
\journaleditor{Helen Nissenbaum}{New York University}
\journaleditor{Michael Reiter}{University of North Carolina}
\journaleditor{Shankar Sastry}{University of California, Berkeley}
\journaleditor{Dawn Song}{University of California, Berkeley}
\journaleditor{Daniel Weitzner}{Massachusetts Institute of Technology}
\end{multicols}
\end{editorialboard} 


==> journaldata/SEC-journaldata.tex <==
\definecolor{bananayellow}{rgb}{1.0, 0.88, 0.21}
\colorlet{SECcolor}{bananayellow}   %new color names can be defined before use
\journalcolor      {SECcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Privacy and Security}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SEC}
\journalurl        {http://nowpublishers.com/SEC}
\journalissnprint  {2474-1558}
\journalissnonline {2474-1566}
\journaldoi        {10.1561/33}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
 Privacy and Security publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Access control}
\item{Accountability}
\item{Anonymity}
\item{Application security}
\item{Artifical intelligence methods in security and privacy}
\item{Authentication}
\item{Big data analytics and privacy}
\item{Cloud security}
\item{Cyber-physical systems security and privacy}
\item{Distributed systems security and privacy}
\item{Embedded systems security and privacy}
\item{Forensics}
\item{Hardware security}
\item{Human factors in security and privacy}
\item{Information flow}
\item{Intrusion detection}
\item{Malware}
\item{Metrics}
\item{Mobile security and privacy}
\item{Language-based security and privacy}
\item{Network security}
\item{Privacy-preserving systems}
\item{Protocol security}
\item{Security and privacy policies}
\item{Security architectures}
\item{System security}
\item{Web security and privacy}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Privacy and Security, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SEC-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Contextual Integrity through the Lens of Computer Science}\\
Sebastian Benthall, Seda Gurses and Helen Nissenbaum\\
ISBN: 978-1-68083-384-3\\
\\
\noindent \textit{Methods for Location Privacy: A comparative overview}\\
Kostantinos Chatzikokolakis, Ehab ElSalamouny, Catuscia Palamidessi and Pazii Anna\\
ISBN: 978-1-68083-366-9\\
\\
\noindent \textit{Principles and Implementation Techniques of Software-Based Fault Isolation}\\
Gang Tan\\
ISBN: 978-1-68083-344-7\\
\\
\noindent \textit{Modeling and Verifying Security Protocols with the Applied Pi\\ Calculus and ProVerif}\\
Bruno Blanchet\\
ISBN: 978-1-68083-206-8

==> journaldata/SIG-editorialboard.tex <==
%SIG-Editorialboard.

\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Yonina Eldar}{Weizmann Institute\\Israel}



\subsection{Editors}
\begin{multicols}{3}\raggedcolumns
\journaleditor{Pao-Chi Chang}{National Central University}
\journaleditor{Pamela Cosman}{University of California, San Diego}
\journaleditor{Michelle Effros}{California Institute of Technology}
\journaleditor{Yariv Ephraim}{George Mason University}
\journaleditor{Alfonso Farina}{Selex ES}
\journaleditor{Sadaoki Furui}{Tokyo Institute of Technology}
\journaleditor{Georgios Giannakis}{University of Minnesota}
\journaleditor{Vivek Goyal}{Boston University}
\journaleditor{Sinan Gunturk}{Courant Institute}
\journaleditor{Christine Guillemot}{INRIA}
\journaleditor{Robert W. Heath, Jr.}{The University of Texas at Austin}
\journaleditor{Sheila Hemami}{Northeastern University}
\journaleditor{Lina Karam}{Arizona State University}
\journaleditor{Nick Kingsbury}{University of Cambridge}
\journaleditor{Alex Kot}{Nanyang Technical University}
\journaleditor{Jelena Kovacevic}{Carnegie Mellon University}
\journaleditor{Geert Leus}{TU Delft}
\journaleditor{Jia Li}{Pennsylvania State University}
\journaleditor{Henrique Malvar}{Microsoft Research}
\journaleditor{B.S. Manjunath}{University of California, Santa Barbara}
\journaleditor{Urbashi Mitra}{University of Southern California}
\journaleditor{Bj\"{o}rn Ottersten}{KTH Stockholm}
\journaleditor{Vincent Poor}{Princeton University}
\journaleditor{Anna Scaglione}{University of California, Davis}
\journaleditor{Mihaela van der Shaar}{University of California, Los Angeles}
\journaleditor{Nicholas D. Sidiropoulos}{Technical University of Crete}
\journaleditor{Michael Unser}{EPFL}
\journaleditor{P.P. Vaidyanathan}{California Institute of Technology}
\journaleditor{Ami Wiesel}{The Hebrew University of Jerusalem}
\journaleditor{Min Wu}{University of Maryland}
\journaleditor{Josiane Zerubia}{INRIA}
\end{multicols}
\end{editorialboard} 


==> journaldata/SIG-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{SIGcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {SIGcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Signal Processing}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SIG}
\journalurl        {http://www.nowpublishers.com/SIG}
\journalissnprint  {1932-8346}
\journalissnonline {1932-8354}
\journaldoi        {10.1561/20}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
\footnotesize
 \begin{itemize}
\item{Adaptive signal processing}
\item{Audio signal processing}
\item{Biological and biomedical signal processing}
\item{Complexity in signal processing}
\item{Digital signal processing}
\item{Distributed and network signal processing}
\item{Image and video processing}
\item{Linear and nonlinear filtering}
\item{Multidimensional signal processing}
\item{Multimodal signal processing}
\item{Multirate signal processing}
\item{Multiresolution signal processing}
\item{Nonlinear signal processing}
\item{Randomized algorithms in signal processing}
\item{Sensor and multiple source signal processing, source separation}
\item{Signal decompositions, subband and transform methods, sparse representations}
\item{Signal processing for communications}
\item{Signal processing for security and forensic analysis, biometric signal processing}
\item{Signal quantization, sampling, analog-to-digital conversion, coding and compression}
\item{Signal reconstruction, digital-to-analog conversion, enhancement, decoding and inverse problems}
\item{Speech/audio/image/video compression}
\item{Speech and spoken language processing}
\item{Statistical/machine learning}
\item{Statistical signal processing}
	\begin{itemize}
	\item{Classification and detection}
	\item{Estimation and regression}
	\item{Tree-structured methods}
	\end{itemize}
\end{itemize}
\normalsize
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Signal Processing, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SIG-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Massive MIMO Networks: Spectral, Energy, and Hardware Efficiency}\\
Emil Bjornson, Jakob Hoydis and Luca Sanguinetti\\
ISBN: 978-1-68083-985-2\\
\\
\noindent \textit{Using Inertial Sensors for Position and Orientation Estimation}\\
Manon Kok, Jeroen D. Hol and Thomas B. Schon\\
ISBN: 978-1-68083-356-0\\
\\
\noindent \textit{Computational Visual Attention Models}\\
Milind S. Gide and Lina J. Karam\\
ISBN: 978-1-68083-280-8\\
\\
\noindent \textit{Video Coding: Part II of Fundamentals of Source and Video Coding}\\
Thomas Wiegand and Heiko Schwarz\\
ISBN: 978-1-68083-178-8

==> journaldata/STP-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Albert N. Link}{University of North Carolina at Greensboro\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{David Audretsch}{Indiana University}
\journaleditor{William Bonvillian}{MIT}
\journaleditor{Barry Bozeman}{Arizona State University}
\journaleditor{Kaye Husbands Fealing}{Georgia Institute of Technology}
\journaleditor{John Hardin}{North Carolina Board of Science and Technology}
\journaleditor{Mariagrazia Squicciarini}{OECD}
\journaleditor{Wolfgang Polt}{Joanneum Research Institute}
\journaleditor{Nicholas Vonortas}{The George Washington University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/STP-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{ASTPcolor}{cobalt}   %new color names can be defined before use
\journalcolor      {ASTPcolor} %a color name. 
\journaltitle      {Annals of Science and Technology Policy}
%\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {ASTP}
\journalurl        {http://www.nowpublishers.com/ASTP}
\journalissnprint  {2475-1820}
\journalissnonline {2475-1812}
\journaldoi        {10.1561/110}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Annals of Science and Technology Policy publishes
 survey and tutorial articles in the following topics:
 %\begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Literature reviews of technology and innovation policies}
\item{Historical case studies of technology development and implementation}
\item{Institutional histories of technology- and innovation-based organizations}
\item{Analyses of policies attendant to technology development and adoption and diffusion}
\item{Studies documenting the adoption and diffusion of technologies and subsequent consequences}
\item{Studies of public and private research partnerships (cross sectional, over time, or case based)}
\item{Assessments and evaluations of specific technology and innovation policies}
\item{Analyses of ecosystems associated with the technology and/or innovation development}
\item{Cross observational (e.g., cross-agency or cross-country) comparisons of technology and innovation policies}
\end{itemize}
% \end{multicols}
 }


\journallibraryinfo
 {%
  Annals of Science and Technology Policy, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SYS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\journalchiefeditor{Panos J. Antsaklis}{University of Notre Dame\\United States}
\journalchiefeditor{Alessandro Astolfi}{Imperial College London, United Kingdom\\ University of Rome ''Tor Vergata'', Italy}



\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{John Baillieuli}{Boston University}
\journaleditor{Peter Caines}{McGill University}
\journaleditor{Christos Cassandras}{Boston University}
\journaleditor{Denis Dochain}{UC Louvain}
\journaleditor{Magnus Egerstedt}{Georgia Institute of Technology}
\journaleditor{Karl Henrik Johansson}{KTH Stockholm}
\journaleditor{Miroslav Krstic}{University of California, San Diego}
\journaleditor{Jan Maciejowski}{University of Cambridge}
\columnbreak
\journaleditor{Dragan Nesic}{The University of Melbourne}
\journaleditor{Marios Polycarpou}{University of Cyprus}
\journaleditor{J\"{o}rg Raisch}{Technical University Berlin}
\journaleditor{Arjan van der Schaft}{University of Groningen}
\journaleditor{M. Elena Valcher}{University of Padova}
\journaleditor{Richard Vinter}{Imperial College London}
\journaleditor{George Weiss}{Tel Aviv University}
\end{multicols*}
\end{editorialboard} 

==> journaldata/SYS-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet {SYScolor}{cobalt} %new color names can be defined before use
\journalcolor      {SYScolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Systems and Control}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {SYS}
\journalurl        {http://www.nowpublishers.com/SYS}
\journalissnprint  {2325-6818}
\journalissnonline {2325-6826}
\journaldoi        {10.1561/26}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
 Foundations and Trends\textsuperscript{\textregistered} in
Systems and Control publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Control of:}
	\begin{itemize}
	\item{Hybrid and Discrete Event Systems}
	\item{Nonlinear Systems}
	\item{Network Systems}
	\item{Stochastic Systems}
	\item{Multi-agent Systems}
	\item{Distributed Parameter Systems}
	\item{Delay Systems}
	\end{itemize}
\item{Filtering, Estimation, Identification}
\item{Optimal Control}
\item{Systems Theory}
\item{Control Applications}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Systems and Control, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/SYS-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Economic Model Predictive Control}\\
Helen Durand and Panagiotis D. Christofides\\
ISBN: 978-1-68083-432-1\\
\\
\noindent \textit{Distributed Averaging and Balancing in Network Systems}\\
Christoforos N. Hadjicostis, Alejandro D. Dominguez-Garcia and\\ Themistokis Charalambous\\
ISBN: 978-1-68083-438-3\\
\\
\noindent \textit{Economic Nonlinear Model Predictive Control}\\
Timm Faulwasser, Lars Grune and Matthias A. Muller\\
ISBN: 978-1-68083-392-8


==> journaldata/TCS-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Madhu Sudan}{Harvard University\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Bernard Chazelle}{Princeton University}
\journaleditor{Oded Goldreich}{Weizmann Institute}
\journaleditor{Shafi Goldwasser}{Massachusetts Institute of Technology and Weizmann Institute}
\journaleditor{Sanjeev Khanna}{University of Pennsylvania}
\journaleditor{Jon Kleinberg}{Cornell University}
\journaleditor{L\'aszl\'o Lov\'asz}{Eötvös Lor\'and University}
\journaleditor{Christos Papadimitriou}{University of California, Berkeley}
\journaleditor{Peter Shor}{Massachusetts Institute of Technology}
\journaleditor{Eva Tardos}{Cornell University}
\journaleditor{Avi Wigderson}{AIS, Princeton University}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/TCS-journaldata.tex <==
\definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
\colorlet{TCScolor}{cobalt}   %new color names can be defined before use
\journalcolor      {TCScolor} %a color name. 
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {TCS}
\journalurl        {http://www.nowpublishers.com/TCS}
\journalissnprint  {1551-305X}
\journalissnonline {1551-3068}
\journaldoi        {10.1561/04}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{numeric} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Algorithmic game theory}
    \item{Computational algebra}
    \item{Computational aspects of combinatorics and graph theory}
    \item{Computational aspects of communication}
    \item{Computational biology}
    \item{Computational complexity}
    \item{Computational geometry}
    \item{Computational learning}
    \item{Computational Models and Complexity}
    \item{Computational Number Theory}
    \item{Cryptography and information security}
    \item{Data structures}
    \item{Database theory}
    \item{Design and analysis of algorithms}
    \item{Distributed computing}
    \item{Information retrieval}
    \item{Operations Research}
    \item{Parallel algorithms}
    \item{Quantum Computation}
    \item{Randomness in Computation}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in Theoretical Computer Science, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/TCS-seriespage.tex <==
\vspace{12pt}

\noindent \textit{Coding for Interactive Communication: A Survey}\\
Ran Gelles\\
ISBN: 978-1-68083-346-1\\
\\
\noindent \textit{Hashing, Load Balancing and Multiple Choice}\\
Udi Wieder\\
ISBN: 978-1-68083-282-2\\
\\
\noindent \textit{Scalable Algorithms for Data and Network Analysis}\\
Shang-Hua Teng\\
ISBN: 978-1-68083-130-6\\
\\
\noindent \textit{Communication Complexity (for Algorithm Designers)}\\
Tim Roughgarden \\
ISBN: 978-1-68083-114-6\\
\\
\noindent \textit{Quantum Proofs}\\
Thomas Vidick and John Watrous\\
ISBN: 978-1-68083-126-9

==> journaldata/TOM-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Charles Corbett}{UCLA, Anderson School of Management\\United States}



\subsection{Editors}
%\begin{multicols*}{2}\raggedcolumns
\journaleditor{Fernando Bernstein}{Duke University}
\journaleditor{Cheryl Gaimon}{Georgia Institute of Technology}
\journaleditor{Uday Karmarkar}{University of California, Los Angeles}
\journaleditor{Sunder Kekre}{Carnegie Mellon University}
\journaleditor{Panos Kouvelis}{Washington University}
\journaleditor{Michael Lapré}{Vanderbilt University}
\journaleditor{Karl Ulrich}{University of Pennsylvania}
\journaleditor{Luk van Wassenhove}{INSEAD}
%\end{multicols*}
\end{editorialboard} 

==> journaldata/TOM-journaldata.tex <==
\definecolor{cerise}{rgb}{0.87, 0.19, 0.39}
\colorlet{TOMcolor}{cerise}   %new color names can be defined before use
\journalcolor      {TOMcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Technology, Information and Operations Management}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {TOM}
\journalurl        {http://www.nowpublishers.com/TOM}
\journalissnprint  {1571-9545}
\journalissnonline {1571-9553}
\journaldoi        {10.1561/02}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Technology, Information and Operations Management publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{B2B Commerce}
\item{Business Process Engineering and Design}
\item{Business Process Outsourcing}
\item{Capacity Planning}
\item{Competitive Operations}
\item{Contracting in Supply Chains}
\item{E-Commerce and E-Business Models}
\item{Electronic markets, auctions and exchanges}
\item{Enterprise Management Systems}
\item{Facility Location}
\item{Information Chain Structure and Competition}
\item{International Operations}
\item{Marketing/Manufacturing Interfaces}
\item{Multi-location inventory theory}
\item{New Product \& Service Design}
\item{Queuing Networks}
\item{Reverse Logistics}
\item{Service Logistics and Product Support}
\item{Supply Chain Management}
\item{Technology Management and Strategy}
\item{Technology, Information and Operations in:}
	\begin{itemize}
	\item{Automotive Industries}
	\item{Electronics manufacturing}
	\item{Financial Services}
	\item{Health Care}
	\item{Media and Entertainment}
	\item{Process Industries}
	\item{Retailing}
	\item{Telecommunications}
	\end{itemize}
\end{itemize}
 \end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Technology, Information and Operations Management, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/TOM-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Inventory Management:  Modeling Real-life Supply Chains and Empirical Validity}\\
Ton de Kok
\\ISBN: 978-1-68083-416-1
\\
\\
\noindent \textit{Operations in Financial Services: Processes, Technologies, and Risks}\\
Michael Pinedo and Yuqian Xu
\\ISBN: 978-1-68083-336-2
\\
\\
\noindent \textit{Integrated Risk Management in Supply Chains}\\
Panos Kouvelis, Ling Dong and Danko Turcic (eds.)
\\ISBN: 978-1-68083-378-2
\\
\\
\noindent \textit{Supply Chain Finance}\\
Panos Kouvelis, Ling Dong and Danko Turcic (eds.)
\\ISBN: 978-1-68083-376-8

==> journaldata/WEB-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editors-in-Chief}

\begin{multicols}{1}%\raggedcolumns
\journalchiefeditor{Wendy Hall}{University of Southampton, UK}
\journalchiefeditor{Noshir R. Contractor}{Northwestern University, USA}
\journalchiefeditor{Kieron O'Hara}{University of Southampton, UK}
\end{multicols}

\subsection{Editors}
\begin{multicols*}{2}\raggedcolumns
\journaleditor{Tim Berners-Lee}{Massachusetts Institute of Technology}
\journaleditor{Noshir Contractor}{Northwestern University}
\journaleditor{Lorrie Crano}{Carnegie Mellon University}
\journaleditor{Dieter Fensel}{University of Innsbruck}
\journaleditor{Carole Goble}{University of Manchester}
\journaleditor{Pat Hayes}{IHMC}
\journaleditor{James Hendler}{Rensselaer Polytechnic Institute}
\journaleditor{Arun Iyengar}{IBM Research}
%\columnbreak
\journaleditor{Craig Knoblock}{University of Southern California}
\journaleditor{Ora Lassila}{Pegasystems}
\journaleditor{Sun Maosong}{Tsinghua University}
\journaleditor{Cathy Marshall}{Microsoft}
\journaleditor{Peter Monge}{University of Southern California}
\journaleditor{Ben Shneiderman}{University of Maryland}
\journaleditor{Danny Weitzner}{Massachusetts Institute of Technology}
\journaleditor{Yorick Wilks}{University of Sheffield}
\end{multicols*}
\end{editorialboard} 

==> journaldata/WEB-journaldata.tex <==
\definecolor{brickred}{rgb}{0.8, 0.25, 0.33}
\colorlet{WEBcolor}{brickred}   %new color names can be defined before use
\journalcolor      {WEBcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Web Science}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {WEB}
\journalurl        {http://www.nowpublishers.com/WEB}
\journalissnprint  {1551-3939}
\journalissnonline {1551-3947}
\journaldoi        {10.1561/10}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Web Science publishes
 survey and tutorial articles in the following topics: 
\begin{multicols}{2}\raggedcolumns
\begin{itemize}
\item{Agents and the Semantic Web}
    \item{Collective Intelligence}
    \item{Content Management}
    \item{Databases on the Web}
    \item{Data Mining}
    \item{Democracy and the Web}
    \item{Dependability}
    \item{Economics of information and the Web}
    \item{E-Crime}
    \item{E-Government}
    \item{Emergent behaviour}
    \item{Ethics}
    \item{Hypertext/Hypermedia}
    \item{Identity}
    \item{Languages on the Web}
    \item{Memories for Life}
    \item{Mobile/Pervasive}
    \item{Network Infrastructures}
    \item{Performance}
    \item{Privacy}
    \item{Scalability}
    \item{Security}
    \item{Semantic Web}
    \item{Social Networking}
    \item{Standards}
    \item{The Law and the Web}
    \item{The Web as an Educational Tool}
    \item{The Web in the Developing World}
    \item{Trust and Provenance}
    \item{Universal Usability}
    \item{User Interfaces}
    \item{Virtual Reality}
    \item{Web Art}
    \item{Web Governance}
    \item{Search}
    \item{Web Services}
\end{itemize}
\end{multicols}
 }

\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Web Science, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 4 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> journaldata/WEB-seriespage.tex <==
\vspace{12pt}
\noindent \textit{An Introduction to Hybrid Human-Machine Information Systems}\\
Gianluca Demartini, Djellel Eddine Difallah, Ujwal Gadiraju and\\ Michele Catasta\\
ISBN: 978-1-68083-374-4\\
\\
\noindent \textit{Minds Online: The Interface between Web Science, Cognitive Science and the Philosophy of Mind}\\
Paul Smart, Robert Clowes and Richard Heersmink\\
ISBN: 978-1-68083-322-5\\
\\
\noindent \textit{Collective Attention on the Web}\\
Christian Bauckhage and Kristian Kersting\\
ISBN: 978-1-68083-204-4
